SRE-Marathon: A Continuous, Change-Driven Benchmark for Autonomous Site Reliability Agents

Benchmarks for site reliability engineering (SRE) agents are typically episodic: one fault is injected, the agent receives an incident task, and its response is scored. Production operation is not. Incidents surface through noisy alerts, overlap in time, and often originate from code or configuration changes. We present SRE-Marathon, a benchmark for long-horizon, continuous SRE operation. An agent is invoked at a fixed cadence with cumulative alert history and a persistent workspace while operating a live two-zone Kubernetes deployment as a fault orchestrator injects overlapping faults according to a seeded, production-calibrated schedule. Curated code and configuration changes deployed through the same build pipeline available for repair. Each run is recorded into a sealed bundle and scored offline: Marathon-Score credits each injected fault for ordered progress through correlation, localization, and repair, with all metrics computed deterministically from recorded system evidence. Across three applications and about sixty faults per run, the best of 10 methods reaches only 41.3 out of 100. Agents often correlate and localize faults, but almost never complete repairs while the faults remain active.

==> results/macros.tex <==
% Generated by 12_tables.py from the analysis CSVs. Use \val{key}; never type a result by hand.
\makeatletter
\newcommand{\val}[1]{\@ifundefined{val@#1}{\textbf{??#1??}}{\csname val@#1\endcsname}}
\expandafter\def\csname val@pool.long.runs\endcsname{16}
\expandafter\def\csname val@pool.long.agents\endcsname{5}
\expandafter\def\csname val@pool.matched.runs\endcsname{12}
\expandafter\def\csname val@pool.seed17.runs\endcsname{5}
\expandafter\def\csname val@pool.short5.episodes\endcsname{6}
\expandafter\def\csname val@pool.short10.episodes\endcsname{6}
\expandafter\def\csname val@pool.short.episodes\endcsname{12}
\expandafter\def\csname val@pool.crossrelease.runs\endcsname{1}
\expandafter\def\csname val@pool.not_rescored\endcsname{4}
\expandafter\def\csname val@pool.all_bundles\endcsname{79}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.alerts_in_denominator\endcsname{89}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m4.uim\endcsname{8062}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m6.mitigated.median_s\endcsname{244}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.smash_score\endcsname{2.52}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.smash_lo_r1\endcsname{2.52}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.smash_hi_r0\endcsname{2.52}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.f1\endcsname{0.04}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.nrr\endcsname{0.32}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.precision\endcsname{0.02}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.incidents_declared\endcsname{63}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.alerts_in_denominator\endcsname{92}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m2.mean_credit\endcsname{0.07}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m3.fsr_symptomatic\endcsname{0.06}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m4.uim\endcsname{7818}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m4.regret\endcsname{0.97}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m4.regret_raw\endcsname{0.97}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m5.median_s\endcsname{155}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m6.mitigated.median_s\endcsname{246}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.blast_radius\endcsname{0.29}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.claim_calls\endcsname{1540}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m1.ambiguous_excluded\endcsname{53}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.m7.executed_mutating_actions\endcsname{14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.dollars\endcsname{4.39}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.llm_calls\endcsname{305}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.smash_score\endcsname{-8.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.smash_lo_r1\endcsname{-8.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.smash_hi_r0\endcsname{-8.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.f1\endcsname{0.32}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.nrr\endcsname{0.72}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.precision\endcsname{0.21}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.recall\endcsname{0.71}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.incidents_declared\endcsname{49}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.alerts_in_denominator\endcsname{177}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m2.acc_at_1\endcsname{0.19}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m2.mean_credit\endcsname{0.69}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m2.false_diagnoses\endcsname{142}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m4.uim\endcsname{12129}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m4.regret_raw\endcsname{1.50}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m5.reached\endcsname{11}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m5.median_s\endcsname{80}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.claim_calls\endcsname{2034}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.refused_actions\endcsname{25}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.unlinked_citations\endcsname{21}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m1.ambiguous_excluded\endcsname{62}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.m7.executed_mutating_actions\endcsname{66}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.dollars\endcsname{0.70}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.llm_calls\endcsname{45}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.smash_score\endcsname{3.45}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.smash_lo_r1\endcsname{3.45}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.smash_hi_r0\endcsname{3.45}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.f1\endcsname{0.06}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.nrr\endcsname{-0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.precision\endcsname{0.43}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.recall\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.incidents_declared\endcsname{134}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.alerts_in_denominator\endcsname{90}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m4.uim\endcsname{7478}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m4.regret\endcsname{0.93}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m4.regret_raw\endcsname{0.93}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m6.mitigated.median_s\endcsname{250}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m7.claim_calls\endcsname{4036}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m1.ambiguous_excluded\endcsname{54}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.dollars\endcsname{3.95}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.llm_calls\endcsname{128}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.smash_score\endcsname{7.39}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.smash_lo_r1\endcsname{7.39}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.smash_hi_r0\endcsname{7.39}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.f1\endcsname{0.40}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.nrr\endcsname{0.42}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.precision\endcsname{0.42}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.recall\endcsname{0.38}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.incidents_declared\endcsname{102}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.alerts_in_denominator\endcsname{177}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m2.mean_credit\endcsname{0.58}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m2.false_diagnoses\endcsname{11}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m3.mitigated_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m4.uim\endcsname{7930}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m4.regret\endcsname{0.98}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m4.regret_raw\endcsname{0.98}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m5.median_s\endcsname{132}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m6.mitigated.reached\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m6.mitigated.median_s\endcsname{371}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.claim_calls\endcsname{651}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.unlinked_citations\endcsname{32}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m1.ambiguous_excluded\endcsname{102}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.m7.executed_mutating_actions\endcsname{95}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-tt-seed7-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.alerts_in_denominator\endcsname{57}
\expandafter\def\csname val@run.storm-tt-seed7-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m3.fsr_symptomatic\endcsname{0.04}
\expandafter\def\csname val@run.storm-tt-seed7-null.m3.mitigated_rate\endcsname{0.17}
\expandafter\def\csname val@run.storm-tt-seed7-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m4.uim\endcsname{38181}
\expandafter\def\csname val@run.storm-tt-seed7-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.storm-tt-seed7-null.m6.mitigated.median_s\endcsname{286}
\expandafter\def\csname val@run.storm-tt-seed7-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m1.ambiguous_excluded\endcsname{184}
\expandafter\def\csname val@run.storm-tt-seed7-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-null.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.smash_score\endcsname{-2.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.smash_lo_r1\endcsname{-2.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.smash_hi_r0\endcsname{-2.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.f1\endcsname{0.35}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.nrr\endcsname{0.63}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.precision\endcsname{0.28}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.recall\endcsname{0.46}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.incidents_declared\endcsname{33}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.alerts_in_denominator\endcsname{90}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m2.mean_credit\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m2.false_diagnoses\endcsname{21}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m3.fsr_symptomatic\endcsname{0.04}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m3.mitigated_rate\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m3.root_fixed_rate\endcsname{0.07}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m3.agent_attributed_rate\endcsname{0.29}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m4.uim\endcsname{47197}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m4.regret_raw\endcsname{1.24}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m6.mitigated.reached\endcsname{7}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m6.mitigated.median_s\endcsname{467}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.blast_radius\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.claim_calls\endcsname{313}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.unlinked_citations\endcsname{16}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m1.ambiguous_excluded\endcsname{163}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.m7.executed_mutating_actions\endcsname{37}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.problems_injected\endcsname{55}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.smash_score\endcsname{10.35}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.smash_lo_r1\endcsname{10.35}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.smash_hi_r0\endcsname{10.35}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.f1\endcsname{0.06}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.nrr\endcsname{0.11}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.incidents_declared\endcsname{49}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.alerts_in_denominator\endcsname{55}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m2.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m2.mean_credit\endcsname{0.14}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m2.false_diagnoses\endcsname{10}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m3.fsr_symptomatic\endcsname{0.02}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m3.mitigated_rate\endcsname{0.17}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m4.uim\endcsname{29297}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m4.regret\endcsname{0.77}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m4.regret_raw\endcsname{0.77}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m5.reached\endcsname{3}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m5.median_s\endcsname{359}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m6.mitigated.median_s\endcsname{260}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.blast_radius\endcsname{0.30}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.claim_calls\endcsname{1318}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.unlinked_citations\endcsname{3}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m1.ambiguous_excluded\endcsname{172}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.m7.executed_mutating_actions\endcsname{10}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.dollars\endcsname{4.06}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.llm_calls\endcsname{256}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.smash_score\endcsname{19.77}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.smash_lo_r1\endcsname{19.77}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.smash_hi_r0\endcsname{19.77}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.f1\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.nrr\endcsname{0.80}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.precision\endcsname{0.08}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.recall\endcsname{0.33}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.incidents_declared\endcsname{25}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.alerts_in_denominator\endcsname{128}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m2.mean_credit\endcsname{0.57}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m2.false_diagnoses\endcsname{443}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m3.fsr_symptomatic\endcsname{0.02}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m3.mitigated_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m3.root_fixed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m4.uim\endcsname{18782}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m4.regret\endcsname{0.49}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m4.regret_raw\endcsname{0.49}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m5.reached\endcsname{1}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m5.median_s\endcsname{376}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m6.mitigated.reached\endcsname{2}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m6.mitigated.median_s\endcsname{389}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.blast_radius\endcsname{0.05}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.claim_calls\endcsname{2221}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.refused_actions\endcsname{31}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.unlinked_citations\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m1.ambiguous_excluded\endcsname{290}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.m7.executed_mutating_actions\endcsname{152}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.dollars\endcsname{1.25}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.llm_calls\endcsname{45}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.alerts_in_denominator\endcsname{55}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m3.fsr_symptomatic\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m4.uim\endcsname{1244}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m6.mitigated.reached\endcsname{39}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m6.mitigated.median_s\endcsname{375}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m1.ambiguous_excluded\endcsname{49}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.smash_score\endcsname{14.33}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.smash_lo_r1\endcsname{14.33}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.smash_hi_r0\endcsname{14.33}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.f1\endcsname{0.64}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.nrr\endcsname{0.57}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.precision\endcsname{0.68}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.recall\endcsname{0.60}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.incidents_declared\endcsname{49}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.alerts_in_denominator\endcsname{114}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m2.mean_credit\endcsname{0.28}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m2.false_diagnoses\endcsname{7}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m3.fsr_symptomatic\endcsname{0.23}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m3.mitigated_rate\endcsname{0.57}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m3.root_fixed_rate\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m3.agent_attributed_rate\endcsname{0.18}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m4.uim\endcsname{1155}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m4.regret\endcsname{0.93}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m4.regret_raw\endcsname{0.93}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m6.mitigated.reached\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m6.mitigated.median_s\endcsname{491}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.blast_radius\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.claim_calls\endcsname{284}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.unlinked_citations\endcsname{30}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m1.ambiguous_excluded\endcsname{114}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.m7.executed_mutating_actions\endcsname{47}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.smash_score\endcsname{13.06}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.smash_lo_r1\endcsname{13.06}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.smash_hi_r0\endcsname{13.06}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.f1\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.nrr\endcsname{0.30}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.precision\endcsname{0.05}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.incidents_declared\endcsname{37}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.alerts_in_denominator\endcsname{53}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m2.acc_at_1\endcsname{0.12}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m2.mean_credit\endcsname{0.24}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m2.false_diagnoses\endcsname{24}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m3.fsr_symptomatic\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m3.agent_attributed_rate\endcsname{0.11}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m4.uim\endcsname{960}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m4.regret\endcsname{0.77}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m4.regret_raw\endcsname{0.77}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m5.reached\endcsname{9}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m5.median_s\endcsname{350}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m6.mitigated.reached\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m6.mitigated.median_s\endcsname{407}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.blast_radius\endcsname{0.14}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.claim_calls\endcsname{356}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.unlinked_citations\endcsname{13}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m1.ambiguous_excluded\endcsname{63}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.m7.executed_mutating_actions\endcsname{22}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.dollars\endcsname{3.61}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.llm_calls\endcsname{335}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.smash_score\endcsname{-8.73}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.smash_lo_r1\endcsname{-8.73}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.smash_hi_r0\endcsname{-8.73}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.f1\endcsname{0.42}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.nrr\endcsname{0.72}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.precision\endcsname{0.27}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.recall\endcsname{0.91}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.incidents_declared\endcsname{16}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.alerts_in_denominator\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m2.mean_credit\endcsname{0.13}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m2.false_diagnoses\endcsname{115}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m3.fsr_symptomatic\endcsname{0.28}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m4.uim\endcsname{1778}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m4.regret_raw\endcsname{1.43}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m6.mitigated.reached\endcsname{39}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m6.mitigated.median_s\endcsname{452}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.blast_radius\endcsname{0.50}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.claim_calls\endcsname{648}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.refused_actions\endcsname{5}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.unlinked_citations\endcsname{14}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m1.ambiguous_excluded\endcsname{52}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.m7.executed_mutating_actions\endcsname{2}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.dollars\endcsname{0.22}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.llm_calls\endcsname{24}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.smash_score\endcsname{1.92}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.smash_lo_r1\endcsname{1.92}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.smash_hi_r0\endcsname{1.92}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.f1\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.nrr\endcsname{-0.89}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.precision\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.recall\endcsname{0.02}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.incidents_declared\endcsname{102}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.alerts_in_denominator\endcsname{54}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m3.fsr_symptomatic\endcsname{0.30}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m3.mitigated_rate\endcsname{0.71}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m4.uim\endcsname{1192}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m4.regret\endcsname{0.96}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m4.regret_raw\endcsname{0.96}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m6.mitigated.reached\endcsname{41}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m6.mitigated.median_s\endcsname{441}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m7.claim_calls\endcsname{4260}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m1.ambiguous_excluded\endcsname{48}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.dollars\endcsname{2.75}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.llm_calls\endcsname{119}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.smash_score\endcsname{6.46}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.smash_lo_r1\endcsname{6.46}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.smash_hi_r0\endcsname{6.46}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.f1\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.nrr\endcsname{0.99}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.precision\endcsname{0.02}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.incidents_declared\endcsname{1}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.alerts_in_denominator\endcsname{85}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m2.acc_at_1\endcsname{0.19}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m2.mean_credit\endcsname{0.33}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m2.false_diagnoses\endcsname{29}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m4.uim\endcsname{7804}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m4.regret\endcsname{0.97}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m4.regret_raw\endcsname{0.97}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m5.reached\endcsname{12}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m5.median_s\endcsname{152}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m6.mitigated.median_s\endcsname{243}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.claim_calls\endcsname{545}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m1.ambiguous_excluded\endcsname{54}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.m7.executed_mutating_actions\endcsname{7}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.dollars\endcsname{4.37}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.llm_calls\endcsname{282}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.smash_score\endcsname{-7.75}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.smash_lo_r1\endcsname{-7.75}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.smash_hi_r0\endcsname{-7.75}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.f1\endcsname{0.36}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.nrr\endcsname{0.90}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.precision\endcsname{0.27}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.recall\endcsname{0.54}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.incidents_declared\endcsname{6}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.alerts_in_denominator\endcsname{60}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m2.acc_at_1\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m2.mean_credit\endcsname{0.29}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m2.false_diagnoses\endcsname{31}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m3.fsr_symptomatic\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m3.mitigated_rate\endcsname{0.62}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m3.root_fixed_rate\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m3.agent_attributed_rate\endcsname{0.12}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m4.uim\endcsname{1793}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m4.regret_raw\endcsname{1.44}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m5.reached\endcsname{5}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m5.median_s\endcsname{193}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m6.mitigated.reached\endcsname{34}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m6.mitigated.median_s\endcsname{402}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.claim_calls\endcsname{546}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.unlinked_citations\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m1.ambiguous_excluded\endcsname{67}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.m7.executed_mutating_actions\endcsname{15}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.dollars\endcsname{4.37}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.llm_calls\endcsname{302}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.problems_injected\endcsname{55}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.smash_score\endcsname{4.65}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.smash_lo_r1\endcsname{4.65}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.smash_hi_r0\endcsname{4.65}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.f1\endcsname{0.15}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.nrr\endcsname{0.90}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.precision\endcsname{0.18}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.recall\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.incidents_declared\endcsname{7}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.alerts_in_denominator\endcsname{70}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m2.acc_at_1\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m2.mean_credit\endcsname{0.17}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m2.false_diagnoses\endcsname{19}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m3.mitigated_rate\endcsname{0.12}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m3.agent_attributed_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m4.uim\endcsname{32657}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m4.regret_raw\endcsname{1.03}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m5.reached\endcsname{8}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m5.median_s\endcsname{239}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m6.mitigated.reached\endcsname{7}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m6.mitigated.median_s\endcsname{319}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.claim_calls\endcsname{447}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m1.ambiguous_excluded\endcsname{165}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.m7.executed_mutating_actions\endcsname{8}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.dollars\endcsname{4.47}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.llm_calls\endcsname{239}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.alerts_in_denominator\endcsname{44}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m3.mitigated_rate\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m4.uim\endcsname{886}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m6.mitigated.reached\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m6.mitigated.median_s\endcsname{511}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m1.ambiguous_excluded\endcsname{55}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.smash_score\endcsname{0.64}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.smash_lo_r1\endcsname{0.64}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.smash_hi_r0\endcsname{0.64}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.f1\endcsname{0.85}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.nrr\endcsname{0.42}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.precision\endcsname{0.85}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.recall\endcsname{0.86}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.incidents_declared\endcsname{45}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.alerts_in_denominator\endcsname{78}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m2.mean_credit\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m2.false_diagnoses\endcsname{6}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m3.mitigated_rate\endcsname{0.51}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m3.root_fixed_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m3.agent_attributed_rate\endcsname{0.10}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m4.uim\endcsname{1270}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m4.regret_raw\endcsname{1.43}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m6.mitigated.reached\endcsname{30}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m6.mitigated.median_s\endcsname{580}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.blast_radius\endcsname{0.02}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.claim_calls\endcsname{290}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.unlinked_citations\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m1.ambiguous_excluded\endcsname{113}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.m7.executed_mutating_actions\endcsname{41}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.smash_score\endcsname{-9.02}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.smash_lo_r1\endcsname{-9.02}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.smash_hi_r0\endcsname{-9.02}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.f1\endcsname{0.11}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.nrr\endcsname{0.65}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.precision\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.incidents_declared\endcsname{17}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.alerts_in_denominator\endcsname{48}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m2.mean_credit\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m2.false_diagnoses\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m3.mitigated_rate\endcsname{0.47}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m3.root_fixed_rate\endcsname{0.07}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m3.agent_attributed_rate\endcsname{0.04}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m4.uim\endcsname{1225}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m4.regret_raw\endcsname{1.38}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m5.median_s\endcsname{625}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m6.mitigated.reached\endcsname{28}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m6.mitigated.median_s\endcsname{443}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.blast_radius\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.claim_calls\endcsname{172}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.unlinked_citations\endcsname{6}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m1.ambiguous_excluded\endcsname{62}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.m7.executed_mutating_actions\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.dollars\endcsname{3.09}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.llm_calls\endcsname{313}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.smash_score\endcsname{-12.03}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.smash_lo_r1\endcsname{-12.03}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.smash_hi_r0\endcsname{-12.03}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.f1\endcsname{0.65}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.nrr\endcsname{0.63}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.precision\endcsname{0.53}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.recall\endcsname{0.83}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.incidents_declared\endcsname{23}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.alerts_in_denominator\endcsname{63}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m2.mean_credit\endcsname{0.27}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m2.false_diagnoses\endcsname{130}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m3.mitigated_rate\endcsname{0.54}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m3.root_fixed_rate\endcsname{0.12}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m4.uim\endcsname{1539}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m4.regret_raw\endcsname{1.74}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m5.reached\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m5.median_s\endcsname{609}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m6.mitigated.reached\endcsname{32}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m6.mitigated.median_s\endcsname{547}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.blast_radius\endcsname{0.11}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.claim_calls\endcsname{791}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.refused_actions\endcsname{12}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.unlinked_citations\endcsname{17}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m1.ambiguous_excluded\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.m7.executed_mutating_actions\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.dollars\endcsname{0.24}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.llm_calls\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.smash_score\endcsname{-31.95}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.smash_lo_r1\endcsname{-31.95}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.smash_hi_r0\endcsname{-31.95}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.f1\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.nrr\endcsname{-1.20}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.precision\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.recall\endcsname{0.11}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.incidents_declared\endcsname{97}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.alerts_in_denominator\endcsname{44}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m3.mitigated_rate\endcsname{0.63}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m4.uim\endcsname{2543}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m4.regret_raw\endcsname{2.87}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m6.mitigated.reached\endcsname{37}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m6.mitigated.median_s\endcsname{455}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m7.claim_calls\endcsname{3887}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.dollars\endcsname{2.10}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.llm_calls\endcsname{102}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.smash_score\endcsname{1.37}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.smash_lo_r1\endcsname{1.37}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.smash_hi_r0\endcsname{1.37}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.alerts_in_denominator\endcsname{88}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m4.uim\endcsname{7747}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m4.regret\endcsname{0.96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m4.regret_raw\endcsname{0.96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m6.mitigated.median_s\endcsname{241}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m1.ambiguous_excluded\endcsname{53}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.alerts_in_denominator\endcsname{105}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m3.mitigated_rate\endcsname{0.10}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m4.uim\endcsname{8836}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m6.mitigated.reached\endcsname{6}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m6.mitigated.median_s\endcsname{253}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m1.ambiguous_excluded\endcsname{61}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.smash_score\endcsname{6.89}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.smash_lo_r1\endcsname{6.89}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.smash_hi_r0\endcsname{6.89}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.f1\endcsname{0.04}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.nrr\endcsname{0.26}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.precision\endcsname{0.02}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.incidents_declared\endcsname{64}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.alerts_in_denominator\endcsname{87}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m2.acc_at_1\endcsname{0.08}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m2.mean_credit\endcsname{0.22}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m2.false_diagnoses\endcsname{7}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m3.fsr_symptomatic\endcsname{0.07}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m3.mitigated_rate\endcsname{0.17}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m3.root_fixed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m4.uim\endcsname{7918}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m4.regret\endcsname{0.90}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m4.regret_raw\endcsname{0.90}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m5.reached\endcsname{5}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m5.median_s\endcsname{290}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m6.mitigated.median_s\endcsname{375}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.blast_radius\endcsname{0.10}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.claim_calls\endcsname{1336}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.unlinked_citations\endcsname{6}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m1.ambiguous_excluded\endcsname{55}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.m7.executed_mutating_actions\endcsname{21}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.dollars\endcsname{4.32}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.llm_calls\endcsname{312}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.smash_score\endcsname{-1.60}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.smash_lo_r1\endcsname{-1.60}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.smash_hi_r0\endcsname{-1.60}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.f1\endcsname{0.51}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.nrr\endcsname{0.72}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.precision\endcsname{0.34}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.incidents_declared\endcsname{35}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.alerts_in_denominator\endcsname{125}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m2.acc_at_1\endcsname{0.21}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m2.mean_credit\endcsname{0.62}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m2.false_diagnoses\endcsname{191}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m4.uim\endcsname{12486}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m4.regret_raw\endcsname{1.41}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m5.reached\endcsname{12}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m5.median_s\endcsname{181}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.claim_calls\endcsname{1838}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.refused_actions\endcsname{23}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.unlinked_citations\endcsname{33}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m1.ambiguous_excluded\endcsname{73}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.m7.executed_mutating_actions\endcsname{55}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.dollars\endcsname{0.60}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.llm_calls\endcsname{45}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.problems_injected\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.alerts_in_denominator\endcsname{51}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m3.fsr_symptomatic\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m3.mitigated_rate\endcsname{0.70}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m4.uim\endcsname{902}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m6.mitigated.reached\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m6.mitigated.median_s\endcsname{713}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m1.ambiguous_excluded\endcsname{38}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.problems_injected\endcsname{47}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.smash_score\endcsname{-22.22}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.smash_lo_r1\endcsname{-22.22}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.smash_hi_r0\endcsname{-22.22}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.f1\endcsname{0.70}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.nrr\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.precision\endcsname{0.66}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.recall\endcsname{0.76}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.incidents_declared\endcsname{40}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.alerts_in_denominator\endcsname{97}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m2.mean_credit\endcsname{0.22}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m2.false_diagnoses\endcsname{11}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m3.fsr_symptomatic\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m3.mitigated_rate\endcsname{0.62}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m3.root_fixed_rate\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m3.agent_attributed_rate\endcsname{0.18}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m4.uim\endcsname{1874}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m4.regret_raw\endcsname{2.08}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m6.mitigated.reached\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m6.mitigated.median_s\endcsname{475}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.blast_radius\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.claim_calls\endcsname{319}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.unlinked_citations\endcsname{17}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m1.ambiguous_excluded\endcsname{76}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.m7.executed_mutating_actions\endcsname{36}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.problems_injected\endcsname{53}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.smash_score\endcsname{-31.70}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.smash_lo_r1\endcsname{-31.70}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.smash_hi_r0\endcsname{-31.70}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.f1\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.nrr\endcsname{0.62}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.incidents_declared\endcsname{26}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.alerts_in_denominator\endcsname{69}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m2.acc_at_1\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m2.mean_credit\endcsname{0.24}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m2.false_diagnoses\endcsname{7}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m3.fsr_symptomatic\endcsname{0.24}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m3.mitigated_rate\endcsname{0.66}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m3.root_fixed_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m4.uim\endcsname{2703}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m4.regret_raw\endcsname{3.00}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m5.reached\endcsname{5}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m5.median_s\endcsname{326}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m6.mitigated.reached\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m6.mitigated.median_s\endcsname{390}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.blast_radius\endcsname{0.28}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.claim_calls\endcsname{541}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.unlinked_citations\endcsname{5}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m1.ambiguous_excluded\endcsname{44}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.m7.executed_mutating_actions\endcsname{18}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.dollars\endcsname{3.47}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.llm_calls\endcsname{320}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.problems_injected\endcsname{53}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.alerts_in_denominator\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m3.fsr_symptomatic\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m4.uim\endcsname{2369}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m6.mitigated.reached\endcsname{39}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m6.mitigated.median_s\endcsname{481}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m1.ambiguous_excluded\endcsname{48}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.smash_score\endcsname{7.86}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.smash_lo_r1\endcsname{7.86}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.smash_hi_r0\endcsname{7.86}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.f1\endcsname{0.74}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.nrr\endcsname{0.53}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.precision\endcsname{0.76}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.recall\endcsname{0.73}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.incidents_declared\endcsname{50}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.alerts_in_denominator\endcsname{106}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m2.mean_credit\endcsname{0.29}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m2.false_diagnoses\endcsname{9}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m3.fsr_symptomatic\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m3.root_fixed_rate\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m3.agent_attributed_rate\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m4.uim\endcsname{2712}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m4.regret_raw\endcsname{1.15}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m6.mitigated.reached\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m6.mitigated.median_s\endcsname{502}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.blast_radius\endcsname{0.08}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.claim_calls\endcsname{286}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.unlinked_citations\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m1.ambiguous_excluded\endcsname{105}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.m7.executed_mutating_actions\endcsname{48}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.smash_score\endcsname{24.57}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.smash_lo_r1\endcsname{24.57}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.smash_hi_r0\endcsname{24.57}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.f1\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.nrr\endcsname{0.62}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.incidents_declared\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.alerts_in_denominator\endcsname{92}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m2.acc_at_1\endcsname{0.19}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m2.mean_credit\endcsname{0.32}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m2.false_diagnoses\endcsname{22}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m3.mitigated_rate\endcsname{0.52}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m3.agent_attributed_rate\endcsname{0.07}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m4.uim\endcsname{1165}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m4.regret\endcsname{0.49}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m4.regret_raw\endcsname{0.49}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m5.reached\endcsname{11}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m5.median_s\endcsname{311}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m6.mitigated.reached\endcsname{30}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m6.mitigated.median_s\endcsname{351}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.blast_radius\endcsname{0.13}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.claim_calls\endcsname{652}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.refused_actions\endcsname{6}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.unlinked_citations\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m1.ambiguous_excluded\endcsname{68}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.m7.executed_mutating_actions\endcsname{52}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.dollars\endcsname{3.68}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.llm_calls\endcsname{338}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.smash_score\endcsname{22.29}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.smash_lo_r1\endcsname{22.29}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.smash_hi_r0\endcsname{22.29}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.f1\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.nrr\endcsname{0.82}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.precision\endcsname{0.16}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.recall\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.incidents_declared\endcsname{21}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.alerts_in_denominator\endcsname{116}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m2.mean_credit\endcsname{0.29}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m2.false_diagnoses\endcsname{308}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m3.fsr_symptomatic\endcsname{0.24}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m3.root_fixed_rate\endcsname{0.04}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m3.agent_attributed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m4.uim\endcsname{1191}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m4.regret\endcsname{0.50}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m4.regret_raw\endcsname{0.50}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m6.mitigated.reached\endcsname{34}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m6.mitigated.median_s\endcsname{406}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.blast_radius\endcsname{0.07}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.claim_calls\endcsname{1578}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.refused_actions\endcsname{20}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.unlinked_citations\endcsname{31}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m1.ambiguous_excluded\endcsname{82}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.m7.executed_mutating_actions\endcsname{70}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.dollars\endcsname{0.54}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.llm_calls\endcsname{41}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.problems_injected\endcsname{57}
\expandafter\def\csname val@run.astro-episode1.smash_score\endcsname{16.05}
\expandafter\def\csname val@run.astro-episode1.smash_lo_r1\endcsname{16.05}
\expandafter\def\csname val@run.astro-episode1.smash_hi_r0\endcsname{16.05}
\expandafter\def\csname val@run.astro-episode1.m1.f1\endcsname{0.24}
\expandafter\def\csname val@run.astro-episode1.m1.nrr\endcsname{0.67}
\expandafter\def\csname val@run.astro-episode1.m1.precision\endcsname{0.13}
\expandafter\def\csname val@run.astro-episode1.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode1.m1.incidents_declared\endcsname{2}
\expandafter\def\csname val@run.astro-episode1.m1.alerts_in_denominator\endcsname{6}
\expandafter\def\csname val@run.astro-episode1.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1.m2.mean_credit\endcsname{0.18}
\expandafter\def\csname val@run.astro-episode1.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode1.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1.m3.mitigated_rate\endcsname{0.40}
\expandafter\def\csname val@run.astro-episode1.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1.m3.agent_attributed_rate\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode1.m4.uim\endcsname{648}
\expandafter\def\csname val@run.astro-episode1.m4.regret\endcsname{0.64}
\expandafter\def\csname val@run.astro-episode1.m4.regret_raw\endcsname{0.64}
\expandafter\def\csname val@run.astro-episode1.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode1.m6.mitigated.reached\endcsname{2}
\expandafter\def\csname val@run.astro-episode1.m6.mitigated.median_s\endcsname{216}
\expandafter\def\csname val@run.astro-episode1.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1.m7.claim_calls\endcsname{50}
\expandafter\def\csname val@run.astro-episode1.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode1.m7.unlinked_citations\endcsname{3}
\expandafter\def\csname val@run.astro-episode1.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.astro-episode1.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode1.m7.executed_mutating_actions\endcsname{3}
\expandafter\def\csname val@run.astro-episode1.dollars\endcsname{1.40}
\expandafter\def\csname val@run.astro-episode1.llm_calls\endcsname{175}
\expandafter\def\csname val@run.astro-episode1.problems_injected\endcsname{5}
\expandafter\def\csname val@run.astro-episode2.smash_score\endcsname{30.04}
\expandafter\def\csname val@run.astro-episode2.smash_lo_r1\endcsname{30.04}
\expandafter\def\csname val@run.astro-episode2.smash_hi_r0\endcsname{30.04}
\expandafter\def\csname val@run.astro-episode2.m1.f1\endcsname{0.20}
\expandafter\def\csname val@run.astro-episode2.m1.nrr\endcsname{0.18}
\expandafter\def\csname val@run.astro-episode2.m1.precision\endcsname{0.11}
\expandafter\def\csname val@run.astro-episode2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode2.m1.incidents_declared\endcsname{9}
\expandafter\def\csname val@run.astro-episode2.m1.alerts_in_denominator\endcsname{11}
\expandafter\def\csname val@run.astro-episode2.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2.m2.mean_credit\endcsname{0.06}
\expandafter\def\csname val@run.astro-episode2.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode2.m3.fsr_symptomatic\endcsname{0.50}
\expandafter\def\csname val@run.astro-episode2.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode2.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2.m3.agent_attributed_rate\endcsname{0.40}
\expandafter\def\csname val@run.astro-episode2.m4.uim\endcsname{101}
\expandafter\def\csname val@run.astro-episode2.m4.regret\endcsname{0.58}
\expandafter\def\csname val@run.astro-episode2.m4.regret_raw\endcsname{0.58}
\expandafter\def\csname val@run.astro-episode2.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode2.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.astro-episode2.m6.mitigated.median_s\endcsname{685}
\expandafter\def\csname val@run.astro-episode2.m7.blast_radius\endcsname{0.11}
\expandafter\def\csname val@run.astro-episode2.m7.claim_calls\endcsname{61}
\expandafter\def\csname val@run.astro-episode2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode2.m7.unlinked_citations\endcsname{4}
\expandafter\def\csname val@run.astro-episode2.m1.ambiguous_excluded\endcsname{9}
\expandafter\def\csname val@run.astro-episode2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode2.m7.executed_mutating_actions\endcsname{9}
\expandafter\def\csname val@run.astro-episode2.dollars\endcsname{1.37}
\expandafter\def\csname val@run.astro-episode2.llm_calls\endcsname{181}
\expandafter\def\csname val@run.astro-episode2.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode1.smash_score\endcsname{42.27}
\expandafter\def\csname val@run.ob-episode1.smash_lo_r1\endcsname{42.27}
\expandafter\def\csname val@run.ob-episode1.smash_hi_r0\endcsname{42.27}
\expandafter\def\csname val@run.ob-episode1.m1.f1\endcsname{0.36}
\expandafter\def\csname val@run.ob-episode1.m1.nrr\endcsname{0.27}
\expandafter\def\csname val@run.ob-episode1.m1.precision\endcsname{0.22}
\expandafter\def\csname val@run.ob-episode1.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode1.m1.incidents_declared\endcsname{8}
\expandafter\def\csname val@run.ob-episode1.m1.alerts_in_denominator\endcsname{11}
\expandafter\def\csname val@run.ob-episode1.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1.m2.mean_credit\endcsname{0.20}
\expandafter\def\csname val@run.ob-episode1.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.ob-episode1.m3.fsr_symptomatic\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode1.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode1.m3.root_fixed_rate\endcsname{0.40}
\expandafter\def\csname val@run.ob-episode1.m3.agent_attributed_rate\endcsname{0.40}
\expandafter\def\csname val@run.ob-episode1.m4.uim\endcsname{70}
\expandafter\def\csname val@run.ob-episode1.m4.regret\endcsname{0.66}
\expandafter\def\csname val@run.ob-episode1.m4.regret_raw\endcsname{0.66}
\expandafter\def\csname val@run.ob-episode1.m5.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode1.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.ob-episode1.m6.mitigated.median_s\endcsname{431}
\expandafter\def\csname val@run.ob-episode1.m7.blast_radius\endcsname{0.60}
\expandafter\def\csname val@run.ob-episode1.m7.claim_calls\endcsname{47}
\expandafter\def\csname val@run.ob-episode1.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode1.m7.unlinked_citations\endcsname{2}
\expandafter\def\csname val@run.ob-episode1.m1.ambiguous_excluded\endcsname{5}
\expandafter\def\csname val@run.ob-episode1.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode1.m7.executed_mutating_actions\endcsname{5}
\expandafter\def\csname val@run.ob-episode1.dollars\endcsname{1.08}
\expandafter\def\csname val@run.ob-episode1.llm_calls\endcsname{143}
\expandafter\def\csname val@run.ob-episode1.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode2.smash_score\endcsname{51.85}
\expandafter\def\csname val@run.ob-episode2.smash_lo_r1\endcsname{51.85}
\expandafter\def\csname val@run.ob-episode2.smash_hi_r0\endcsname{51.85}
\expandafter\def\csname val@run.ob-episode2.m1.f1\endcsname{0.34}
\expandafter\def\csname val@run.ob-episode2.m1.nrr\endcsname{0.15}
\expandafter\def\csname val@run.ob-episode2.m1.precision\endcsname{0.21}
\expandafter\def\csname val@run.ob-episode2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode2.m1.incidents_declared\endcsname{11}
\expandafter\def\csname val@run.ob-episode2.m1.alerts_in_denominator\endcsname{13}
\expandafter\def\csname val@run.ob-episode2.m2.acc_at_1\endcsname{0.20}
\expandafter\def\csname val@run.ob-episode2.m2.mean_credit\endcsname{0.56}
\expandafter\def\csname val@run.ob-episode2.m2.false_diagnoses\endcsname{1}
\expandafter\def\csname val@run.ob-episode2.m3.fsr_symptomatic\endcsname{0.90}
\expandafter\def\csname val@run.ob-episode2.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode2.m3.root_fixed_rate\endcsname{0.80}
\expandafter\def\csname val@run.ob-episode2.m3.agent_attributed_rate\endcsname{0.40}
\expandafter\def\csname val@run.ob-episode2.m4.uim\endcsname{1129}
\expandafter\def\csname val@run.ob-episode2.m4.regret\endcsname{0.45}
\expandafter\def\csname val@run.ob-episode2.m4.regret_raw\endcsname{0.45}
\expandafter\def\csname val@run.ob-episode2.m5.reached\endcsname{1}
\expandafter\def\csname val@run.ob-episode2.m5.median_s\endcsname{176}
\expandafter\def\csname val@run.ob-episode2.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.ob-episode2.m6.mitigated.median_s\endcsname{560}
\expandafter\def\csname val@run.ob-episode2.m7.blast_radius\endcsname{0.40}
\expandafter\def\csname val@run.ob-episode2.m7.claim_calls\endcsname{73}
\expandafter\def\csname val@run.ob-episode2.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.ob-episode2.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.ob-episode2.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.ob-episode2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode2.m7.executed_mutating_actions\endcsname{5}
\expandafter\def\csname val@run.ob-episode2.dollars\endcsname{1.05}
\expandafter\def\csname val@run.ob-episode2.llm_calls\endcsname{151}
\expandafter\def\csname val@run.ob-episode2.problems_injected\endcsname{5}
\expandafter\def\csname val@run.tt-episode1.smash_score\endcsname{54.74}
\expandafter\def\csname val@run.tt-episode1.smash_lo_r1\endcsname{54.74}
\expandafter\def\csname val@run.tt-episode1.smash_hi_r0\endcsname{54.74}
\expandafter\def\csname val@run.tt-episode1.m1.f1\endcsname{0.44}
\expandafter\def\csname val@run.tt-episode1.m1.nrr\endcsname{0.79}
\expandafter\def\csname val@run.tt-episode1.m1.precision\endcsname{0.29}
\expandafter\def\csname val@run.tt-episode1.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode1.m1.incidents_declared\endcsname{3}
\expandafter\def\csname val@run.tt-episode1.m1.alerts_in_denominator\endcsname{14}
\expandafter\def\csname val@run.tt-episode1.m2.acc_at_1\endcsname{0.40}
\expandafter\def\csname val@run.tt-episode1.m2.mean_credit\endcsname{0.52}
\expandafter\def\csname val@run.tt-episode1.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode1.m3.fsr_symptomatic\endcsname{0.75}
\expandafter\def\csname val@run.tt-episode1.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode1.m3.root_fixed_rate\endcsname{0.60}
\expandafter\def\csname val@run.tt-episode1.m3.agent_attributed_rate\endcsname{0.60}
\expandafter\def\csname val@run.tt-episode1.m4.uim\endcsname{1532}
\expandafter\def\csname val@run.tt-episode1.m4.regret\endcsname{0.45}
\expandafter\def\csname val@run.tt-episode1.m4.regret_raw\endcsname{0.45}
\expandafter\def\csname val@run.tt-episode1.m5.reached\endcsname{2}
\expandafter\def\csname val@run.tt-episode1.m5.median_s\endcsname{129}
\expandafter\def\csname val@run.tt-episode1.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.tt-episode1.m6.mitigated.median_s\endcsname{957}
\expandafter\def\csname val@run.tt-episode1.m7.blast_radius\endcsname{0.44}
\expandafter\def\csname val@run.tt-episode1.m7.claim_calls\endcsname{61}
\expandafter\def\csname val@run.tt-episode1.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode1.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.tt-episode1.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.tt-episode1.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode1.m7.executed_mutating_actions\endcsname{9}
\expandafter\def\csname val@run.tt-episode1.dollars\endcsname{1.19}
\expandafter\def\csname val@run.tt-episode1.llm_calls\endcsname{155}
\expandafter\def\csname val@run.tt-episode1.problems_injected\endcsname{5}
\expandafter\def\csname val@run.tt-episode2.smash_score\endcsname{53.17}
\expandafter\def\csname val@run.tt-episode2.smash_lo_r1\endcsname{53.17}
\expandafter\def\csname val@run.tt-episode2.smash_hi_r0\endcsname{53.17}
\expandafter\def\csname val@run.tt-episode2.m1.f1\endcsname{0.25}
\expandafter\def\csname val@run.tt-episode2.m1.nrr\endcsname{0.18}
\expandafter\def\csname val@run.tt-episode2.m1.precision\endcsname{0.14}
\expandafter\def\csname val@run.tt-episode2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode2.m1.incidents_declared\endcsname{14}
\expandafter\def\csname val@run.tt-episode2.m1.alerts_in_denominator\endcsname{17}
\expandafter\def\csname val@run.tt-episode2.m2.acc_at_1\endcsname{0.40}
\expandafter\def\csname val@run.tt-episode2.m2.mean_credit\endcsname{0.66}
\expandafter\def\csname val@run.tt-episode2.m2.false_diagnoses\endcsname{2}
\expandafter\def\csname val@run.tt-episode2.m3.fsr_symptomatic\endcsname{0.80}
\expandafter\def\csname val@run.tt-episode2.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode2.m3.root_fixed_rate\endcsname{0.60}
\expandafter\def\csname val@run.tt-episode2.m3.agent_attributed_rate\endcsname{0.40}
\expandafter\def\csname val@run.tt-episode2.m4.uim\endcsname{1820}
\expandafter\def\csname val@run.tt-episode2.m4.regret\endcsname{0.44}
\expandafter\def\csname val@run.tt-episode2.m4.regret_raw\endcsname{0.44}
\expandafter\def\csname val@run.tt-episode2.m5.reached\endcsname{2}
\expandafter\def\csname val@run.tt-episode2.m5.median_s\endcsname{176}
\expandafter\def\csname val@run.tt-episode2.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.tt-episode2.m6.mitigated.median_s\endcsname{380}
\expandafter\def\csname val@run.tt-episode2.m7.blast_radius\endcsname{0.33}
\expandafter\def\csname val@run.tt-episode2.m7.claim_calls\endcsname{83}
\expandafter\def\csname val@run.tt-episode2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode2.m7.unlinked_citations\endcsname{2}
\expandafter\def\csname val@run.tt-episode2.m1.ambiguous_excluded\endcsname{9}
\expandafter\def\csname val@run.tt-episode2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode2.m7.executed_mutating_actions\endcsname{6}
\expandafter\def\csname val@run.tt-episode2.dollars\endcsname{1.32}
\expandafter\def\csname val@run.tt-episode2.llm_calls\endcsname{158}
\expandafter\def\csname val@run.tt-episode2.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode3.smash_score\endcsname{15.73}
\expandafter\def\csname val@run.ob-episode3.smash_lo_r1\endcsname{15.73}
\expandafter\def\csname val@run.ob-episode3.smash_hi_r0\endcsname{15.73}
\expandafter\def\csname val@run.ob-episode3.m1.f1\endcsname{0.19}
\expandafter\def\csname val@run.ob-episode3.m1.nrr\endcsname{0.95}
\expandafter\def\csname val@run.ob-episode3.m1.precision\endcsname{0.10}
\expandafter\def\csname val@run.ob-episode3.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode3.m1.incidents_declared\endcsname{1}
\expandafter\def\csname val@run.ob-episode3.m1.alerts_in_denominator\endcsname{22}
\expandafter\def\csname val@run.ob-episode3.m2.acc_at_1\endcsname{0.20}
\expandafter\def\csname val@run.ob-episode3.m2.mean_credit\endcsname{0.40}
\expandafter\def\csname val@run.ob-episode3.m2.false_diagnoses\endcsname{2}
\expandafter\def\csname val@run.ob-episode3.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3.m4.uim\endcsname{3515}
\expandafter\def\csname val@run.ob-episode3.m4.regret\endcsname{0.77}
\expandafter\def\csname val@run.ob-episode3.m4.regret_raw\endcsname{0.77}
\expandafter\def\csname val@run.ob-episode3.m5.reached\endcsname{2}
\expandafter\def\csname val@run.ob-episode3.m5.median_s\endcsname{210}
\expandafter\def\csname val@run.ob-episode3.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode3.m7.blast_radius\endcsname{0.50}
\expandafter\def\csname val@run.ob-episode3.m7.claim_calls\endcsname{86}
\expandafter\def\csname val@run.ob-episode3.m7.refused_actions\endcsname{9}
\expandafter\def\csname val@run.ob-episode3.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.ob-episode3.m1.ambiguous_excluded\endcsname{20}
\expandafter\def\csname val@run.ob-episode3.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode3.m7.executed_mutating_actions\endcsname{18}
\expandafter\def\csname val@run.ob-episode3.dollars\endcsname{2.28}
\expandafter\def\csname val@run.ob-episode3.llm_calls\endcsname{270}
\expandafter\def\csname val@run.ob-episode3.problems_injected\endcsname{10}
\expandafter\def\csname val@run.ob-episode4.smash_score\endcsname{-20.70}
\expandafter\def\csname val@run.ob-episode4.smash_lo_r1\endcsname{-20.70}
\expandafter\def\csname val@run.ob-episode4.smash_hi_r0\endcsname{-20.70}
\expandafter\def\csname val@run.ob-episode4.m1.f1\endcsname{0.13}
\expandafter\def\csname val@run.ob-episode4.m1.nrr\endcsname{0.70}
\expandafter\def\csname val@run.ob-episode4.m1.precision\endcsname{0.07}
\expandafter\def\csname val@run.ob-episode4.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode4.m1.incidents_declared\endcsname{14}
\expandafter\def\csname val@run.ob-episode4.m1.alerts_in_denominator\endcsname{46}
\expandafter\def\csname val@run.ob-episode4.m2.acc_at_1\endcsname{0.20}
\expandafter\def\csname val@run.ob-episode4.m2.mean_credit\endcsname{0.37}
\expandafter\def\csname val@run.ob-episode4.m2.false_diagnoses\endcsname{1}
\expandafter\def\csname val@run.ob-episode4.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4.m4.uim\endcsname{7421}
\expandafter\def\csname val@run.ob-episode4.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode4.m4.regret_raw\endcsname{1.79}
\expandafter\def\csname val@run.ob-episode4.m5.reached\endcsname{4}
\expandafter\def\csname val@run.ob-episode4.m5.median_s\endcsname{154}
\expandafter\def\csname val@run.ob-episode4.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode4.m7.blast_radius\endcsname{0.13}
\expandafter\def\csname val@run.ob-episode4.m7.claim_calls\endcsname{220}
\expandafter\def\csname val@run.ob-episode4.m7.refused_actions\endcsname{3}
\expandafter\def\csname val@run.ob-episode4.m7.unlinked_citations\endcsname{2}
\expandafter\def\csname val@run.ob-episode4.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.ob-episode4.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode4.m7.executed_mutating_actions\endcsname{15}
\expandafter\def\csname val@run.ob-episode4.dollars\endcsname{2.72}
\expandafter\def\csname val@run.ob-episode4.llm_calls\endcsname{255}
\expandafter\def\csname val@run.ob-episode4.problems_injected\endcsname{10}
\expandafter\def\csname val@run.tt-episode3.smash_score\endcsname{56.16}
\expandafter\def\csname val@run.tt-episode3.smash_lo_r1\endcsname{56.16}
\expandafter\def\csname val@run.tt-episode3.smash_hi_r0\endcsname{56.16}
\expandafter\def\csname val@run.tt-episode3.m1.f1\endcsname{0.21}
\expandafter\def\csname val@run.tt-episode3.m1.nrr\endcsname{0.18}
\expandafter\def\csname val@run.tt-episode3.m1.precision\endcsname{0.12}
\expandafter\def\csname val@run.tt-episode3.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode3.m1.incidents_declared\endcsname{14}
\expandafter\def\csname val@run.tt-episode3.m1.alerts_in_denominator\endcsname{17}
\expandafter\def\csname val@run.tt-episode3.m2.acc_at_1\endcsname{0.30}
\expandafter\def\csname val@run.tt-episode3.m2.mean_credit\endcsname{0.54}
\expandafter\def\csname val@run.tt-episode3.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode3.m3.fsr_symptomatic\endcsname{0.65}
\expandafter\def\csname val@run.tt-episode3.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode3.m3.root_fixed_rate\endcsname{0.30}
\expandafter\def\csname val@run.tt-episode3.m3.agent_attributed_rate\endcsname{0.20}
\expandafter\def\csname val@run.tt-episode3.m4.uim\endcsname{2743}
\expandafter\def\csname val@run.tt-episode3.m4.regret\endcsname{0.16}
\expandafter\def\csname val@run.tt-episode3.m4.regret_raw\endcsname{0.16}
\expandafter\def\csname val@run.tt-episode3.m5.reached\endcsname{3}
\expandafter\def\csname val@run.tt-episode3.m5.median_s\endcsname{153}
\expandafter\def\csname val@run.tt-episode3.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.tt-episode3.m6.mitigated.median_s\endcsname{560}
\expandafter\def\csname val@run.tt-episode3.m7.blast_radius\endcsname{0.50}
\expandafter\def\csname val@run.tt-episode3.m7.claim_calls\endcsname{106}
\expandafter\def\csname val@run.tt-episode3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode3.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.tt-episode3.m1.ambiguous_excluded\endcsname{20}
\expandafter\def\csname val@run.tt-episode3.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode3.m7.executed_mutating_actions\endcsname{14}
\expandafter\def\csname val@run.tt-episode3.dollars\endcsname{2.05}
\expandafter\def\csname val@run.tt-episode3.llm_calls\endcsname{224}
\expandafter\def\csname val@run.tt-episode3.problems_injected\endcsname{10}
\expandafter\def\csname val@run.tt-episode4.smash_score\endcsname{-5.18}
\expandafter\def\csname val@run.tt-episode4.smash_lo_r1\endcsname{-5.18}
\expandafter\def\csname val@run.tt-episode4.smash_hi_r0\endcsname{-5.18}
\expandafter\def\csname val@run.tt-episode4.m1.f1\endcsname{0.57}
\expandafter\def\csname val@run.tt-episode4.m1.nrr\endcsname{-7.83}
\expandafter\def\csname val@run.tt-episode4.m1.precision\endcsname{0.40}
\expandafter\def\csname val@run.tt-episode4.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode4.m1.incidents_declared\endcsname{53}
\expandafter\def\csname val@run.tt-episode4.m1.alerts_in_denominator\endcsname{6}
\expandafter\def\csname val@run.tt-episode4.m2.acc_at_1\endcsname{0.60}
\expandafter\def\csname val@run.tt-episode4.m2.mean_credit\endcsname{0.77}
\expandafter\def\csname val@run.tt-episode4.m2.false_diagnoses\endcsname{4}
\expandafter\def\csname val@run.tt-episode4.m3.mitigated_rate\endcsname{0.50}
\expandafter\def\csname val@run.tt-episode4.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4.m3.agent_attributed_rate\endcsname{0.20}
\expandafter\def\csname val@run.tt-episode4.m4.uim\endcsname{27672}
\expandafter\def\csname val@run.tt-episode4.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode4.m4.regret_raw\endcsname{8.54}
\expandafter\def\csname val@run.tt-episode4.m5.reached\endcsname{6}
\expandafter\def\csname val@run.tt-episode4.m5.median_s\endcsname{333}
\expandafter\def\csname val@run.tt-episode4.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.tt-episode4.m6.mitigated.median_s\endcsname{918}
\expandafter\def\csname val@run.tt-episode4.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4.m7.claim_calls\endcsname{881}
\expandafter\def\csname val@run.tt-episode4.m7.refused_actions\endcsname{3}
\expandafter\def\csname val@run.tt-episode4.m7.unlinked_citations\endcsname{6}
\expandafter\def\csname val@run.tt-episode4.m1.ambiguous_excluded\endcsname{74}
\expandafter\def\csname val@run.tt-episode4.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode4.m7.executed_mutating_actions\endcsname{16}
\expandafter\def\csname val@run.tt-episode4.dollars\endcsname{2.50}
\expandafter\def\csname val@run.tt-episode4.llm_calls\endcsname{227}
\expandafter\def\csname val@run.tt-episode4.problems_injected\endcsname{10}
\expandafter\def\csname val@run.astro-episode1-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.astro-episode1-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode1-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m1.alerts_in_denominator\endcsname{7}
\expandafter\def\csname val@run.astro-episode1-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m3.mitigated_rate\endcsname{0.40}
\expandafter\def\csname val@run.astro-episode1-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.m4.uim\endcsname{1009}
\expandafter\def\csname val@run.astro-episode1-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m6.mitigated.reached\endcsname{2}
\expandafter\def\csname val@run.astro-episode1-null.m6.mitigated.median_s\endcsname{195}
\expandafter\def\csname val@run.astro-episode1-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.astro-episode1-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode1-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode1-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.astro-episode2-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.astro-episode2-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode2-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m1.alerts_in_denominator\endcsname{14}
\expandafter\def\csname val@run.astro-episode2-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m3.fsr_symptomatic\endcsname{0.50}
\expandafter\def\csname val@run.astro-episode2-null.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode2-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.m4.uim\endcsname{173}
\expandafter\def\csname val@run.astro-episode2-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.astro-episode2-null.m6.mitigated.median_s\endcsname{246}
\expandafter\def\csname val@run.astro-episode2-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m1.ambiguous_excluded\endcsname{8}
\expandafter\def\csname val@run.astro-episode2-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode2-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode2-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode1-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.ob-episode1-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode1-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m1.alerts_in_denominator\endcsname{12}
\expandafter\def\csname val@run.ob-episode1-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.ob-episode1-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.m4.uim\endcsname{106}
\expandafter\def\csname val@run.ob-episode1-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m6.mitigated.reached\endcsname{3}
\expandafter\def\csname val@run.ob-episode1-null.m6.mitigated.median_s\endcsname{307}
\expandafter\def\csname val@run.ob-episode1-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m1.ambiguous_excluded\endcsname{5}
\expandafter\def\csname val@run.ob-episode1-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode1-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode1-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode2-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.ob-episode2-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode2-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m1.alerts_in_denominator\endcsname{21}
\expandafter\def\csname val@run.ob-episode2-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.m4.uim\endcsname{2508}
\expandafter\def\csname val@run.ob-episode2-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m1.ambiguous_excluded\endcsname{3}
\expandafter\def\csname val@run.ob-episode2-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode2-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode2-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.ob-episode3-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.ob-episode3-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode3-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m1.alerts_in_denominator\endcsname{45}
\expandafter\def\csname val@run.ob-episode3-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.m4.uim\endcsname{4542}
\expandafter\def\csname val@run.ob-episode3-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m1.ambiguous_excluded\endcsname{6}
\expandafter\def\csname val@run.ob-episode3-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode3-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode3-null.problems_injected\endcsname{10}
\expandafter\def\csname val@run.ob-episode4-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.ob-episode4-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.ob-episode4-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m1.alerts_in_denominator\endcsname{45}
\expandafter\def\csname val@run.ob-episode4-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.m4.uim\endcsname{4144}
\expandafter\def\csname val@run.ob-episode4-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m1.ambiguous_excluded\endcsname{13}
\expandafter\def\csname val@run.ob-episode4-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.ob-episode4-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.ob-episode4-null.problems_injected\endcsname{10}
\expandafter\def\csname val@run.tt-episode1-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.tt-episode1-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode1-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m1.alerts_in_denominator\endcsname{14}
\expandafter\def\csname val@run.tt-episode1-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.tt-episode1-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.m4.uim\endcsname{3419}
\expandafter\def\csname val@run.tt-episode1-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m6.mitigated.reached\endcsname{3}
\expandafter\def\csname val@run.tt-episode1-null.m6.mitigated.median_s\endcsname{726}
\expandafter\def\csname val@run.tt-episode1-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m1.ambiguous_excluded\endcsname{9}
\expandafter\def\csname val@run.tt-episode1-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode1-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode1-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.tt-episode2-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.tt-episode2-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode2-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m1.alerts_in_denominator\endcsname{26}
\expandafter\def\csname val@run.tt-episode2-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m3.fsr_symptomatic\endcsname{0.10}
\expandafter\def\csname val@run.tt-episode2-null.m3.mitigated_rate\endcsname{0.20}
\expandafter\def\csname val@run.tt-episode2-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.m4.uim\endcsname{4108}
\expandafter\def\csname val@run.tt-episode2-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m6.mitigated.reached\endcsname{1}
\expandafter\def\csname val@run.tt-episode2-null.m6.mitigated.median_s\endcsname{369}
\expandafter\def\csname val@run.tt-episode2-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m1.ambiguous_excluded\endcsname{9}
\expandafter\def\csname val@run.tt-episode2-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode2-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode2-null.problems_injected\endcsname{5}
\expandafter\def\csname val@run.tt-episode3-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.tt-episode3-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode3-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m1.alerts_in_denominator\endcsname{35}
\expandafter\def\csname val@run.tt-episode3-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.m4.uim\endcsname{16714}
\expandafter\def\csname val@run.tt-episode3-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m1.ambiguous_excluded\endcsname{11}
\expandafter\def\csname val@run.tt-episode3-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode3-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode3-null.problems_injected\endcsname{9}
\expandafter\def\csname val@run.tt-episode4-null.smash_lo_r1\endcsname{6.25}
\expandafter\def\csname val@run.tt-episode4-null.smash_hi_r0\endcsname{41.25}
\expandafter\def\csname val@run.tt-episode4-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.tt-episode4-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m1.alerts_in_denominator\endcsname{14}
\expandafter\def\csname val@run.tt-episode4-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m3.mitigated_rate\endcsname{0.50}
\expandafter\def\csname val@run.tt-episode4-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.m4.uim\endcsname{3240}
\expandafter\def\csname val@run.tt-episode4-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.tt-episode4-null.m6.mitigated.median_s\endcsname{306}
\expandafter\def\csname val@run.tt-episode4-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m1.ambiguous_excluded\endcsname{43}
\expandafter\def\csname val@run.tt-episode4-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.tt-episode4-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.tt-episode4-null.problems_injected\endcsname{10}
\expandafter\def\csname val@run.astro-episode3.smash_score\endcsname{-14.10}
\expandafter\def\csname val@run.astro-episode3.smash_lo_r1\endcsname{-14.10}
\expandafter\def\csname val@run.astro-episode3.smash_hi_r0\endcsname{-14.10}
\expandafter\def\csname val@run.astro-episode3.m1.f1\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode3.m1.nrr\endcsname{-3.00}
\expandafter\def\csname val@run.astro-episode3.m1.precision\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode3.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode3.m1.incidents_declared\endcsname{8}
\expandafter\def\csname val@run.astro-episode3.m1.alerts_in_denominator\endcsname{2}
\expandafter\def\csname val@run.astro-episode3.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3.m2.mean_credit\endcsname{0.18}
\expandafter\def\csname val@run.astro-episode3.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode3.m3.fsr_symptomatic\endcsname{0.20}
\expandafter\def\csname val@run.astro-episode3.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.astro-episode3.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3.m3.agent_attributed_rate\endcsname{0.17}
\expandafter\def\csname val@run.astro-episode3.m4.uim\endcsname{873}
\expandafter\def\csname val@run.astro-episode3.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode3.m4.regret_raw\endcsname{1.83}
\expandafter\def\csname val@run.astro-episode3.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode3.m6.mitigated.reached\endcsname{6}
\expandafter\def\csname val@run.astro-episode3.m6.mitigated.median_s\endcsname{185}
\expandafter\def\csname val@run.astro-episode3.m7.blast_radius\endcsname{0.25}
\expandafter\def\csname val@run.astro-episode3.m7.claim_calls\endcsname{84}
\expandafter\def\csname val@run.astro-episode3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode3.m7.unlinked_citations\endcsname{3}
\expandafter\def\csname val@run.astro-episode3.m1.ambiguous_excluded\endcsname{7}
\expandafter\def\csname val@run.astro-episode3.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode3.m7.executed_mutating_actions\endcsname{4}
\expandafter\def\csname val@run.astro-episode3.dollars\endcsname{2.00}
\expandafter\def\csname val@run.astro-episode3.llm_calls\endcsname{265}
\expandafter\def\csname val@run.astro-episode3.problems_injected\endcsname{9}
\expandafter\def\csname val@run.astro-episode4.smash_score\endcsname{-2.51}
\expandafter\def\csname val@run.astro-episode4.smash_lo_r1\endcsname{-2.51}
\expandafter\def\csname val@run.astro-episode4.smash_hi_r0\endcsname{-2.51}
\expandafter\def\csname val@run.astro-episode4.m1.f1\endcsname{0.80}
\expandafter\def\csname val@run.astro-episode4.m1.nrr\endcsname{-2.17}
\expandafter\def\csname val@run.astro-episode4.m1.precision\endcsname{0.67}
\expandafter\def\csname val@run.astro-episode4.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode4.m1.incidents_declared\endcsname{19}
\expandafter\def\csname val@run.astro-episode4.m1.alerts_in_denominator\endcsname{6}
\expandafter\def\csname val@run.astro-episode4.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4.m2.mean_credit\endcsname{0.18}
\expandafter\def\csname val@run.astro-episode4.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode4.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode4.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@run.astro-episode4.m3.agent_attributed_rate\endcsname{0.10}
\expandafter\def\csname val@run.astro-episode4.m4.uim\endcsname{69}
\expandafter\def\csname val@run.astro-episode4.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode4.m4.regret_raw\endcsname{1.81}
\expandafter\def\csname val@run.astro-episode4.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode4.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.astro-episode4.m6.mitigated.median_s\endcsname{202}
\expandafter\def\csname val@run.astro-episode4.m7.blast_radius\endcsname{0.43}
\expandafter\def\csname val@run.astro-episode4.m7.claim_calls\endcsname{100}
\expandafter\def\csname val@run.astro-episode4.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode4.m7.unlinked_citations\endcsname{2}
\expandafter\def\csname val@run.astro-episode4.m1.ambiguous_excluded\endcsname{14}
\expandafter\def\csname val@run.astro-episode4.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode4.m7.executed_mutating_actions\endcsname{7}
\expandafter\def\csname val@run.astro-episode4.dollars\endcsname{1.76}
\expandafter\def\csname val@run.astro-episode4.llm_calls\endcsname{228}
\expandafter\def\csname val@run.astro-episode4.problems_injected\endcsname{10}
\expandafter\def\csname val@run.astro-episode3-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.astro-episode3-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode3-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m1.alerts_in_denominator\endcsname{4}
\expandafter\def\csname val@run.astro-episode3-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m3.fsr_symptomatic\endcsname{0.10}
\expandafter\def\csname val@run.astro-episode3-null.m3.mitigated_rate\endcsname{0.56}
\expandafter\def\csname val@run.astro-episode3-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.m4.uim\endcsname{477}
\expandafter\def\csname val@run.astro-episode3-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m6.mitigated.reached\endcsname{5}
\expandafter\def\csname val@run.astro-episode3-null.m6.mitigated.median_s\endcsname{884}
\expandafter\def\csname val@run.astro-episode3-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m1.ambiguous_excluded\endcsname{7}
\expandafter\def\csname val@run.astro-episode3-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode3-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode3-null.problems_injected\endcsname{9}
\expandafter\def\csname val@run.astro-episode4-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@run.astro-episode4-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode4-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m1.alerts_in_denominator\endcsname{5}
\expandafter\def\csname val@run.astro-episode4-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m3.fsr_symptomatic\endcsname{0.50}
\expandafter\def\csname val@run.astro-episode4-null.m3.mitigated_rate\endcsname{1.00}
\expandafter\def\csname val@run.astro-episode4-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.m4.uim\endcsname{38}
\expandafter\def\csname val@run.astro-episode4-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m6.mitigated.reached\endcsname{10}
\expandafter\def\csname val@run.astro-episode4-null.m6.mitigated.median_s\endcsname{195}
\expandafter\def\csname val@run.astro-episode4-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m1.ambiguous_excluded\endcsname{19}
\expandafter\def\csname val@run.astro-episode4-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.astro-episode4-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.astro-episode4-null.problems_injected\endcsname{10}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.smash_score\endcsname{-24.23}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.smash_lo_r1\endcsname{-24.23}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.smash_hi_r0\endcsname{-24.23}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.f1\endcsname{0.37}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.nrr\endcsname{0.40}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.precision\endcsname{0.54}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.recall\endcsname{0.28}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.incidents_declared\endcsname{44}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.alerts_in_denominator\endcsname{73}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m2.mean_credit\endcsname{0.14}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m2.false_diagnoses\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m3.mitigated_rate\endcsname{0.55}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m3.root_fixed_rate\endcsname{0.07}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m3.agent_attributed_rate\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m4.uim\endcsname{2323}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m4.regret_raw\endcsname{1.87}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m6.mitigated.reached\endcsname{32}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m6.mitigated.median_s\endcsname{591}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.claim_calls\endcsname{152}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.unlinked_citations\endcsname{23}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m1.ambiguous_excluded\endcsname{96}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.m7.executed_mutating_actions\endcsname{34}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.smash_score\endcsname{-19.81}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.smash_lo_r1\endcsname{-19.81}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.smash_hi_r0\endcsname{-19.81}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.f1\endcsname{0.40}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.nrr\endcsname{0.39}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.precision\endcsname{0.32}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.recall\endcsname{0.52}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.incidents_declared\endcsname{52}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.alerts_in_denominator\endcsname{85}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m2.mean_credit\endcsname{0.29}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m2.false_diagnoses\endcsname{627}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m3.fsr_symptomatic\endcsname{0.26}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m3.mitigated_rate\endcsname{0.66}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m3.agent_attributed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m4.uim\endcsname{2179}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m4.regret_raw\endcsname{1.75}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m6.mitigated.reached\endcsname{38}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m6.mitigated.median_s\endcsname{464}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.claim_calls\endcsname{2405}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.refused_actions\endcsname{11}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.unlinked_citations\endcsname{34}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.m7.executed_mutating_actions\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.dollars\endcsname{0.63}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.llm_calls\endcsname{36}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.smash_score\endcsname{-22.63}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.smash_lo_r1\endcsname{-22.63}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.smash_hi_r0\endcsname{-22.63}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.f1\endcsname{0.27}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.nrr\endcsname{0.51}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.precision\endcsname{0.18}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.recall\endcsname{0.50}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.incidents_declared\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.alerts_in_denominator\endcsname{67}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m2.mean_credit\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m2.false_diagnoses\endcsname{94}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m3.fsr_symptomatic\endcsname{0.26}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m3.mitigated_rate\endcsname{0.47}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m3.root_fixed_rate\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m3.agent_attributed_rate\endcsname{0.04}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m4.uim\endcsname{2190}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m4.regret_raw\endcsname{1.76}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m6.mitigated.reached\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m6.mitigated.median_s\endcsname{547}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.claim_calls\endcsname{540}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.refused_actions\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.unlinked_citations\endcsname{14}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m1.ambiguous_excluded\endcsname{60}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.m7.executed_mutating_actions\endcsname{14}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.dollars\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.llm_calls\endcsname{18}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.problems_injected\endcsname{57}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.alerts_in_denominator\endcsname{89}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m4.uim\endcsname{7649}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m6.mitigated.median_s\endcsname{243}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m1.ambiguous_excluded\endcsname{53}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.smash_score\endcsname{-21.34}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.smash_lo_r1\endcsname{-21.34}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.smash_hi_r0\endcsname{-21.34}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.f1\endcsname{0.30}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.nrr\endcsname{0.28}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.precision\endcsname{0.28}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.recall\endcsname{0.31}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.incidents_declared\endcsname{126}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.alerts_in_denominator\endcsname{174}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m2.mean_credit\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m2.false_diagnoses\endcsname{113}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m3.mitigated_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m4.uim\endcsname{13473}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m4.regret_raw\endcsname{1.76}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m5.median_s\endcsname{160}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m6.mitigated.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.claim_calls\endcsname{664}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.unlinked_citations\endcsname{72}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m1.ambiguous_excluded\endcsname{104}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.m7.executed_mutating_actions\endcsname{178}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.smash_score\endcsname{13.80}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.smash_lo_r1\endcsname{13.80}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.smash_hi_r0\endcsname{13.80}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.f1\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.nrr\endcsname{0.27}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.precision\endcsname{0.48}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.recall\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.incidents_declared\endcsname{72}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.alerts_in_denominator\endcsname{99}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m2.mean_credit\endcsname{0.72}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m2.false_diagnoses\endcsname{899}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m3.mitigated_rate\endcsname{0.12}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m3.agent_attributed_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m4.uim\endcsname{7048}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m4.regret\endcsname{0.92}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m4.regret_raw\endcsname{0.92}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m5.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m5.median_s\endcsname{204}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m6.mitigated.reached\endcsname{7}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m6.mitigated.median_s\endcsname{364}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.blast_radius\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.claim_calls\endcsname{4327}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.refused_actions\endcsname{28}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.unlinked_citations\endcsname{25}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m1.ambiguous_excluded\endcsname{61}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.m7.executed_mutating_actions\endcsname{36}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.dollars\endcsname{0.81}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.llm_calls\endcsname{39}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.problems_injected\endcsname{57}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.alerts_in_denominator\endcsname{48}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m3.fsr_symptomatic\endcsname{0.01}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m3.mitigated_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m4.uim\endcsname{30658}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m6.mitigated.reached\endcsname{9}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m6.mitigated.median_s\endcsname{244}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m1.ambiguous_excluded\endcsname{163}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.smash_score\endcsname{3.12}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.smash_lo_r1\endcsname{3.12}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.smash_hi_r0\endcsname{3.12}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.f1\endcsname{0.27}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.nrr\endcsname{0.74}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.precision\endcsname{0.45}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.recall\endcsname{0.19}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.incidents_declared\endcsname{15}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.alerts_in_denominator\endcsname{57}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m2.mean_credit\endcsname{0.06}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m2.false_diagnoses\endcsname{4}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m3.fsr_symptomatic\endcsname{0.01}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m4.uim\endcsname{31428}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m4.regret_raw\endcsname{1.03}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m6.mitigated.median_s\endcsname{276}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.claim_calls\endcsname{26}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.unlinked_citations\endcsname{4}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m1.ambiguous_excluded\endcsname{165}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.m7.executed_mutating_actions\endcsname{12}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.smash_score\endcsname{-1.13}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.smash_lo_r1\endcsname{-1.13}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.smash_hi_r0\endcsname{-1.13}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.alerts_in_denominator\endcsname{55}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m3.fsr_symptomatic\endcsname{0.01}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m3.mitigated_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m4.uim\endcsname{31644}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m4.regret_raw\endcsname{1.03}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m6.mitigated.reached\endcsname{9}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m6.mitigated.median_s\endcsname{245}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m1.ambiguous_excluded\endcsname{156}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.alerts_in_denominator\endcsname{53}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m3.fsr_symptomatic\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m4.uim\endcsname{1270}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m6.mitigated.reached\endcsname{39}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m6.mitigated.median_s\endcsname{392}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m1.ambiguous_excluded\endcsname{56}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.smash_score\endcsname{-9.06}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.smash_lo_r1\endcsname{-9.06}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.smash_hi_r0\endcsname{-9.06}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.f1\endcsname{0.08}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.nrr\endcsname{0.55}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.precision\endcsname{0.04}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.incidents_declared\endcsname{31}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.alerts_in_denominator\endcsname{69}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m2.acc_at_1\endcsname{0.10}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m2.mean_credit\endcsname{0.21}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m2.false_diagnoses\endcsname{23}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m3.fsr_symptomatic\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m3.mitigated_rate\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m3.root_fixed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m3.agent_attributed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m4.uim\endcsname{1738}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m4.regret_raw\endcsname{1.37}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m5.reached\endcsname{8}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m5.median_s\endcsname{283}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m6.mitigated.reached\endcsname{34}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m6.mitigated.median_s\endcsname{471}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.blast_radius\endcsname{0.56}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.claim_calls\endcsname{626}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.unlinked_citations\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m1.ambiguous_excluded\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.m7.executed_mutating_actions\endcsname{9}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.dollars\endcsname{1.21}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.llm_calls\endcsname{264}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.smash_score\endcsname{-13.86}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.smash_lo_r1\endcsname{-13.86}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.smash_hi_r0\endcsname{-13.86}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.nrr\endcsname{-1.04}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.incidents_declared\endcsname{110}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.alerts_in_denominator\endcsname{54}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m2.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m2.mean_credit\endcsname{0.02}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m3.fsr_symptomatic\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m3.mitigated_rate\endcsname{0.66}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m4.uim\endcsname{1789}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m4.regret_raw\endcsname{1.41}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m5.reached\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m5.median_s\endcsname{249}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m6.mitigated.reached\endcsname{38}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m6.mitigated.median_s\endcsname{393}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m7.claim_calls\endcsname{2996}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m1.ambiguous_excluded\endcsname{56}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.dollars\endcsname{1.54}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.llm_calls\endcsname{356}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.smash_score\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.smash_lo_r1\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.smash_hi_r0\endcsname{0.09}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.f1\endcsname{0.35}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.nrr\endcsname{0.81}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.precision\endcsname{0.22}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.recall\endcsname{0.83}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.incidents_declared\endcsname{10}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.alerts_in_denominator\endcsname{52}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m2.mean_credit\endcsname{0.16}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m2.false_diagnoses\endcsname{17}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m3.fsr_symptomatic\endcsname{0.23}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m3.mitigated_rate\endcsname{0.66}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m4.uim\endcsname{1486}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m4.regret_raw\endcsname{1.17}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m5.median_s\endcsname{173}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m6.mitigated.reached\endcsname{38}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m6.mitigated.median_s\endcsname{436}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.claim_calls\endcsname{515}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.m7.executed_mutating_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.dollars\endcsname{1.49}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.llm_calls\endcsname{306}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.problems_injected\endcsname{58}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.alerts_in_denominator\endcsname{86}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m4.uim\endcsname{7820}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m6.mitigated.median_s\endcsname{242}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m1.ambiguous_excluded\endcsname{56}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.smash_score\endcsname{4.43}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.smash_lo_r1\endcsname{4.43}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.smash_hi_r0\endcsname{4.43}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.f1\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.nrr\endcsname{-0.31}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.incidents_declared\endcsname{123}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.alerts_in_denominator\endcsname{94}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m2.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m2.mean_credit\endcsname{0.39}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m2.false_diagnoses\endcsname{87}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m3.fsr_symptomatic\endcsname{0.07}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m3.mitigated_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m3.agent_attributed_rate\endcsname{0.11}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m4.uim\endcsname{7381}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m4.regret\endcsname{0.94}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m4.regret_raw\endcsname{0.94}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m5.reached\endcsname{5}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m5.median_s\endcsname{166}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m6.mitigated.reached\endcsname{9}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m6.mitigated.median_s\endcsname{242}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.blast_radius\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.claim_calls\endcsname{2432}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.refused_actions\endcsname{25}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.unlinked_citations\endcsname{12}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m1.ambiguous_excluded\endcsname{55}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.m7.executed_mutating_actions\endcsname{35}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.dollars\endcsname{1.60}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.llm_calls\endcsname{255}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.smash_score\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.smash_lo_r1\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.smash_hi_r0\endcsname{0.49}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.nrr\endcsname{-0.63}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.incidents_declared\endcsname{142}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.alerts_in_denominator\endcsname{87}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m3.fsr_symptomatic\endcsname{0.05}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m3.mitigated_rate\endcsname{0.14}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m4.uim\endcsname{7712}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m4.regret\endcsname{0.99}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m4.regret_raw\endcsname{0.99}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m6.mitigated.median_s\endcsname{241}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m7.claim_calls\endcsname{4222}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m1.ambiguous_excluded\endcsname{55}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.dollars\endcsname{1.73}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.llm_calls\endcsname{238}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.problems_injected\endcsname{59}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.smash_score\endcsname{1.07}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.smash_lo_r1\endcsname{1.07}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.smash_hi_r0\endcsname{1.07}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.f1\endcsname{0.05}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.nrr\endcsname{0.95}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.incidents_declared\endcsname{4}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.alerts_in_denominator\endcsname{81}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m2.acc_at_1\endcsname{0.08}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m2.mean_credit\endcsname{0.16}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m2.false_diagnoses\endcsname{4}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m3.fsr_symptomatic\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m3.mitigated_rate\endcsname{0.12}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m3.root_fixed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m4.uim\endcsname{33540}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m4.regret_raw\endcsname{1.07}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m5.reached\endcsname{5}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m5.median_s\endcsname{292}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m6.mitigated.reached\endcsname{7}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m6.mitigated.median_s\endcsname{382}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.blast_radius\endcsname{0.63}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.claim_calls\endcsname{207}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.unlinked_citations\endcsname{3}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m1.ambiguous_excluded\endcsname{173}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.m7.executed_mutating_actions\endcsname{19}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.dollars\endcsname{1.53}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.llm_calls\endcsname{216}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.smash_score\endcsname{24.45}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.smash_lo_r1\endcsname{24.45}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.smash_hi_r0\endcsname{24.45}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.f1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.nrr\endcsname{-2.29}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.precision\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.recall\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.incidents_declared\endcsname{227}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.alerts_in_denominator\endcsname{69}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m3.fsr_symptomatic\endcsname{0.01}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m3.mitigated_rate\endcsname{0.15}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m4.uim\endcsname{9664}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m4.regret\endcsname{0.31}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m4.regret_raw\endcsname{0.31}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m6.mitigated.reached\endcsname{9}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m6.mitigated.median_s\endcsname{368}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m7.claim_calls\endcsname{4172}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m1.ambiguous_excluded\endcsname{158}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.dollars\endcsname{1.54}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.llm_calls\endcsname{216}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.smash_score\endcsname{24.58}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.smash_lo_r1\endcsname{24.58}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.smash_hi_r0\endcsname{24.58}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.f1\endcsname{0.06}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.nrr\endcsname{0.98}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.precision\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.incidents_declared\endcsname{1}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.alerts_in_denominator\endcsname{62}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m2.mean_credit\endcsname{0.12}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m2.false_diagnoses\endcsname{4}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m3.fsr_symptomatic\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m3.mitigated_rate\endcsname{0.13}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m4.uim\endcsname{10876}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m4.regret\endcsname{0.35}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m4.regret_raw\endcsname{0.35}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m5.reached\endcsname{2}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m5.median_s\endcsname{188}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m6.mitigated.reached\endcsname{8}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m6.mitigated.median_s\endcsname{255}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.blast_radius\endcsname{0.07}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.claim_calls\endcsname{174}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.unlinked_citations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m1.ambiguous_excluded\endcsname{161}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.m7.executed_mutating_actions\endcsname{14}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.dollars\endcsname{1.67}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.llm_calls\endcsname{234}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.problems_injected\endcsname{60}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.smash_lo_r1\endcsname{11.83}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.smash_hi_r0\endcsname{46.83}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.f1\endcsname{0.59}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.nrr\endcsname{0.65}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.precision\endcsname{0.55}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.recall\endcsname{0.64}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.incidents_declared\endcsname{50}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.alerts_in_denominator\endcsname{144}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m2.mean_credit\endcsname{0.31}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m2.false_diagnoses\endcsname{12}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m3.fsr_symptomatic\endcsname{0.29}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m3.mitigated_rate\endcsname{0.67}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m3.root_fixed_rate\endcsname{0.33}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m3.agent_attributed_rate\endcsname{0.16}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m4.uim\endcsname{2944}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m5.reached\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m6.mitigated.reached\endcsname{37}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m6.mitigated.median_s\endcsname{755}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.blast_radius\endcsname{0.15}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.claim_calls\endcsname{412}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.unlinked_citations\endcsname{29}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m1.ambiguous_excluded\endcsname{105}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.m7.executed_mutating_actions\endcsname{46}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.problems_injected\endcsname{55}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.smash_lo_r1\endcsname{4.85}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.smash_hi_r0\endcsname{39.85}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.f1\endcsname{0.15}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.nrr\endcsname{0.71}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.precision\endcsname{0.08}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.incidents_declared\endcsname{26}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.alerts_in_denominator\endcsname{91}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m2.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m2.mean_credit\endcsname{0.11}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m3.fsr_symptomatic\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m3.mitigated_rate\endcsname{0.60}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m3.root_fixed_rate\endcsname{0.13}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m4.uim\endcsname{8544}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m5.reached\endcsname{4}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m5.median_s\endcsname{324}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m6.mitigated.reached\endcsname{33}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m6.mitigated.median_s\endcsname{685}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.blast_radius\endcsname{0.25}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.claim_calls\endcsname{347}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.unlinked_citations\endcsname{7}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.m7.executed_mutating_actions\endcsname{16}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.dollars\endcsname{3.56}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.llm_calls\endcsname{309}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.problems_injected\endcsname{55}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.smash_lo_r1\endcsname{13.74}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.smash_hi_r0\endcsname{48.74}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.f1\endcsname{0.31}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.nrr\endcsname{0.89}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.precision\endcsname{0.20}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.recall\endcsname{0.69}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.incidents_declared\endcsname{19}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.alerts_in_denominator\endcsname{168}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m2.acc_at_1\endcsname{0.33}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m2.mean_credit\endcsname{0.46}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m2.false_diagnoses\endcsname{175}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m3.fsr_symptomatic\endcsname{0.23}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m3.mitigated_rate\endcsname{0.65}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m3.agent_attributed_rate\endcsname{0.03}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m4.uim\endcsname{4703}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m5.reached\endcsname{18}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m5.median_s\endcsname{113}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m6.mitigated.reached\endcsname{36}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m6.mitigated.median_s\endcsname{624}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.blast_radius\endcsname{0.17}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.claim_calls\endcsname{882}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.refused_actions\endcsname{14}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.unlinked_citations\endcsname{27}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m1.ambiguous_excluded\endcsname{59}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.violations\endcsname{0}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.m7.executed_mutating_actions\endcsname{94}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.dollars\endcsname{0.39}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.llm_calls\endcsname{35}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.problems_injected\endcsname{55}
\expandafter\def\csname val@long.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m1.alerts_in_denominator\endcsname{67}
\expandafter\def\csname val@long.b0-null.m1.alerts_in_denominator.min\endcsname{55}
\expandafter\def\csname val@long.b0-null.m1.alerts_in_denominator.max\endcsname{89}
\expandafter\def\csname val@long.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_excluded\endcsname{97}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_excluded.min\endcsname{49}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_excluded.max\endcsname{184}
\expandafter\def\csname val@long.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_share\endcsname{0.54}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long.b0-null.m1.ambiguous_share.max\endcsname{0.76}
\expandafter\def\csname val@long.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.fsr\endcsname{0.16}
\expandafter\def\csname val@long.b0-null.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long.b0-null.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long.b0-null.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@long.b0-null.m3.fsr_symptomatic.min\endcsname{0.04}
\expandafter\def\csname val@long.b0-null.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate\endcsname{0.32}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.08}
\expandafter\def\csname val@long.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m3.cleared_without_agent_count\endcsname{2.67}
\expandafter\def\csname val@long.b0-null.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m3.cleared_without_agent_count.max\endcsname{4.00}
\expandafter\def\csname val@long.b0-null.m3.repairable_count\endcsname{27.33}
\expandafter\def\csname val@long.b0-null.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long.b0-null.m3.repairable_count.max\endcsname{40.00}
\expandafter\def\csname val@long.b0-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.regret_raw.min\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.regret_raw.max\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m4.uim\endcsname{15829}
\expandafter\def\csname val@long.b0-null.m4.uim.min\endcsname{1244}
\expandafter\def\csname val@long.b0-null.m4.uim.max\endcsname{38181}
\expandafter\def\csname val@long.b0-null.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long.b0-null.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.b0-null.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long.b0-null.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.b0-null.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m4.offered_requests\endcsname{28212.10}
\expandafter\def\csname val@long.b0-null.m4.offered_requests.min\endcsname{1530.35}
\expandafter\def\csname val@long.b0-null.m4.offered_requests.max\endcsname{67092.50}
\expandafter\def\csname val@long.b0-null.m4.load_live_share\endcsname{0.85}
\expandafter\def\csname val@long.b0-null.m4.load_live_share.min\endcsname{0.56}
\expandafter\def\csname val@long.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m5.injected\endcsname{59}
\expandafter\def\csname val@long.b0-null.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long.b0-null.m5.injected.max\endcsname{60}
\expandafter\def\csname val@long.b0-null.m6.mitigated.median_s\endcsname{302}
\expandafter\def\csname val@long.b0-null.m6.mitigated.median_s.min\endcsname{244}
\expandafter\def\csname val@long.b0-null.m6.mitigated.median_s.max\endcsname{375}
\expandafter\def\csname val@long.b0-null.m6.mitigated.p90_s\endcsname{777}
\expandafter\def\csname val@long.b0-null.m6.mitigated.p90_s.min\endcsname{451}
\expandafter\def\csname val@long.b0-null.m6.mitigated.p90_s.max\endcsname{1268}
\expandafter\def\csname val@long.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m6.mitigated.reached\endcsname{19.0}
\expandafter\def\csname val@long.b0-null.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long.b0-null.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long.b0-null.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long.b0-null.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long.b0-null.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long.b0-null.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@long.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m1.f1\endcsname{0.46}
\expandafter\def\csname val@long.b1-runbook.m1.f1.min\endcsname{0.35}
\expandafter\def\csname val@long.b1-runbook.m1.f1.max\endcsname{0.64}
\expandafter\def\csname val@long.b1-runbook.m1.precision\endcsname{0.46}
\expandafter\def\csname val@long.b1-runbook.m1.precision.min\endcsname{0.28}
\expandafter\def\csname val@long.b1-runbook.m1.precision.max\endcsname{0.68}
\expandafter\def\csname val@long.b1-runbook.m1.recall\endcsname{0.48}
\expandafter\def\csname val@long.b1-runbook.m1.recall.min\endcsname{0.38}
\expandafter\def\csname val@long.b1-runbook.m1.recall.max\endcsname{0.60}
\expandafter\def\csname val@long.b1-runbook.m1.nrr\endcsname{0.54}
\expandafter\def\csname val@long.b1-runbook.m1.nrr.min\endcsname{0.42}
\expandafter\def\csname val@long.b1-runbook.m1.nrr.max\endcsname{0.63}
\expandafter\def\csname val@long.b1-runbook.m1.alerts_in_denominator\endcsname{127}
\expandafter\def\csname val@long.b1-runbook.m1.alerts_in_denominator.min\endcsname{90}
\expandafter\def\csname val@long.b1-runbook.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long.b1-runbook.m1.incidents_declared\endcsname{61}
\expandafter\def\csname val@long.b1-runbook.m1.incidents_declared.min\endcsname{33}
\expandafter\def\csname val@long.b1-runbook.m1.incidents_declared.max\endcsname{102}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_excluded\endcsname{126}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_excluded.min\endcsname{102}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_excluded.max\endcsname{163}
\expandafter\def\csname val@long.b1-runbook.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_share\endcsname{0.50}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long.b1-runbook.m1.ambiguous_share.max\endcsname{0.64}
\expandafter\def\csname val@long.b1-runbook.m1.f1_overlap\endcsname{0.56}
\expandafter\def\csname val@long.b1-runbook.m1.f1_overlap.min\endcsname{0.41}
\expandafter\def\csname val@long.b1-runbook.m1.f1_overlap.max\endcsname{0.82}
\expandafter\def\csname val@long.b1-runbook.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m1.incident_precision\endcsname{0.90}
\expandafter\def\csname val@long.b1-runbook.m1.incident_precision.min\endcsname{0.79}
\expandafter\def\csname val@long.b1-runbook.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m2.mean_credit\endcsname{0.33}
\expandafter\def\csname val@long.b1-runbook.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@long.b1-runbook.m2.mean_credit.max\endcsname{0.58}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_1\endcsname{0.01}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_3\endcsname{0.01}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m2.acc_at_3.max\endcsname{0.03}
\expandafter\def\csname val@long.b1-runbook.m2.services_overlap_mean\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m2.services_overlap_mean.min\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.category\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.category.min\endcsname{0.03}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.category.max\endcsname{0.16}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.services\endcsname{0.53}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.services.min\endcsname{0.29}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.services.max\endcsname{0.83}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.artifact\endcsname{0.36}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.artifact.min\endcsname{0.05}
\expandafter\def\csname val@long.b1-runbook.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@long.b1-runbook.m2.false_diagnoses\endcsname{13}
\expandafter\def\csname val@long.b1-runbook.m2.false_diagnoses.min\endcsname{7}
\expandafter\def\csname val@long.b1-runbook.m2.false_diagnoses.max\endcsname{21}
\expandafter\def\csname val@long.b1-runbook.m2.loc_at_1\endcsname{0.36}
\expandafter\def\csname val@long.b1-runbook.m2.loc_at_1.min\endcsname{0.05}
\expandafter\def\csname val@long.b1-runbook.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long.b1-runbook.m2.committed_claims\endcsname{60.67}
\expandafter\def\csname val@long.b1-runbook.m2.committed_claims.min\endcsname{37.00}
\expandafter\def\csname val@long.b1-runbook.m2.committed_claims.max\endcsname{97.00}
\expandafter\def\csname val@long.b1-runbook.m2.claim_precision\endcsname{0.72}
\expandafter\def\csname val@long.b1-runbook.m2.claim_precision.min\endcsname{0.43}
\expandafter\def\csname val@long.b1-runbook.m2.claim_precision.max\endcsname{0.89}
\expandafter\def\csname val@long.b1-runbook.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@long.b1-runbook.m3.fsr.min\endcsname{0.02}
\expandafter\def\csname val@long.b1-runbook.m3.fsr.max\endcsname{0.39}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_symptomatic\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_symptomatic.max\endcsname{0.23}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate\endcsname{0.24}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate.min\endcsname{0.03}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate.max\endcsname{0.57}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate_symptomatic\endcsname{0.14}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long.b1-runbook.m3.agent_attributed_rate\endcsname{0.16}
\expandafter\def\csname val@long.b1-runbook.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.agent_attributed_rate.max\endcsname{0.29}
\expandafter\def\csname val@long.b1-runbook.m3.root_fixed_rate\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.root_fixed_rate.max\endcsname{0.21}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_agent\endcsname{0.04}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.fsr_agent.max\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m3.repaired_rate\endcsname{0.04}
\expandafter\def\csname val@long.b1-runbook.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.repaired_rate.max\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m3.cleared_without_agent_count\endcsname{0.33}
\expandafter\def\csname val@long.b1-runbook.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m3.repairable_count\endcsname{26.33}
\expandafter\def\csname val@long.b1-runbook.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long.b1-runbook.m3.repairable_count.max\endcsname{38.00}
\expandafter\def\csname val@long.b1-runbook.m4.regret\endcsname{0.97}
\expandafter\def\csname val@long.b1-runbook.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long.b1-runbook.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m4.regret_raw\endcsname{1.05}
\expandafter\def\csname val@long.b1-runbook.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long.b1-runbook.m4.regret_raw.max\endcsname{1.24}
\expandafter\def\csname val@long.b1-runbook.m4.uim\endcsname{18761}
\expandafter\def\csname val@long.b1-runbook.m4.uim.min\endcsname{1155}
\expandafter\def\csname val@long.b1-runbook.m4.uim.max\endcsname{47197}
\expandafter\def\csname val@long.b1-runbook.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long.b1-runbook.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.b1-runbook.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long.b1-runbook.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m4.offered_requests\endcsname{27462.55}
\expandafter\def\csname val@long.b1-runbook.m4.offered_requests.min\endcsname{1454.79}
\expandafter\def\csname val@long.b1-runbook.m4.offered_requests.max\endcsname{65898.40}
\expandafter\def\csname val@long.b1-runbook.m4.load_live_share\endcsname{0.78}
\expandafter\def\csname val@long.b1-runbook.m4.load_live_share.min\endcsname{0.35}
\expandafter\def\csname val@long.b1-runbook.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.b1-runbook.m5.median_s\endcsname{132}
\expandafter\def\csname val@long.b1-runbook.m5.median_s.min\endcsname{132}
\expandafter\def\csname val@long.b1-runbook.m5.median_s.max\endcsname{132}
\expandafter\def\csname val@long.b1-runbook.m5.p90_s\endcsname{563}
\expandafter\def\csname val@long.b1-runbook.m5.p90_s.min\endcsname{563}
\expandafter\def\csname val@long.b1-runbook.m5.p90_s.max\endcsname{563}
\expandafter\def\csname val@long.b1-runbook.m5.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m5.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m5.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m5.reached\endcsname{0.7}
\expandafter\def\csname val@long.b1-runbook.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.b1-runbook.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@long.b1-runbook.m5.injected\endcsname{57}
\expandafter\def\csname val@long.b1-runbook.m5.injected.min\endcsname{55}
\expandafter\def\csname val@long.b1-runbook.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.median_s\endcsname{443}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.median_s.min\endcsname{371}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.median_s.max\endcsname{491}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.p90_s\endcsname{780}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.p90_s.min\endcsname{374}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.p90_s.max\endcsname{1353}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.reached\endcsname{14.0}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.reached.min\endcsname{2.0}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.reached.max\endcsname{33.0}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@long.b1-runbook.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.median_s\endcsname{486}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.median_s.min\endcsname{483}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.median_s.max\endcsname{489}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.p90_s\endcsname{1460}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.p90_s.min\endcsname{920}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.p90_s.max\endcsname{2001}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.reached\endcsname{5.3}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.reached.max\endcsname{12.0}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@long.b1-runbook.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long.b1-runbook.m7.blast_radius\endcsname{0.04}
\expandafter\def\csname val@long.b1-runbook.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m7.blast_radius.max\endcsname{0.09}
\expandafter\def\csname val@long.b1-runbook.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.m7.out_of_scope_actions\endcsname{2}
\expandafter\def\csname val@long.b1-runbook.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long.b1-runbook.m7.unscoped_actions\endcsname{2}
\expandafter\def\csname val@long.b1-runbook.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.unscoped_actions.max\endcsname{4}
\expandafter\def\csname val@long.b1-runbook.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.executed_mutating_actions\endcsname{60}
\expandafter\def\csname val@long.b1-runbook.m7.executed_mutating_actions.min\endcsname{37}
\expandafter\def\csname val@long.b1-runbook.m7.executed_mutating_actions.max\endcsname{95}
\expandafter\def\csname val@long.b1-runbook.m7.claim_calls\endcsname{416}
\expandafter\def\csname val@long.b1-runbook.m7.claim_calls.min\endcsname{284}
\expandafter\def\csname val@long.b1-runbook.m7.claim_calls.max\endcsname{651}
\expandafter\def\csname val@long.b1-runbook.m7.max_mutations_per_tick\endcsname{9.33}
\expandafter\def\csname val@long.b1-runbook.m7.max_mutations_per_tick.min\endcsname{7.00}
\expandafter\def\csname val@long.b1-runbook.m7.max_mutations_per_tick.max\endcsname{13.00}
\expandafter\def\csname val@long.b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@long.b1-runbook.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.m7.refused_actions.max\endcsname{2}
\expandafter\def\csname val@long.b1-runbook.m7.unlinked_citations\endcsname{26.00}
\expandafter\def\csname val@long.b1-runbook.m7.unlinked_citations.min\endcsname{16.00}
\expandafter\def\csname val@long.b1-runbook.m7.unlinked_citations.max\endcsname{32.00}
\expandafter\def\csname val@long.react-b2.m1.f1\endcsname{0.07}
\expandafter\def\csname val@long.react-b2.m1.f1.min\endcsname{0.04}
\expandafter\def\csname val@long.react-b2.m1.f1.max\endcsname{0.09}
\expandafter\def\csname val@long.react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@long.react-b2.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long.react-b2.m1.precision.max\endcsname{0.05}
\expandafter\def\csname val@long.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.nrr\endcsname{0.24}
\expandafter\def\csname val@long.react-b2.m1.nrr.min\endcsname{0.11}
\expandafter\def\csname val@long.react-b2.m1.nrr.max\endcsname{0.32}
\expandafter\def\csname val@long.react-b2.m1.alerts_in_denominator\endcsname{67}
\expandafter\def\csname val@long.react-b2.m1.alerts_in_denominator.min\endcsname{53}
\expandafter\def\csname val@long.react-b2.m1.alerts_in_denominator.max\endcsname{92}
\expandafter\def\csname val@long.react-b2.m1.incidents_declared\endcsname{50}
\expandafter\def\csname val@long.react-b2.m1.incidents_declared.min\endcsname{37}
\expandafter\def\csname val@long.react-b2.m1.incidents_declared.max\endcsname{63}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_excluded\endcsname{96}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_excluded.min\endcsname{53}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_excluded.max\endcsname{172}
\expandafter\def\csname val@long.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_share\endcsname{0.56}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long.react-b2.m1.ambiguous_share.max\endcsname{0.76}
\expandafter\def\csname val@long.react-b2.m1.f1_overlap\endcsname{0.20}
\expandafter\def\csname val@long.react-b2.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long.react-b2.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long.react-b2.m1.incident_precision.min\endcsname{0.92}
\expandafter\def\csname val@long.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m2.mean_credit\endcsname{0.15}
\expandafter\def\csname val@long.react-b2.m2.mean_credit.min\endcsname{0.07}
\expandafter\def\csname val@long.react-b2.m2.mean_credit.max\endcsname{0.24}
\expandafter\def\csname val@long.react-b2.m2.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@long.react-b2.m2.acc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long.react-b2.m2.acc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long.react-b2.m2.acc_at_3\endcsname{0.08}
\expandafter\def\csname val@long.react-b2.m2.acc_at_3.min\endcsname{0.05}
\expandafter\def\csname val@long.react-b2.m2.acc_at_3.max\endcsname{0.14}
\expandafter\def\csname val@long.react-b2.m2.services_overlap_mean\endcsname{0.84}
\expandafter\def\csname val@long.react-b2.m2.services_overlap_mean.min\endcsname{0.67}
\expandafter\def\csname val@long.react-b2.m2.services_overlap_mean.max\endcsname{0.97}
\expandafter\def\csname val@long.react-b2.m2.component_rates.category\endcsname{0.18}
\expandafter\def\csname val@long.react-b2.m2.component_rates.category.min\endcsname{0.10}
\expandafter\def\csname val@long.react-b2.m2.component_rates.category.max\endcsname{0.29}
\expandafter\def\csname val@long.react-b2.m2.component_rates.services\endcsname{0.19}
\expandafter\def\csname val@long.react-b2.m2.component_rates.services.min\endcsname{0.05}
\expandafter\def\csname val@long.react-b2.m2.component_rates.services.max\endcsname{0.33}
\expandafter\def\csname val@long.react-b2.m2.component_rates.artifact\endcsname{0.10}
\expandafter\def\csname val@long.react-b2.m2.component_rates.artifact.min\endcsname{0.07}
\expandafter\def\csname val@long.react-b2.m2.component_rates.artifact.max\endcsname{0.14}
\expandafter\def\csname val@long.react-b2.m2.false_diagnoses\endcsname{11}
\expandafter\def\csname val@long.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m2.false_diagnoses.max\endcsname{24}
\expandafter\def\csname val@long.react-b2.m2.loc_at_1\endcsname{0.08}
\expandafter\def\csname val@long.react-b2.m2.loc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long.react-b2.m2.loc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long.react-b2.m2.committed_claims\endcsname{29.67}
\expandafter\def\csname val@long.react-b2.m2.committed_claims.min\endcsname{6.00}
\expandafter\def\csname val@long.react-b2.m2.committed_claims.max\endcsname{58.00}
\expandafter\def\csname val@long.react-b2.m2.claim_precision\endcsname{0.73}
\expandafter\def\csname val@long.react-b2.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m3.fsr\endcsname{0.18}
\expandafter\def\csname val@long.react-b2.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long.react-b2.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long.react-b2.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@long.react-b2.m3.fsr_symptomatic.min\endcsname{0.02}
\expandafter\def\csname val@long.react-b2.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate\endcsname{0.30}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate.max\endcsname{0.60}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.22}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.02}
\expandafter\def\csname val@long.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long.react-b2.m3.agent_attributed_rate\endcsname{0.04}
\expandafter\def\csname val@long.react-b2.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m3.agent_attributed_rate.max\endcsname{0.11}
\expandafter\def\csname val@long.react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@long.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m3.root_fixed_rate.max\endcsname{0.10}
\expandafter\def\csname val@long.react-b2.m3.fsr_agent\endcsname{0.01}
\expandafter\def\csname val@long.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m3.fsr_agent.max\endcsname{0.03}
\expandafter\def\csname val@long.react-b2.m3.repaired_rate\endcsname{0.02}
\expandafter\def\csname val@long.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m3.repaired_rate.max\endcsname{0.06}
\expandafter\def\csname val@long.react-b2.m3.cleared_without_agent_count\endcsname{1.33}
\expandafter\def\csname val@long.react-b2.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m3.cleared_without_agent_count.max\endcsname{2.00}
\expandafter\def\csname val@long.react-b2.m3.repairable_count\endcsname{24.33}
\expandafter\def\csname val@long.react-b2.m3.repairable_count.min\endcsname{10.00}
\expandafter\def\csname val@long.react-b2.m3.repairable_count.max\endcsname{36.00}
\expandafter\def\csname val@long.react-b2.m4.regret\endcsname{0.84}
\expandafter\def\csname val@long.react-b2.m4.regret.min\endcsname{0.77}
\expandafter\def\csname val@long.react-b2.m4.regret.max\endcsname{0.97}
\expandafter\def\csname val@long.react-b2.m4.regret_raw\endcsname{0.84}
\expandafter\def\csname val@long.react-b2.m4.regret_raw.min\endcsname{0.77}
\expandafter\def\csname val@long.react-b2.m4.regret_raw.max\endcsname{0.97}
\expandafter\def\csname val@long.react-b2.m4.uim\endcsname{12692}
\expandafter\def\csname val@long.react-b2.m4.uim.min\endcsname{960}
\expandafter\def\csname val@long.react-b2.m4.uim.max\endcsname{29297}
\expandafter\def\csname val@long.react-b2.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long.react-b2.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.react-b2.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.react-b2.m4.offered_requests\endcsname{23936.84}
\expandafter\def\csname val@long.react-b2.m4.offered_requests.min\endcsname{1378.15}
\expandafter\def\csname val@long.react-b2.m4.offered_requests.max\endcsname{54239.20}
\expandafter\def\csname val@long.react-b2.m4.load_live_share\endcsname{0.89}
\expandafter\def\csname val@long.react-b2.m4.load_live_share.min\endcsname{0.67}
\expandafter\def\csname val@long.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m5.median_s\endcsname{288}
\expandafter\def\csname val@long.react-b2.m5.median_s.min\endcsname{155}
\expandafter\def\csname val@long.react-b2.m5.median_s.max\endcsname{359}
\expandafter\def\csname val@long.react-b2.m5.p90_s\endcsname{499}
\expandafter\def\csname val@long.react-b2.m5.p90_s.min\endcsname{435}
\expandafter\def\csname val@long.react-b2.m5.p90_s.max\endcsname{561}
\expandafter\def\csname val@long.react-b2.m5.dollars_median\endcsname{0.69}
\expandafter\def\csname val@long.react-b2.m5.dollars_median.min\endcsname{0.03}
\expandafter\def\csname val@long.react-b2.m5.dollars_median.max\endcsname{1.79}
\expandafter\def\csname val@long.react-b2.m5.reached\endcsname{4.7}
\expandafter\def\csname val@long.react-b2.m5.reached.min\endcsname{2.0}
\expandafter\def\csname val@long.react-b2.m5.reached.max\endcsname{9.0}
\expandafter\def\csname val@long.react-b2.m5.injected\endcsname{59}
\expandafter\def\csname val@long.react-b2.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long.react-b2.m5.injected.max\endcsname{60}
\expandafter\def\csname val@long.react-b2.m6.mitigated.median_s\endcsname{304}
\expandafter\def\csname val@long.react-b2.m6.mitigated.median_s.min\endcsname{246}
\expandafter\def\csname val@long.react-b2.m6.mitigated.median_s.max\endcsname{407}
\expandafter\def\csname val@long.react-b2.m6.mitigated.p90_s\endcsname{678}
\expandafter\def\csname val@long.react-b2.m6.mitigated.p90_s.min\endcsname{397}
\expandafter\def\csname val@long.react-b2.m6.mitigated.p90_s.max\endcsname{1143}
\expandafter\def\csname val@long.react-b2.m6.mitigated.dollars_median\endcsname{1.89}
\expandafter\def\csname val@long.react-b2.m6.mitigated.dollars_median.min\endcsname{1.41}
\expandafter\def\csname val@long.react-b2.m6.mitigated.dollars_median.max\endcsname{2.50}
\expandafter\def\csname val@long.react-b2.m6.mitigated.reached\endcsname{17.7}
\expandafter\def\csname val@long.react-b2.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long.react-b2.m6.mitigated.reached.max\endcsname{35.0}
\expandafter\def\csname val@long.react-b2.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long.react-b2.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long.react-b2.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.median_s\endcsname{777}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.median_s.min\endcsname{547}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.median_s.max\endcsname{1007}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.p90_s\endcsname{3304}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.p90_s.min\endcsname{1129}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.p90_s.max\endcsname{5479}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.dollars_median\endcsname{0.83}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.12}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.54}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.reached\endcsname{3.0}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.reached.max\endcsname{6.0}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long.react-b2.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@long.react-b2.m7.blast_radius\endcsname{0.24}
\expandafter\def\csname val@long.react-b2.m7.blast_radius.min\endcsname{0.14}
\expandafter\def\csname val@long.react-b2.m7.blast_radius.max\endcsname{0.30}
\expandafter\def\csname val@long.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.react-b2.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@long.react-b2.m7.out_of_scope_actions.min\endcsname{3}
\expandafter\def\csname val@long.react-b2.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.executed_mutating_actions\endcsname{15}
\expandafter\def\csname val@long.react-b2.m7.executed_mutating_actions.min\endcsname{10}
\expandafter\def\csname val@long.react-b2.m7.executed_mutating_actions.max\endcsname{22}
\expandafter\def\csname val@long.react-b2.m7.claim_calls\endcsname{1071}
\expandafter\def\csname val@long.react-b2.m7.claim_calls.min\endcsname{356}
\expandafter\def\csname val@long.react-b2.m7.claim_calls.max\endcsname{1540}
\expandafter\def\csname val@long.react-b2.m7.max_mutations_per_tick\endcsname{3.67}
\expandafter\def\csname val@long.react-b2.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long.react-b2.m7.max_mutations_per_tick.max\endcsname{5.00}
\expandafter\def\csname val@long.react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long.react-b2.m7.unlinked_citations\endcsname{5.67}
\expandafter\def\csname val@long.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@long.react-b2.m7.unlinked_citations.max\endcsname{13.00}
\expandafter\def\csname val@long.rag-b2r.m1.f1\endcsname{0.29}
\expandafter\def\csname val@long.rag-b2r.m1.f1.min\endcsname{0.13}
\expandafter\def\csname val@long.rag-b2r.m1.f1.max\endcsname{0.42}
\expandafter\def\csname val@long.rag-b2r.m1.precision\endcsname{0.19}
\expandafter\def\csname val@long.rag-b2r.m1.precision.min\endcsname{0.08}
\expandafter\def\csname val@long.rag-b2r.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long.rag-b2r.m1.recall\endcsname{0.65}
\expandafter\def\csname val@long.rag-b2r.m1.recall.min\endcsname{0.33}
\expandafter\def\csname val@long.rag-b2r.m1.recall.max\endcsname{0.91}
\expandafter\def\csname val@long.rag-b2r.m1.nrr\endcsname{0.75}
\expandafter\def\csname val@long.rag-b2r.m1.nrr.min\endcsname{0.72}
\expandafter\def\csname val@long.rag-b2r.m1.nrr.max\endcsname{0.80}
\expandafter\def\csname val@long.rag-b2r.m1.alerts_in_denominator\endcsname{121}
\expandafter\def\csname val@long.rag-b2r.m1.alerts_in_denominator.min\endcsname{57}
\expandafter\def\csname val@long.rag-b2r.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long.rag-b2r.m1.incidents_declared\endcsname{30}
\expandafter\def\csname val@long.rag-b2r.m1.incidents_declared.min\endcsname{16}
\expandafter\def\csname val@long.rag-b2r.m1.incidents_declared.max\endcsname{49}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_excluded\endcsname{135}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_excluded.min\endcsname{52}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_excluded.max\endcsname{290}
\expandafter\def\csname val@long.rag-b2r.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_share\endcsname{0.48}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_share.min\endcsname{0.26}
\expandafter\def\csname val@long.rag-b2r.m1.ambiguous_share.max\endcsname{0.69}
\expandafter\def\csname val@long.rag-b2r.m1.f1_overlap\endcsname{0.37}
\expandafter\def\csname val@long.rag-b2r.m1.f1_overlap.min\endcsname{0.34}
\expandafter\def\csname val@long.rag-b2r.m1.f1_overlap.max\endcsname{0.42}
\expandafter\def\csname val@long.rag-b2r.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long.rag-b2r.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long.rag-b2r.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long.rag-b2r.m1.incident_precision\endcsname{0.87}
\expandafter\def\csname val@long.rag-b2r.m1.incident_precision.min\endcsname{0.81}
\expandafter\def\csname val@long.rag-b2r.m1.incident_precision.max\endcsname{0.96}
\expandafter\def\csname val@long.rag-b2r.m2.mean_credit\endcsname{0.46}
\expandafter\def\csname val@long.rag-b2r.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@long.rag-b2r.m2.mean_credit.max\endcsname{0.69}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_1\endcsname{0.06}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_3\endcsname{0.06}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m2.acc_at_3.max\endcsname{0.19}
\expandafter\def\csname val@long.rag-b2r.m2.services_overlap_mean\endcsname{0.83}
\expandafter\def\csname val@long.rag-b2r.m2.services_overlap_mean.min\endcsname{0.70}
\expandafter\def\csname val@long.rag-b2r.m2.services_overlap_mean.max\endcsname{0.94}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.category\endcsname{0.15}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.category.max\endcsname{0.24}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.services\endcsname{0.62}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.services.min\endcsname{0.22}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.artifact\endcsname{0.58}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m2.component_rates.artifact.max\endcsname{0.88}
\expandafter\def\csname val@long.rag-b2r.m2.false_diagnoses\endcsname{233}
\expandafter\def\csname val@long.rag-b2r.m2.false_diagnoses.min\endcsname{115}
\expandafter\def\csname val@long.rag-b2r.m2.false_diagnoses.max\endcsname{443}
\expandafter\def\csname val@long.rag-b2r.m2.loc_at_1\endcsname{0.51}
\expandafter\def\csname val@long.rag-b2r.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long.rag-b2r.m2.committed_claims\endcsname{470.33}
\expandafter\def\csname val@long.rag-b2r.m2.committed_claims.min\endcsname{196.00}
\expandafter\def\csname val@long.rag-b2r.m2.committed_claims.max\endcsname{711.00}
\expandafter\def\csname val@long.rag-b2r.m2.claim_precision\endcsname{0.50}
\expandafter\def\csname val@long.rag-b2r.m2.claim_precision.min\endcsname{0.38}
\expandafter\def\csname val@long.rag-b2r.m2.claim_precision.max\endcsname{0.72}
\expandafter\def\csname val@long.rag-b2r.m3.fsr\endcsname{0.12}
\expandafter\def\csname val@long.rag-b2r.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_symptomatic\endcsname{0.10}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_symptomatic.max\endcsname{0.28}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate\endcsname{0.24}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate_symptomatic\endcsname{0.19}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.mitigated_rate_symptomatic.max\endcsname{0.56}
\expandafter\def\csname val@long.rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.root_fixed_rate\endcsname{0.01}
\expandafter\def\csname val@long.rag-b2r.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.root_fixed_rate.max\endcsname{0.03}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.cleared_without_agent_count\endcsname{1.33}
\expandafter\def\csname val@long.rag-b2r.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long.rag-b2r.m3.repairable_count\endcsname{30.33}
\expandafter\def\csname val@long.rag-b2r.m3.repairable_count.min\endcsname{11.00}
\expandafter\def\csname val@long.rag-b2r.m3.repairable_count.max\endcsname{43.00}
\expandafter\def\csname val@long.rag-b2r.m4.regret\endcsname{0.83}
\expandafter\def\csname val@long.rag-b2r.m4.regret.min\endcsname{0.49}
\expandafter\def\csname val@long.rag-b2r.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long.rag-b2r.m4.regret_raw\endcsname{1.14}
\expandafter\def\csname val@long.rag-b2r.m4.regret_raw.min\endcsname{0.49}
\expandafter\def\csname val@long.rag-b2r.m4.regret_raw.max\endcsname{1.50}
\expandafter\def\csname val@long.rag-b2r.m4.uim\endcsname{10896}
\expandafter\def\csname val@long.rag-b2r.m4.uim.min\endcsname{1778}
\expandafter\def\csname val@long.rag-b2r.m4.uim.max\endcsname{18782}
\expandafter\def\csname val@long.rag-b2r.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long.rag-b2r.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.rag-b2r.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long.rag-b2r.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m4.offered_requests\endcsname{15187.06}
\expandafter\def\csname val@long.rag-b2r.m4.offered_requests.min\endcsname{2900.59}
\expandafter\def\csname val@long.rag-b2r.m4.offered_requests.max\endcsname{27505.40}
\expandafter\def\csname val@long.rag-b2r.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@long.rag-b2r.m4.load_live_share.min\endcsname{0.29}
\expandafter\def\csname val@long.rag-b2r.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.rag-b2r.m5.median_s\endcsname{228}
\expandafter\def\csname val@long.rag-b2r.m5.median_s.min\endcsname{80}
\expandafter\def\csname val@long.rag-b2r.m5.median_s.max\endcsname{376}
\expandafter\def\csname val@long.rag-b2r.m5.p90_s\endcsname{279}
\expandafter\def\csname val@long.rag-b2r.m5.p90_s.min\endcsname{183}
\expandafter\def\csname val@long.rag-b2r.m5.p90_s.max\endcsname{376}
\expandafter\def\csname val@long.rag-b2r.m5.dollars_median\endcsname{0.16}
\expandafter\def\csname val@long.rag-b2r.m5.dollars_median.min\endcsname{0.02}
\expandafter\def\csname val@long.rag-b2r.m5.dollars_median.max\endcsname{0.30}
\expandafter\def\csname val@long.rag-b2r.m5.reached\endcsname{4.0}
\expandafter\def\csname val@long.rag-b2r.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.rag-b2r.m5.reached.max\endcsname{11.0}
\expandafter\def\csname val@long.rag-b2r.m5.injected\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.median_s\endcsname{420}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.median_s.min\endcsname{389}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.median_s.max\endcsname{452}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.p90_s\endcsname{978}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.p90_s.min\endcsname{529}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.p90_s.max\endcsname{1426}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.dollars_median\endcsname{0.05}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.dollars_median.min\endcsname{0.01}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.dollars_median.max\endcsname{0.09}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.reached\endcsname{13.7}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.median_s\endcsname{636}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.median_s.min\endcsname{636}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.median_s.max\endcsname{636}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.p90_s\endcsname{5947}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.p90_s.min\endcsname{5947}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.p90_s.max\endcsname{5947}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.dollars_median\endcsname{0.02}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.dollars_median.min\endcsname{0.02}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.dollars_median.max\endcsname{0.02}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.reached\endcsname{0.7}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.reached.max\endcsname{2.0}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long.rag-b2r.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long.rag-b2r.m7.blast_radius\endcsname{0.18}
\expandafter\def\csname val@long.rag-b2r.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m7.blast_radius.max\endcsname{0.50}
\expandafter\def\csname val@long.rag-b2r.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.rag-b2r.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@long.rag-b2r.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m7.out_of_scope_actions.max\endcsname{7}
\expandafter\def\csname val@long.rag-b2r.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long.rag-b2r.m7.no_target_actions\endcsname{13}
\expandafter\def\csname val@long.rag-b2r.m7.no_target_actions.min\endcsname{2}
\expandafter\def\csname val@long.rag-b2r.m7.no_target_actions.max\endcsname{23}
\expandafter\def\csname val@long.rag-b2r.m7.executed_mutating_actions\endcsname{73}
\expandafter\def\csname val@long.rag-b2r.m7.executed_mutating_actions.min\endcsname{2}
\expandafter\def\csname val@long.rag-b2r.m7.executed_mutating_actions.max\endcsname{152}
\expandafter\def\csname val@long.rag-b2r.m7.claim_calls\endcsname{1634}
\expandafter\def\csname val@long.rag-b2r.m7.claim_calls.min\endcsname{648}
\expandafter\def\csname val@long.rag-b2r.m7.claim_calls.max\endcsname{2221}
\expandafter\def\csname val@long.rag-b2r.m7.max_mutations_per_tick\endcsname{9.33}
\expandafter\def\csname val@long.rag-b2r.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long.rag-b2r.m7.max_mutations_per_tick.max\endcsname{17.00}
\expandafter\def\csname val@long.rag-b2r.m7.refused_actions\endcsname{20}
\expandafter\def\csname val@long.rag-b2r.m7.refused_actions.min\endcsname{5}
\expandafter\def\csname val@long.rag-b2r.m7.refused_actions.max\endcsname{31}
\expandafter\def\csname val@long.rag-b2r.m7.unlinked_citations\endcsname{31.67}
\expandafter\def\csname val@long.rag-b2r.m7.unlinked_citations.min\endcsname{14.00}
\expandafter\def\csname val@long.rag-b2r.m7.unlinked_citations.max\endcsname{60.00}
\expandafter\def\csname val@long.opensre-x3.m1.f1\endcsname{0.20}
\expandafter\def\csname val@long.opensre-x3.m1.f1.min\endcsname{0.05}
\expandafter\def\csname val@long.opensre-x3.m1.f1.max\endcsname{0.36}
\expandafter\def\csname val@long.opensre-x3.m1.precision\endcsname{0.15}
\expandafter\def\csname val@long.opensre-x3.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long.opensre-x3.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long.opensre-x3.m1.recall\endcsname{0.77}
\expandafter\def\csname val@long.opensre-x3.m1.recall.min\endcsname{0.54}
\expandafter\def\csname val@long.opensre-x3.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m1.nrr\endcsname{0.94}
\expandafter\def\csname val@long.opensre-x3.m1.nrr.min\endcsname{0.90}
\expandafter\def\csname val@long.opensre-x3.m1.nrr.max\endcsname{0.99}
\expandafter\def\csname val@long.opensre-x3.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long.opensre-x3.m1.alerts_in_denominator.min\endcsname{60}
\expandafter\def\csname val@long.opensre-x3.m1.alerts_in_denominator.max\endcsname{85}
\expandafter\def\csname val@long.opensre-x3.m1.incidents_declared\endcsname{4}
\expandafter\def\csname val@long.opensre-x3.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@long.opensre-x3.m1.incidents_declared.max\endcsname{6}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_excluded\endcsname{60}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_excluded.min\endcsname{54}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_excluded.max\endcsname{67}
\expandafter\def\csname val@long.opensre-x3.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_share\endcsname{0.46}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long.opensre-x3.m1.ambiguous_share.max\endcsname{0.53}
\expandafter\def\csname val@long.opensre-x3.m1.f1_overlap\endcsname{0.27}
\expandafter\def\csname val@long.opensre-x3.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long.opensre-x3.m1.f1_overlap.max\endcsname{0.39}
\expandafter\def\csname val@long.opensre-x3.m1.detection_recall\endcsname{0.97}
\expandafter\def\csname val@long.opensre-x3.m1.detection_recall.min\endcsname{0.93}
\expandafter\def\csname val@long.opensre-x3.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m1.incident_precision\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m1.incident_precision.min\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m2.mean_credit\endcsname{0.31}
\expandafter\def\csname val@long.opensre-x3.m2.mean_credit.min\endcsname{0.29}
\expandafter\def\csname val@long.opensre-x3.m2.mean_credit.max\endcsname{0.33}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_1.min\endcsname{0.09}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_3\endcsname{0.16}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_3.min\endcsname{0.09}
\expandafter\def\csname val@long.opensre-x3.m2.acc_at_3.max\endcsname{0.22}
\expandafter\def\csname val@long.opensre-x3.m2.services_overlap_mean\endcsname{0.90}
\expandafter\def\csname val@long.opensre-x3.m2.services_overlap_mean.min\endcsname{0.85}
\expandafter\def\csname val@long.opensre-x3.m2.services_overlap_mean.max\endcsname{0.95}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.category\endcsname{0.34}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.category.min\endcsname{0.27}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.category.max\endcsname{0.40}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.services\endcsname{0.40}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.services.min\endcsname{0.40}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.services.max\endcsname{0.41}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.artifact.min\endcsname{0.13}
\expandafter\def\csname val@long.opensre-x3.m2.component_rates.artifact.max\endcsname{0.32}
\expandafter\def\csname val@long.opensre-x3.m2.false_diagnoses\endcsname{30}
\expandafter\def\csname val@long.opensre-x3.m2.false_diagnoses.min\endcsname{29}
\expandafter\def\csname val@long.opensre-x3.m2.false_diagnoses.max\endcsname{31}
\expandafter\def\csname val@long.opensre-x3.m2.loc_at_1\endcsname{0.22}
\expandafter\def\csname val@long.opensre-x3.m2.loc_at_1.min\endcsname{0.13}
\expandafter\def\csname val@long.opensre-x3.m2.loc_at_1.max\endcsname{0.32}
\expandafter\def\csname val@long.opensre-x3.m2.committed_claims\endcsname{72.50}
\expandafter\def\csname val@long.opensre-x3.m2.committed_claims.min\endcsname{70.00}
\expandafter\def\csname val@long.opensre-x3.m2.committed_claims.max\endcsname{75.00}
\expandafter\def\csname val@long.opensre-x3.m2.claim_precision\endcsname{0.59}
\expandafter\def\csname val@long.opensre-x3.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long.opensre-x3.m2.claim_precision.max\endcsname{0.59}
\expandafter\def\csname val@long.opensre-x3.m3.fsr\endcsname{0.24}
\expandafter\def\csname val@long.opensre-x3.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long.opensre-x3.m3.fsr.max\endcsname{0.41}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_symptomatic\endcsname{0.13}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_symptomatic.max\endcsname{0.20}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate\endcsname{0.38}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate.max\endcsname{0.62}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long.opensre-x3.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long.opensre-x3.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@long.opensre-x3.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.agent_attributed_rate.max\endcsname{0.12}
\expandafter\def\csname val@long.opensre-x3.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@long.opensre-x3.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.root_fixed_rate.max\endcsname{0.20}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long.opensre-x3.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long.opensre-x3.m3.repairable_count\endcsname{21.50}
\expandafter\def\csname val@long.opensre-x3.m3.repairable_count.min\endcsname{13.00}
\expandafter\def\csname val@long.opensre-x3.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long.opensre-x3.m4.regret\endcsname{0.98}
\expandafter\def\csname val@long.opensre-x3.m4.regret.min\endcsname{0.97}
\expandafter\def\csname val@long.opensre-x3.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m4.regret_raw\endcsname{1.20}
\expandafter\def\csname val@long.opensre-x3.m4.regret_raw.min\endcsname{0.97}
\expandafter\def\csname val@long.opensre-x3.m4.regret_raw.max\endcsname{1.44}
\expandafter\def\csname val@long.opensre-x3.m4.uim\endcsname{4798}
\expandafter\def\csname val@long.opensre-x3.m4.uim.min\endcsname{1793}
\expandafter\def\csname val@long.opensre-x3.m4.uim.max\endcsname{7804}
\expandafter\def\csname val@long.opensre-x3.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long.opensre-x3.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.opensre-x3.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long.opensre-x3.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m4.offered_requests\endcsname{9003.38}
\expandafter\def\csname val@long.opensre-x3.m4.offered_requests.min\endcsname{2332.84}
\expandafter\def\csname val@long.opensre-x3.m4.offered_requests.max\endcsname{15673.90}
\expandafter\def\csname val@long.opensre-x3.m4.load_live_share\endcsname{0.68}
\expandafter\def\csname val@long.opensre-x3.m4.load_live_share.min\endcsname{0.36}
\expandafter\def\csname val@long.opensre-x3.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.opensre-x3.m5.median_s\endcsname{172}
\expandafter\def\csname val@long.opensre-x3.m5.median_s.min\endcsname{152}
\expandafter\def\csname val@long.opensre-x3.m5.median_s.max\endcsname{193}
\expandafter\def\csname val@long.opensre-x3.m5.p90_s\endcsname{766}
\expandafter\def\csname val@long.opensre-x3.m5.p90_s.min\endcsname{306}
\expandafter\def\csname val@long.opensre-x3.m5.p90_s.max\endcsname{1225}
\expandafter\def\csname val@long.opensre-x3.m5.dollars_median\endcsname{0.55}
\expandafter\def\csname val@long.opensre-x3.m5.dollars_median.min\endcsname{0.47}
\expandafter\def\csname val@long.opensre-x3.m5.dollars_median.max\endcsname{0.64}
\expandafter\def\csname val@long.opensre-x3.m5.reached\endcsname{8.5}
\expandafter\def\csname val@long.opensre-x3.m5.reached.min\endcsname{5.0}
\expandafter\def\csname val@long.opensre-x3.m5.reached.max\endcsname{12.0}
\expandafter\def\csname val@long.opensre-x3.m5.injected\endcsname{57}
\expandafter\def\csname val@long.opensre-x3.m5.injected.min\endcsname{55}
\expandafter\def\csname val@long.opensre-x3.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.median_s\endcsname{322}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.median_s.min\endcsname{243}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.median_s.max\endcsname{402}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.p90_s\endcsname{1987}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.p90_s.min\endcsname{490}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.p90_s.max\endcsname{3483}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.dollars_median\endcsname{1.65}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.dollars_median.min\endcsname{1.54}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.dollars_median.max\endcsname{1.76}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.reached\endcsname{21.0}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.reached.max\endcsname{34.0}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@long.opensre-x3.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.median_s\endcsname{196}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.median_s.min\endcsname{196}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.median_s.max\endcsname{196}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.p90_s\endcsname{4950}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.p90_s.min\endcsname{4950}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.p90_s.max\endcsname{4950}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.dollars_median\endcsname{1.14}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.dollars_median.min\endcsname{1.14}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.dollars_median.max\endcsname{1.14}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.reached\endcsname{5.5}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.reached.max\endcsname{11.0}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@long.opensre-x3.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long.opensre-x3.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.blast_radius.max\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.executed_mutating_actions\endcsname{11}
\expandafter\def\csname val@long.opensre-x3.m7.executed_mutating_actions.min\endcsname{7}
\expandafter\def\csname val@long.opensre-x3.m7.executed_mutating_actions.max\endcsname{15}
\expandafter\def\csname val@long.opensre-x3.m7.claim_calls\endcsname{546}
\expandafter\def\csname val@long.opensre-x3.m7.claim_calls.min\endcsname{545}
\expandafter\def\csname val@long.opensre-x3.m7.claim_calls.max\endcsname{546}
\expandafter\def\csname val@long.opensre-x3.m7.max_mutations_per_tick\endcsname{3.00}
\expandafter\def\csname val@long.opensre-x3.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@long.opensre-x3.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@long.opensre-x3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long.opensre-x3.m7.unlinked_citations\endcsname{4.00}
\expandafter\def\csname val@long.opensre-x3.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long.opensre-x3.m7.unlinked_citations.max\endcsname{8.00}
\expandafter\def\csname val@long.orbit-0.m1.f1\endcsname{0.05}
\expandafter\def\csname val@long.orbit-0.m1.f1.min\endcsname{0.03}
\expandafter\def\csname val@long.orbit-0.m1.f1.max\endcsname{0.06}
\expandafter\def\csname val@long.orbit-0.m1.precision\endcsname{0.71}
\expandafter\def\csname val@long.orbit-0.m1.precision.min\endcsname{0.43}
\expandafter\def\csname val@long.orbit-0.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m1.recall\endcsname{0.02}
\expandafter\def\csname val@long.orbit-0.m1.recall.min\endcsname{0.02}
\expandafter\def\csname val@long.orbit-0.m1.recall.max\endcsname{0.03}
\expandafter\def\csname val@long.orbit-0.m1.nrr\endcsname{-0.69}
\expandafter\def\csname val@long.orbit-0.m1.nrr.min\endcsname{-0.89}
\expandafter\def\csname val@long.orbit-0.m1.nrr.max\endcsname{-0.49}
\expandafter\def\csname val@long.orbit-0.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long.orbit-0.m1.alerts_in_denominator.min\endcsname{54}
\expandafter\def\csname val@long.orbit-0.m1.alerts_in_denominator.max\endcsname{90}
\expandafter\def\csname val@long.orbit-0.m1.incidents_declared\endcsname{118}
\expandafter\def\csname val@long.orbit-0.m1.incidents_declared.min\endcsname{102}
\expandafter\def\csname val@long.orbit-0.m1.incidents_declared.max\endcsname{134}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_excluded\endcsname{51}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_excluded.min\endcsname{48}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_excluded.max\endcsname{54}
\expandafter\def\csname val@long.orbit-0.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_share\endcsname{0.42}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_share.min\endcsname{0.38}
\expandafter\def\csname val@long.orbit-0.m1.ambiguous_share.max\endcsname{0.47}
\expandafter\def\csname val@long.orbit-0.m1.f1_overlap\endcsname{0.22}
\expandafter\def\csname val@long.orbit-0.m1.f1_overlap.min\endcsname{0.16}
\expandafter\def\csname val@long.orbit-0.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long.orbit-0.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long.orbit-0.m1.incident_precision.min\endcsname{0.91}
\expandafter\def\csname val@long.orbit-0.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.fsr\endcsname{0.21}
\expandafter\def\csname val@long.orbit-0.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long.orbit-0.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long.orbit-0.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@long.orbit-0.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long.orbit-0.m3.fsr_symptomatic.max\endcsname{0.30}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate\endcsname{0.42}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate.max\endcsname{0.71}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate_symptomatic\endcsname{0.35}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long.orbit-0.m3.mitigated_rate_symptomatic.max\endcsname{0.59}
\expandafter\def\csname val@long.orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long.orbit-0.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long.orbit-0.m3.repairable_count\endcsname{21.00}
\expandafter\def\csname val@long.orbit-0.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long.orbit-0.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long.orbit-0.m4.regret\endcsname{0.94}
\expandafter\def\csname val@long.orbit-0.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long.orbit-0.m4.regret.max\endcsname{0.96}
\expandafter\def\csname val@long.orbit-0.m4.regret_raw\endcsname{0.94}
\expandafter\def\csname val@long.orbit-0.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long.orbit-0.m4.regret_raw.max\endcsname{0.96}
\expandafter\def\csname val@long.orbit-0.m4.uim\endcsname{4335}
\expandafter\def\csname val@long.orbit-0.m4.uim.min\endcsname{1192}
\expandafter\def\csname val@long.orbit-0.m4.uim.max\endcsname{7478}
\expandafter\def\csname val@long.orbit-0.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long.orbit-0.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long.orbit-0.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long.orbit-0.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m4.offered_requests\endcsname{8129.78}
\expandafter\def\csname val@long.orbit-0.m4.offered_requests.min\endcsname{1525.92}
\expandafter\def\csname val@long.orbit-0.m4.offered_requests.max\endcsname{14733.60}
\expandafter\def\csname val@long.orbit-0.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@long.orbit-0.m4.load_live_share.min\endcsname{0.45}
\expandafter\def\csname val@long.orbit-0.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long.orbit-0.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m5.injected\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.median_s\endcsname{345}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.median_s.min\endcsname{250}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.median_s.max\endcsname{441}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.p90_s\endcsname{912}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.p90_s.min\endcsname{493}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.p90_s.max\endcsname{1331}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.dollars_median\endcsname{0.86}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.dollars_median.min\endcsname{0.59}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.dollars_median.max\endcsname{1.13}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.reached\endcsname{24.5}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.reached.max\endcsname{41.0}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long.orbit-0.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long.orbit-0.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.claim_calls\endcsname{4148}
\expandafter\def\csname val@long.orbit-0.m7.claim_calls.min\endcsname{4036}
\expandafter\def\csname val@long.orbit-0.m7.claim_calls.max\endcsname{4260}
\expandafter\def\csname val@long.orbit-0.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long.orbit-0.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long.orbit-0.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@long.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.smash_score\endcsname{6.57}
\expandafter\def\csname val@long.b1-runbook.smash_lo_r1\endcsname{6.57}
\expandafter\def\csname val@long.b1-runbook.smash_hi_r0\endcsname{6.57}
\expandafter\def\csname val@long.b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@long.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@long.b1-runbook.rank\endcsname{2}
\expandafter\def\csname val@long.react-b2.smash_score\endcsname{8.64}
\expandafter\def\csname val@long.react-b2.smash_lo_r1\endcsname{8.64}
\expandafter\def\csname val@long.react-b2.smash_hi_r0\endcsname{8.64}
\expandafter\def\csname val@long.react-b2.dollars\endcsname{4.02}
\expandafter\def\csname val@long.react-b2.llm_calls\endcsname{299}
\expandafter\def\csname val@long.react-b2.rank\endcsname{1}
\expandafter\def\csname val@long.rag-b2r.smash_score\endcsname{0.97}
\expandafter\def\csname val@long.rag-b2r.smash_lo_r1\endcsname{0.97}
\expandafter\def\csname val@long.rag-b2r.smash_hi_r0\endcsname{0.97}
\expandafter\def\csname val@long.rag-b2r.dollars\endcsname{0.72}
\expandafter\def\csname val@long.rag-b2r.llm_calls\endcsname{38}
\expandafter\def\csname val@long.rag-b2r.rank\endcsname{4}
\expandafter\def\csname val@long.opensre-x3.smash_score\endcsname{-0.64}
\expandafter\def\csname val@long.opensre-x3.smash_lo_r1\endcsname{-0.64}
\expandafter\def\csname val@long.opensre-x3.smash_hi_r0\endcsname{-0.64}
\expandafter\def\csname val@long.opensre-x3.dollars\endcsname{4.37}
\expandafter\def\csname val@long.opensre-x3.llm_calls\endcsname{292}
\expandafter\def\csname val@long.opensre-x3.rank\endcsname{5}
\expandafter\def\csname val@long.orbit-0.smash_score\endcsname{2.69}
\expandafter\def\csname val@long.orbit-0.smash_lo_r1\endcsname{2.69}
\expandafter\def\csname val@long.orbit-0.smash_hi_r0\endcsname{2.69}
\expandafter\def\csname val@long.orbit-0.dollars\endcsname{3.35}
\expandafter\def\csname val@long.orbit-0.llm_calls\endcsname{124}
\expandafter\def\csname val@long.orbit-0.rank\endcsname{3}
\expandafter\def\csname val@long-valid.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m1.alerts_in_denominator\endcsname{67}
\expandafter\def\csname val@long-valid.b0-null.m1.alerts_in_denominator.min\endcsname{55}
\expandafter\def\csname val@long-valid.b0-null.m1.alerts_in_denominator.max\endcsname{89}
\expandafter\def\csname val@long-valid.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_excluded\endcsname{97}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_excluded.min\endcsname{49}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_excluded.max\endcsname{184}
\expandafter\def\csname val@long-valid.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_share\endcsname{0.54}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long-valid.b0-null.m1.ambiguous_share.max\endcsname{0.76}
\expandafter\def\csname val@long-valid.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr\endcsname{0.16}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_symptomatic.min\endcsname{0.04}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate\endcsname{0.32}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.08}
\expandafter\def\csname val@long-valid.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long-valid.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m3.cleared_without_agent_count\endcsname{2.67}
\expandafter\def\csname val@long-valid.b0-null.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m3.cleared_without_agent_count.max\endcsname{4.00}
\expandafter\def\csname val@long-valid.b0-null.m3.repairable_count\endcsname{27.33}
\expandafter\def\csname val@long-valid.b0-null.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-valid.b0-null.m3.repairable_count.max\endcsname{40.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret_raw.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.regret_raw.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m4.uim\endcsname{15829}
\expandafter\def\csname val@long-valid.b0-null.m4.uim.min\endcsname{1244}
\expandafter\def\csname val@long-valid.b0-null.m4.uim.max\endcsname{38181}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m4.offered_requests\endcsname{28212.10}
\expandafter\def\csname val@long-valid.b0-null.m4.offered_requests.min\endcsname{1530.35}
\expandafter\def\csname val@long-valid.b0-null.m4.offered_requests.max\endcsname{67092.50}
\expandafter\def\csname val@long-valid.b0-null.m4.load_live_share\endcsname{0.85}
\expandafter\def\csname val@long-valid.b0-null.m4.load_live_share.min\endcsname{0.56}
\expandafter\def\csname val@long-valid.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m5.injected\endcsname{59}
\expandafter\def\csname val@long-valid.b0-null.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.b0-null.m5.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.median_s\endcsname{302}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.median_s.min\endcsname{244}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.median_s.max\endcsname{375}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.p90_s\endcsname{777}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.p90_s.min\endcsname{451}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.p90_s.max\endcsname{1268}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.reached\endcsname{19.0}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.b0-null.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.b0-null.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1\endcsname{0.46}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1.min\endcsname{0.35}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1.max\endcsname{0.64}
\expandafter\def\csname val@long-valid.b1-runbook.m1.precision\endcsname{0.46}
\expandafter\def\csname val@long-valid.b1-runbook.m1.precision.min\endcsname{0.28}
\expandafter\def\csname val@long-valid.b1-runbook.m1.precision.max\endcsname{0.68}
\expandafter\def\csname val@long-valid.b1-runbook.m1.recall\endcsname{0.48}
\expandafter\def\csname val@long-valid.b1-runbook.m1.recall.min\endcsname{0.38}
\expandafter\def\csname val@long-valid.b1-runbook.m1.recall.max\endcsname{0.60}
\expandafter\def\csname val@long-valid.b1-runbook.m1.nrr\endcsname{0.54}
\expandafter\def\csname val@long-valid.b1-runbook.m1.nrr.min\endcsname{0.42}
\expandafter\def\csname val@long-valid.b1-runbook.m1.nrr.max\endcsname{0.63}
\expandafter\def\csname val@long-valid.b1-runbook.m1.alerts_in_denominator\endcsname{127}
\expandafter\def\csname val@long-valid.b1-runbook.m1.alerts_in_denominator.min\endcsname{90}
\expandafter\def\csname val@long-valid.b1-runbook.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incidents_declared\endcsname{61}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incidents_declared.min\endcsname{33}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incidents_declared.max\endcsname{102}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_excluded\endcsname{126}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_excluded.min\endcsname{102}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_excluded.max\endcsname{163}
\expandafter\def\csname val@long-valid.b1-runbook.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_share\endcsname{0.50}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long-valid.b1-runbook.m1.ambiguous_share.max\endcsname{0.64}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1_overlap\endcsname{0.56}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1_overlap.min\endcsname{0.41}
\expandafter\def\csname val@long-valid.b1-runbook.m1.f1_overlap.max\endcsname{0.82}
\expandafter\def\csname val@long-valid.b1-runbook.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incident_precision\endcsname{0.90}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incident_precision.min\endcsname{0.79}
\expandafter\def\csname val@long-valid.b1-runbook.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.mean_credit\endcsname{0.33}
\expandafter\def\csname val@long-valid.b1-runbook.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@long-valid.b1-runbook.m2.mean_credit.max\endcsname{0.58}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_1\endcsname{0.01}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_3\endcsname{0.01}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.acc_at_3.max\endcsname{0.03}
\expandafter\def\csname val@long-valid.b1-runbook.m2.services_overlap_mean\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.services_overlap_mean.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.category\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.category.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.category.max\endcsname{0.16}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.services\endcsname{0.53}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.services.min\endcsname{0.29}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.services.max\endcsname{0.83}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.artifact\endcsname{0.36}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.artifact.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.b1-runbook.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@long-valid.b1-runbook.m2.false_diagnoses\endcsname{13}
\expandafter\def\csname val@long-valid.b1-runbook.m2.false_diagnoses.min\endcsname{7}
\expandafter\def\csname val@long-valid.b1-runbook.m2.false_diagnoses.max\endcsname{21}
\expandafter\def\csname val@long-valid.b1-runbook.m2.loc_at_1\endcsname{0.36}
\expandafter\def\csname val@long-valid.b1-runbook.m2.loc_at_1.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.b1-runbook.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long-valid.b1-runbook.m2.committed_claims\endcsname{60.67}
\expandafter\def\csname val@long-valid.b1-runbook.m2.committed_claims.min\endcsname{37.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.committed_claims.max\endcsname{97.00}
\expandafter\def\csname val@long-valid.b1-runbook.m2.claim_precision\endcsname{0.72}
\expandafter\def\csname val@long-valid.b1-runbook.m2.claim_precision.min\endcsname{0.43}
\expandafter\def\csname val@long-valid.b1-runbook.m2.claim_precision.max\endcsname{0.89}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr.max\endcsname{0.39}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_symptomatic\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_symptomatic.max\endcsname{0.23}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate\endcsname{0.24}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate.max\endcsname{0.57}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate_symptomatic\endcsname{0.14}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long-valid.b1-runbook.m3.agent_attributed_rate\endcsname{0.16}
\expandafter\def\csname val@long-valid.b1-runbook.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.agent_attributed_rate.max\endcsname{0.29}
\expandafter\def\csname val@long-valid.b1-runbook.m3.root_fixed_rate\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.root_fixed_rate.max\endcsname{0.21}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_agent\endcsname{0.04}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.fsr_agent.max\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repaired_rate\endcsname{0.04}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repaired_rate.max\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m3.cleared_without_agent_count\endcsname{0.33}
\expandafter\def\csname val@long-valid.b1-runbook.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repairable_count\endcsname{26.33}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-valid.b1-runbook.m3.repairable_count.max\endcsname{38.00}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret\endcsname{0.97}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret_raw\endcsname{1.05}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long-valid.b1-runbook.m4.regret_raw.max\endcsname{1.24}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim\endcsname{18761}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim.min\endcsname{1155}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim.max\endcsname{47197}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m4.offered_requests\endcsname{27462.55}
\expandafter\def\csname val@long-valid.b1-runbook.m4.offered_requests.min\endcsname{1454.79}
\expandafter\def\csname val@long-valid.b1-runbook.m4.offered_requests.max\endcsname{65898.40}
\expandafter\def\csname val@long-valid.b1-runbook.m4.load_live_share\endcsname{0.78}
\expandafter\def\csname val@long-valid.b1-runbook.m4.load_live_share.min\endcsname{0.35}
\expandafter\def\csname val@long-valid.b1-runbook.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.b1-runbook.m5.median_s\endcsname{132}
\expandafter\def\csname val@long-valid.b1-runbook.m5.median_s.min\endcsname{132}
\expandafter\def\csname val@long-valid.b1-runbook.m5.median_s.max\endcsname{132}
\expandafter\def\csname val@long-valid.b1-runbook.m5.p90_s\endcsname{563}
\expandafter\def\csname val@long-valid.b1-runbook.m5.p90_s.min\endcsname{563}
\expandafter\def\csname val@long-valid.b1-runbook.m5.p90_s.max\endcsname{563}
\expandafter\def\csname val@long-valid.b1-runbook.m5.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m5.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m5.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m5.reached\endcsname{0.7}
\expandafter\def\csname val@long-valid.b1-runbook.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.b1-runbook.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@long-valid.b1-runbook.m5.injected\endcsname{57}
\expandafter\def\csname val@long-valid.b1-runbook.m5.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.b1-runbook.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.median_s\endcsname{443}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.median_s.min\endcsname{371}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.median_s.max\endcsname{491}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.p90_s\endcsname{780}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.p90_s.min\endcsname{374}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.p90_s.max\endcsname{1353}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.reached\endcsname{14.0}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.reached.min\endcsname{2.0}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.reached.max\endcsname{33.0}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.b1-runbook.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.median_s\endcsname{486}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.median_s.min\endcsname{483}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.median_s.max\endcsname{489}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.p90_s\endcsname{1460}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.p90_s.min\endcsname{920}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.p90_s.max\endcsname{2001}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.reached\endcsname{5.3}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.reached.max\endcsname{12.0}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.b1-runbook.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.b1-runbook.m7.blast_radius\endcsname{0.04}
\expandafter\def\csname val@long-valid.b1-runbook.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.blast_radius.max\endcsname{0.09}
\expandafter\def\csname val@long-valid.b1-runbook.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.out_of_scope_actions\endcsname{2}
\expandafter\def\csname val@long-valid.b1-runbook.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unscoped_actions\endcsname{2}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unscoped_actions.max\endcsname{4}
\expandafter\def\csname val@long-valid.b1-runbook.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.executed_mutating_actions\endcsname{60}
\expandafter\def\csname val@long-valid.b1-runbook.m7.executed_mutating_actions.min\endcsname{37}
\expandafter\def\csname val@long-valid.b1-runbook.m7.executed_mutating_actions.max\endcsname{95}
\expandafter\def\csname val@long-valid.b1-runbook.m7.claim_calls\endcsname{416}
\expandafter\def\csname val@long-valid.b1-runbook.m7.claim_calls.min\endcsname{284}
\expandafter\def\csname val@long-valid.b1-runbook.m7.claim_calls.max\endcsname{651}
\expandafter\def\csname val@long-valid.b1-runbook.m7.max_mutations_per_tick\endcsname{9.33}
\expandafter\def\csname val@long-valid.b1-runbook.m7.max_mutations_per_tick.min\endcsname{7.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.max_mutations_per_tick.max\endcsname{13.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@long-valid.b1-runbook.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.m7.refused_actions.max\endcsname{2}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unlinked_citations\endcsname{26.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unlinked_citations.min\endcsname{16.00}
\expandafter\def\csname val@long-valid.b1-runbook.m7.unlinked_citations.max\endcsname{32.00}
\expandafter\def\csname val@long-valid.react-b2.m1.f1\endcsname{0.07}
\expandafter\def\csname val@long-valid.react-b2.m1.f1.min\endcsname{0.04}
\expandafter\def\csname val@long-valid.react-b2.m1.f1.max\endcsname{0.09}
\expandafter\def\csname val@long-valid.react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@long-valid.react-b2.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.react-b2.m1.precision.max\endcsname{0.05}
\expandafter\def\csname val@long-valid.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.nrr\endcsname{0.24}
\expandafter\def\csname val@long-valid.react-b2.m1.nrr.min\endcsname{0.11}
\expandafter\def\csname val@long-valid.react-b2.m1.nrr.max\endcsname{0.32}
\expandafter\def\csname val@long-valid.react-b2.m1.alerts_in_denominator\endcsname{67}
\expandafter\def\csname val@long-valid.react-b2.m1.alerts_in_denominator.min\endcsname{53}
\expandafter\def\csname val@long-valid.react-b2.m1.alerts_in_denominator.max\endcsname{92}
\expandafter\def\csname val@long-valid.react-b2.m1.incidents_declared\endcsname{50}
\expandafter\def\csname val@long-valid.react-b2.m1.incidents_declared.min\endcsname{37}
\expandafter\def\csname val@long-valid.react-b2.m1.incidents_declared.max\endcsname{63}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_excluded\endcsname{96}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_excluded.min\endcsname{53}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_excluded.max\endcsname{172}
\expandafter\def\csname val@long-valid.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_share\endcsname{0.56}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long-valid.react-b2.m1.ambiguous_share.max\endcsname{0.76}
\expandafter\def\csname val@long-valid.react-b2.m1.f1_overlap\endcsname{0.20}
\expandafter\def\csname val@long-valid.react-b2.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.react-b2.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long-valid.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long-valid.react-b2.m1.incident_precision.min\endcsname{0.92}
\expandafter\def\csname val@long-valid.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m2.mean_credit\endcsname{0.15}
\expandafter\def\csname val@long-valid.react-b2.m2.mean_credit.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.react-b2.m2.mean_credit.max\endcsname{0.24}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_3\endcsname{0.08}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_3.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.react-b2.m2.acc_at_3.max\endcsname{0.14}
\expandafter\def\csname val@long-valid.react-b2.m2.services_overlap_mean\endcsname{0.84}
\expandafter\def\csname val@long-valid.react-b2.m2.services_overlap_mean.min\endcsname{0.67}
\expandafter\def\csname val@long-valid.react-b2.m2.services_overlap_mean.max\endcsname{0.97}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.category\endcsname{0.18}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.category.min\endcsname{0.10}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.category.max\endcsname{0.29}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.services\endcsname{0.19}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.services.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.services.max\endcsname{0.33}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.artifact\endcsname{0.10}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.artifact.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.react-b2.m2.component_rates.artifact.max\endcsname{0.14}
\expandafter\def\csname val@long-valid.react-b2.m2.false_diagnoses\endcsname{11}
\expandafter\def\csname val@long-valid.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m2.false_diagnoses.max\endcsname{24}
\expandafter\def\csname val@long-valid.react-b2.m2.loc_at_1\endcsname{0.08}
\expandafter\def\csname val@long-valid.react-b2.m2.loc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.react-b2.m2.loc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long-valid.react-b2.m2.committed_claims\endcsname{29.67}
\expandafter\def\csname val@long-valid.react-b2.m2.committed_claims.min\endcsname{6.00}
\expandafter\def\csname val@long-valid.react-b2.m2.committed_claims.max\endcsname{58.00}
\expandafter\def\csname val@long-valid.react-b2.m2.claim_precision\endcsname{0.73}
\expandafter\def\csname val@long-valid.react-b2.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long-valid.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr\endcsname{0.18}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_symptomatic.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate\endcsname{0.30}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate.max\endcsname{0.60}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.22}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long-valid.react-b2.m3.agent_attributed_rate\endcsname{0.04}
\expandafter\def\csname val@long-valid.react-b2.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m3.agent_attributed_rate.max\endcsname{0.11}
\expandafter\def\csname val@long-valid.react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@long-valid.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m3.root_fixed_rate.max\endcsname{0.10}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_agent\endcsname{0.01}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m3.fsr_agent.max\endcsname{0.03}
\expandafter\def\csname val@long-valid.react-b2.m3.repaired_rate\endcsname{0.02}
\expandafter\def\csname val@long-valid.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m3.repaired_rate.max\endcsname{0.06}
\expandafter\def\csname val@long-valid.react-b2.m3.cleared_without_agent_count\endcsname{1.33}
\expandafter\def\csname val@long-valid.react-b2.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m3.cleared_without_agent_count.max\endcsname{2.00}
\expandafter\def\csname val@long-valid.react-b2.m3.repairable_count\endcsname{24.33}
\expandafter\def\csname val@long-valid.react-b2.m3.repairable_count.min\endcsname{10.00}
\expandafter\def\csname val@long-valid.react-b2.m3.repairable_count.max\endcsname{36.00}
\expandafter\def\csname val@long-valid.react-b2.m4.regret\endcsname{0.84}
\expandafter\def\csname val@long-valid.react-b2.m4.regret.min\endcsname{0.77}
\expandafter\def\csname val@long-valid.react-b2.m4.regret.max\endcsname{0.97}
\expandafter\def\csname val@long-valid.react-b2.m4.regret_raw\endcsname{0.84}
\expandafter\def\csname val@long-valid.react-b2.m4.regret_raw.min\endcsname{0.77}
\expandafter\def\csname val@long-valid.react-b2.m4.regret_raw.max\endcsname{0.97}
\expandafter\def\csname val@long-valid.react-b2.m4.uim\endcsname{12692}
\expandafter\def\csname val@long-valid.react-b2.m4.uim.min\endcsname{960}
\expandafter\def\csname val@long-valid.react-b2.m4.uim.max\endcsname{29297}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m4.offered_requests\endcsname{23936.84}
\expandafter\def\csname val@long-valid.react-b2.m4.offered_requests.min\endcsname{1378.15}
\expandafter\def\csname val@long-valid.react-b2.m4.offered_requests.max\endcsname{54239.20}
\expandafter\def\csname val@long-valid.react-b2.m4.load_live_share\endcsname{0.89}
\expandafter\def\csname val@long-valid.react-b2.m4.load_live_share.min\endcsname{0.67}
\expandafter\def\csname val@long-valid.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m5.median_s\endcsname{288}
\expandafter\def\csname val@long-valid.react-b2.m5.median_s.min\endcsname{155}
\expandafter\def\csname val@long-valid.react-b2.m5.median_s.max\endcsname{359}
\expandafter\def\csname val@long-valid.react-b2.m5.p90_s\endcsname{499}
\expandafter\def\csname val@long-valid.react-b2.m5.p90_s.min\endcsname{435}
\expandafter\def\csname val@long-valid.react-b2.m5.p90_s.max\endcsname{561}
\expandafter\def\csname val@long-valid.react-b2.m5.dollars_median\endcsname{0.69}
\expandafter\def\csname val@long-valid.react-b2.m5.dollars_median.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.react-b2.m5.dollars_median.max\endcsname{1.79}
\expandafter\def\csname val@long-valid.react-b2.m5.reached\endcsname{4.7}
\expandafter\def\csname val@long-valid.react-b2.m5.reached.min\endcsname{2.0}
\expandafter\def\csname val@long-valid.react-b2.m5.reached.max\endcsname{9.0}
\expandafter\def\csname val@long-valid.react-b2.m5.injected\endcsname{59}
\expandafter\def\csname val@long-valid.react-b2.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.react-b2.m5.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.median_s\endcsname{304}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.median_s.min\endcsname{246}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.median_s.max\endcsname{407}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.p90_s\endcsname{678}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.p90_s.min\endcsname{397}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.p90_s.max\endcsname{1143}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.dollars_median\endcsname{1.89}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.dollars_median.min\endcsname{1.41}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.dollars_median.max\endcsname{2.50}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.reached\endcsname{17.7}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.reached.max\endcsname{35.0}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.react-b2.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.median_s\endcsname{777}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.median_s.min\endcsname{547}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.median_s.max\endcsname{1007}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.p90_s\endcsname{3304}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.p90_s.min\endcsname{1129}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.p90_s.max\endcsname{5479}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.dollars_median\endcsname{0.83}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.12}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.54}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.reached\endcsname{3.0}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.reached.max\endcsname{6.0}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.react-b2.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@long-valid.react-b2.m7.blast_radius\endcsname{0.24}
\expandafter\def\csname val@long-valid.react-b2.m7.blast_radius.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.react-b2.m7.blast_radius.max\endcsname{0.30}
\expandafter\def\csname val@long-valid.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.react-b2.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@long-valid.react-b2.m7.out_of_scope_actions.min\endcsname{3}
\expandafter\def\csname val@long-valid.react-b2.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long-valid.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.executed_mutating_actions\endcsname{15}
\expandafter\def\csname val@long-valid.react-b2.m7.executed_mutating_actions.min\endcsname{10}
\expandafter\def\csname val@long-valid.react-b2.m7.executed_mutating_actions.max\endcsname{22}
\expandafter\def\csname val@long-valid.react-b2.m7.claim_calls\endcsname{1071}
\expandafter\def\csname val@long-valid.react-b2.m7.claim_calls.min\endcsname{356}
\expandafter\def\csname val@long-valid.react-b2.m7.claim_calls.max\endcsname{1540}
\expandafter\def\csname val@long-valid.react-b2.m7.max_mutations_per_tick\endcsname{3.67}
\expandafter\def\csname val@long-valid.react-b2.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long-valid.react-b2.m7.max_mutations_per_tick.max\endcsname{5.00}
\expandafter\def\csname val@long-valid.react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.react-b2.m7.unlinked_citations\endcsname{5.67}
\expandafter\def\csname val@long-valid.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.react-b2.m7.unlinked_citations.max\endcsname{13.00}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1\endcsname{0.37}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1.min\endcsname{0.32}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1.max\endcsname{0.42}
\expandafter\def\csname val@long-valid.rag-b2r.m1.precision\endcsname{0.24}
\expandafter\def\csname val@long-valid.rag-b2r.m1.precision.min\endcsname{0.21}
\expandafter\def\csname val@long-valid.rag-b2r.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long-valid.rag-b2r.m1.recall\endcsname{0.81}
\expandafter\def\csname val@long-valid.rag-b2r.m1.recall.min\endcsname{0.71}
\expandafter\def\csname val@long-valid.rag-b2r.m1.recall.max\endcsname{0.91}
\expandafter\def\csname val@long-valid.rag-b2r.m1.nrr\endcsname{0.72}
\expandafter\def\csname val@long-valid.rag-b2r.m1.nrr.min\endcsname{0.72}
\expandafter\def\csname val@long-valid.rag-b2r.m1.nrr.max\endcsname{0.72}
\expandafter\def\csname val@long-valid.rag-b2r.m1.alerts_in_denominator\endcsname{117}
\expandafter\def\csname val@long-valid.rag-b2r.m1.alerts_in_denominator.min\endcsname{57}
\expandafter\def\csname val@long-valid.rag-b2r.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incidents_declared\endcsname{32}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incidents_declared.min\endcsname{16}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incidents_declared.max\endcsname{49}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_excluded.min\endcsname{52}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_excluded.max\endcsname{62}
\expandafter\def\csname val@long-valid.rag-b2r.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_share\endcsname{0.37}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_share.min\endcsname{0.26}
\expandafter\def\csname val@long-valid.rag-b2r.m1.ambiguous_share.max\endcsname{0.48}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1_overlap\endcsname{0.39}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1_overlap.min\endcsname{0.35}
\expandafter\def\csname val@long-valid.rag-b2r.m1.f1_overlap.max\endcsname{0.42}
\expandafter\def\csname val@long-valid.rag-b2r.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incident_precision\endcsname{0.82}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incident_precision.min\endcsname{0.81}
\expandafter\def\csname val@long-valid.rag-b2r.m1.incident_precision.max\endcsname{0.84}
\expandafter\def\csname val@long-valid.rag-b2r.m2.mean_credit\endcsname{0.41}
\expandafter\def\csname val@long-valid.rag-b2r.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@long-valid.rag-b2r.m2.mean_credit.max\endcsname{0.69}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_1\endcsname{0.09}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_3\endcsname{0.09}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.acc_at_3.max\endcsname{0.19}
\expandafter\def\csname val@long-valid.rag-b2r.m2.services_overlap_mean\endcsname{0.82}
\expandafter\def\csname val@long-valid.rag-b2r.m2.services_overlap_mean.min\endcsname{0.70}
\expandafter\def\csname val@long-valid.rag-b2r.m2.services_overlap_mean.max\endcsname{0.94}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.category\endcsname{0.23}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.category.min\endcsname{0.22}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.category.max\endcsname{0.24}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.services\endcsname{0.56}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.services.min\endcsname{0.22}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.artifact\endcsname{0.44}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.component_rates.artifact.max\endcsname{0.88}
\expandafter\def\csname val@long-valid.rag-b2r.m2.false_diagnoses\endcsname{128}
\expandafter\def\csname val@long-valid.rag-b2r.m2.false_diagnoses.min\endcsname{115}
\expandafter\def\csname val@long-valid.rag-b2r.m2.false_diagnoses.max\endcsname{142}
\expandafter\def\csname val@long-valid.rag-b2r.m2.loc_at_1\endcsname{0.40}
\expandafter\def\csname val@long-valid.rag-b2r.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long-valid.rag-b2r.m2.committed_claims\endcsname{350.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.committed_claims.min\endcsname{196.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.committed_claims.max\endcsname{504.00}
\expandafter\def\csname val@long-valid.rag-b2r.m2.claim_precision\endcsname{0.57}
\expandafter\def\csname val@long-valid.rag-b2r.m2.claim_precision.min\endcsname{0.41}
\expandafter\def\csname val@long-valid.rag-b2r.m2.claim_precision.max\endcsname{0.72}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_symptomatic\endcsname{0.14}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_symptomatic.max\endcsname{0.28}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate\endcsname{0.34}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate_symptomatic\endcsname{0.28}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.mitigated_rate_symptomatic.max\endcsname{0.56}
\expandafter\def\csname val@long-valid.rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.cleared_without_agent_count\endcsname{1.50}
\expandafter\def\csname val@long-valid.rag-b2r.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repairable_count\endcsname{24.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repairable_count.min\endcsname{11.00}
\expandafter\def\csname val@long-valid.rag-b2r.m3.repairable_count.max\endcsname{37.00}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret_raw\endcsname{1.47}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret_raw.min\endcsname{1.43}
\expandafter\def\csname val@long-valid.rag-b2r.m4.regret_raw.max\endcsname{1.50}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim\endcsname{6954}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim.min\endcsname{1778}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim.max\endcsname{12130}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m4.offered_requests\endcsname{9027.90}
\expandafter\def\csname val@long-valid.rag-b2r.m4.offered_requests.min\endcsname{2900.59}
\expandafter\def\csname val@long-valid.rag-b2r.m4.offered_requests.max\endcsname{15155.20}
\expandafter\def\csname val@long-valid.rag-b2r.m4.load_live_share\endcsname{0.65}
\expandafter\def\csname val@long-valid.rag-b2r.m4.load_live_share.min\endcsname{0.29}
\expandafter\def\csname val@long-valid.rag-b2r.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.rag-b2r.m5.median_s\endcsname{80}
\expandafter\def\csname val@long-valid.rag-b2r.m5.median_s.min\endcsname{80}
\expandafter\def\csname val@long-valid.rag-b2r.m5.median_s.max\endcsname{80}
\expandafter\def\csname val@long-valid.rag-b2r.m5.p90_s\endcsname{183}
\expandafter\def\csname val@long-valid.rag-b2r.m5.p90_s.min\endcsname{183}
\expandafter\def\csname val@long-valid.rag-b2r.m5.p90_s.max\endcsname{183}
\expandafter\def\csname val@long-valid.rag-b2r.m5.dollars_median\endcsname{0.30}
\expandafter\def\csname val@long-valid.rag-b2r.m5.dollars_median.min\endcsname{0.30}
\expandafter\def\csname val@long-valid.rag-b2r.m5.dollars_median.max\endcsname{0.30}
\expandafter\def\csname val@long-valid.rag-b2r.m5.reached\endcsname{5.5}
\expandafter\def\csname val@long-valid.rag-b2r.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.rag-b2r.m5.reached.max\endcsname{11.0}
\expandafter\def\csname val@long-valid.rag-b2r.m5.injected\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.median_s\endcsname{452}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.median_s.min\endcsname{452}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.median_s.max\endcsname{452}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.p90_s\endcsname{1426}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.p90_s.min\endcsname{1426}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.p90_s.max\endcsname{1426}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.dollars_median\endcsname{0.09}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.dollars_median.min\endcsname{0.09}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.dollars_median.max\endcsname{0.09}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.reached\endcsname{19.5}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.rag-b2r.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.rag-b2r.m7.blast_radius\endcsname{0.25}
\expandafter\def\csname val@long-valid.rag-b2r.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.blast_radius.max\endcsname{0.50}
\expandafter\def\csname val@long-valid.rag-b2r.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m7.out_of_scope_actions.max\endcsname{1}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.rag-b2r.m7.no_target_actions\endcsname{18}
\expandafter\def\csname val@long-valid.rag-b2r.m7.no_target_actions.min\endcsname{13}
\expandafter\def\csname val@long-valid.rag-b2r.m7.no_target_actions.max\endcsname{23}
\expandafter\def\csname val@long-valid.rag-b2r.m7.executed_mutating_actions\endcsname{34}
\expandafter\def\csname val@long-valid.rag-b2r.m7.executed_mutating_actions.min\endcsname{2}
\expandafter\def\csname val@long-valid.rag-b2r.m7.executed_mutating_actions.max\endcsname{66}
\expandafter\def\csname val@long-valid.rag-b2r.m7.claim_calls\endcsname{1341}
\expandafter\def\csname val@long-valid.rag-b2r.m7.claim_calls.min\endcsname{648}
\expandafter\def\csname val@long-valid.rag-b2r.m7.claim_calls.max\endcsname{2034}
\expandafter\def\csname val@long-valid.rag-b2r.m7.max_mutations_per_tick\endcsname{5.50}
\expandafter\def\csname val@long-valid.rag-b2r.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.refused_actions\endcsname{15}
\expandafter\def\csname val@long-valid.rag-b2r.m7.refused_actions.min\endcsname{5}
\expandafter\def\csname val@long-valid.rag-b2r.m7.refused_actions.max\endcsname{25}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unlinked_citations\endcsname{17.50}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unlinked_citations.min\endcsname{14.00}
\expandafter\def\csname val@long-valid.rag-b2r.m7.unlinked_citations.max\endcsname{21.00}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1\endcsname{0.20}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1.max\endcsname{0.36}
\expandafter\def\csname val@long-valid.opensre-x3.m1.precision\endcsname{0.15}
\expandafter\def\csname val@long-valid.opensre-x3.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.opensre-x3.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long-valid.opensre-x3.m1.recall\endcsname{0.77}
\expandafter\def\csname val@long-valid.opensre-x3.m1.recall.min\endcsname{0.54}
\expandafter\def\csname val@long-valid.opensre-x3.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m1.nrr\endcsname{0.94}
\expandafter\def\csname val@long-valid.opensre-x3.m1.nrr.min\endcsname{0.90}
\expandafter\def\csname val@long-valid.opensre-x3.m1.nrr.max\endcsname{0.99}
\expandafter\def\csname val@long-valid.opensre-x3.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-valid.opensre-x3.m1.alerts_in_denominator.min\endcsname{60}
\expandafter\def\csname val@long-valid.opensre-x3.m1.alerts_in_denominator.max\endcsname{85}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incidents_declared\endcsname{4}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incidents_declared.max\endcsname{6}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_excluded\endcsname{60}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_excluded.min\endcsname{54}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_excluded.max\endcsname{67}
\expandafter\def\csname val@long-valid.opensre-x3.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_share\endcsname{0.46}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long-valid.opensre-x3.m1.ambiguous_share.max\endcsname{0.53}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1_overlap\endcsname{0.27}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.opensre-x3.m1.f1_overlap.max\endcsname{0.39}
\expandafter\def\csname val@long-valid.opensre-x3.m1.detection_recall\endcsname{0.97}
\expandafter\def\csname val@long-valid.opensre-x3.m1.detection_recall.min\endcsname{0.93}
\expandafter\def\csname val@long-valid.opensre-x3.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incident_precision\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incident_precision.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m2.mean_credit\endcsname{0.31}
\expandafter\def\csname val@long-valid.opensre-x3.m2.mean_credit.min\endcsname{0.29}
\expandafter\def\csname val@long-valid.opensre-x3.m2.mean_credit.max\endcsname{0.33}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_1.min\endcsname{0.09}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_3\endcsname{0.16}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_3.min\endcsname{0.09}
\expandafter\def\csname val@long-valid.opensre-x3.m2.acc_at_3.max\endcsname{0.22}
\expandafter\def\csname val@long-valid.opensre-x3.m2.services_overlap_mean\endcsname{0.90}
\expandafter\def\csname val@long-valid.opensre-x3.m2.services_overlap_mean.min\endcsname{0.85}
\expandafter\def\csname val@long-valid.opensre-x3.m2.services_overlap_mean.max\endcsname{0.95}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.category\endcsname{0.34}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.category.min\endcsname{0.27}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.category.max\endcsname{0.40}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.services\endcsname{0.40}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.services.min\endcsname{0.40}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.services.max\endcsname{0.41}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.artifact.min\endcsname{0.13}
\expandafter\def\csname val@long-valid.opensre-x3.m2.component_rates.artifact.max\endcsname{0.32}
\expandafter\def\csname val@long-valid.opensre-x3.m2.false_diagnoses\endcsname{30}
\expandafter\def\csname val@long-valid.opensre-x3.m2.false_diagnoses.min\endcsname{29}
\expandafter\def\csname val@long-valid.opensre-x3.m2.false_diagnoses.max\endcsname{31}
\expandafter\def\csname val@long-valid.opensre-x3.m2.loc_at_1\endcsname{0.22}
\expandafter\def\csname val@long-valid.opensre-x3.m2.loc_at_1.min\endcsname{0.13}
\expandafter\def\csname val@long-valid.opensre-x3.m2.loc_at_1.max\endcsname{0.32}
\expandafter\def\csname val@long-valid.opensre-x3.m2.committed_claims\endcsname{72.50}
\expandafter\def\csname val@long-valid.opensre-x3.m2.committed_claims.min\endcsname{70.00}
\expandafter\def\csname val@long-valid.opensre-x3.m2.committed_claims.max\endcsname{75.00}
\expandafter\def\csname val@long-valid.opensre-x3.m2.claim_precision\endcsname{0.59}
\expandafter\def\csname val@long-valid.opensre-x3.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long-valid.opensre-x3.m2.claim_precision.max\endcsname{0.59}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr\endcsname{0.24}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr.max\endcsname{0.41}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_symptomatic\endcsname{0.13}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_symptomatic.max\endcsname{0.20}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate\endcsname{0.38}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate.max\endcsname{0.62}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long-valid.opensre-x3.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long-valid.opensre-x3.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@long-valid.opensre-x3.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.agent_attributed_rate.max\endcsname{0.12}
\expandafter\def\csname val@long-valid.opensre-x3.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@long-valid.opensre-x3.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.root_fixed_rate.max\endcsname{0.20}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repairable_count\endcsname{21.50}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repairable_count.min\endcsname{13.00}
\expandafter\def\csname val@long-valid.opensre-x3.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret\endcsname{0.98}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret.min\endcsname{0.97}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret_raw\endcsname{1.20}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret_raw.min\endcsname{0.97}
\expandafter\def\csname val@long-valid.opensre-x3.m4.regret_raw.max\endcsname{1.44}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim\endcsname{4798}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim.min\endcsname{1793}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim.max\endcsname{7804}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m4.offered_requests\endcsname{9003.38}
\expandafter\def\csname val@long-valid.opensre-x3.m4.offered_requests.min\endcsname{2332.84}
\expandafter\def\csname val@long-valid.opensre-x3.m4.offered_requests.max\endcsname{15673.90}
\expandafter\def\csname val@long-valid.opensre-x3.m4.load_live_share\endcsname{0.68}
\expandafter\def\csname val@long-valid.opensre-x3.m4.load_live_share.min\endcsname{0.36}
\expandafter\def\csname val@long-valid.opensre-x3.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.opensre-x3.m5.median_s\endcsname{172}
\expandafter\def\csname val@long-valid.opensre-x3.m5.median_s.min\endcsname{152}
\expandafter\def\csname val@long-valid.opensre-x3.m5.median_s.max\endcsname{193}
\expandafter\def\csname val@long-valid.opensre-x3.m5.p90_s\endcsname{766}
\expandafter\def\csname val@long-valid.opensre-x3.m5.p90_s.min\endcsname{306}
\expandafter\def\csname val@long-valid.opensre-x3.m5.p90_s.max\endcsname{1225}
\expandafter\def\csname val@long-valid.opensre-x3.m5.dollars_median\endcsname{0.55}
\expandafter\def\csname val@long-valid.opensre-x3.m5.dollars_median.min\endcsname{0.47}
\expandafter\def\csname val@long-valid.opensre-x3.m5.dollars_median.max\endcsname{0.64}
\expandafter\def\csname val@long-valid.opensre-x3.m5.reached\endcsname{8.5}
\expandafter\def\csname val@long-valid.opensre-x3.m5.reached.min\endcsname{5.0}
\expandafter\def\csname val@long-valid.opensre-x3.m5.reached.max\endcsname{12.0}
\expandafter\def\csname val@long-valid.opensre-x3.m5.injected\endcsname{57}
\expandafter\def\csname val@long-valid.opensre-x3.m5.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.opensre-x3.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.median_s\endcsname{322}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.median_s.min\endcsname{243}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.median_s.max\endcsname{402}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.p90_s\endcsname{1987}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.p90_s.min\endcsname{490}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.p90_s.max\endcsname{3483}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.dollars_median\endcsname{1.65}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.dollars_median.min\endcsname{1.54}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.dollars_median.max\endcsname{1.76}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.reached\endcsname{21.0}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.reached.max\endcsname{34.0}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.opensre-x3.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.median_s\endcsname{196}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.median_s.min\endcsname{196}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.median_s.max\endcsname{196}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.p90_s\endcsname{4950}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.p90_s.min\endcsname{4950}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.p90_s.max\endcsname{4950}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.dollars_median\endcsname{1.14}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.dollars_median.min\endcsname{1.14}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.dollars_median.max\endcsname{1.14}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.reached\endcsname{5.5}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.reached.max\endcsname{11.0}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@long-valid.opensre-x3.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.opensre-x3.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.blast_radius.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.executed_mutating_actions\endcsname{11}
\expandafter\def\csname val@long-valid.opensre-x3.m7.executed_mutating_actions.min\endcsname{7}
\expandafter\def\csname val@long-valid.opensre-x3.m7.executed_mutating_actions.max\endcsname{15}
\expandafter\def\csname val@long-valid.opensre-x3.m7.claim_calls\endcsname{546}
\expandafter\def\csname val@long-valid.opensre-x3.m7.claim_calls.min\endcsname{545}
\expandafter\def\csname val@long-valid.opensre-x3.m7.claim_calls.max\endcsname{546}
\expandafter\def\csname val@long-valid.opensre-x3.m7.max_mutations_per_tick\endcsname{3.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unlinked_citations\endcsname{4.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.opensre-x3.m7.unlinked_citations.max\endcsname{8.00}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1\endcsname{0.05}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1.min\endcsname{0.03}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1.max\endcsname{0.06}
\expandafter\def\csname val@long-valid.orbit-0.m1.precision\endcsname{0.71}
\expandafter\def\csname val@long-valid.orbit-0.m1.precision.min\endcsname{0.43}
\expandafter\def\csname val@long-valid.orbit-0.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m1.recall\endcsname{0.02}
\expandafter\def\csname val@long-valid.orbit-0.m1.recall.min\endcsname{0.02}
\expandafter\def\csname val@long-valid.orbit-0.m1.recall.max\endcsname{0.03}
\expandafter\def\csname val@long-valid.orbit-0.m1.nrr\endcsname{-0.69}
\expandafter\def\csname val@long-valid.orbit-0.m1.nrr.min\endcsname{-0.89}
\expandafter\def\csname val@long-valid.orbit-0.m1.nrr.max\endcsname{-0.49}
\expandafter\def\csname val@long-valid.orbit-0.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-valid.orbit-0.m1.alerts_in_denominator.min\endcsname{54}
\expandafter\def\csname val@long-valid.orbit-0.m1.alerts_in_denominator.max\endcsname{90}
\expandafter\def\csname val@long-valid.orbit-0.m1.incidents_declared\endcsname{118}
\expandafter\def\csname val@long-valid.orbit-0.m1.incidents_declared.min\endcsname{102}
\expandafter\def\csname val@long-valid.orbit-0.m1.incidents_declared.max\endcsname{134}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_excluded\endcsname{51}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_excluded.min\endcsname{48}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_excluded.max\endcsname{54}
\expandafter\def\csname val@long-valid.orbit-0.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_share\endcsname{0.42}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_share.min\endcsname{0.38}
\expandafter\def\csname val@long-valid.orbit-0.m1.ambiguous_share.max\endcsname{0.47}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1_overlap\endcsname{0.22}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1_overlap.min\endcsname{0.16}
\expandafter\def\csname val@long-valid.orbit-0.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long-valid.orbit-0.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long-valid.orbit-0.m1.incident_precision.min\endcsname{0.91}
\expandafter\def\csname val@long-valid.orbit-0.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr\endcsname{0.21}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_symptomatic.max\endcsname{0.30}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate\endcsname{0.42}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate.max\endcsname{0.71}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate_symptomatic\endcsname{0.35}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long-valid.orbit-0.m3.mitigated_rate_symptomatic.max\endcsname{0.59}
\expandafter\def\csname val@long-valid.orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repairable_count\endcsname{21.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-valid.orbit-0.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret\endcsname{0.94}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret.max\endcsname{0.96}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret_raw\endcsname{0.94}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long-valid.orbit-0.m4.regret_raw.max\endcsname{0.96}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim\endcsname{4335}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim.min\endcsname{1192}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim.max\endcsname{7478}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m4.offered_requests\endcsname{8129.78}
\expandafter\def\csname val@long-valid.orbit-0.m4.offered_requests.min\endcsname{1525.92}
\expandafter\def\csname val@long-valid.orbit-0.m4.offered_requests.max\endcsname{14733.60}
\expandafter\def\csname val@long-valid.orbit-0.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@long-valid.orbit-0.m4.load_live_share.min\endcsname{0.45}
\expandafter\def\csname val@long-valid.orbit-0.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-valid.orbit-0.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m5.injected\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.median_s\endcsname{345}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.median_s.min\endcsname{250}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.median_s.max\endcsname{441}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.p90_s\endcsname{912}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.p90_s.min\endcsname{493}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.p90_s.max\endcsname{1331}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.dollars_median\endcsname{0.86}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.dollars_median.min\endcsname{0.59}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.dollars_median.max\endcsname{1.13}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.reached\endcsname{24.5}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.reached.max\endcsname{41.0}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-valid.orbit-0.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-valid.orbit-0.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.claim_calls\endcsname{4148}
\expandafter\def\csname val@long-valid.orbit-0.m7.claim_calls.min\endcsname{4036}
\expandafter\def\csname val@long-valid.orbit-0.m7.claim_calls.max\endcsname{4260}
\expandafter\def\csname val@long-valid.orbit-0.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-valid.orbit-0.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-valid.orbit-0.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@long-valid.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.smash_score\endcsname{6.57}
\expandafter\def\csname val@long-valid.b1-runbook.smash_lo_r1\endcsname{6.57}
\expandafter\def\csname val@long-valid.b1-runbook.smash_hi_r0\endcsname{6.57}
\expandafter\def\csname val@long-valid.b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@long-valid.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@long-valid.b1-runbook.rank\endcsname{2}
\expandafter\def\csname val@long-valid.react-b2.smash_score\endcsname{8.64}
\expandafter\def\csname val@long-valid.react-b2.smash_lo_r1\endcsname{8.64}
\expandafter\def\csname val@long-valid.react-b2.smash_hi_r0\endcsname{8.64}
\expandafter\def\csname val@long-valid.react-b2.dollars\endcsname{4.02}
\expandafter\def\csname val@long-valid.react-b2.llm_calls\endcsname{299}
\expandafter\def\csname val@long-valid.react-b2.rank\endcsname{1}
\expandafter\def\csname val@long-valid.rag-b2r.smash_score\endcsname{-8.43}
\expandafter\def\csname val@long-valid.rag-b2r.smash_lo_r1\endcsname{-8.43}
\expandafter\def\csname val@long-valid.rag-b2r.smash_hi_r0\endcsname{-8.43}
\expandafter\def\csname val@long-valid.rag-b2r.dollars\endcsname{0.46}
\expandafter\def\csname val@long-valid.rag-b2r.llm_calls\endcsname{34}
\expandafter\def\csname val@long-valid.rag-b2r.rank\endcsname{5}
\expandafter\def\csname val@long-valid.opensre-x3.smash_score\endcsname{-0.64}
\expandafter\def\csname val@long-valid.opensre-x3.smash_lo_r1\endcsname{-0.64}
\expandafter\def\csname val@long-valid.opensre-x3.smash_hi_r0\endcsname{-0.64}
\expandafter\def\csname val@long-valid.opensre-x3.dollars\endcsname{4.37}
\expandafter\def\csname val@long-valid.opensre-x3.llm_calls\endcsname{292}
\expandafter\def\csname val@long-valid.opensre-x3.rank\endcsname{4}
\expandafter\def\csname val@long-valid.orbit-0.smash_score\endcsname{2.69}
\expandafter\def\csname val@long-valid.orbit-0.smash_lo_r1\endcsname{2.69}
\expandafter\def\csname val@long-valid.orbit-0.smash_hi_r0\endcsname{2.69}
\expandafter\def\csname val@long-valid.orbit-0.dollars\endcsname{3.35}
\expandafter\def\csname val@long-valid.orbit-0.llm_calls\endcsname{124}
\expandafter\def\csname val@long-valid.orbit-0.rank\endcsname{3}
\expandafter\def\csname val@long-matched.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-matched.b0-null.m1.alerts_in_denominator.min\endcsname{55}
\expandafter\def\csname val@long-matched.b0-null.m1.alerts_in_denominator.max\endcsname{89}
\expandafter\def\csname val@long-matched.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_excluded\endcsname{53}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_excluded.min\endcsname{49}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_excluded.max\endcsname{57}
\expandafter\def\csname val@long-matched.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_share\endcsname{0.43}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long-matched.b0-null.m1.ambiguous_share.max\endcsname{0.47}
\expandafter\def\csname val@long-matched.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr\endcsname{0.20}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_symptomatic\endcsname{0.15}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate\endcsname{0.40}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.30}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long-matched.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long-matched.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long-matched.b0-null.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repairable_count\endcsname{21.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-matched.b0-null.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret_raw.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.regret_raw.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m4.uim\endcsname{4653}
\expandafter\def\csname val@long-matched.b0-null.m4.uim.min\endcsname{1244}
\expandafter\def\csname val@long-matched.b0-null.m4.uim.max\endcsname{8062}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m4.offered_requests\endcsname{8771.91}
\expandafter\def\csname val@long-matched.b0-null.m4.offered_requests.min\endcsname{1530.35}
\expandafter\def\csname val@long-matched.b0-null.m4.offered_requests.max\endcsname{16013.50}
\expandafter\def\csname val@long-matched.b0-null.m4.load_live_share\endcsname{0.78}
\expandafter\def\csname val@long-matched.b0-null.m4.load_live_share.min\endcsname{0.56}
\expandafter\def\csname val@long-matched.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m5.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.median_s\endcsname{310}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.median_s.min\endcsname{244}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.median_s.max\endcsname{375}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.p90_s\endcsname{940}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.p90_s.min\endcsname{613}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.p90_s.max\endcsname{1268}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.reached\endcsname{23.5}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b0-null.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1\endcsname{0.52}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1.min\endcsname{0.40}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1.max\endcsname{0.64}
\expandafter\def\csname val@long-matched.b1-runbook.m1.precision\endcsname{0.55}
\expandafter\def\csname val@long-matched.b1-runbook.m1.precision.min\endcsname{0.42}
\expandafter\def\csname val@long-matched.b1-runbook.m1.precision.max\endcsname{0.68}
\expandafter\def\csname val@long-matched.b1-runbook.m1.recall\endcsname{0.49}
\expandafter\def\csname val@long-matched.b1-runbook.m1.recall.min\endcsname{0.38}
\expandafter\def\csname val@long-matched.b1-runbook.m1.recall.max\endcsname{0.60}
\expandafter\def\csname val@long-matched.b1-runbook.m1.nrr\endcsname{0.50}
\expandafter\def\csname val@long-matched.b1-runbook.m1.nrr.min\endcsname{0.42}
\expandafter\def\csname val@long-matched.b1-runbook.m1.nrr.max\endcsname{0.57}
\expandafter\def\csname val@long-matched.b1-runbook.m1.alerts_in_denominator\endcsname{146}
\expandafter\def\csname val@long-matched.b1-runbook.m1.alerts_in_denominator.min\endcsname{114}
\expandafter\def\csname val@long-matched.b1-runbook.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incidents_declared\endcsname{76}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incidents_declared.min\endcsname{49}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incidents_declared.max\endcsname{102}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_excluded\endcsname{108}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_excluded.min\endcsname{102}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_excluded.max\endcsname{114}
\expandafter\def\csname val@long-matched.b1-runbook.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_share\endcsname{0.43}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long-matched.b1-runbook.m1.ambiguous_share.max\endcsname{0.50}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1_overlap\endcsname{0.63}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1_overlap.min\endcsname{0.44}
\expandafter\def\csname val@long-matched.b1-runbook.m1.f1_overlap.max\endcsname{0.82}
\expandafter\def\csname val@long-matched.b1-runbook.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incident_precision\endcsname{0.95}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incident_precision.min\endcsname{0.90}
\expandafter\def\csname val@long-matched.b1-runbook.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.mean_credit\endcsname{0.43}
\expandafter\def\csname val@long-matched.b1-runbook.m2.mean_credit.min\endcsname{0.28}
\expandafter\def\csname val@long-matched.b1-runbook.m2.mean_credit.max\endcsname{0.58}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_3\endcsname{0.02}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.acc_at_3.max\endcsname{0.03}
\expandafter\def\csname val@long-matched.b1-runbook.m2.services_overlap_mean\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.services_overlap_mean.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.category\endcsname{0.09}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.category.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.category.max\endcsname{0.16}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.services\endcsname{0.65}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.services.min\endcsname{0.47}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.services.max\endcsname{0.83}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.artifact\endcsname{0.52}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.artifact.min\endcsname{0.24}
\expandafter\def\csname val@long-matched.b1-runbook.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@long-matched.b1-runbook.m2.false_diagnoses\endcsname{9}
\expandafter\def\csname val@long-matched.b1-runbook.m2.false_diagnoses.min\endcsname{7}
\expandafter\def\csname val@long-matched.b1-runbook.m2.false_diagnoses.max\endcsname{11}
\expandafter\def\csname val@long-matched.b1-runbook.m2.loc_at_1\endcsname{0.52}
\expandafter\def\csname val@long-matched.b1-runbook.m2.loc_at_1.min\endcsname{0.24}
\expandafter\def\csname val@long-matched.b1-runbook.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long-matched.b1-runbook.m2.committed_claims\endcsname{72.50}
\expandafter\def\csname val@long-matched.b1-runbook.m2.committed_claims.min\endcsname{48.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.committed_claims.max\endcsname{97.00}
\expandafter\def\csname val@long-matched.b1-runbook.m2.claim_precision\endcsname{0.87}
\expandafter\def\csname val@long-matched.b1-runbook.m2.claim_precision.min\endcsname{0.85}
\expandafter\def\csname val@long-matched.b1-runbook.m2.claim_precision.max\endcsname{0.89}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr\endcsname{0.20}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr.min\endcsname{0.02}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr.max\endcsname{0.39}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_symptomatic.max\endcsname{0.23}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate\endcsname{0.30}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate.max\endcsname{0.57}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate_symptomatic\endcsname{0.18}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long-matched.b1-runbook.m3.agent_attributed_rate\endcsname{0.09}
\expandafter\def\csname val@long-matched.b1-runbook.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.agent_attributed_rate.max\endcsname{0.18}
\expandafter\def\csname val@long-matched.b1-runbook.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@long-matched.b1-runbook.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.root_fixed_rate.max\endcsname{0.21}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_agent\endcsname{0.05}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.fsr_agent.max\endcsname{0.09}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repaired_rate\endcsname{0.05}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repaired_rate.max\endcsname{0.09}
\expandafter\def\csname val@long-matched.b1-runbook.m3.cleared_without_agent_count\endcsname{0.50}
\expandafter\def\csname val@long-matched.b1-runbook.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repairable_count\endcsname{20.50}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-matched.b1-runbook.m3.repairable_count.max\endcsname{29.00}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret\endcsname{0.96}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret.max\endcsname{0.98}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret_raw\endcsname{0.96}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long-matched.b1-runbook.m4.regret_raw.max\endcsname{0.98}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim\endcsname{4542}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim.min\endcsname{1155}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim.max\endcsname{7930}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m4.offered_requests\endcsname{8244.61}
\expandafter\def\csname val@long-matched.b1-runbook.m4.offered_requests.min\endcsname{1454.79}
\expandafter\def\csname val@long-matched.b1-runbook.m4.offered_requests.max\endcsname{15034.40}
\expandafter\def\csname val@long-matched.b1-runbook.m4.load_live_share\endcsname{0.67}
\expandafter\def\csname val@long-matched.b1-runbook.m4.load_live_share.min\endcsname{0.35}
\expandafter\def\csname val@long-matched.b1-runbook.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.b1-runbook.m5.median_s\endcsname{132}
\expandafter\def\csname val@long-matched.b1-runbook.m5.median_s.min\endcsname{132}
\expandafter\def\csname val@long-matched.b1-runbook.m5.median_s.max\endcsname{132}
\expandafter\def\csname val@long-matched.b1-runbook.m5.p90_s\endcsname{563}
\expandafter\def\csname val@long-matched.b1-runbook.m5.p90_s.min\endcsname{563}
\expandafter\def\csname val@long-matched.b1-runbook.m5.p90_s.max\endcsname{563}
\expandafter\def\csname val@long-matched.b1-runbook.m5.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m5.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m5.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m5.reached\endcsname{1.0}
\expandafter\def\csname val@long-matched.b1-runbook.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.b1-runbook.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@long-matched.b1-runbook.m5.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.median_s\endcsname{431}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.median_s.min\endcsname{371}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.median_s.max\endcsname{491}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.p90_s\endcsname{863}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.p90_s.min\endcsname{374}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.p90_s.max\endcsname{1353}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.reached\endcsname{17.5}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.reached.min\endcsname{2.0}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.reached.max\endcsname{33.0}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.median_s\endcsname{489}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.median_s.min\endcsname{489}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.median_s.max\endcsname{489}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.p90_s\endcsname{920}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.p90_s.min\endcsname{920}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.p90_s.max\endcsname{920}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.reached\endcsname{6.0}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.reached.max\endcsname{12.0}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.b1-runbook.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.b1-runbook.m7.blast_radius\endcsname{0.04}
\expandafter\def\csname val@long-matched.b1-runbook.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.blast_radius.max\endcsname{0.09}
\expandafter\def\csname val@long-matched.b1-runbook.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.out_of_scope_actions\endcsname{2}
\expandafter\def\csname val@long-matched.b1-runbook.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unscoped_actions\endcsname{2}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unscoped_actions.max\endcsname{4}
\expandafter\def\csname val@long-matched.b1-runbook.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.m7.executed_mutating_actions\endcsname{71}
\expandafter\def\csname val@long-matched.b1-runbook.m7.executed_mutating_actions.min\endcsname{47}
\expandafter\def\csname val@long-matched.b1-runbook.m7.executed_mutating_actions.max\endcsname{95}
\expandafter\def\csname val@long-matched.b1-runbook.m7.claim_calls\endcsname{468}
\expandafter\def\csname val@long-matched.b1-runbook.m7.claim_calls.min\endcsname{284}
\expandafter\def\csname val@long-matched.b1-runbook.m7.claim_calls.max\endcsname{651}
\expandafter\def\csname val@long-matched.b1-runbook.m7.max_mutations_per_tick\endcsname{7.50}
\expandafter\def\csname val@long-matched.b1-runbook.m7.max_mutations_per_tick.min\endcsname{7.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@long-matched.b1-runbook.m7.refused_actions.min\endcsname{1}
\expandafter\def\csname val@long-matched.b1-runbook.m7.refused_actions.max\endcsname{2}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unlinked_citations\endcsname{31.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unlinked_citations.min\endcsname{30.00}
\expandafter\def\csname val@long-matched.b1-runbook.m7.unlinked_citations.max\endcsname{32.00}
\expandafter\def\csname val@long-matched.react-b2.m1.f1\endcsname{0.07}
\expandafter\def\csname val@long-matched.react-b2.m1.f1.min\endcsname{0.04}
\expandafter\def\csname val@long-matched.react-b2.m1.f1.max\endcsname{0.09}
\expandafter\def\csname val@long-matched.react-b2.m1.precision\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long-matched.react-b2.m1.precision.max\endcsname{0.05}
\expandafter\def\csname val@long-matched.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.nrr\endcsname{0.31}
\expandafter\def\csname val@long-matched.react-b2.m1.nrr.min\endcsname{0.30}
\expandafter\def\csname val@long-matched.react-b2.m1.nrr.max\endcsname{0.32}
\expandafter\def\csname val@long-matched.react-b2.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-matched.react-b2.m1.alerts_in_denominator.min\endcsname{53}
\expandafter\def\csname val@long-matched.react-b2.m1.alerts_in_denominator.max\endcsname{92}
\expandafter\def\csname val@long-matched.react-b2.m1.incidents_declared\endcsname{50}
\expandafter\def\csname val@long-matched.react-b2.m1.incidents_declared.min\endcsname{37}
\expandafter\def\csname val@long-matched.react-b2.m1.incidents_declared.max\endcsname{63}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_excluded\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_excluded.min\endcsname{53}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_excluded.max\endcsname{63}
\expandafter\def\csname val@long-matched.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_share\endcsname{0.45}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@long-matched.react-b2.m1.ambiguous_share.max\endcsname{0.54}
\expandafter\def\csname val@long-matched.react-b2.m1.f1_overlap\endcsname{0.16}
\expandafter\def\csname val@long-matched.react-b2.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.react-b2.m1.f1_overlap.max\endcsname{0.17}
\expandafter\def\csname val@long-matched.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long-matched.react-b2.m1.incident_precision.min\endcsname{0.92}
\expandafter\def\csname val@long-matched.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m2.mean_credit\endcsname{0.16}
\expandafter\def\csname val@long-matched.react-b2.m2.mean_credit.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.react-b2.m2.mean_credit.max\endcsname{0.24}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_1\endcsname{0.08}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_3\endcsname{0.09}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_3.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.react-b2.m2.acc_at_3.max\endcsname{0.14}
\expandafter\def\csname val@long-matched.react-b2.m2.services_overlap_mean\endcsname{0.82}
\expandafter\def\csname val@long-matched.react-b2.m2.services_overlap_mean.min\endcsname{0.67}
\expandafter\def\csname val@long-matched.react-b2.m2.services_overlap_mean.max\endcsname{0.97}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.category\endcsname{0.20}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.category.min\endcsname{0.10}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.category.max\endcsname{0.29}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.services\endcsname{0.19}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.services.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.services.max\endcsname{0.33}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.artifact\endcsname{0.10}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.artifact.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.react-b2.m2.component_rates.artifact.max\endcsname{0.14}
\expandafter\def\csname val@long-matched.react-b2.m2.false_diagnoses\endcsname{12}
\expandafter\def\csname val@long-matched.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m2.false_diagnoses.max\endcsname{24}
\expandafter\def\csname val@long-matched.react-b2.m2.loc_at_1\endcsname{0.08}
\expandafter\def\csname val@long-matched.react-b2.m2.loc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m2.loc_at_1.max\endcsname{0.12}
\expandafter\def\csname val@long-matched.react-b2.m2.committed_claims\endcsname{32.00}
\expandafter\def\csname val@long-matched.react-b2.m2.committed_claims.min\endcsname{6.00}
\expandafter\def\csname val@long-matched.react-b2.m2.committed_claims.max\endcsname{58.00}
\expandafter\def\csname val@long-matched.react-b2.m2.claim_precision\endcsname{0.79}
\expandafter\def\csname val@long-matched.react-b2.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long-matched.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr\endcsname{0.21}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_symptomatic\endcsname{0.16}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_symptomatic.min\endcsname{0.06}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_symptomatic.max\endcsname{0.25}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate\endcsname{0.37}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate.max\endcsname{0.60}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.31}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.12}
\expandafter\def\csname val@long-matched.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@long-matched.react-b2.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@long-matched.react-b2.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m3.agent_attributed_rate.max\endcsname{0.11}
\expandafter\def\csname val@long-matched.react-b2.m3.root_fixed_rate\endcsname{0.05}
\expandafter\def\csname val@long-matched.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m3.root_fixed_rate.max\endcsname{0.10}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_agent\endcsname{0.01}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m3.fsr_agent.max\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m3.repaired_rate\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m3.repaired_rate.max\endcsname{0.06}
\expandafter\def\csname val@long-matched.react-b2.m3.cleared_without_agent_count\endcsname{1.50}
\expandafter\def\csname val@long-matched.react-b2.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m3.cleared_without_agent_count.max\endcsname{2.00}
\expandafter\def\csname val@long-matched.react-b2.m3.repairable_count\endcsname{18.50}
\expandafter\def\csname val@long-matched.react-b2.m3.repairable_count.min\endcsname{10.00}
\expandafter\def\csname val@long-matched.react-b2.m3.repairable_count.max\endcsname{27.00}
\expandafter\def\csname val@long-matched.react-b2.m4.regret\endcsname{0.87}
\expandafter\def\csname val@long-matched.react-b2.m4.regret.min\endcsname{0.77}
\expandafter\def\csname val@long-matched.react-b2.m4.regret.max\endcsname{0.97}
\expandafter\def\csname val@long-matched.react-b2.m4.regret_raw\endcsname{0.87}
\expandafter\def\csname val@long-matched.react-b2.m4.regret_raw.min\endcsname{0.77}
\expandafter\def\csname val@long-matched.react-b2.m4.regret_raw.max\endcsname{0.97}
\expandafter\def\csname val@long-matched.react-b2.m4.uim\endcsname{4389}
\expandafter\def\csname val@long-matched.react-b2.m4.uim.min\endcsname{960}
\expandafter\def\csname val@long-matched.react-b2.m4.uim.max\endcsname{7818}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m4.offered_requests\endcsname{8785.66}
\expandafter\def\csname val@long-matched.react-b2.m4.offered_requests.min\endcsname{1378.15}
\expandafter\def\csname val@long-matched.react-b2.m4.offered_requests.max\endcsname{16193.20}
\expandafter\def\csname val@long-matched.react-b2.m4.load_live_share\endcsname{0.84}
\expandafter\def\csname val@long-matched.react-b2.m4.load_live_share.min\endcsname{0.67}
\expandafter\def\csname val@long-matched.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m5.median_s\endcsname{253}
\expandafter\def\csname val@long-matched.react-b2.m5.median_s.min\endcsname{155}
\expandafter\def\csname val@long-matched.react-b2.m5.median_s.max\endcsname{350}
\expandafter\def\csname val@long-matched.react-b2.m5.p90_s\endcsname{498}
\expandafter\def\csname val@long-matched.react-b2.m5.p90_s.min\endcsname{435}
\expandafter\def\csname val@long-matched.react-b2.m5.p90_s.max\endcsname{561}
\expandafter\def\csname val@long-matched.react-b2.m5.dollars_median\endcsname{0.91}
\expandafter\def\csname val@long-matched.react-b2.m5.dollars_median.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.react-b2.m5.dollars_median.max\endcsname{1.79}
\expandafter\def\csname val@long-matched.react-b2.m5.reached\endcsname{5.5}
\expandafter\def\csname val@long-matched.react-b2.m5.reached.min\endcsname{2.0}
\expandafter\def\csname val@long-matched.react-b2.m5.reached.max\endcsname{9.0}
\expandafter\def\csname val@long-matched.react-b2.m5.injected\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.median_s\endcsname{326}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.median_s.min\endcsname{246}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.median_s.max\endcsname{407}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.p90_s\endcsname{819}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.p90_s.min\endcsname{496}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.p90_s.max\endcsname{1143}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.dollars_median\endcsname{1.58}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.dollars_median.min\endcsname{1.41}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.dollars_median.max\endcsname{1.75}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.reached\endcsname{21.5}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.reached.max\endcsname{35.0}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.median_s\endcsname{1007}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.median_s.min\endcsname{1007}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.median_s.max\endcsname{1007}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.p90_s\endcsname{5479}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.p90_s.min\endcsname{5479}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.p90_s.max\endcsname{5479}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.dollars_median\endcsname{1.54}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.dollars_median.min\endcsname{1.54}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.54}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.reached\endcsname{3.0}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.reached.max\endcsname{6.0}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.react-b2.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.react-b2.m7.blast_radius\endcsname{0.21}
\expandafter\def\csname val@long-matched.react-b2.m7.blast_radius.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.react-b2.m7.blast_radius.max\endcsname{0.29}
\expandafter\def\csname val@long-matched.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.react-b2.m7.out_of_scope_actions\endcsname{4}
\expandafter\def\csname val@long-matched.react-b2.m7.out_of_scope_actions.min\endcsname{3}
\expandafter\def\csname val@long-matched.react-b2.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@long-matched.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.executed_mutating_actions\endcsname{18}
\expandafter\def\csname val@long-matched.react-b2.m7.executed_mutating_actions.min\endcsname{14}
\expandafter\def\csname val@long-matched.react-b2.m7.executed_mutating_actions.max\endcsname{22}
\expandafter\def\csname val@long-matched.react-b2.m7.claim_calls\endcsname{948}
\expandafter\def\csname val@long-matched.react-b2.m7.claim_calls.min\endcsname{356}
\expandafter\def\csname val@long-matched.react-b2.m7.claim_calls.max\endcsname{1540}
\expandafter\def\csname val@long-matched.react-b2.m7.max_mutations_per_tick\endcsname{4.00}
\expandafter\def\csname val@long-matched.react-b2.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long-matched.react-b2.m7.max_mutations_per_tick.max\endcsname{5.00}
\expandafter\def\csname val@long-matched.react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.react-b2.m7.unlinked_citations\endcsname{7.00}
\expandafter\def\csname val@long-matched.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.react-b2.m7.unlinked_citations.max\endcsname{13.00}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1\endcsname{0.37}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1.min\endcsname{0.32}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1.max\endcsname{0.42}
\expandafter\def\csname val@long-matched.rag-b2r.m1.precision\endcsname{0.24}
\expandafter\def\csname val@long-matched.rag-b2r.m1.precision.min\endcsname{0.21}
\expandafter\def\csname val@long-matched.rag-b2r.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long-matched.rag-b2r.m1.recall\endcsname{0.81}
\expandafter\def\csname val@long-matched.rag-b2r.m1.recall.min\endcsname{0.71}
\expandafter\def\csname val@long-matched.rag-b2r.m1.recall.max\endcsname{0.91}
\expandafter\def\csname val@long-matched.rag-b2r.m1.nrr\endcsname{0.72}
\expandafter\def\csname val@long-matched.rag-b2r.m1.nrr.min\endcsname{0.72}
\expandafter\def\csname val@long-matched.rag-b2r.m1.nrr.max\endcsname{0.72}
\expandafter\def\csname val@long-matched.rag-b2r.m1.alerts_in_denominator\endcsname{117}
\expandafter\def\csname val@long-matched.rag-b2r.m1.alerts_in_denominator.min\endcsname{57}
\expandafter\def\csname val@long-matched.rag-b2r.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incidents_declared\endcsname{32}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incidents_declared.min\endcsname{16}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incidents_declared.max\endcsname{49}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_excluded.min\endcsname{52}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_excluded.max\endcsname{62}
\expandafter\def\csname val@long-matched.rag-b2r.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_share\endcsname{0.37}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_share.min\endcsname{0.26}
\expandafter\def\csname val@long-matched.rag-b2r.m1.ambiguous_share.max\endcsname{0.48}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1_overlap\endcsname{0.39}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1_overlap.min\endcsname{0.35}
\expandafter\def\csname val@long-matched.rag-b2r.m1.f1_overlap.max\endcsname{0.42}
\expandafter\def\csname val@long-matched.rag-b2r.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incident_precision\endcsname{0.82}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incident_precision.min\endcsname{0.81}
\expandafter\def\csname val@long-matched.rag-b2r.m1.incident_precision.max\endcsname{0.84}
\expandafter\def\csname val@long-matched.rag-b2r.m2.mean_credit\endcsname{0.41}
\expandafter\def\csname val@long-matched.rag-b2r.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@long-matched.rag-b2r.m2.mean_credit.max\endcsname{0.69}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_1\endcsname{0.09}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_3\endcsname{0.09}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.acc_at_3.max\endcsname{0.19}
\expandafter\def\csname val@long-matched.rag-b2r.m2.services_overlap_mean\endcsname{0.82}
\expandafter\def\csname val@long-matched.rag-b2r.m2.services_overlap_mean.min\endcsname{0.70}
\expandafter\def\csname val@long-matched.rag-b2r.m2.services_overlap_mean.max\endcsname{0.94}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.category\endcsname{0.23}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.category.min\endcsname{0.22}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.category.max\endcsname{0.24}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.services\endcsname{0.56}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.services.min\endcsname{0.22}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.artifact\endcsname{0.44}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.component_rates.artifact.max\endcsname{0.88}
\expandafter\def\csname val@long-matched.rag-b2r.m2.false_diagnoses\endcsname{128}
\expandafter\def\csname val@long-matched.rag-b2r.m2.false_diagnoses.min\endcsname{115}
\expandafter\def\csname val@long-matched.rag-b2r.m2.false_diagnoses.max\endcsname{142}
\expandafter\def\csname val@long-matched.rag-b2r.m2.loc_at_1\endcsname{0.40}
\expandafter\def\csname val@long-matched.rag-b2r.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@long-matched.rag-b2r.m2.committed_claims\endcsname{350.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.committed_claims.min\endcsname{196.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.committed_claims.max\endcsname{504.00}
\expandafter\def\csname val@long-matched.rag-b2r.m2.claim_precision\endcsname{0.57}
\expandafter\def\csname val@long-matched.rag-b2r.m2.claim_precision.min\endcsname{0.41}
\expandafter\def\csname val@long-matched.rag-b2r.m2.claim_precision.max\endcsname{0.72}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_symptomatic\endcsname{0.14}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_symptomatic.max\endcsname{0.28}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate\endcsname{0.34}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate_symptomatic\endcsname{0.28}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.mitigated_rate_symptomatic.max\endcsname{0.56}
\expandafter\def\csname val@long-matched.rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.cleared_without_agent_count\endcsname{1.50}
\expandafter\def\csname val@long-matched.rag-b2r.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repairable_count\endcsname{24.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repairable_count.min\endcsname{11.00}
\expandafter\def\csname val@long-matched.rag-b2r.m3.repairable_count.max\endcsname{37.00}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret_raw\endcsname{1.47}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret_raw.min\endcsname{1.43}
\expandafter\def\csname val@long-matched.rag-b2r.m4.regret_raw.max\endcsname{1.50}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim\endcsname{6954}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim.min\endcsname{1778}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim.max\endcsname{12130}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m4.offered_requests\endcsname{9027.90}
\expandafter\def\csname val@long-matched.rag-b2r.m4.offered_requests.min\endcsname{2900.59}
\expandafter\def\csname val@long-matched.rag-b2r.m4.offered_requests.max\endcsname{15155.20}
\expandafter\def\csname val@long-matched.rag-b2r.m4.load_live_share\endcsname{0.65}
\expandafter\def\csname val@long-matched.rag-b2r.m4.load_live_share.min\endcsname{0.29}
\expandafter\def\csname val@long-matched.rag-b2r.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.rag-b2r.m5.median_s\endcsname{80}
\expandafter\def\csname val@long-matched.rag-b2r.m5.median_s.min\endcsname{80}
\expandafter\def\csname val@long-matched.rag-b2r.m5.median_s.max\endcsname{80}
\expandafter\def\csname val@long-matched.rag-b2r.m5.p90_s\endcsname{183}
\expandafter\def\csname val@long-matched.rag-b2r.m5.p90_s.min\endcsname{183}
\expandafter\def\csname val@long-matched.rag-b2r.m5.p90_s.max\endcsname{183}
\expandafter\def\csname val@long-matched.rag-b2r.m5.dollars_median\endcsname{0.30}
\expandafter\def\csname val@long-matched.rag-b2r.m5.dollars_median.min\endcsname{0.30}
\expandafter\def\csname val@long-matched.rag-b2r.m5.dollars_median.max\endcsname{0.30}
\expandafter\def\csname val@long-matched.rag-b2r.m5.reached\endcsname{5.5}
\expandafter\def\csname val@long-matched.rag-b2r.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.rag-b2r.m5.reached.max\endcsname{11.0}
\expandafter\def\csname val@long-matched.rag-b2r.m5.injected\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.median_s\endcsname{452}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.median_s.min\endcsname{452}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.median_s.max\endcsname{452}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.p90_s\endcsname{1426}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.p90_s.min\endcsname{1426}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.p90_s.max\endcsname{1426}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.dollars_median\endcsname{0.09}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.dollars_median.min\endcsname{0.09}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.dollars_median.max\endcsname{0.09}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.reached\endcsname{19.5}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.rag-b2r.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.rag-b2r.m7.blast_radius\endcsname{0.25}
\expandafter\def\csname val@long-matched.rag-b2r.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.blast_radius.max\endcsname{0.50}
\expandafter\def\csname val@long-matched.rag-b2r.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m7.out_of_scope_actions.max\endcsname{1}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.rag-b2r.m7.no_target_actions\endcsname{18}
\expandafter\def\csname val@long-matched.rag-b2r.m7.no_target_actions.min\endcsname{13}
\expandafter\def\csname val@long-matched.rag-b2r.m7.no_target_actions.max\endcsname{23}
\expandafter\def\csname val@long-matched.rag-b2r.m7.executed_mutating_actions\endcsname{34}
\expandafter\def\csname val@long-matched.rag-b2r.m7.executed_mutating_actions.min\endcsname{2}
\expandafter\def\csname val@long-matched.rag-b2r.m7.executed_mutating_actions.max\endcsname{66}
\expandafter\def\csname val@long-matched.rag-b2r.m7.claim_calls\endcsname{1341}
\expandafter\def\csname val@long-matched.rag-b2r.m7.claim_calls.min\endcsname{648}
\expandafter\def\csname val@long-matched.rag-b2r.m7.claim_calls.max\endcsname{2034}
\expandafter\def\csname val@long-matched.rag-b2r.m7.max_mutations_per_tick\endcsname{5.50}
\expandafter\def\csname val@long-matched.rag-b2r.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.refused_actions\endcsname{15}
\expandafter\def\csname val@long-matched.rag-b2r.m7.refused_actions.min\endcsname{5}
\expandafter\def\csname val@long-matched.rag-b2r.m7.refused_actions.max\endcsname{25}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unlinked_citations\endcsname{17.50}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unlinked_citations.min\endcsname{14.00}
\expandafter\def\csname val@long-matched.rag-b2r.m7.unlinked_citations.max\endcsname{21.00}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1\endcsname{0.20}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1.max\endcsname{0.36}
\expandafter\def\csname val@long-matched.opensre-x3.m1.precision\endcsname{0.15}
\expandafter\def\csname val@long-matched.opensre-x3.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@long-matched.opensre-x3.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@long-matched.opensre-x3.m1.recall\endcsname{0.77}
\expandafter\def\csname val@long-matched.opensre-x3.m1.recall.min\endcsname{0.54}
\expandafter\def\csname val@long-matched.opensre-x3.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m1.nrr\endcsname{0.94}
\expandafter\def\csname val@long-matched.opensre-x3.m1.nrr.min\endcsname{0.90}
\expandafter\def\csname val@long-matched.opensre-x3.m1.nrr.max\endcsname{0.99}
\expandafter\def\csname val@long-matched.opensre-x3.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-matched.opensre-x3.m1.alerts_in_denominator.min\endcsname{60}
\expandafter\def\csname val@long-matched.opensre-x3.m1.alerts_in_denominator.max\endcsname{85}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incidents_declared\endcsname{4}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incidents_declared.max\endcsname{6}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_excluded\endcsname{60}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_excluded.min\endcsname{54}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_excluded.max\endcsname{67}
\expandafter\def\csname val@long-matched.opensre-x3.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_share\endcsname{0.46}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@long-matched.opensre-x3.m1.ambiguous_share.max\endcsname{0.53}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1_overlap\endcsname{0.27}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.opensre-x3.m1.f1_overlap.max\endcsname{0.39}
\expandafter\def\csname val@long-matched.opensre-x3.m1.detection_recall\endcsname{0.97}
\expandafter\def\csname val@long-matched.opensre-x3.m1.detection_recall.min\endcsname{0.93}
\expandafter\def\csname val@long-matched.opensre-x3.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incident_precision\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incident_precision.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m2.mean_credit\endcsname{0.31}
\expandafter\def\csname val@long-matched.opensre-x3.m2.mean_credit.min\endcsname{0.29}
\expandafter\def\csname val@long-matched.opensre-x3.m2.mean_credit.max\endcsname{0.33}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_1.min\endcsname{0.09}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_3\endcsname{0.16}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_3.min\endcsname{0.09}
\expandafter\def\csname val@long-matched.opensre-x3.m2.acc_at_3.max\endcsname{0.22}
\expandafter\def\csname val@long-matched.opensre-x3.m2.services_overlap_mean\endcsname{0.90}
\expandafter\def\csname val@long-matched.opensre-x3.m2.services_overlap_mean.min\endcsname{0.85}
\expandafter\def\csname val@long-matched.opensre-x3.m2.services_overlap_mean.max\endcsname{0.95}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.category\endcsname{0.34}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.category.min\endcsname{0.27}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.category.max\endcsname{0.40}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.services\endcsname{0.40}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.services.min\endcsname{0.40}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.services.max\endcsname{0.41}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.artifact.min\endcsname{0.13}
\expandafter\def\csname val@long-matched.opensre-x3.m2.component_rates.artifact.max\endcsname{0.32}
\expandafter\def\csname val@long-matched.opensre-x3.m2.false_diagnoses\endcsname{30}
\expandafter\def\csname val@long-matched.opensre-x3.m2.false_diagnoses.min\endcsname{29}
\expandafter\def\csname val@long-matched.opensre-x3.m2.false_diagnoses.max\endcsname{31}
\expandafter\def\csname val@long-matched.opensre-x3.m2.loc_at_1\endcsname{0.22}
\expandafter\def\csname val@long-matched.opensre-x3.m2.loc_at_1.min\endcsname{0.13}
\expandafter\def\csname val@long-matched.opensre-x3.m2.loc_at_1.max\endcsname{0.32}
\expandafter\def\csname val@long-matched.opensre-x3.m2.committed_claims\endcsname{72.50}
\expandafter\def\csname val@long-matched.opensre-x3.m2.committed_claims.min\endcsname{70.00}
\expandafter\def\csname val@long-matched.opensre-x3.m2.committed_claims.max\endcsname{75.00}
\expandafter\def\csname val@long-matched.opensre-x3.m2.claim_precision\endcsname{0.59}
\expandafter\def\csname val@long-matched.opensre-x3.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@long-matched.opensre-x3.m2.claim_precision.max\endcsname{0.59}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr\endcsname{0.24}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr.max\endcsname{0.41}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_symptomatic\endcsname{0.13}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_symptomatic.max\endcsname{0.20}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate\endcsname{0.38}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate.max\endcsname{0.62}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long-matched.opensre-x3.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@long-matched.opensre-x3.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@long-matched.opensre-x3.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.agent_attributed_rate.max\endcsname{0.12}
\expandafter\def\csname val@long-matched.opensre-x3.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@long-matched.opensre-x3.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.root_fixed_rate.max\endcsname{0.20}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repairable_count\endcsname{21.50}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repairable_count.min\endcsname{13.00}
\expandafter\def\csname val@long-matched.opensre-x3.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret\endcsname{0.98}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret.min\endcsname{0.97}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret_raw\endcsname{1.20}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret_raw.min\endcsname{0.97}
\expandafter\def\csname val@long-matched.opensre-x3.m4.regret_raw.max\endcsname{1.44}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim\endcsname{4798}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim.min\endcsname{1793}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim.max\endcsname{7804}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m4.offered_requests\endcsname{9003.38}
\expandafter\def\csname val@long-matched.opensre-x3.m4.offered_requests.min\endcsname{2332.84}
\expandafter\def\csname val@long-matched.opensre-x3.m4.offered_requests.max\endcsname{15673.90}
\expandafter\def\csname val@long-matched.opensre-x3.m4.load_live_share\endcsname{0.68}
\expandafter\def\csname val@long-matched.opensre-x3.m4.load_live_share.min\endcsname{0.36}
\expandafter\def\csname val@long-matched.opensre-x3.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.opensre-x3.m5.median_s\endcsname{172}
\expandafter\def\csname val@long-matched.opensre-x3.m5.median_s.min\endcsname{152}
\expandafter\def\csname val@long-matched.opensre-x3.m5.median_s.max\endcsname{193}
\expandafter\def\csname val@long-matched.opensre-x3.m5.p90_s\endcsname{766}
\expandafter\def\csname val@long-matched.opensre-x3.m5.p90_s.min\endcsname{306}
\expandafter\def\csname val@long-matched.opensre-x3.m5.p90_s.max\endcsname{1225}
\expandafter\def\csname val@long-matched.opensre-x3.m5.dollars_median\endcsname{0.55}
\expandafter\def\csname val@long-matched.opensre-x3.m5.dollars_median.min\endcsname{0.47}
\expandafter\def\csname val@long-matched.opensre-x3.m5.dollars_median.max\endcsname{0.64}
\expandafter\def\csname val@long-matched.opensre-x3.m5.reached\endcsname{8.5}
\expandafter\def\csname val@long-matched.opensre-x3.m5.reached.min\endcsname{5.0}
\expandafter\def\csname val@long-matched.opensre-x3.m5.reached.max\endcsname{12.0}
\expandafter\def\csname val@long-matched.opensre-x3.m5.injected\endcsname{57}
\expandafter\def\csname val@long-matched.opensre-x3.m5.injected.min\endcsname{55}
\expandafter\def\csname val@long-matched.opensre-x3.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.median_s\endcsname{322}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.median_s.min\endcsname{243}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.median_s.max\endcsname{402}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.p90_s\endcsname{1987}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.p90_s.min\endcsname{490}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.p90_s.max\endcsname{3483}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.dollars_median\endcsname{1.65}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.dollars_median.min\endcsname{1.54}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.dollars_median.max\endcsname{1.76}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.reached\endcsname{21.0}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.reached.max\endcsname{34.0}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@long-matched.opensre-x3.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.median_s\endcsname{196}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.median_s.min\endcsname{196}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.median_s.max\endcsname{196}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.p90_s\endcsname{4950}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.p90_s.min\endcsname{4950}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.p90_s.max\endcsname{4950}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.dollars_median\endcsname{1.14}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.dollars_median.min\endcsname{1.14}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.dollars_median.max\endcsname{1.14}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.reached\endcsname{5.5}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.reached.max\endcsname{11.0}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@long-matched.opensre-x3.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.opensre-x3.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.blast_radius.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.executed_mutating_actions\endcsname{11}
\expandafter\def\csname val@long-matched.opensre-x3.m7.executed_mutating_actions.min\endcsname{7}
\expandafter\def\csname val@long-matched.opensre-x3.m7.executed_mutating_actions.max\endcsname{15}
\expandafter\def\csname val@long-matched.opensre-x3.m7.claim_calls\endcsname{546}
\expandafter\def\csname val@long-matched.opensre-x3.m7.claim_calls.min\endcsname{545}
\expandafter\def\csname val@long-matched.opensre-x3.m7.claim_calls.max\endcsname{546}
\expandafter\def\csname val@long-matched.opensre-x3.m7.max_mutations_per_tick\endcsname{3.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unlinked_citations\endcsname{4.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.opensre-x3.m7.unlinked_citations.max\endcsname{8.00}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1\endcsname{0.05}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1.min\endcsname{0.03}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1.max\endcsname{0.06}
\expandafter\def\csname val@long-matched.orbit-0.m1.precision\endcsname{0.71}
\expandafter\def\csname val@long-matched.orbit-0.m1.precision.min\endcsname{0.43}
\expandafter\def\csname val@long-matched.orbit-0.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m1.recall\endcsname{0.02}
\expandafter\def\csname val@long-matched.orbit-0.m1.recall.min\endcsname{0.02}
\expandafter\def\csname val@long-matched.orbit-0.m1.recall.max\endcsname{0.03}
\expandafter\def\csname val@long-matched.orbit-0.m1.nrr\endcsname{-0.69}
\expandafter\def\csname val@long-matched.orbit-0.m1.nrr.min\endcsname{-0.89}
\expandafter\def\csname val@long-matched.orbit-0.m1.nrr.max\endcsname{-0.49}
\expandafter\def\csname val@long-matched.orbit-0.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@long-matched.orbit-0.m1.alerts_in_denominator.min\endcsname{54}
\expandafter\def\csname val@long-matched.orbit-0.m1.alerts_in_denominator.max\endcsname{90}
\expandafter\def\csname val@long-matched.orbit-0.m1.incidents_declared\endcsname{118}
\expandafter\def\csname val@long-matched.orbit-0.m1.incidents_declared.min\endcsname{102}
\expandafter\def\csname val@long-matched.orbit-0.m1.incidents_declared.max\endcsname{134}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_excluded\endcsname{51}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_excluded.min\endcsname{48}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_excluded.max\endcsname{54}
\expandafter\def\csname val@long-matched.orbit-0.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_share\endcsname{0.42}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_share.min\endcsname{0.38}
\expandafter\def\csname val@long-matched.orbit-0.m1.ambiguous_share.max\endcsname{0.47}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1_overlap\endcsname{0.22}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1_overlap.min\endcsname{0.16}
\expandafter\def\csname val@long-matched.orbit-0.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long-matched.orbit-0.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long-matched.orbit-0.m1.incident_precision.min\endcsname{0.91}
\expandafter\def\csname val@long-matched.orbit-0.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr\endcsname{0.21}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_symptomatic.max\endcsname{0.30}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate\endcsname{0.42}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate.max\endcsname{0.71}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate_symptomatic\endcsname{0.35}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@long-matched.orbit-0.m3.mitigated_rate_symptomatic.max\endcsname{0.59}
\expandafter\def\csname val@long-matched.orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repairable_count\endcsname{21.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@long-matched.orbit-0.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret\endcsname{0.94}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret.max\endcsname{0.96}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret_raw\endcsname{0.94}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@long-matched.orbit-0.m4.regret_raw.max\endcsname{0.96}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim\endcsname{4335}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim.min\endcsname{1192}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim.max\endcsname{7478}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m4.offered_requests\endcsname{8129.78}
\expandafter\def\csname val@long-matched.orbit-0.m4.offered_requests.min\endcsname{1525.92}
\expandafter\def\csname val@long-matched.orbit-0.m4.offered_requests.max\endcsname{14733.60}
\expandafter\def\csname val@long-matched.orbit-0.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@long-matched.orbit-0.m4.load_live_share.min\endcsname{0.45}
\expandafter\def\csname val@long-matched.orbit-0.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@long-matched.orbit-0.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m5.injected\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m5.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.median_s\endcsname{345}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.median_s.min\endcsname{250}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.median_s.max\endcsname{441}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.p90_s\endcsname{912}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.p90_s.min\endcsname{493}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.p90_s.max\endcsname{1331}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.dollars_median\endcsname{0.86}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.dollars_median.min\endcsname{0.59}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.dollars_median.max\endcsname{1.13}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.reached\endcsname{24.5}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.reached.max\endcsname{41.0}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@long-matched.orbit-0.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-matched.orbit-0.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.claim_calls\endcsname{4148}
\expandafter\def\csname val@long-matched.orbit-0.m7.claim_calls.min\endcsname{4036}
\expandafter\def\csname val@long-matched.orbit-0.m7.claim_calls.max\endcsname{4260}
\expandafter\def\csname val@long-matched.orbit-0.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-matched.orbit-0.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-matched.orbit-0.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@long-matched.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.smash_score\endcsname{10.86}
\expandafter\def\csname val@long-matched.b1-runbook.smash_lo_r1\endcsname{10.86}
\expandafter\def\csname val@long-matched.b1-runbook.smash_hi_r0\endcsname{10.86}
\expandafter\def\csname val@long-matched.b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@long-matched.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@long-matched.b1-runbook.rank\endcsname{1}
\expandafter\def\csname val@long-matched.react-b2.smash_score\endcsname{7.79}
\expandafter\def\csname val@long-matched.react-b2.smash_lo_r1\endcsname{7.79}
\expandafter\def\csname val@long-matched.react-b2.smash_hi_r0\endcsname{7.79}
\expandafter\def\csname val@long-matched.react-b2.dollars\endcsname{4.00}
\expandafter\def\csname val@long-matched.react-b2.llm_calls\endcsname{320}
\expandafter\def\csname val@long-matched.react-b2.rank\endcsname{2}
\expandafter\def\csname val@long-matched.rag-b2r.smash_score\endcsname{-8.43}
\expandafter\def\csname val@long-matched.rag-b2r.smash_lo_r1\endcsname{-8.43}
\expandafter\def\csname val@long-matched.rag-b2r.smash_hi_r0\endcsname{-8.43}
\expandafter\def\csname val@long-matched.rag-b2r.dollars\endcsname{0.46}
\expandafter\def\csname val@long-matched.rag-b2r.llm_calls\endcsname{34}
\expandafter\def\csname val@long-matched.rag-b2r.rank\endcsname{5}
\expandafter\def\csname val@long-matched.opensre-x3.smash_score\endcsname{-0.64}
\expandafter\def\csname val@long-matched.opensre-x3.smash_lo_r1\endcsname{-0.64}
\expandafter\def\csname val@long-matched.opensre-x3.smash_hi_r0\endcsname{-0.64}
\expandafter\def\csname val@long-matched.opensre-x3.dollars\endcsname{4.37}
\expandafter\def\csname val@long-matched.opensre-x3.llm_calls\endcsname{292}
\expandafter\def\csname val@long-matched.opensre-x3.rank\endcsname{4}
\expandafter\def\csname val@long-matched.orbit-0.smash_score\endcsname{2.69}
\expandafter\def\csname val@long-matched.orbit-0.smash_lo_r1\endcsname{2.69}
\expandafter\def\csname val@long-matched.orbit-0.smash_hi_r0\endcsname{2.69}
\expandafter\def\csname val@long-matched.orbit-0.dollars\endcsname{3.35}
\expandafter\def\csname val@long-matched.orbit-0.llm_calls\endcsname{124}
\expandafter\def\csname val@long-matched.orbit-0.rank\endcsname{3}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.alerts_in_denominator\endcsname{44}
\expandafter\def\csname val@long-seed17.b0-null.m1.alerts_in_denominator.min\endcsname{44}
\expandafter\def\csname val@long-seed17.b0-null.m1.alerts_in_denominator.max\endcsname{44}
\expandafter\def\csname val@long-seed17.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_excluded\endcsname{55}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_excluded.min\endcsname{55}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_excluded.max\endcsname{55}
\expandafter\def\csname val@long-seed17.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_share\endcsname{0.56}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_share.min\endcsname{0.56}
\expandafter\def\csname val@long-seed17.b0-null.m1.ambiguous_share.max\endcsname{0.56}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr\endcsname{0.30}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr.min\endcsname{0.30}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr.max\endcsname{0.30}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_symptomatic.min\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_symptomatic.max\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate.min\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate.max\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.38}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.38}
\expandafter\def\csname val@long-seed17.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{0.38}
\expandafter\def\csname val@long-seed17.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.cleared_without_agent_count\endcsname{4.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.cleared_without_agent_count.min\endcsname{4.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.cleared_without_agent_count.max\endcsname{4.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repairable_count\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repairable_count.min\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b0-null.m3.repairable_count.max\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret_raw.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.regret_raw.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim.min\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim.max\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_null\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_null.min\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_null.max\endcsname{886}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m4.offered_requests\endcsname{1184.43}
\expandafter\def\csname val@long-seed17.b0-null.m4.offered_requests.min\endcsname{1184.43}
\expandafter\def\csname val@long-seed17.b0-null.m4.offered_requests.max\endcsname{1184.43}
\expandafter\def\csname val@long-seed17.b0-null.m4.load_live_share\endcsname{0.43}
\expandafter\def\csname val@long-seed17.b0-null.m4.load_live_share.min\endcsname{0.43}
\expandafter\def\csname val@long-seed17.b0-null.m4.load_live_share.max\endcsname{0.43}
\expandafter\def\csname val@long-seed17.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m5.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m5.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.median_s\endcsname{511}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.median_s.min\endcsname{511}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.median_s.max\endcsname{511}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.p90_s\endcsname{1298}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.p90_s.min\endcsname{1298}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.p90_s.max\endcsname{1298}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.reached\endcsname{35.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.reached.min\endcsname{35.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.reached.max\endcsname{35.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1.min\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1.max\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.precision\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.precision.min\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.precision.max\endcsname{0.85}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.recall\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.recall.min\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.recall.max\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.nrr\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.nrr.min\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.nrr.max\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.alerts_in_denominator\endcsname{78}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.alerts_in_denominator.min\endcsname{78}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.alerts_in_denominator.max\endcsname{78}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incidents_declared\endcsname{45}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incidents_declared.min\endcsname{45}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incidents_declared.max\endcsname{45}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_excluded\endcsname{113}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_excluded.min\endcsname{113}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_excluded.max\endcsname{113}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_share\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_share.min\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.ambiguous_share.max\endcsname{0.59}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1_overlap\endcsname{0.94}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1_overlap.min\endcsname{0.94}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.f1_overlap.max\endcsname{0.94}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incident_precision\endcsname{0.98}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incident_precision.min\endcsname{0.98}
\expandafter\def\csname val@long-seed17.b1-runbook.m1.incident_precision.max\endcsname{0.98}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.mean_credit\endcsname{0.25}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.mean_credit.min\endcsname{0.25}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.mean_credit.max\endcsname{0.25}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.services_overlap_mean\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.services_overlap_mean.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.category\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.category.min\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.category.max\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.services\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.services.min\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.services.max\endcsname{0.42}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.artifact.min\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.component_rates.artifact.max\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.false_diagnoses\endcsname{6}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.false_diagnoses.min\endcsname{6}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.false_diagnoses.max\endcsname{6}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.loc_at_1\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.loc_at_1.min\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.loc_at_1.max\endcsname{0.22}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.committed_claims\endcsname{42.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.committed_claims.min\endcsname{42.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.committed_claims.max\endcsname{42.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.claim_precision\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.claim_precision.min\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m2.claim_precision.max\endcsname{0.86}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr\endcsname{0.33}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr.min\endcsname{0.33}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr.max\endcsname{0.33}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_symptomatic.min\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_symptomatic.max\endcsname{0.19}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate\endcsname{0.51}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate.min\endcsname{0.51}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate.max\endcsname{0.51}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate_symptomatic\endcsname{0.29}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate_symptomatic.min\endcsname{0.29}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.mitigated_rate_symptomatic.max\endcsname{0.29}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.agent_attributed_rate\endcsname{0.10}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.agent_attributed_rate.min\endcsname{0.10}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.agent_attributed_rate.max\endcsname{0.10}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.root_fixed_rate\endcsname{0.15}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.root_fixed_rate.min\endcsname{0.15}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.root_fixed_rate.max\endcsname{0.15}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_agent\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_agent.min\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.fsr_agent.max\endcsname{0.12}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repaired_rate\endcsname{0.14}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repaired_rate.min\endcsname{0.14}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repaired_rate.max\endcsname{0.14}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.cleared_without_agent_count\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repairable_count\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repairable_count.min\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m3.repairable_count.max\endcsname{15.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret_raw\endcsname{1.43}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret_raw.min\endcsname{1.43}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.regret_raw.max\endcsname{1.43}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim\endcsname{1270}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim.min\endcsname{1270}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim.max\endcsname{1270}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_null\endcsname{886}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_null.min\endcsname{886}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_null.max\endcsname{886}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.offered_requests\endcsname{1644.01}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.offered_requests.min\endcsname{1644.01}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.offered_requests.max\endcsname{1644.01}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.load_live_share\endcsname{0.40}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.load_live_share.min\endcsname{0.40}
\expandafter\def\csname val@long-seed17.b1-runbook.m4.load_live_share.max\endcsname{0.40}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.median_s\endcsname{580}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.median_s.min\endcsname{580}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.median_s.max\endcsname{580}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.p90_s\endcsname{1245}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.p90_s.min\endcsname{1245}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.p90_s.max\endcsname{1245}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.reached\endcsname{30.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.reached.min\endcsname{30.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.reached.max\endcsname{30.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.median_s\endcsname{416}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.median_s.min\endcsname{416}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.median_s.max\endcsname{416}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.p90_s\endcsname{2410}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.p90_s.min\endcsname{2410}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.p90_s.max\endcsname{2410}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.dollars_median\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.reached\endcsname{9.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.reached.min\endcsname{9.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.reached.max\endcsname{9.0}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.blast_radius\endcsname{0.02}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.blast_radius.min\endcsname{0.02}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.blast_radius.max\endcsname{0.02}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.out_of_scope_actions\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.out_of_scope_actions.min\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.out_of_scope_actions.max\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unscoped_actions\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unscoped_actions.min\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unscoped_actions.max\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.executed_mutating_actions\endcsname{41}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.executed_mutating_actions.min\endcsname{41}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.executed_mutating_actions.max\endcsname{41}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.claim_calls\endcsname{290}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.claim_calls.min\endcsname{290}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.claim_calls.max\endcsname{290}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.max_mutations_per_tick\endcsname{6.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.max_mutations_per_tick.min\endcsname{6.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.max_mutations_per_tick.max\endcsname{6.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.refused_actions.min\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.refused_actions.max\endcsname{1}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unlinked_citations\endcsname{27.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unlinked_citations.min\endcsname{27.00}
\expandafter\def\csname val@long-seed17.b1-runbook.m7.unlinked_citations.max\endcsname{27.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m1.precision\endcsname{0.06}
\expandafter\def\csname val@long-seed17.react-b2.m1.precision.min\endcsname{0.06}
\expandafter\def\csname val@long-seed17.react-b2.m1.precision.max\endcsname{0.06}
\expandafter\def\csname val@long-seed17.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.nrr\endcsname{0.65}
\expandafter\def\csname val@long-seed17.react-b2.m1.nrr.min\endcsname{0.65}
\expandafter\def\csname val@long-seed17.react-b2.m1.nrr.max\endcsname{0.65}
\expandafter\def\csname val@long-seed17.react-b2.m1.alerts_in_denominator\endcsname{48}
\expandafter\def\csname val@long-seed17.react-b2.m1.alerts_in_denominator.min\endcsname{48}
\expandafter\def\csname val@long-seed17.react-b2.m1.alerts_in_denominator.max\endcsname{48}
\expandafter\def\csname val@long-seed17.react-b2.m1.incidents_declared\endcsname{17}
\expandafter\def\csname val@long-seed17.react-b2.m1.incidents_declared.min\endcsname{17}
\expandafter\def\csname val@long-seed17.react-b2.m1.incidents_declared.max\endcsname{17}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_excluded\endcsname{62}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_excluded.min\endcsname{62}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_excluded.max\endcsname{62}
\expandafter\def\csname val@long-seed17.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_share\endcsname{0.56}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_share.min\endcsname{0.56}
\expandafter\def\csname val@long-seed17.react-b2.m1.ambiguous_share.max\endcsname{0.56}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1_overlap\endcsname{0.19}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1_overlap.min\endcsname{0.19}
\expandafter\def\csname val@long-seed17.react-b2.m1.f1_overlap.max\endcsname{0.19}
\expandafter\def\csname val@long-seed17.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m1.incident_precision\endcsname{0.71}
\expandafter\def\csname val@long-seed17.react-b2.m1.incident_precision.min\endcsname{0.71}
\expandafter\def\csname val@long-seed17.react-b2.m1.incident_precision.max\endcsname{0.71}
\expandafter\def\csname val@long-seed17.react-b2.m2.mean_credit\endcsname{0.09}
\expandafter\def\csname val@long-seed17.react-b2.m2.mean_credit.min\endcsname{0.09}
\expandafter\def\csname val@long-seed17.react-b2.m2.mean_credit.max\endcsname{0.09}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_3\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_3.min\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.acc_at_3.max\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.services_overlap_mean\endcsname{0.60}
\expandafter\def\csname val@long-seed17.react-b2.m2.services_overlap_mean.min\endcsname{0.60}
\expandafter\def\csname val@long-seed17.react-b2.m2.services_overlap_mean.max\endcsname{0.60}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.category\endcsname{0.15}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.category.min\endcsname{0.15}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.category.max\endcsname{0.15}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.services\endcsname{0.08}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.services.min\endcsname{0.08}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.services.max\endcsname{0.08}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.artifact\endcsname{0.05}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.artifact.min\endcsname{0.05}
\expandafter\def\csname val@long-seed17.react-b2.m2.component_rates.artifact.max\endcsname{0.05}
\expandafter\def\csname val@long-seed17.react-b2.m2.false_diagnoses\endcsname{8}
\expandafter\def\csname val@long-seed17.react-b2.m2.false_diagnoses.min\endcsname{8}
\expandafter\def\csname val@long-seed17.react-b2.m2.false_diagnoses.max\endcsname{8}
\expandafter\def\csname val@long-seed17.react-b2.m2.loc_at_1\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.loc_at_1.min\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.loc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@long-seed17.react-b2.m2.committed_claims\endcsname{27.00}
\expandafter\def\csname val@long-seed17.react-b2.m2.committed_claims.min\endcsname{27.00}
\expandafter\def\csname val@long-seed17.react-b2.m2.committed_claims.max\endcsname{27.00}
\expandafter\def\csname val@long-seed17.react-b2.m2.claim_precision\endcsname{0.70}
\expandafter\def\csname val@long-seed17.react-b2.m2.claim_precision.min\endcsname{0.70}
\expandafter\def\csname val@long-seed17.react-b2.m2.claim_precision.max\endcsname{0.70}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr\endcsname{0.27}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr.min\endcsname{0.27}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr.max\endcsname{0.27}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_symptomatic.min\endcsname{0.17}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_symptomatic.max\endcsname{0.17}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate\endcsname{0.47}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate.min\endcsname{0.47}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate.max\endcsname{0.47}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.30}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.30}
\expandafter\def\csname val@long-seed17.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{0.30}
\expandafter\def\csname val@long-seed17.react-b2.m3.agent_attributed_rate\endcsname{0.04}
\expandafter\def\csname val@long-seed17.react-b2.m3.agent_attributed_rate.min\endcsname{0.04}
\expandafter\def\csname val@long-seed17.react-b2.m3.agent_attributed_rate.max\endcsname{0.04}
\expandafter\def\csname val@long-seed17.react-b2.m3.root_fixed_rate\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.root_fixed_rate.min\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.root_fixed_rate.max\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_agent\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_agent.min\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.fsr_agent.max\endcsname{0.07}
\expandafter\def\csname val@long-seed17.react-b2.m3.repaired_rate\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m3.repaired_rate.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m3.repaired_rate.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.react-b2.m3.cleared_without_agent_count\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m3.repairable_count\endcsname{16.00}
\expandafter\def\csname val@long-seed17.react-b2.m3.repairable_count.min\endcsname{16.00}
\expandafter\def\csname val@long-seed17.react-b2.m3.repairable_count.max\endcsname{16.00}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret_raw\endcsname{1.38}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret_raw.min\endcsname{1.38}
\expandafter\def\csname val@long-seed17.react-b2.m4.regret_raw.max\endcsname{1.38}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim\endcsname{1225}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim.min\endcsname{1225}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim.max\endcsname{1225}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_null\endcsname{886}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_null.min\endcsname{886}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_null.max\endcsname{886}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m4.offered_requests\endcsname{1651.24}
\expandafter\def\csname val@long-seed17.react-b2.m4.offered_requests.min\endcsname{1651.24}
\expandafter\def\csname val@long-seed17.react-b2.m4.offered_requests.max\endcsname{1651.24}
\expandafter\def\csname val@long-seed17.react-b2.m4.load_live_share\endcsname{0.48}
\expandafter\def\csname val@long-seed17.react-b2.m4.load_live_share.min\endcsname{0.48}
\expandafter\def\csname val@long-seed17.react-b2.m4.load_live_share.max\endcsname{0.48}
\expandafter\def\csname val@long-seed17.react-b2.m5.median_s\endcsname{625}
\expandafter\def\csname val@long-seed17.react-b2.m5.median_s.min\endcsname{625}
\expandafter\def\csname val@long-seed17.react-b2.m5.median_s.max\endcsname{625}
\expandafter\def\csname val@long-seed17.react-b2.m5.p90_s\endcsname{916}
\expandafter\def\csname val@long-seed17.react-b2.m5.p90_s.min\endcsname{916}
\expandafter\def\csname val@long-seed17.react-b2.m5.p90_s.max\endcsname{916}
\expandafter\def\csname val@long-seed17.react-b2.m5.dollars_median\endcsname{0.44}
\expandafter\def\csname val@long-seed17.react-b2.m5.dollars_median.min\endcsname{0.44}
\expandafter\def\csname val@long-seed17.react-b2.m5.dollars_median.max\endcsname{0.44}
\expandafter\def\csname val@long-seed17.react-b2.m5.reached\endcsname{2.0}
\expandafter\def\csname val@long-seed17.react-b2.m5.reached.min\endcsname{2.0}
\expandafter\def\csname val@long-seed17.react-b2.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@long-seed17.react-b2.m5.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m5.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.median_s\endcsname{443}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.median_s.min\endcsname{443}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.median_s.max\endcsname{443}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.p90_s\endcsname{2404}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.p90_s.min\endcsname{2404}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.p90_s.max\endcsname{2404}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.dollars_median\endcsname{1.18}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.dollars_median.min\endcsname{1.18}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.dollars_median.max\endcsname{1.18}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.reached\endcsname{28.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.reached.min\endcsname{28.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.reached.max\endcsname{28.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.median_s\endcsname{611}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.median_s.min\endcsname{611}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.median_s.max\endcsname{611}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.p90_s\endcsname{2911}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.p90_s.min\endcsname{2911}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.p90_s.max\endcsname{2911}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.dollars_median\endcsname{0.31}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.31}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.dollars_median.max\endcsname{0.31}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.reached\endcsname{4.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.reached.min\endcsname{4.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.reached.max\endcsname{4.0}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.react-b2.m7.blast_radius\endcsname{0.59}
\expandafter\def\csname val@long-seed17.react-b2.m7.blast_radius.min\endcsname{0.59}
\expandafter\def\csname val@long-seed17.react-b2.m7.blast_radius.max\endcsname{0.59}
\expandafter\def\csname val@long-seed17.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.out_of_scope_actions\endcsname{16}
\expandafter\def\csname val@long-seed17.react-b2.m7.out_of_scope_actions.min\endcsname{16}
\expandafter\def\csname val@long-seed17.react-b2.m7.out_of_scope_actions.max\endcsname{16}
\expandafter\def\csname val@long-seed17.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.react-b2.m7.executed_mutating_actions\endcsname{27}
\expandafter\def\csname val@long-seed17.react-b2.m7.executed_mutating_actions.min\endcsname{27}
\expandafter\def\csname val@long-seed17.react-b2.m7.executed_mutating_actions.max\endcsname{27}
\expandafter\def\csname val@long-seed17.react-b2.m7.claim_calls\endcsname{172}
\expandafter\def\csname val@long-seed17.react-b2.m7.claim_calls.min\endcsname{172}
\expandafter\def\csname val@long-seed17.react-b2.m7.claim_calls.max\endcsname{172}
\expandafter\def\csname val@long-seed17.react-b2.m7.max_mutations_per_tick\endcsname{4.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.max_mutations_per_tick.min\endcsname{4.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@long-seed17.react-b2.m7.refused_actions.min\endcsname{2}
\expandafter\def\csname val@long-seed17.react-b2.m7.refused_actions.max\endcsname{2}
\expandafter\def\csname val@long-seed17.react-b2.m7.unlinked_citations\endcsname{6.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.unlinked_citations.min\endcsname{6.00}
\expandafter\def\csname val@long-seed17.react-b2.m7.unlinked_citations.max\endcsname{6.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1\endcsname{0.65}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1.min\endcsname{0.65}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1.max\endcsname{0.65}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.precision\endcsname{0.53}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.precision.min\endcsname{0.53}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.precision.max\endcsname{0.53}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.recall\endcsname{0.83}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.recall.min\endcsname{0.83}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.recall.max\endcsname{0.83}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.nrr\endcsname{0.63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.nrr.min\endcsname{0.63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.nrr.max\endcsname{0.63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.alerts_in_denominator\endcsname{63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.alerts_in_denominator.min\endcsname{63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.alerts_in_denominator.max\endcsname{63}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incidents_declared\endcsname{23}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incidents_declared.min\endcsname{23}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incidents_declared.max\endcsname{23}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_excluded\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_excluded.min\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_excluded.max\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_share\endcsname{0.48}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_share.min\endcsname{0.48}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.ambiguous_share.max\endcsname{0.48}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1_overlap\endcsname{0.73}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1_overlap.min\endcsname{0.73}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.f1_overlap.max\endcsname{0.73}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incident_precision.min\endcsname{0.96}
\expandafter\def\csname val@long-seed17.rag-b2r.m1.incident_precision.max\endcsname{0.96}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.mean_credit\endcsname{0.27}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.mean_credit.min\endcsname{0.27}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.mean_credit.max\endcsname{0.27}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_1.min\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_1.max\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_3\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_3.min\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.acc_at_3.max\endcsname{0.14}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.services_overlap_mean\endcsname{0.76}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.services_overlap_mean.min\endcsname{0.76}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.services_overlap_mean.max\endcsname{0.76}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.category\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.category.min\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.category.max\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.services\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.services.min\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.services.max\endcsname{0.31}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.artifact.min\endcsname{0.22}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.component_rates.artifact.max\endcsname{0.22}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.false_diagnoses\endcsname{130}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.false_diagnoses.min\endcsname{130}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.false_diagnoses.max\endcsname{130}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.loc_at_1\endcsname{0.15}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.loc_at_1.min\endcsname{0.15}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.loc_at_1.max\endcsname{0.15}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.committed_claims\endcsname{232.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.committed_claims.min\endcsname{232.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.committed_claims.max\endcsname{232.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.claim_precision\endcsname{0.44}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.claim_precision.min\endcsname{0.44}
\expandafter\def\csname val@long-seed17.rag-b2r.m2.claim_precision.max\endcsname{0.44}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr\endcsname{0.33}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr.min\endcsname{0.33}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr.max\endcsname{0.33}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_symptomatic.min\endcsname{0.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_symptomatic.max\endcsname{0.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate\endcsname{0.54}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate.min\endcsname{0.54}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate.max\endcsname{0.54}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate_symptomatic\endcsname{0.29}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate_symptomatic.min\endcsname{0.29}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.mitigated_rate_symptomatic.max\endcsname{0.29}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.root_fixed_rate\endcsname{0.12}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.root_fixed_rate.min\endcsname{0.12}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.root_fixed_rate.max\endcsname{0.12}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_agent\endcsname{0.02}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_agent.min\endcsname{0.02}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.fsr_agent.max\endcsname{0.02}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repaired_rate\endcsname{0.05}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repaired_rate.min\endcsname{0.05}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repaired_rate.max\endcsname{0.05}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.cleared_without_agent_count\endcsname{3.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.cleared_without_agent_count.min\endcsname{3.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repairable_count\endcsname{15.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repairable_count.min\endcsname{15.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m3.repairable_count.max\endcsname{15.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret_raw\endcsname{1.74}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret_raw.min\endcsname{1.74}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.regret_raw.max\endcsname{1.74}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim\endcsname{1539}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim.min\endcsname{1539}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim.max\endcsname{1539}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_null\endcsname{886}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_null.min\endcsname{886}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_null.max\endcsname{886}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.offered_requests\endcsname{1986.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.offered_requests.min\endcsname{1986.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.offered_requests.max\endcsname{1986.17}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.load_live_share\endcsname{0.49}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.load_live_share.min\endcsname{0.49}
\expandafter\def\csname val@long-seed17.rag-b2r.m4.load_live_share.max\endcsname{0.49}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.median_s\endcsname{609}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.median_s.min\endcsname{609}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.median_s.max\endcsname{609}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.p90_s\endcsname{1711}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.p90_s.min\endcsname{1711}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.p90_s.max\endcsname{1711}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.dollars_median\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.dollars_median.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.dollars_median.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.reached\endcsname{8.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.reached.min\endcsname{8.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.reached.max\endcsname{8.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.median_s\endcsname{547}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.median_s.min\endcsname{547}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.median_s.max\endcsname{547}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.p90_s\endcsname{1306}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.p90_s.min\endcsname{1306}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.p90_s.max\endcsname{1306}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.dollars_median\endcsname{0.06}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.dollars_median.min\endcsname{0.06}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.dollars_median.max\endcsname{0.06}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.reached\endcsname{32.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.reached.min\endcsname{32.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.reached.max\endcsname{32.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.median_s\endcsname{7019}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.median_s.min\endcsname{7019}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.median_s.max\endcsname{7019}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.p90_s\endcsname{10556}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.p90_s.min\endcsname{10556}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.p90_s.max\endcsname{10556}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.dollars_median\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.dollars_median.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.dollars_median.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.reached\endcsname{7.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.reached.min\endcsname{7.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.reached.max\endcsname{7.0}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.blast_radius\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.blast_radius.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.blast_radius.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.out_of_scope_actions.min\endcsname{3}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.out_of_scope_actions.max\endcsname{3}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unscoped_actions\endcsname{2}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unscoped_actions.min\endcsname{2}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unscoped_actions.max\endcsname{2}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.no_target_actions\endcsname{1}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.no_target_actions.min\endcsname{1}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.no_target_actions.max\endcsname{1}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.executed_mutating_actions\endcsname{27}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.executed_mutating_actions.min\endcsname{27}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.executed_mutating_actions.max\endcsname{27}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.claim_calls\endcsname{791}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.claim_calls.min\endcsname{791}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.claim_calls.max\endcsname{791}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.max_mutations_per_tick\endcsname{16.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.max_mutations_per_tick.min\endcsname{16.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.max_mutations_per_tick.max\endcsname{16.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.refused_actions\endcsname{12}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.refused_actions.min\endcsname{12}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.refused_actions.max\endcsname{12}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unlinked_citations\endcsname{17.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unlinked_citations.min\endcsname{17.00}
\expandafter\def\csname val@long-seed17.rag-b2r.m7.unlinked_citations.max\endcsname{17.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1\endcsname{0.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1.min\endcsname{0.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1.max\endcsname{0.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.precision\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.precision.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.recall\endcsname{0.11}
\expandafter\def\csname val@long-seed17.orbit-0.m1.recall.min\endcsname{0.11}
\expandafter\def\csname val@long-seed17.orbit-0.m1.recall.max\endcsname{0.11}
\expandafter\def\csname val@long-seed17.orbit-0.m1.nrr\endcsname{-1.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.nrr.min\endcsname{-1.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.nrr.max\endcsname{-1.20}
\expandafter\def\csname val@long-seed17.orbit-0.m1.alerts_in_denominator\endcsname{44}
\expandafter\def\csname val@long-seed17.orbit-0.m1.alerts_in_denominator.min\endcsname{44}
\expandafter\def\csname val@long-seed17.orbit-0.m1.alerts_in_denominator.max\endcsname{44}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incidents_declared\endcsname{97}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incidents_declared.min\endcsname{97}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incidents_declared.max\endcsname{97}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_excluded\endcsname{57}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_excluded.min\endcsname{57}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_excluded.max\endcsname{57}
\expandafter\def\csname val@long-seed17.orbit-0.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_share\endcsname{0.56}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_share.min\endcsname{0.56}
\expandafter\def\csname val@long-seed17.orbit-0.m1.ambiguous_share.max\endcsname{0.56}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1_overlap\endcsname{0.28}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1_overlap.min\endcsname{0.28}
\expandafter\def\csname val@long-seed17.orbit-0.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@long-seed17.orbit-0.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incident_precision\endcsname{0.94}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incident_precision.min\endcsname{0.94}
\expandafter\def\csname val@long-seed17.orbit-0.m1.incident_precision.max\endcsname{0.94}
\expandafter\def\csname val@long-seed17.orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr\endcsname{0.31}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr.min\endcsname{0.31}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr.max\endcsname{0.31}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_symptomatic\endcsname{0.19}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_symptomatic.min\endcsname{0.19}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_symptomatic.max\endcsname{0.19}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate\endcsname{0.63}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate.min\endcsname{0.63}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate.max\endcsname{0.63}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate_symptomatic\endcsname{0.38}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate_symptomatic.min\endcsname{0.38}
\expandafter\def\csname val@long-seed17.orbit-0.m3.mitigated_rate_symptomatic.max\endcsname{0.38}
\expandafter\def\csname val@long-seed17.orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.cleared_without_agent_count\endcsname{4.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.cleared_without_agent_count.min\endcsname{4.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.cleared_without_agent_count.max\endcsname{4.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repairable_count\endcsname{15.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repairable_count.min\endcsname{15.00}
\expandafter\def\csname val@long-seed17.orbit-0.m3.repairable_count.max\endcsname{15.00}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret_raw\endcsname{2.87}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret_raw.min\endcsname{2.87}
\expandafter\def\csname val@long-seed17.orbit-0.m4.regret_raw.max\endcsname{2.87}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim\endcsname{2543}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim.min\endcsname{2543}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim.max\endcsname{2543}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_null\endcsname{886}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_null.min\endcsname{886}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_null.max\endcsname{886}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m4.offered_requests\endcsname{3233.16}
\expandafter\def\csname val@long-seed17.orbit-0.m4.offered_requests.min\endcsname{3233.16}
\expandafter\def\csname val@long-seed17.orbit-0.m4.offered_requests.max\endcsname{3233.16}
\expandafter\def\csname val@long-seed17.orbit-0.m4.load_live_share\endcsname{0.47}
\expandafter\def\csname val@long-seed17.orbit-0.m4.load_live_share.min\endcsname{0.47}
\expandafter\def\csname val@long-seed17.orbit-0.m4.load_live_share.max\endcsname{0.47}
\expandafter\def\csname val@long-seed17.orbit-0.m5.reached\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m5.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m5.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m5.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.median_s\endcsname{455}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.median_s.min\endcsname{455}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.median_s.max\endcsname{455}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.p90_s\endcsname{1226}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.p90_s.min\endcsname{1226}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.p90_s.max\endcsname{1226}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.dollars_median\endcsname{0.67}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.dollars_median.min\endcsname{0.67}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.dollars_median.max\endcsname{0.67}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.reached\endcsname{37.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.reached.min\endcsname{37.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.reached.max\endcsname{37.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.injected\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.injected.min\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@long-seed17.orbit-0.m7.violations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.claim_calls\endcsname{3887}
\expandafter\def\csname val@long-seed17.orbit-0.m7.claim_calls.min\endcsname{3887}
\expandafter\def\csname val@long-seed17.orbit-0.m7.claim_calls.max\endcsname{3887}
\expandafter\def\csname val@long-seed17.orbit-0.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@long-seed17.orbit-0.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.smash_hi_r0\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.smash_score\endcsname{0.64}
\expandafter\def\csname val@long-seed17.b1-runbook.smash_lo_r1\endcsname{0.64}
\expandafter\def\csname val@long-seed17.b1-runbook.smash_hi_r0\endcsname{0.64}
\expandafter\def\csname val@long-seed17.b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@long-seed17.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@long-seed17.b1-runbook.rank\endcsname{1}
\expandafter\def\csname val@long-seed17.react-b2.smash_score\endcsname{-9.02}
\expandafter\def\csname val@long-seed17.react-b2.smash_lo_r1\endcsname{-9.02}
\expandafter\def\csname val@long-seed17.react-b2.smash_hi_r0\endcsname{-9.02}
\expandafter\def\csname val@long-seed17.react-b2.dollars\endcsname{3.09}
\expandafter\def\csname val@long-seed17.react-b2.llm_calls\endcsname{313}
\expandafter\def\csname val@long-seed17.react-b2.rank\endcsname{2}
\expandafter\def\csname val@long-seed17.rag-b2r.smash_score\endcsname{-12.03}
\expandafter\def\csname val@long-seed17.rag-b2r.smash_lo_r1\endcsname{-12.03}
\expandafter\def\csname val@long-seed17.rag-b2r.smash_hi_r0\endcsname{-12.03}
\expandafter\def\csname val@long-seed17.rag-b2r.dollars\endcsname{0.24}
\expandafter\def\csname val@long-seed17.rag-b2r.llm_calls\endcsname{27}
\expandafter\def\csname val@long-seed17.rag-b2r.rank\endcsname{3}
\expandafter\def\csname val@long-seed17.orbit-0.smash_score\endcsname{-31.95}
\expandafter\def\csname val@long-seed17.orbit-0.smash_lo_r1\endcsname{-31.95}
\expandafter\def\csname val@long-seed17.orbit-0.smash_hi_r0\endcsname{-31.95}
\expandafter\def\csname val@long-seed17.orbit-0.dollars\endcsname{2.10}
\expandafter\def\csname val@long-seed17.orbit-0.llm_calls\endcsname{102}
\expandafter\def\csname val@long-seed17.orbit-0.rank\endcsname{4}
\expandafter\def\csname val@short.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m1.alerts_in_denominator\endcsname{20}
\expandafter\def\csname val@short.b0-null.m1.alerts_in_denominator.min\endcsname{4}
\expandafter\def\csname val@short.b0-null.m1.alerts_in_denominator.max\endcsname{45}
\expandafter\def\csname val@short.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_excluded\endcsname{12}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_excluded.min\endcsname{3}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_excluded.max\endcsname{43}
\expandafter\def\csname val@short.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_share\endcsname{0.40}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_share.min\endcsname{0.12}
\expandafter\def\csname val@short.b0-null.m1.ambiguous_share.max\endcsname{0.79}
\expandafter\def\csname val@short.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@short.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr\endcsname{0.20}
\expandafter\def\csname val@short.b0-null.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr.max\endcsname{0.50}
\expandafter\def\csname val@short.b0-null.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@short.b0-null.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate\endcsname{0.40}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.22}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.cleared_without_agent_count\endcsname{0.25}
\expandafter\def\csname val@short.b0-null.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m3.repairable_count\endcsname{3.75}
\expandafter\def\csname val@short.b0-null.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m3.repairable_count.max\endcsname{10.00}
\expandafter\def\csname val@short.b0-null.m4.uim\endcsname{3373}
\expandafter\def\csname val@short.b0-null.m4.uim.min\endcsname{38}
\expandafter\def\csname val@short.b0-null.m4.uim.max\endcsname{16714}
\expandafter\def\csname val@short.b0-null.m4.offered_requests\endcsname{5959.34}
\expandafter\def\csname val@short.b0-null.m4.offered_requests.min\endcsname{382.97}
\expandafter\def\csname val@short.b0-null.m4.offered_requests.max\endcsname{21368.60}
\expandafter\def\csname val@short.b0-null.m4.load_live_share\endcsname{0.90}
\expandafter\def\csname val@short.b0-null.m4.load_live_share.min\endcsname{0.19}
\expandafter\def\csname val@short.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m5.injected\endcsname{7}
\expandafter\def\csname val@short.b0-null.m5.injected.min\endcsname{5}
\expandafter\def\csname val@short.b0-null.m5.injected.max\endcsname{10}
\expandafter\def\csname val@short.b0-null.m6.mitigated.median_s\endcsname{404}
\expandafter\def\csname val@short.b0-null.m6.mitigated.median_s.min\endcsname{195}
\expandafter\def\csname val@short.b0-null.m6.mitigated.median_s.max\endcsname{884}
\expandafter\def\csname val@short.b0-null.m6.mitigated.p90_s\endcsname{610}
\expandafter\def\csname val@short.b0-null.m6.mitigated.p90_s.min\endcsname{348}
\expandafter\def\csname val@short.b0-null.m6.mitigated.p90_s.max\endcsname{1089}
\expandafter\def\csname val@short.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m6.mitigated.reached\endcsname{2.8}
\expandafter\def\csname val@short.b0-null.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m6.mitigated.reached.max\endcsname{10.0}
\expandafter\def\csname val@short.b0-null.m6.mitigated.injected\endcsname{7}
\expandafter\def\csname val@short.b0-null.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@short.b0-null.m6.mitigated.injected.max\endcsname{10}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.injected\endcsname{7}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@short.b0-null.m6.root_fixed.injected.max\endcsname{10}
\expandafter\def\csname val@short.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@short.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m1.f1\endcsname{0.39}
\expandafter\def\csname val@short.react-b2.m1.f1.min\endcsname{0.13}
\expandafter\def\csname val@short.react-b2.m1.f1.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.precision\endcsname{0.29}
\expandafter\def\csname val@short.react-b2.m1.precision.min\endcsname{0.07}
\expandafter\def\csname val@short.react-b2.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.nrr\endcsname{-0.74}
\expandafter\def\csname val@short.react-b2.m1.nrr.min\endcsname{-7.83}
\expandafter\def\csname val@short.react-b2.m1.nrr.max\endcsname{0.95}
\expandafter\def\csname val@short.react-b2.m1.alerts_in_denominator\endcsname{14}
\expandafter\def\csname val@short.react-b2.m1.alerts_in_denominator.min\endcsname{2}
\expandafter\def\csname val@short.react-b2.m1.alerts_in_denominator.max\endcsname{46}
\expandafter\def\csname val@short.react-b2.m1.incidents_declared\endcsname{13}
\expandafter\def\csname val@short.react-b2.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@short.react-b2.m1.incidents_declared.max\endcsname{53}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_excluded\endcsname{17}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_excluded.min\endcsname{5}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_excluded.max\endcsname{74}
\expandafter\def\csname val@short.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_share\endcsname{0.52}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_share.min\endcsname{0.19}
\expandafter\def\csname val@short.react-b2.m1.ambiguous_share.max\endcsname{0.93}
\expandafter\def\csname val@short.react-b2.m1.f1_overlap\endcsname{0.65}
\expandafter\def\csname val@short.react-b2.m1.f1_overlap.min\endcsname{0.35}
\expandafter\def\csname val@short.react-b2.m1.f1_overlap.max\endcsname{0.97}
\expandafter\def\csname val@short.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m1.incident_precision\endcsname{0.98}
\expandafter\def\csname val@short.react-b2.m1.incident_precision.min\endcsname{0.86}
\expandafter\def\csname val@short.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m2.mean_credit\endcsname{0.38}
\expandafter\def\csname val@short.react-b2.m2.mean_credit.min\endcsname{0.06}
\expandafter\def\csname val@short.react-b2.m2.mean_credit.max\endcsname{0.77}
\expandafter\def\csname val@short.react-b2.m2.acc_at_1\endcsname{0.19}
\expandafter\def\csname val@short.react-b2.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.acc_at_1.max\endcsname{0.60}
\expandafter\def\csname val@short.react-b2.m2.acc_at_3\endcsname{0.20}
\expandafter\def\csname val@short.react-b2.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.acc_at_3.max\endcsname{0.60}
\expandafter\def\csname val@short.react-b2.m2.services_overlap_mean\endcsname{0.71}
\expandafter\def\csname val@short.react-b2.m2.services_overlap_mean.min\endcsname{0.40}
\expandafter\def\csname val@short.react-b2.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m2.component_rates.category\endcsname{0.42}
\expandafter\def\csname val@short.react-b2.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.component_rates.category.max\endcsname{0.80}
\expandafter\def\csname val@short.react-b2.m2.component_rates.services\endcsname{0.39}
\expandafter\def\csname val@short.react-b2.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@short.react-b2.m2.component_rates.artifact\endcsname{0.36}
\expandafter\def\csname val@short.react-b2.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@short.react-b2.m2.false_diagnoses\endcsname{1}
\expandafter\def\csname val@short.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m2.false_diagnoses.max\endcsname{4}
\expandafter\def\csname val@short.react-b2.m2.loc_at_1\endcsname{0.24}
\expandafter\def\csname val@short.react-b2.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@short.react-b2.m2.committed_claims\endcsname{14.83}
\expandafter\def\csname val@short.react-b2.m2.committed_claims.min\endcsname{3.00}
\expandafter\def\csname val@short.react-b2.m2.committed_claims.max\endcsname{53.00}
\expandafter\def\csname val@short.react-b2.m2.claim_precision\endcsname{0.96}
\expandafter\def\csname val@short.react-b2.m2.claim_precision.min\endcsname{0.87}
\expandafter\def\csname val@short.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.fsr\endcsname{0.47}
\expandafter\def\csname val@short.react-b2.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.fsr.max\endcsname{0.90}
\expandafter\def\csname val@short.react-b2.m3.fsr_symptomatic\endcsname{0.48}
\expandafter\def\csname val@short.react-b2.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.fsr_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate\endcsname{0.71}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.64}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.agent_attributed_rate\endcsname{0.39}
\expandafter\def\csname val@short.react-b2.m3.agent_attributed_rate.min\endcsname{0.10}
\expandafter\def\csname val@short.react-b2.m3.agent_attributed_rate.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.root_fixed_rate\endcsname{0.23}
\expandafter\def\csname val@short.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.root_fixed_rate.max\endcsname{0.80}
\expandafter\def\csname val@short.react-b2.m3.fsr_agent\endcsname{0.46}
\expandafter\def\csname val@short.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.fsr_agent.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.repaired_rate\endcsname{0.60}
\expandafter\def\csname val@short.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.repaired_rate.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m3.cleared_without_agent_count\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.cleared_without_agent_count.max\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.repairable_count\endcsname{4.25}
\expandafter\def\csname val@short.react-b2.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m3.repairable_count.max\endcsname{10.00}
\expandafter\def\csname val@short.react-b2.m4.regret\endcsname{0.68}
\expandafter\def\csname val@short.react-b2.m4.regret.min\endcsname{0.16}
\expandafter\def\csname val@short.react-b2.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m4.regret_raw\endcsname{1.51}
\expandafter\def\csname val@short.react-b2.m4.regret_raw.min\endcsname{0.16}
\expandafter\def\csname val@short.react-b2.m4.regret_raw.max\endcsname{8.54}
\expandafter\def\csname val@short.react-b2.m4.uim\endcsname{3966}
\expandafter\def\csname val@short.react-b2.m4.uim.min\endcsname{69}
\expandafter\def\csname val@short.react-b2.m4.uim.max\endcsname{27672}
\expandafter\def\csname val@short.react-b2.m4.uim_null\endcsname{3373}
\expandafter\def\csname val@short.react-b2.m4.uim_null.min\endcsname{38}
\expandafter\def\csname val@short.react-b2.m4.uim_null.max\endcsname{16714}
\expandafter\def\csname val@short.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@short.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@short.react-b2.m4.offered_requests\endcsname{8419.74}
\expandafter\def\csname val@short.react-b2.m4.offered_requests.min\endcsname{687.81}
\expandafter\def\csname val@short.react-b2.m4.offered_requests.max\endcsname{30956.80}
\expandafter\def\csname val@short.react-b2.m4.load_live_share\endcsname{0.91}
\expandafter\def\csname val@short.react-b2.m4.load_live_share.min\endcsname{0.21}
\expandafter\def\csname val@short.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m5.median_s\endcsname{190}
\expandafter\def\csname val@short.react-b2.m5.median_s.min\endcsname{129}
\expandafter\def\csname val@short.react-b2.m5.median_s.max\endcsname{333}
\expandafter\def\csname val@short.react-b2.m5.p90_s\endcsname{757}
\expandafter\def\csname val@short.react-b2.m5.p90_s.min\endcsname{154}
\expandafter\def\csname val@short.react-b2.m5.p90_s.max\endcsname{2330}
\expandafter\def\csname val@short.react-b2.m5.dollars_median\endcsname{0.41}
\expandafter\def\csname val@short.react-b2.m5.dollars_median.min\endcsname{0.04}
\expandafter\def\csname val@short.react-b2.m5.dollars_median.max\endcsname{0.98}
\expandafter\def\csname val@short.react-b2.m5.reached\endcsname{1.7}
\expandafter\def\csname val@short.react-b2.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.react-b2.m5.reached.max\endcsname{6.0}
\expandafter\def\csname val@short.react-b2.m5.injected\endcsname{7}
\expandafter\def\csname val@short.react-b2.m5.injected.min\endcsname{5}
\expandafter\def\csname val@short.react-b2.m5.injected.max\endcsname{10}
\expandafter\def\csname val@short.react-b2.m6.mitigated.median_s\endcsname{509}
\expandafter\def\csname val@short.react-b2.m6.mitigated.median_s.min\endcsname{185}
\expandafter\def\csname val@short.react-b2.m6.mitigated.median_s.max\endcsname{957}
\expandafter\def\csname val@short.react-b2.m6.mitigated.p90_s\endcsname{790}
\expandafter\def\csname val@short.react-b2.m6.mitigated.p90_s.min\endcsname{341}
\expandafter\def\csname val@short.react-b2.m6.mitigated.p90_s.max\endcsname{1409}
\expandafter\def\csname val@short.react-b2.m6.mitigated.dollars_median\endcsname{0.65}
\expandafter\def\csname val@short.react-b2.m6.mitigated.dollars_median.min\endcsname{0.33}
\expandafter\def\csname val@short.react-b2.m6.mitigated.dollars_median.max\endcsname{1.19}
\expandafter\def\csname val@short.react-b2.m6.mitigated.reached\endcsname{4.8}
\expandafter\def\csname val@short.react-b2.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.react-b2.m6.mitigated.reached.max\endcsname{10.0}
\expandafter\def\csname val@short.react-b2.m6.mitigated.injected\endcsname{7}
\expandafter\def\csname val@short.react-b2.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@short.react-b2.m6.mitigated.injected.max\endcsname{10}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.median_s\endcsname{432}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.median_s.min\endcsname{160}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.median_s.max\endcsname{1055}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.p90_s\endcsname{709}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.p90_s.min\endcsname{160}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.p90_s.max\endcsname{1254}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.dollars_median\endcsname{0.49}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.05}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.31}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.reached\endcsname{1.3}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.reached.max\endcsname{4.0}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.injected\endcsname{7}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@short.react-b2.m6.root_fixed.injected.max\endcsname{10}
\expandafter\def\csname val@short.react-b2.m7.blast_radius\endcsname{0.31}
\expandafter\def\csname val@short.react-b2.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m7.blast_radius.max\endcsname{0.60}
\expandafter\def\csname val@short.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short.react-b2.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@short.react-b2.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.out_of_scope_actions.max\endcsname{9}
\expandafter\def\csname val@short.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.no_target_actions.max\endcsname{1}
\expandafter\def\csname val@short.react-b2.m7.executed_mutating_actions\endcsname{9}
\expandafter\def\csname val@short.react-b2.m7.executed_mutating_actions.min\endcsname{3}
\expandafter\def\csname val@short.react-b2.m7.executed_mutating_actions.max\endcsname{18}
\expandafter\def\csname val@short.react-b2.m7.claim_calls\endcsname{154}
\expandafter\def\csname val@short.react-b2.m7.claim_calls.min\endcsname{47}
\expandafter\def\csname val@short.react-b2.m7.claim_calls.max\endcsname{881}
\expandafter\def\csname val@short.react-b2.m7.max_mutations_per_tick\endcsname{3.00}
\expandafter\def\csname val@short.react-b2.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@short.react-b2.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@short.react-b2.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@short.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short.react-b2.m7.refused_actions.max\endcsname{9}
\expandafter\def\csname val@short.react-b2.m7.unlinked_citations\endcsname{2.33}
\expandafter\def\csname val@short.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@short.react-b2.m7.unlinked_citations.max\endcsname{6.00}
\expandafter\def\csname val@short.b0-null.smash_lo_r1\endcsname{0.52}
\expandafter\def\csname val@short.b0-null.smash_hi_r0\endcsname{35.52}
\expandafter\def\csname val@short.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@short.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@short.react-b2.smash_score\endcsname{23.13}
\expandafter\def\csname val@short.react-b2.smash_lo_r1\endcsname{23.13}
\expandafter\def\csname val@short.react-b2.smash_hi_r0\endcsname{23.13}
\expandafter\def\csname val@short.react-b2.dollars\endcsname{1.73}
\expandafter\def\csname val@short.react-b2.llm_calls\endcsname{203}
\expandafter\def\csname val@short.react-b2.rank\endcsname{1}
\expandafter\def\csname val@short5.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m1.alerts_in_denominator\endcsname{16}
\expandafter\def\csname val@short5.b0-null.m1.alerts_in_denominator.min\endcsname{7}
\expandafter\def\csname val@short5.b0-null.m1.alerts_in_denominator.max\endcsname{26}
\expandafter\def\csname val@short5.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_excluded\endcsname{8}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_excluded.min\endcsname{3}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_excluded.max\endcsname{11}
\expandafter\def\csname val@short5.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_share\endcsname{0.34}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_share.min\endcsname{0.12}
\expandafter\def\csname val@short5.b0-null.m1.ambiguous_share.max\endcsname{0.61}
\expandafter\def\csname val@short5.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr\endcsname{0.23}
\expandafter\def\csname val@short5.b0-null.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr.max\endcsname{0.50}
\expandafter\def\csname val@short5.b0-null.m3.fsr_symptomatic\endcsname{0.10}
\expandafter\def\csname val@short5.b0-null.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate\endcsname{0.47}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.20}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.cleared_without_agent_count\endcsname{0.33}
\expandafter\def\csname val@short5.b0-null.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m3.repairable_count\endcsname{2.00}
\expandafter\def\csname val@short5.b0-null.m3.repairable_count.min\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m3.repairable_count.max\endcsname{5.00}
\expandafter\def\csname val@short5.b0-null.m4.uim\endcsname{1887}
\expandafter\def\csname val@short5.b0-null.m4.uim.min\endcsname{106}
\expandafter\def\csname val@short5.b0-null.m4.uim.max\endcsname{4108}
\expandafter\def\csname val@short5.b0-null.m4.offered_requests\endcsname{5324.95}
\expandafter\def\csname val@short5.b0-null.m4.offered_requests.min\endcsname{1070.81}
\expandafter\def\csname val@short5.b0-null.m4.offered_requests.max\endcsname{11945.60}
\expandafter\def\csname val@short5.b0-null.m4.load_live_share\endcsname{0.94}
\expandafter\def\csname val@short5.b0-null.m4.load_live_share.min\endcsname{0.65}
\expandafter\def\csname val@short5.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short5.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m5.injected\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m5.injected.min\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m5.injected.max\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.median_s\endcsname{369}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.median_s.min\endcsname{195}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.median_s.max\endcsname{726}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.p90_s\endcsname{488}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.p90_s.min\endcsname{348}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.p90_s.max\endcsname{915}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.reached\endcsname{2.3}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.reached.max\endcsname{5.0}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.injected\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.mitigated.injected.max\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.injected\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m6.root_fixed.injected.max\endcsname{5}
\expandafter\def\csname val@short5.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@short5.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m1.f1\endcsname{0.30}
\expandafter\def\csname val@short5.react-b2.m1.f1.min\endcsname{0.20}
\expandafter\def\csname val@short5.react-b2.m1.f1.max\endcsname{0.44}
\expandafter\def\csname val@short5.react-b2.m1.precision\endcsname{0.18}
\expandafter\def\csname val@short5.react-b2.m1.precision.min\endcsname{0.11}
\expandafter\def\csname val@short5.react-b2.m1.precision.max\endcsname{0.29}
\expandafter\def\csname val@short5.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.nrr\endcsname{0.37}
\expandafter\def\csname val@short5.react-b2.m1.nrr.min\endcsname{0.15}
\expandafter\def\csname val@short5.react-b2.m1.nrr.max\endcsname{0.79}
\expandafter\def\csname val@short5.react-b2.m1.alerts_in_denominator\endcsname{12}
\expandafter\def\csname val@short5.react-b2.m1.alerts_in_denominator.min\endcsname{6}
\expandafter\def\csname val@short5.react-b2.m1.alerts_in_denominator.max\endcsname{17}
\expandafter\def\csname val@short5.react-b2.m1.incidents_declared\endcsname{8}
\expandafter\def\csname val@short5.react-b2.m1.incidents_declared.min\endcsname{2}
\expandafter\def\csname val@short5.react-b2.m1.incidents_declared.max\endcsname{14}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_excluded\endcsname{9}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_excluded.min\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_excluded.max\endcsname{11}
\expandafter\def\csname val@short5.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_share\endcsname{0.44}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_share.min\endcsname{0.31}
\expandafter\def\csname val@short5.react-b2.m1.ambiguous_share.max\endcsname{0.65}
\expandafter\def\csname val@short5.react-b2.m1.f1_overlap\endcsname{0.60}
\expandafter\def\csname val@short5.react-b2.m1.f1_overlap.min\endcsname{0.36}
\expandafter\def\csname val@short5.react-b2.m1.f1_overlap.max\endcsname{0.82}
\expandafter\def\csname val@short5.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m1.incident_precision\endcsname{0.98}
\expandafter\def\csname val@short5.react-b2.m1.incident_precision.min\endcsname{0.86}
\expandafter\def\csname val@short5.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m2.mean_credit\endcsname{0.36}
\expandafter\def\csname val@short5.react-b2.m2.mean_credit.min\endcsname{0.06}
\expandafter\def\csname val@short5.react-b2.m2.mean_credit.max\endcsname{0.66}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_1\endcsname{0.17}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_1.max\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_3\endcsname{0.17}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.acc_at_3.max\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m2.services_overlap_mean\endcsname{0.67}
\expandafter\def\csname val@short5.react-b2.m2.services_overlap_mean.min\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m2.services_overlap_mean.max\endcsname{0.88}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.category\endcsname{0.43}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.category.max\endcsname{0.80}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.services\endcsname{0.33}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.services.max\endcsname{0.60}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.artifact\endcsname{0.33}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@short5.react-b2.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m2.false_diagnoses.max\endcsname{2}
\expandafter\def\csname val@short5.react-b2.m2.loc_at_1\endcsname{0.20}
\expandafter\def\csname val@short5.react-b2.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m2.loc_at_1.max\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m2.committed_claims\endcsname{8.50}
\expandafter\def\csname val@short5.react-b2.m2.committed_claims.min\endcsname{3.00}
\expandafter\def\csname val@short5.react-b2.m2.committed_claims.max\endcsname{15.00}
\expandafter\def\csname val@short5.react-b2.m2.claim_precision\endcsname{0.97}
\expandafter\def\csname val@short5.react-b2.m2.claim_precision.min\endcsname{0.87}
\expandafter\def\csname val@short5.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.fsr\endcsname{0.65}
\expandafter\def\csname val@short5.react-b2.m3.fsr.min\endcsname{0.20}
\expandafter\def\csname val@short5.react-b2.m3.fsr.max\endcsname{0.90}
\expandafter\def\csname val@short5.react-b2.m3.fsr_symptomatic\endcsname{0.66}
\expandafter\def\csname val@short5.react-b2.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.fsr_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate\endcsname{0.90}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate.min\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.83}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.agent_attributed_rate\endcsname{0.53}
\expandafter\def\csname val@short5.react-b2.m3.agent_attributed_rate.min\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m3.agent_attributed_rate.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.root_fixed_rate\endcsname{0.40}
\expandafter\def\csname val@short5.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.root_fixed_rate.max\endcsname{0.80}
\expandafter\def\csname val@short5.react-b2.m3.fsr_agent\endcsname{0.66}
\expandafter\def\csname val@short5.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.fsr_agent.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.repaired_rate\endcsname{0.83}
\expandafter\def\csname val@short5.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.repaired_rate.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.cleared_without_agent_count\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.cleared_without_agent_count.max\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m3.repairable_count\endcsname{2.67}
\expandafter\def\csname val@short5.react-b2.m3.repairable_count.min\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m3.repairable_count.max\endcsname{5.00}
\expandafter\def\csname val@short5.react-b2.m4.regret\endcsname{0.54}
\expandafter\def\csname val@short5.react-b2.m4.regret.min\endcsname{0.44}
\expandafter\def\csname val@short5.react-b2.m4.regret.max\endcsname{0.66}
\expandafter\def\csname val@short5.react-b2.m4.regret_raw\endcsname{0.54}
\expandafter\def\csname val@short5.react-b2.m4.regret_raw.min\endcsname{0.44}
\expandafter\def\csname val@short5.react-b2.m4.regret_raw.max\endcsname{0.66}
\expandafter\def\csname val@short5.react-b2.m4.uim\endcsname{883}
\expandafter\def\csname val@short5.react-b2.m4.uim.min\endcsname{70}
\expandafter\def\csname val@short5.react-b2.m4.uim.max\endcsname{1820}
\expandafter\def\csname val@short5.react-b2.m4.uim_null\endcsname{1887}
\expandafter\def\csname val@short5.react-b2.m4.uim_null.min\endcsname{106}
\expandafter\def\csname val@short5.react-b2.m4.uim_null.max\endcsname{4108}
\expandafter\def\csname val@short5.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m4.offered_requests\endcsname{5595.48}
\expandafter\def\csname val@short5.react-b2.m4.offered_requests.min\endcsname{687.81}
\expandafter\def\csname val@short5.react-b2.m4.offered_requests.max\endcsname{12923.20}
\expandafter\def\csname val@short5.react-b2.m4.load_live_share\endcsname{0.95}
\expandafter\def\csname val@short5.react-b2.m4.load_live_share.min\endcsname{0.69}
\expandafter\def\csname val@short5.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m5.median_s\endcsname{161}
\expandafter\def\csname val@short5.react-b2.m5.median_s.min\endcsname{129}
\expandafter\def\csname val@short5.react-b2.m5.median_s.max\endcsname{176}
\expandafter\def\csname val@short5.react-b2.m5.p90_s\endcsname{199}
\expandafter\def\csname val@short5.react-b2.m5.p90_s.min\endcsname{176}
\expandafter\def\csname val@short5.react-b2.m5.p90_s.max\endcsname{238}
\expandafter\def\csname val@short5.react-b2.m5.dollars_median\endcsname{0.14}
\expandafter\def\csname val@short5.react-b2.m5.dollars_median.min\endcsname{0.04}
\expandafter\def\csname val@short5.react-b2.m5.dollars_median.max\endcsname{0.21}
\expandafter\def\csname val@short5.react-b2.m5.reached\endcsname{0.8}
\expandafter\def\csname val@short5.react-b2.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short5.react-b2.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@short5.react-b2.m5.injected\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m5.injected.min\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m5.injected.max\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.median_s\endcsname{538}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.median_s.min\endcsname{216}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.median_s.max\endcsname{957}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.p90_s\endcsname{762}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.p90_s.min\endcsname{341}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.p90_s.max\endcsname{1364}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.dollars_median\endcsname{0.63}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.dollars_median.min\endcsname{0.34}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.dollars_median.max\endcsname{1.19}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.reached\endcsname{4.5}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.reached.min\endcsname{2.0}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.reached.max\endcsname{5.0}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.injected\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.mitigated.injected.max\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.median_s\endcsname{345}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.median_s.min\endcsname{264}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.median_s.max\endcsname{447}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.p90_s\endcsname{710}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.p90_s.min\endcsname{489}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.p90_s.max\endcsname{1111}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.dollars_median\endcsname{0.39}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.10}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.dollars_median.max\endcsname{0.57}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.reached\endcsname{2.0}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.reached.max\endcsname{4.0}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.injected\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m6.root_fixed.injected.max\endcsname{5}
\expandafter\def\csname val@short5.react-b2.m7.blast_radius\endcsname{0.31}
\expandafter\def\csname val@short5.react-b2.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m7.blast_radius.max\endcsname{0.60}
\expandafter\def\csname val@short5.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short5.react-b2.m7.out_of_scope_actions\endcsname{2}
\expandafter\def\csname val@short5.react-b2.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@short5.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.executed_mutating_actions\endcsname{6}
\expandafter\def\csname val@short5.react-b2.m7.executed_mutating_actions.min\endcsname{3}
\expandafter\def\csname val@short5.react-b2.m7.executed_mutating_actions.max\endcsname{9}
\expandafter\def\csname val@short5.react-b2.m7.claim_calls\endcsname{62}
\expandafter\def\csname val@short5.react-b2.m7.claim_calls.min\endcsname{47}
\expandafter\def\csname val@short5.react-b2.m7.claim_calls.max\endcsname{83}
\expandafter\def\csname val@short5.react-b2.m7.max_mutations_per_tick\endcsname{2.50}
\expandafter\def\csname val@short5.react-b2.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@short5.react-b2.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@short5.react-b2.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short5.react-b2.m7.refused_actions.max\endcsname{1}
\expandafter\def\csname val@short5.react-b2.m7.unlinked_citations\endcsname{2.17}
\expandafter\def\csname val@short5.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@short5.react-b2.m7.unlinked_citations.max\endcsname{4.00}
\expandafter\def\csname val@short5.b0-null.smash_lo_r1\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.smash_hi_r0\endcsname{35.00}
\expandafter\def\csname val@short5.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@short5.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@short5.react-b2.smash_score\endcsname{41.35}
\expandafter\def\csname val@short5.react-b2.smash_lo_r1\endcsname{41.35}
\expandafter\def\csname val@short5.react-b2.smash_hi_r0\endcsname{41.35}
\expandafter\def\csname val@short5.react-b2.dollars\endcsname{1.23}
\expandafter\def\csname val@short5.react-b2.llm_calls\endcsname{160}
\expandafter\def\csname val@short5.react-b2.rank\endcsname{1}
\expandafter\def\csname val@short10.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m1.alerts_in_denominator\endcsname{25}
\expandafter\def\csname val@short10.b0-null.m1.alerts_in_denominator.min\endcsname{4}
\expandafter\def\csname val@short10.b0-null.m1.alerts_in_denominator.max\endcsname{45}
\expandafter\def\csname val@short10.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_excluded\endcsname{16}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_excluded.min\endcsname{6}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_excluded.max\endcsname{43}
\expandafter\def\csname val@short10.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_share\endcsname{0.46}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_share.min\endcsname{0.12}
\expandafter\def\csname val@short10.b0-null.m1.ambiguous_share.max\endcsname{0.79}
\expandafter\def\csname val@short10.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@short10.b0-null.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr.max\endcsname{0.50}
\expandafter\def\csname val@short10.b0-null.m3.fsr_symptomatic\endcsname{0.12}
\expandafter\def\csname val@short10.b0-null.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate\endcsname{0.34}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.24}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.cleared_without_agent_count\endcsname{0.17}
\expandafter\def\csname val@short10.b0-null.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m3.repairable_count\endcsname{5.50}
\expandafter\def\csname val@short10.b0-null.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m3.repairable_count.max\endcsname{10.00}
\expandafter\def\csname val@short10.b0-null.m4.uim\endcsname{4859}
\expandafter\def\csname val@short10.b0-null.m4.uim.min\endcsname{38}
\expandafter\def\csname val@short10.b0-null.m4.uim.max\endcsname{16714}
\expandafter\def\csname val@short10.b0-null.m4.offered_requests\endcsname{6593.73}
\expandafter\def\csname val@short10.b0-null.m4.offered_requests.min\endcsname{382.97}
\expandafter\def\csname val@short10.b0-null.m4.offered_requests.max\endcsname{21368.60}
\expandafter\def\csname val@short10.b0-null.m4.load_live_share\endcsname{0.86}
\expandafter\def\csname val@short10.b0-null.m4.load_live_share.min\endcsname{0.19}
\expandafter\def\csname val@short10.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short10.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m5.injected\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m5.injected.min\endcsname{9}
\expandafter\def\csname val@short10.b0-null.m5.injected.max\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.median_s\endcsname{462}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.median_s.min\endcsname{195}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.median_s.max\endcsname{884}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.p90_s\endcsname{811}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.p90_s.min\endcsname{574}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.p90_s.max\endcsname{1089}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.reached\endcsname{3.3}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.reached.max\endcsname{10.0}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.injected\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.injected.min\endcsname{9}
\expandafter\def\csname val@short10.b0-null.m6.mitigated.injected.max\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.injected\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.injected.min\endcsname{9}
\expandafter\def\csname val@short10.b0-null.m6.root_fixed.injected.max\endcsname{10}
\expandafter\def\csname val@short10.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@short10.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m1.f1\endcsname{0.48}
\expandafter\def\csname val@short10.react-b2.m1.f1.min\endcsname{0.13}
\expandafter\def\csname val@short10.react-b2.m1.f1.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.precision\endcsname{0.39}
\expandafter\def\csname val@short10.react-b2.m1.precision.min\endcsname{0.07}
\expandafter\def\csname val@short10.react-b2.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.nrr\endcsname{-1.86}
\expandafter\def\csname val@short10.react-b2.m1.nrr.min\endcsname{-7.83}
\expandafter\def\csname val@short10.react-b2.m1.nrr.max\endcsname{0.95}
\expandafter\def\csname val@short10.react-b2.m1.alerts_in_denominator\endcsname{16}
\expandafter\def\csname val@short10.react-b2.m1.alerts_in_denominator.min\endcsname{2}
\expandafter\def\csname val@short10.react-b2.m1.alerts_in_denominator.max\endcsname{46}
\expandafter\def\csname val@short10.react-b2.m1.incidents_declared\endcsname{18}
\expandafter\def\csname val@short10.react-b2.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@short10.react-b2.m1.incidents_declared.max\endcsname{53}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_excluded\endcsname{24}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_excluded.min\endcsname{7}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_excluded.max\endcsname{74}
\expandafter\def\csname val@short10.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_share\endcsname{0.60}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_share.min\endcsname{0.19}
\expandafter\def\csname val@short10.react-b2.m1.ambiguous_share.max\endcsname{0.93}
\expandafter\def\csname val@short10.react-b2.m1.f1_overlap\endcsname{0.69}
\expandafter\def\csname val@short10.react-b2.m1.f1_overlap.min\endcsname{0.35}
\expandafter\def\csname val@short10.react-b2.m1.f1_overlap.max\endcsname{0.97}
\expandafter\def\csname val@short10.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m1.incident_precision\endcsname{0.98}
\expandafter\def\csname val@short10.react-b2.m1.incident_precision.min\endcsname{0.93}
\expandafter\def\csname val@short10.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m2.mean_credit\endcsname{0.41}
\expandafter\def\csname val@short10.react-b2.m2.mean_credit.min\endcsname{0.18}
\expandafter\def\csname val@short10.react-b2.m2.mean_credit.max\endcsname{0.77}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_1\endcsname{0.22}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_1.max\endcsname{0.60}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_3\endcsname{0.23}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m2.acc_at_3.max\endcsname{0.60}
\expandafter\def\csname val@short10.react-b2.m2.services_overlap_mean\endcsname{0.75}
\expandafter\def\csname val@short10.react-b2.m2.services_overlap_mean.min\endcsname{0.57}
\expandafter\def\csname val@short10.react-b2.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.category\endcsname{0.40}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.category.min\endcsname{0.22}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.category.max\endcsname{0.60}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.services\endcsname{0.44}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.services.min\endcsname{0.22}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.artifact\endcsname{0.39}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@short10.react-b2.m2.false_diagnoses\endcsname{1}
\expandafter\def\csname val@short10.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m2.false_diagnoses.max\endcsname{4}
\expandafter\def\csname val@short10.react-b2.m2.loc_at_1\endcsname{0.28}
\expandafter\def\csname val@short10.react-b2.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@short10.react-b2.m2.committed_claims\endcsname{21.17}
\expandafter\def\csname val@short10.react-b2.m2.committed_claims.min\endcsname{9.00}
\expandafter\def\csname val@short10.react-b2.m2.committed_claims.max\endcsname{53.00}
\expandafter\def\csname val@short10.react-b2.m2.claim_precision\endcsname{0.96}
\expandafter\def\csname val@short10.react-b2.m2.claim_precision.min\endcsname{0.88}
\expandafter\def\csname val@short10.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m3.fsr\endcsname{0.30}
\expandafter\def\csname val@short10.react-b2.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.fsr.max\endcsname{0.65}
\expandafter\def\csname val@short10.react-b2.m3.fsr_symptomatic\endcsname{0.21}
\expandafter\def\csname val@short10.react-b2.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.fsr_symptomatic.max\endcsname{0.65}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate\endcsname{0.53}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.35}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m3.agent_attributed_rate\endcsname{0.17}
\expandafter\def\csname val@short10.react-b2.m3.agent_attributed_rate.min\endcsname{0.10}
\expandafter\def\csname val@short10.react-b2.m3.agent_attributed_rate.max\endcsname{0.20}
\expandafter\def\csname val@short10.react-b2.m3.root_fixed_rate\endcsname{0.07}
\expandafter\def\csname val@short10.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.root_fixed_rate.max\endcsname{0.30}
\expandafter\def\csname val@short10.react-b2.m3.fsr_agent\endcsname{0.16}
\expandafter\def\csname val@short10.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.fsr_agent.max\endcsname{0.65}
\expandafter\def\csname val@short10.react-b2.m3.repaired_rate\endcsname{0.25}
\expandafter\def\csname val@short10.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.repaired_rate.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m3.cleared_without_agent_count\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.cleared_without_agent_count.max\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.repairable_count\endcsname{5.83}
\expandafter\def\csname val@short10.react-b2.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m3.repairable_count.max\endcsname{10.00}
\expandafter\def\csname val@short10.react-b2.m4.regret\endcsname{0.82}
\expandafter\def\csname val@short10.react-b2.m4.regret.min\endcsname{0.16}
\expandafter\def\csname val@short10.react-b2.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m4.regret_raw\endcsname{2.48}
\expandafter\def\csname val@short10.react-b2.m4.regret_raw.min\endcsname{0.16}
\expandafter\def\csname val@short10.react-b2.m4.regret_raw.max\endcsname{8.54}
\expandafter\def\csname val@short10.react-b2.m4.uim\endcsname{7049}
\expandafter\def\csname val@short10.react-b2.m4.uim.min\endcsname{69}
\expandafter\def\csname val@short10.react-b2.m4.uim.max\endcsname{27672}
\expandafter\def\csname val@short10.react-b2.m4.uim_null\endcsname{4859}
\expandafter\def\csname val@short10.react-b2.m4.uim_null.min\endcsname{38}
\expandafter\def\csname val@short10.react-b2.m4.uim_null.max\endcsname{16714}
\expandafter\def\csname val@short10.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m4.offered_requests\endcsname{11243.99}
\expandafter\def\csname val@short10.react-b2.m4.offered_requests.min\endcsname{760.72}
\expandafter\def\csname val@short10.react-b2.m4.offered_requests.max\endcsname{30956.80}
\expandafter\def\csname val@short10.react-b2.m4.load_live_share\endcsname{0.87}
\expandafter\def\csname val@short10.react-b2.m4.load_live_share.min\endcsname{0.21}
\expandafter\def\csname val@short10.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m5.median_s\endcsname{213}
\expandafter\def\csname val@short10.react-b2.m5.median_s.min\endcsname{153}
\expandafter\def\csname val@short10.react-b2.m5.median_s.max\endcsname{333}
\expandafter\def\csname val@short10.react-b2.m5.p90_s\endcsname{1175}
\expandafter\def\csname val@short10.react-b2.m5.p90_s.min\endcsname{154}
\expandafter\def\csname val@short10.react-b2.m5.p90_s.max\endcsname{2330}
\expandafter\def\csname val@short10.react-b2.m5.dollars_median\endcsname{0.61}
\expandafter\def\csname val@short10.react-b2.m5.dollars_median.min\endcsname{0.17}
\expandafter\def\csname val@short10.react-b2.m5.dollars_median.max\endcsname{0.98}
\expandafter\def\csname val@short10.react-b2.m5.reached\endcsname{2.5}
\expandafter\def\csname val@short10.react-b2.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.react-b2.m5.reached.max\endcsname{6.0}
\expandafter\def\csname val@short10.react-b2.m5.injected\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m5.injected.min\endcsname{9}
\expandafter\def\csname val@short10.react-b2.m5.injected.max\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.median_s\endcsname{466}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.median_s.min\endcsname{185}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.median_s.max\endcsname{918}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.p90_s\endcsname{832}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.p90_s.min\endcsname{425}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.p90_s.max\endcsname{1409}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.dollars_median\endcsname{0.69}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.dollars_median.min\endcsname{0.33}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.dollars_median.max\endcsname{1.14}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.reached\endcsname{5.2}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.reached.max\endcsname{10.0}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.injected\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.injected.min\endcsname{9}
\expandafter\def\csname val@short10.react-b2.m6.mitigated.injected.max\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.median_s\endcsname{608}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.median_s.min\endcsname{160}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.median_s.max\endcsname{1055}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.p90_s\endcsname{707}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.p90_s.min\endcsname{160}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.p90_s.max\endcsname{1254}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.dollars_median\endcsname{0.68}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.05}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.31}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.reached\endcsname{0.7}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.reached.max\endcsname{3.0}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.injected\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.injected.min\endcsname{9}
\expandafter\def\csname val@short10.react-b2.m6.root_fixed.injected.max\endcsname{10}
\expandafter\def\csname val@short10.react-b2.m7.blast_radius\endcsname{0.30}
\expandafter\def\csname val@short10.react-b2.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m7.blast_radius.max\endcsname{0.50}
\expandafter\def\csname val@short10.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@short10.react-b2.m7.out_of_scope_actions\endcsname{4}
\expandafter\def\csname val@short10.react-b2.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.out_of_scope_actions.max\endcsname{9}
\expandafter\def\csname val@short10.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.no_target_actions.max\endcsname{1}
\expandafter\def\csname val@short10.react-b2.m7.executed_mutating_actions\endcsname{12}
\expandafter\def\csname val@short10.react-b2.m7.executed_mutating_actions.min\endcsname{4}
\expandafter\def\csname val@short10.react-b2.m7.executed_mutating_actions.max\endcsname{18}
\expandafter\def\csname val@short10.react-b2.m7.claim_calls\endcsname{246}
\expandafter\def\csname val@short10.react-b2.m7.claim_calls.min\endcsname{84}
\expandafter\def\csname val@short10.react-b2.m7.claim_calls.max\endcsname{881}
\expandafter\def\csname val@short10.react-b2.m7.max_mutations_per_tick\endcsname{3.50}
\expandafter\def\csname val@short10.react-b2.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@short10.react-b2.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@short10.react-b2.m7.refused_actions\endcsname{2}
\expandafter\def\csname val@short10.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@short10.react-b2.m7.refused_actions.max\endcsname{9}
\expandafter\def\csname val@short10.react-b2.m7.unlinked_citations\endcsname{2.50}
\expandafter\def\csname val@short10.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@short10.react-b2.m7.unlinked_citations.max\endcsname{6.00}
\expandafter\def\csname val@short10.b0-null.smash_lo_r1\endcsname{1.04}
\expandafter\def\csname val@short10.b0-null.smash_hi_r0\endcsname{36.04}
\expandafter\def\csname val@short10.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@short10.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@short10.react-b2.smash_score\endcsname{4.90}
\expandafter\def\csname val@short10.react-b2.smash_lo_r1\endcsname{4.90}
\expandafter\def\csname val@short10.react-b2.smash_hi_r0\endcsname{4.90}
\expandafter\def\csname val@short10.react-b2.dollars\endcsname{2.22}
\expandafter\def\csname val@short10.react-b2.llm_calls\endcsname{245}
\expandafter\def\csname val@short10.react-b2.rank\endcsname{1}
\expandafter\def\csname val@all.b0-null.m1.f1\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.f1.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.f1.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.precision\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.precision.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.precision.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.recall\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.recall.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.recall.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.nrr\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m1.nrr.min\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m1.nrr.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m1.alerts_in_denominator\endcsname{30}
\expandafter\def\csname val@all.b0-null.m1.alerts_in_denominator.min\endcsname{4}
\expandafter\def\csname val@all.b0-null.m1.alerts_in_denominator.max\endcsname{89}
\expandafter\def\csname val@all.b0-null.m1.incidents_declared\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.incidents_declared.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.incidents_declared.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_excluded\endcsname{29}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_excluded.min\endcsname{3}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_excluded.max\endcsname{184}
\expandafter\def\csname val@all.b0-null.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_share\endcsname{0.43}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_share.min\endcsname{0.12}
\expandafter\def\csname val@all.b0-null.m1.ambiguous_share.max\endcsname{0.79}
\expandafter\def\csname val@all.b0-null.m1.f1_overlap\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.f1_overlap.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.f1_overlap.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.detection_recall\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.detection_recall.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m1.detection_recall.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@all.b0-null.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr\endcsname{0.19}
\expandafter\def\csname val@all.b0-null.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr.max\endcsname{0.50}
\expandafter\def\csname val@all.b0-null.m3.fsr_symptomatic\endcsname{0.11}
\expandafter\def\csname val@all.b0-null.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr_symptomatic.max\endcsname{0.50}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate\endcsname{0.39}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate_symptomatic\endcsname{0.22}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.cleared_without_agent_count\endcsname{0.73}
\expandafter\def\csname val@all.b0-null.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.cleared_without_agent_count.max\endcsname{4.00}
\expandafter\def\csname val@all.b0-null.m3.repairable_count\endcsname{8.47}
\expandafter\def\csname val@all.b0-null.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m3.repairable_count.max\endcsname{40.00}
\expandafter\def\csname val@all.b0-null.m4.regret\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.regret.min\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.regret_raw\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.regret_raw.min\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.regret_raw.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m4.uim\endcsname{5864}
\expandafter\def\csname val@all.b0-null.m4.uim.min\endcsname{38}
\expandafter\def\csname val@all.b0-null.m4.uim.max\endcsname{38181}
\expandafter\def\csname val@all.b0-null.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@all.b0-null.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@all.b0-null.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@all.b0-null.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.b0-null.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m4.offered_requests\endcsname{10409.89}
\expandafter\def\csname val@all.b0-null.m4.offered_requests.min\endcsname{382.97}
\expandafter\def\csname val@all.b0-null.m4.offered_requests.max\endcsname{67092.50}
\expandafter\def\csname val@all.b0-null.m4.load_live_share\endcsname{0.89}
\expandafter\def\csname val@all.b0-null.m4.load_live_share.min\endcsname{0.19}
\expandafter\def\csname val@all.b0-null.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.b0-null.m5.reached\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m5.injected\endcsname{18}
\expandafter\def\csname val@all.b0-null.m5.injected.min\endcsname{5}
\expandafter\def\csname val@all.b0-null.m5.injected.max\endcsname{60}
\expandafter\def\csname val@all.b0-null.m6.mitigated.median_s\endcsname{376}
\expandafter\def\csname val@all.b0-null.m6.mitigated.median_s.min\endcsname{195}
\expandafter\def\csname val@all.b0-null.m6.mitigated.median_s.max\endcsname{884}
\expandafter\def\csname val@all.b0-null.m6.mitigated.p90_s\endcsname{655}
\expandafter\def\csname val@all.b0-null.m6.mitigated.p90_s.min\endcsname{348}
\expandafter\def\csname val@all.b0-null.m6.mitigated.p90_s.max\endcsname{1268}
\expandafter\def\csname val@all.b0-null.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m6.mitigated.reached\endcsname{6.1}
\expandafter\def\csname val@all.b0-null.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@all.b0-null.m6.mitigated.injected\endcsname{18}
\expandafter\def\csname val@all.b0-null.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@all.b0-null.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.injected\endcsname{18}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@all.b0-null.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@all.b0-null.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.claim_calls\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.claim_calls.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.claim_calls.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@all.b0-null.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m1.f1\endcsname{0.46}
\expandafter\def\csname val@all.b1-runbook.m1.f1.min\endcsname{0.35}
\expandafter\def\csname val@all.b1-runbook.m1.f1.max\endcsname{0.64}
\expandafter\def\csname val@all.b1-runbook.m1.precision\endcsname{0.46}
\expandafter\def\csname val@all.b1-runbook.m1.precision.min\endcsname{0.28}
\expandafter\def\csname val@all.b1-runbook.m1.precision.max\endcsname{0.68}
\expandafter\def\csname val@all.b1-runbook.m1.recall\endcsname{0.48}
\expandafter\def\csname val@all.b1-runbook.m1.recall.min\endcsname{0.38}
\expandafter\def\csname val@all.b1-runbook.m1.recall.max\endcsname{0.60}
\expandafter\def\csname val@all.b1-runbook.m1.nrr\endcsname{0.54}
\expandafter\def\csname val@all.b1-runbook.m1.nrr.min\endcsname{0.42}
\expandafter\def\csname val@all.b1-runbook.m1.nrr.max\endcsname{0.63}
\expandafter\def\csname val@all.b1-runbook.m1.alerts_in_denominator\endcsname{127}
\expandafter\def\csname val@all.b1-runbook.m1.alerts_in_denominator.min\endcsname{90}
\expandafter\def\csname val@all.b1-runbook.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@all.b1-runbook.m1.incidents_declared\endcsname{61}
\expandafter\def\csname val@all.b1-runbook.m1.incidents_declared.min\endcsname{33}
\expandafter\def\csname val@all.b1-runbook.m1.incidents_declared.max\endcsname{102}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_excluded\endcsname{126}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_excluded.min\endcsname{102}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_excluded.max\endcsname{163}
\expandafter\def\csname val@all.b1-runbook.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_share\endcsname{0.50}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_share.min\endcsname{0.37}
\expandafter\def\csname val@all.b1-runbook.m1.ambiguous_share.max\endcsname{0.64}
\expandafter\def\csname val@all.b1-runbook.m1.f1_overlap\endcsname{0.56}
\expandafter\def\csname val@all.b1-runbook.m1.f1_overlap.min\endcsname{0.41}
\expandafter\def\csname val@all.b1-runbook.m1.f1_overlap.max\endcsname{0.82}
\expandafter\def\csname val@all.b1-runbook.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m1.incident_precision\endcsname{0.90}
\expandafter\def\csname val@all.b1-runbook.m1.incident_precision.min\endcsname{0.79}
\expandafter\def\csname val@all.b1-runbook.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m2.mean_credit\endcsname{0.33}
\expandafter\def\csname val@all.b1-runbook.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@all.b1-runbook.m2.mean_credit.max\endcsname{0.58}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_1\endcsname{0.01}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_1.max\endcsname{0.03}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_3\endcsname{0.01}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m2.acc_at_3.max\endcsname{0.03}
\expandafter\def\csname val@all.b1-runbook.m2.services_overlap_mean\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m2.services_overlap_mean.min\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.category\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.category.min\endcsname{0.03}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.category.max\endcsname{0.16}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.services\endcsname{0.53}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.services.min\endcsname{0.29}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.services.max\endcsname{0.83}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.artifact\endcsname{0.36}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.artifact.min\endcsname{0.05}
\expandafter\def\csname val@all.b1-runbook.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@all.b1-runbook.m2.false_diagnoses\endcsname{13}
\expandafter\def\csname val@all.b1-runbook.m2.false_diagnoses.min\endcsname{7}
\expandafter\def\csname val@all.b1-runbook.m2.false_diagnoses.max\endcsname{21}
\expandafter\def\csname val@all.b1-runbook.m2.loc_at_1\endcsname{0.36}
\expandafter\def\csname val@all.b1-runbook.m2.loc_at_1.min\endcsname{0.05}
\expandafter\def\csname val@all.b1-runbook.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@all.b1-runbook.m2.committed_claims\endcsname{60.67}
\expandafter\def\csname val@all.b1-runbook.m2.committed_claims.min\endcsname{37.00}
\expandafter\def\csname val@all.b1-runbook.m2.committed_claims.max\endcsname{97.00}
\expandafter\def\csname val@all.b1-runbook.m2.claim_precision\endcsname{0.72}
\expandafter\def\csname val@all.b1-runbook.m2.claim_precision.min\endcsname{0.43}
\expandafter\def\csname val@all.b1-runbook.m2.claim_precision.max\endcsname{0.89}
\expandafter\def\csname val@all.b1-runbook.m3.fsr\endcsname{0.17}
\expandafter\def\csname val@all.b1-runbook.m3.fsr.min\endcsname{0.02}
\expandafter\def\csname val@all.b1-runbook.m3.fsr.max\endcsname{0.39}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_symptomatic\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_symptomatic.max\endcsname{0.23}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate\endcsname{0.24}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate.min\endcsname{0.03}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate.max\endcsname{0.57}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate_symptomatic\endcsname{0.14}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@all.b1-runbook.m3.agent_attributed_rate\endcsname{0.16}
\expandafter\def\csname val@all.b1-runbook.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.agent_attributed_rate.max\endcsname{0.29}
\expandafter\def\csname val@all.b1-runbook.m3.root_fixed_rate\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.root_fixed_rate.max\endcsname{0.21}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_agent\endcsname{0.04}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.fsr_agent.max\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m3.repaired_rate\endcsname{0.04}
\expandafter\def\csname val@all.b1-runbook.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.repaired_rate.max\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m3.cleared_without_agent_count\endcsname{0.33}
\expandafter\def\csname val@all.b1-runbook.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m3.cleared_without_agent_count.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m3.repairable_count\endcsname{26.33}
\expandafter\def\csname val@all.b1-runbook.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@all.b1-runbook.m3.repairable_count.max\endcsname{38.00}
\expandafter\def\csname val@all.b1-runbook.m4.regret\endcsname{0.97}
\expandafter\def\csname val@all.b1-runbook.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@all.b1-runbook.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m4.regret_raw\endcsname{1.05}
\expandafter\def\csname val@all.b1-runbook.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@all.b1-runbook.m4.regret_raw.max\endcsname{1.24}
\expandafter\def\csname val@all.b1-runbook.m4.uim\endcsname{18761}
\expandafter\def\csname val@all.b1-runbook.m4.uim.min\endcsname{1155}
\expandafter\def\csname val@all.b1-runbook.m4.uim.max\endcsname{47197}
\expandafter\def\csname val@all.b1-runbook.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@all.b1-runbook.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@all.b1-runbook.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@all.b1-runbook.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m4.offered_requests\endcsname{27462.55}
\expandafter\def\csname val@all.b1-runbook.m4.offered_requests.min\endcsname{1454.79}
\expandafter\def\csname val@all.b1-runbook.m4.offered_requests.max\endcsname{65898.40}
\expandafter\def\csname val@all.b1-runbook.m4.load_live_share\endcsname{0.78}
\expandafter\def\csname val@all.b1-runbook.m4.load_live_share.min\endcsname{0.35}
\expandafter\def\csname val@all.b1-runbook.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.b1-runbook.m5.median_s\endcsname{132}
\expandafter\def\csname val@all.b1-runbook.m5.median_s.min\endcsname{132}
\expandafter\def\csname val@all.b1-runbook.m5.median_s.max\endcsname{132}
\expandafter\def\csname val@all.b1-runbook.m5.p90_s\endcsname{563}
\expandafter\def\csname val@all.b1-runbook.m5.p90_s.min\endcsname{563}
\expandafter\def\csname val@all.b1-runbook.m5.p90_s.max\endcsname{563}
\expandafter\def\csname val@all.b1-runbook.m5.dollars_median\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m5.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m5.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m5.reached\endcsname{0.7}
\expandafter\def\csname val@all.b1-runbook.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.b1-runbook.m5.reached.max\endcsname{2.0}
\expandafter\def\csname val@all.b1-runbook.m5.injected\endcsname{57}
\expandafter\def\csname val@all.b1-runbook.m5.injected.min\endcsname{55}
\expandafter\def\csname val@all.b1-runbook.m5.injected.max\endcsname{59}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.median_s\endcsname{443}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.median_s.min\endcsname{371}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.median_s.max\endcsname{491}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.p90_s\endcsname{780}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.p90_s.min\endcsname{374}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.p90_s.max\endcsname{1353}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.dollars_median\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.reached\endcsname{14.0}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.reached.min\endcsname{2.0}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.reached.max\endcsname{33.0}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@all.b1-runbook.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.median_s\endcsname{486}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.median_s.min\endcsname{483}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.median_s.max\endcsname{489}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.p90_s\endcsname{1460}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.p90_s.min\endcsname{920}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.p90_s.max\endcsname{2001}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.dollars_median\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.dollars_median.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.dollars_median.max\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.reached\endcsname{5.3}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.reached.max\endcsname{12.0}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@all.b1-runbook.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@all.b1-runbook.m7.blast_radius\endcsname{0.04}
\expandafter\def\csname val@all.b1-runbook.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m7.blast_radius.max\endcsname{0.09}
\expandafter\def\csname val@all.b1-runbook.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.m7.out_of_scope_actions\endcsname{2}
\expandafter\def\csname val@all.b1-runbook.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.out_of_scope_actions.max\endcsname{4}
\expandafter\def\csname val@all.b1-runbook.m7.unscoped_actions\endcsname{2}
\expandafter\def\csname val@all.b1-runbook.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.unscoped_actions.max\endcsname{4}
\expandafter\def\csname val@all.b1-runbook.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.executed_mutating_actions\endcsname{60}
\expandafter\def\csname val@all.b1-runbook.m7.executed_mutating_actions.min\endcsname{37}
\expandafter\def\csname val@all.b1-runbook.m7.executed_mutating_actions.max\endcsname{95}
\expandafter\def\csname val@all.b1-runbook.m7.claim_calls\endcsname{416}
\expandafter\def\csname val@all.b1-runbook.m7.claim_calls.min\endcsname{284}
\expandafter\def\csname val@all.b1-runbook.m7.claim_calls.max\endcsname{651}
\expandafter\def\csname val@all.b1-runbook.m7.max_mutations_per_tick\endcsname{9.33}
\expandafter\def\csname val@all.b1-runbook.m7.max_mutations_per_tick.min\endcsname{7.00}
\expandafter\def\csname val@all.b1-runbook.m7.max_mutations_per_tick.max\endcsname{13.00}
\expandafter\def\csname val@all.b1-runbook.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@all.b1-runbook.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.m7.refused_actions.max\endcsname{2}
\expandafter\def\csname val@all.b1-runbook.m7.unlinked_citations\endcsname{26.00}
\expandafter\def\csname val@all.b1-runbook.m7.unlinked_citations.min\endcsname{16.00}
\expandafter\def\csname val@all.b1-runbook.m7.unlinked_citations.max\endcsname{32.00}
\expandafter\def\csname val@all.react-b2.m1.f1\endcsname{0.33}
\expandafter\def\csname val@all.react-b2.m1.f1.min\endcsname{0.04}
\expandafter\def\csname val@all.react-b2.m1.f1.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.precision\endcsname{0.24}
\expandafter\def\csname val@all.react-b2.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@all.react-b2.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.recall\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.recall.min\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.nrr\endcsname{-0.55}
\expandafter\def\csname val@all.react-b2.m1.nrr.min\endcsname{-7.83}
\expandafter\def\csname val@all.react-b2.m1.nrr.max\endcsname{0.95}
\expandafter\def\csname val@all.react-b2.m1.alerts_in_denominator\endcsname{25}
\expandafter\def\csname val@all.react-b2.m1.alerts_in_denominator.min\endcsname{2}
\expandafter\def\csname val@all.react-b2.m1.alerts_in_denominator.max\endcsname{92}
\expandafter\def\csname val@all.react-b2.m1.incidents_declared\endcsname{20}
\expandafter\def\csname val@all.react-b2.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@all.react-b2.m1.incidents_declared.max\endcsname{63}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_excluded\endcsname{33}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_excluded.min\endcsname{5}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_excluded.max\endcsname{172}
\expandafter\def\csname val@all.react-b2.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.react-b2.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_share\endcsname{0.53}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_share.min\endcsname{0.19}
\expandafter\def\csname val@all.react-b2.m1.ambiguous_share.max\endcsname{0.93}
\expandafter\def\csname val@all.react-b2.m1.f1_overlap\endcsname{0.56}
\expandafter\def\csname val@all.react-b2.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@all.react-b2.m1.f1_overlap.max\endcsname{0.97}
\expandafter\def\csname val@all.react-b2.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m1.incident_precision\endcsname{0.97}
\expandafter\def\csname val@all.react-b2.m1.incident_precision.min\endcsname{0.86}
\expandafter\def\csname val@all.react-b2.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m2.mean_credit\endcsname{0.34}
\expandafter\def\csname val@all.react-b2.m2.mean_credit.min\endcsname{0.06}
\expandafter\def\csname val@all.react-b2.m2.mean_credit.max\endcsname{0.77}
\expandafter\def\csname val@all.react-b2.m2.acc_at_1\endcsname{0.17}
\expandafter\def\csname val@all.react-b2.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.acc_at_1.max\endcsname{0.60}
\expandafter\def\csname val@all.react-b2.m2.acc_at_3\endcsname{0.18}
\expandafter\def\csname val@all.react-b2.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.acc_at_3.max\endcsname{0.60}
\expandafter\def\csname val@all.react-b2.m2.services_overlap_mean\endcsname{0.74}
\expandafter\def\csname val@all.react-b2.m2.services_overlap_mean.min\endcsname{0.40}
\expandafter\def\csname val@all.react-b2.m2.services_overlap_mean.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m2.component_rates.category\endcsname{0.37}
\expandafter\def\csname val@all.react-b2.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.component_rates.category.max\endcsname{0.80}
\expandafter\def\csname val@all.react-b2.m2.component_rates.services\endcsname{0.35}
\expandafter\def\csname val@all.react-b2.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@all.react-b2.m2.component_rates.artifact\endcsname{0.31}
\expandafter\def\csname val@all.react-b2.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.component_rates.artifact.max\endcsname{0.80}
\expandafter\def\csname val@all.react-b2.m2.false_diagnoses\endcsname{3}
\expandafter\def\csname val@all.react-b2.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m2.false_diagnoses.max\endcsname{24}
\expandafter\def\csname val@all.react-b2.m2.loc_at_1\endcsname{0.21}
\expandafter\def\csname val@all.react-b2.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@all.react-b2.m2.committed_claims\endcsname{17.80}
\expandafter\def\csname val@all.react-b2.m2.committed_claims.min\endcsname{3.00}
\expandafter\def\csname val@all.react-b2.m2.committed_claims.max\endcsname{58.00}
\expandafter\def\csname val@all.react-b2.m2.claim_precision\endcsname{0.91}
\expandafter\def\csname val@all.react-b2.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@all.react-b2.m2.claim_precision.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.fsr\endcsname{0.41}
\expandafter\def\csname val@all.react-b2.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.fsr.max\endcsname{0.90}
\expandafter\def\csname val@all.react-b2.m3.fsr_symptomatic\endcsname{0.39}
\expandafter\def\csname val@all.react-b2.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.fsr_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate\endcsname{0.63}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate_symptomatic\endcsname{0.54}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.mitigated_rate_symptomatic.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.agent_attributed_rate\endcsname{0.31}
\expandafter\def\csname val@all.react-b2.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.agent_attributed_rate.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.root_fixed_rate\endcsname{0.20}
\expandafter\def\csname val@all.react-b2.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.root_fixed_rate.max\endcsname{0.80}
\expandafter\def\csname val@all.react-b2.m3.fsr_agent\endcsname{0.36}
\expandafter\def\csname val@all.react-b2.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.fsr_agent.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.repaired_rate\endcsname{0.47}
\expandafter\def\csname val@all.react-b2.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.repaired_rate.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m3.cleared_without_agent_count\endcsname{0.27}
\expandafter\def\csname val@all.react-b2.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.cleared_without_agent_count.max\endcsname{2.00}
\expandafter\def\csname val@all.react-b2.m3.repairable_count\endcsname{8.27}
\expandafter\def\csname val@all.react-b2.m3.repairable_count.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m3.repairable_count.max\endcsname{36.00}
\expandafter\def\csname val@all.react-b2.m4.regret\endcsname{0.71}
\expandafter\def\csname val@all.react-b2.m4.regret.min\endcsname{0.16}
\expandafter\def\csname val@all.react-b2.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m4.regret_raw\endcsname{1.38}
\expandafter\def\csname val@all.react-b2.m4.regret_raw.min\endcsname{0.16}
\expandafter\def\csname val@all.react-b2.m4.regret_raw.max\endcsname{8.54}
\expandafter\def\csname val@all.react-b2.m4.uim\endcsname{5711}
\expandafter\def\csname val@all.react-b2.m4.uim.min\endcsname{69}
\expandafter\def\csname val@all.react-b2.m4.uim.max\endcsname{29297}
\expandafter\def\csname val@all.react-b2.m4.uim_null\endcsname{5864}
\expandafter\def\csname val@all.react-b2.m4.uim_null.min\endcsname{38}
\expandafter\def\csname val@all.react-b2.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@all.react-b2.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.react-b2.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.react-b2.m4.offered_requests\endcsname{11523.16}
\expandafter\def\csname val@all.react-b2.m4.offered_requests.min\endcsname{687.81}
\expandafter\def\csname val@all.react-b2.m4.offered_requests.max\endcsname{54239.20}
\expandafter\def\csname val@all.react-b2.m4.load_live_share\endcsname{0.90}
\expandafter\def\csname val@all.react-b2.m4.load_live_share.min\endcsname{0.21}
\expandafter\def\csname val@all.react-b2.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m5.median_s\endcsname{220}
\expandafter\def\csname val@all.react-b2.m5.median_s.min\endcsname{129}
\expandafter\def\csname val@all.react-b2.m5.median_s.max\endcsname{359}
\expandafter\def\csname val@all.react-b2.m5.p90_s\endcsname{680}
\expandafter\def\csname val@all.react-b2.m5.p90_s.min\endcsname{154}
\expandafter\def\csname val@all.react-b2.m5.p90_s.max\endcsname{2330}
\expandafter\def\csname val@all.react-b2.m5.dollars_median\endcsname{0.50}
\expandafter\def\csname val@all.react-b2.m5.dollars_median.min\endcsname{0.03}
\expandafter\def\csname val@all.react-b2.m5.dollars_median.max\endcsname{1.79}
\expandafter\def\csname val@all.react-b2.m5.reached\endcsname{2.3}
\expandafter\def\csname val@all.react-b2.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.react-b2.m5.reached.max\endcsname{9.0}
\expandafter\def\csname val@all.react-b2.m5.injected\endcsname{18}
\expandafter\def\csname val@all.react-b2.m5.injected.min\endcsname{5}
\expandafter\def\csname val@all.react-b2.m5.injected.max\endcsname{60}
\expandafter\def\csname val@all.react-b2.m6.mitigated.median_s\endcsname{462}
\expandafter\def\csname val@all.react-b2.m6.mitigated.median_s.min\endcsname{185}
\expandafter\def\csname val@all.react-b2.m6.mitigated.median_s.max\endcsname{957}
\expandafter\def\csname val@all.react-b2.m6.mitigated.p90_s\endcsname{764}
\expandafter\def\csname val@all.react-b2.m6.mitigated.p90_s.min\endcsname{341}
\expandafter\def\csname val@all.react-b2.m6.mitigated.p90_s.max\endcsname{1409}
\expandafter\def\csname val@all.react-b2.m6.mitigated.dollars_median\endcsname{0.94}
\expandafter\def\csname val@all.react-b2.m6.mitigated.dollars_median.min\endcsname{0.33}
\expandafter\def\csname val@all.react-b2.m6.mitigated.dollars_median.max\endcsname{2.50}
\expandafter\def\csname val@all.react-b2.m6.mitigated.reached\endcsname{7.4}
\expandafter\def\csname val@all.react-b2.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.react-b2.m6.mitigated.reached.max\endcsname{35.0}
\expandafter\def\csname val@all.react-b2.m6.mitigated.injected\endcsname{18}
\expandafter\def\csname val@all.react-b2.m6.mitigated.injected.min\endcsname{5}
\expandafter\def\csname val@all.react-b2.m6.mitigated.injected.max\endcsname{60}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.median_s\endcsname{518}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.median_s.min\endcsname{160}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.median_s.max\endcsname{1055}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.p90_s\endcsname{1358}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.p90_s.min\endcsname{160}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.p90_s.max\endcsname{5479}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.dollars_median\endcsname{0.57}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.dollars_median.min\endcsname{0.05}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.dollars_median.max\endcsname{1.54}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.reached\endcsname{1.7}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.reached.max\endcsname{6.0}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.injected\endcsname{18}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.injected.min\endcsname{5}
\expandafter\def\csname val@all.react-b2.m6.root_fixed.injected.max\endcsname{60}
\expandafter\def\csname val@all.react-b2.m7.blast_radius\endcsname{0.29}
\expandafter\def\csname val@all.react-b2.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m7.blast_radius.max\endcsname{0.60}
\expandafter\def\csname val@all.react-b2.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.react-b2.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@all.react-b2.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.out_of_scope_actions.max\endcsname{9}
\expandafter\def\csname val@all.react-b2.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.no_target_actions.max\endcsname{1}
\expandafter\def\csname val@all.react-b2.m7.executed_mutating_actions\endcsname{10}
\expandafter\def\csname val@all.react-b2.m7.executed_mutating_actions.min\endcsname{3}
\expandafter\def\csname val@all.react-b2.m7.executed_mutating_actions.max\endcsname{22}
\expandafter\def\csname val@all.react-b2.m7.claim_calls\endcsname{338}
\expandafter\def\csname val@all.react-b2.m7.claim_calls.min\endcsname{47}
\expandafter\def\csname val@all.react-b2.m7.claim_calls.max\endcsname{1540}
\expandafter\def\csname val@all.react-b2.m7.max_mutations_per_tick\endcsname{3.13}
\expandafter\def\csname val@all.react-b2.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@all.react-b2.m7.max_mutations_per_tick.max\endcsname{8.00}
\expandafter\def\csname val@all.react-b2.m7.refused_actions\endcsname{1}
\expandafter\def\csname val@all.react-b2.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@all.react-b2.m7.refused_actions.max\endcsname{9}
\expandafter\def\csname val@all.react-b2.m7.unlinked_citations\endcsname{3.00}
\expandafter\def\csname val@all.react-b2.m7.unlinked_citations.min\endcsname{1.00}
\expandafter\def\csname val@all.react-b2.m7.unlinked_citations.max\endcsname{13.00}
\expandafter\def\csname val@all.rag-b2r.m1.f1\endcsname{0.29}
\expandafter\def\csname val@all.rag-b2r.m1.f1.min\endcsname{0.13}
\expandafter\def\csname val@all.rag-b2r.m1.f1.max\endcsname{0.42}
\expandafter\def\csname val@all.rag-b2r.m1.precision\endcsname{0.19}
\expandafter\def\csname val@all.rag-b2r.m1.precision.min\endcsname{0.08}
\expandafter\def\csname val@all.rag-b2r.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@all.rag-b2r.m1.recall\endcsname{0.65}
\expandafter\def\csname val@all.rag-b2r.m1.recall.min\endcsname{0.33}
\expandafter\def\csname val@all.rag-b2r.m1.recall.max\endcsname{0.91}
\expandafter\def\csname val@all.rag-b2r.m1.nrr\endcsname{0.75}
\expandafter\def\csname val@all.rag-b2r.m1.nrr.min\endcsname{0.72}
\expandafter\def\csname val@all.rag-b2r.m1.nrr.max\endcsname{0.80}
\expandafter\def\csname val@all.rag-b2r.m1.alerts_in_denominator\endcsname{121}
\expandafter\def\csname val@all.rag-b2r.m1.alerts_in_denominator.min\endcsname{57}
\expandafter\def\csname val@all.rag-b2r.m1.alerts_in_denominator.max\endcsname{177}
\expandafter\def\csname val@all.rag-b2r.m1.incidents_declared\endcsname{30}
\expandafter\def\csname val@all.rag-b2r.m1.incidents_declared.min\endcsname{16}
\expandafter\def\csname val@all.rag-b2r.m1.incidents_declared.max\endcsname{49}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_excluded\endcsname{135}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_excluded.min\endcsname{52}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_excluded.max\endcsname{290}
\expandafter\def\csname val@all.rag-b2r.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_share\endcsname{0.48}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_share.min\endcsname{0.26}
\expandafter\def\csname val@all.rag-b2r.m1.ambiguous_share.max\endcsname{0.69}
\expandafter\def\csname val@all.rag-b2r.m1.f1_overlap\endcsname{0.37}
\expandafter\def\csname val@all.rag-b2r.m1.f1_overlap.min\endcsname{0.34}
\expandafter\def\csname val@all.rag-b2r.m1.f1_overlap.max\endcsname{0.42}
\expandafter\def\csname val@all.rag-b2r.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@all.rag-b2r.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@all.rag-b2r.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@all.rag-b2r.m1.incident_precision\endcsname{0.87}
\expandafter\def\csname val@all.rag-b2r.m1.incident_precision.min\endcsname{0.81}
\expandafter\def\csname val@all.rag-b2r.m1.incident_precision.max\endcsname{0.96}
\expandafter\def\csname val@all.rag-b2r.m2.mean_credit\endcsname{0.46}
\expandafter\def\csname val@all.rag-b2r.m2.mean_credit.min\endcsname{0.13}
\expandafter\def\csname val@all.rag-b2r.m2.mean_credit.max\endcsname{0.69}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_1\endcsname{0.06}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_3\endcsname{0.06}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m2.acc_at_3.max\endcsname{0.19}
\expandafter\def\csname val@all.rag-b2r.m2.services_overlap_mean\endcsname{0.83}
\expandafter\def\csname val@all.rag-b2r.m2.services_overlap_mean.min\endcsname{0.70}
\expandafter\def\csname val@all.rag-b2r.m2.services_overlap_mean.max\endcsname{0.94}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.category\endcsname{0.15}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.category.max\endcsname{0.24}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.services\endcsname{0.62}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.services.min\endcsname{0.22}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.services.max\endcsname{0.90}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.artifact\endcsname{0.58}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m2.component_rates.artifact.max\endcsname{0.88}
\expandafter\def\csname val@all.rag-b2r.m2.false_diagnoses\endcsname{233}
\expandafter\def\csname val@all.rag-b2r.m2.false_diagnoses.min\endcsname{115}
\expandafter\def\csname val@all.rag-b2r.m2.false_diagnoses.max\endcsname{443}
\expandafter\def\csname val@all.rag-b2r.m2.loc_at_1\endcsname{0.51}
\expandafter\def\csname val@all.rag-b2r.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m2.loc_at_1.max\endcsname{0.80}
\expandafter\def\csname val@all.rag-b2r.m2.committed_claims\endcsname{470.33}
\expandafter\def\csname val@all.rag-b2r.m2.committed_claims.min\endcsname{196.00}
\expandafter\def\csname val@all.rag-b2r.m2.committed_claims.max\endcsname{711.00}
\expandafter\def\csname val@all.rag-b2r.m2.claim_precision\endcsname{0.50}
\expandafter\def\csname val@all.rag-b2r.m2.claim_precision.min\endcsname{0.38}
\expandafter\def\csname val@all.rag-b2r.m2.claim_precision.max\endcsname{0.72}
\expandafter\def\csname val@all.rag-b2r.m3.fsr\endcsname{0.12}
\expandafter\def\csname val@all.rag-b2r.m3.fsr.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.fsr.max\endcsname{0.34}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_symptomatic\endcsname{0.10}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_symptomatic.max\endcsname{0.28}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate\endcsname{0.24}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate.max\endcsname{0.67}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate_symptomatic\endcsname{0.19}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate_symptomatic.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.mitigated_rate_symptomatic.max\endcsname{0.56}
\expandafter\def\csname val@all.rag-b2r.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.root_fixed_rate\endcsname{0.01}
\expandafter\def\csname val@all.rag-b2r.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.root_fixed_rate.max\endcsname{0.03}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.cleared_without_agent_count\endcsname{1.33}
\expandafter\def\csname val@all.rag-b2r.m3.cleared_without_agent_count.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@all.rag-b2r.m3.repairable_count\endcsname{30.33}
\expandafter\def\csname val@all.rag-b2r.m3.repairable_count.min\endcsname{11.00}
\expandafter\def\csname val@all.rag-b2r.m3.repairable_count.max\endcsname{43.00}
\expandafter\def\csname val@all.rag-b2r.m4.regret\endcsname{0.83}
\expandafter\def\csname val@all.rag-b2r.m4.regret.min\endcsname{0.49}
\expandafter\def\csname val@all.rag-b2r.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@all.rag-b2r.m4.regret_raw\endcsname{1.14}
\expandafter\def\csname val@all.rag-b2r.m4.regret_raw.min\endcsname{0.49}
\expandafter\def\csname val@all.rag-b2r.m4.regret_raw.max\endcsname{1.50}
\expandafter\def\csname val@all.rag-b2r.m4.uim\endcsname{10896}
\expandafter\def\csname val@all.rag-b2r.m4.uim.min\endcsname{1778}
\expandafter\def\csname val@all.rag-b2r.m4.uim.max\endcsname{18782}
\expandafter\def\csname val@all.rag-b2r.m4.uim_null\endcsname{15829}
\expandafter\def\csname val@all.rag-b2r.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@all.rag-b2r.m4.uim_null.max\endcsname{38181}
\expandafter\def\csname val@all.rag-b2r.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m4.offered_requests\endcsname{15187.06}
\expandafter\def\csname val@all.rag-b2r.m4.offered_requests.min\endcsname{2900.59}
\expandafter\def\csname val@all.rag-b2r.m4.offered_requests.max\endcsname{27505.40}
\expandafter\def\csname val@all.rag-b2r.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@all.rag-b2r.m4.load_live_share.min\endcsname{0.29}
\expandafter\def\csname val@all.rag-b2r.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.rag-b2r.m5.median_s\endcsname{228}
\expandafter\def\csname val@all.rag-b2r.m5.median_s.min\endcsname{80}
\expandafter\def\csname val@all.rag-b2r.m5.median_s.max\endcsname{376}
\expandafter\def\csname val@all.rag-b2r.m5.p90_s\endcsname{279}
\expandafter\def\csname val@all.rag-b2r.m5.p90_s.min\endcsname{183}
\expandafter\def\csname val@all.rag-b2r.m5.p90_s.max\endcsname{376}
\expandafter\def\csname val@all.rag-b2r.m5.dollars_median\endcsname{0.16}
\expandafter\def\csname val@all.rag-b2r.m5.dollars_median.min\endcsname{0.02}
\expandafter\def\csname val@all.rag-b2r.m5.dollars_median.max\endcsname{0.30}
\expandafter\def\csname val@all.rag-b2r.m5.reached\endcsname{4.0}
\expandafter\def\csname val@all.rag-b2r.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.rag-b2r.m5.reached.max\endcsname{11.0}
\expandafter\def\csname val@all.rag-b2r.m5.injected\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m5.injected.min\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m5.injected.max\endcsname{59}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.median_s\endcsname{420}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.median_s.min\endcsname{389}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.median_s.max\endcsname{452}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.p90_s\endcsname{978}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.p90_s.min\endcsname{529}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.p90_s.max\endcsname{1426}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.dollars_median\endcsname{0.05}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.dollars_median.min\endcsname{0.01}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.dollars_median.max\endcsname{0.09}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.reached\endcsname{13.7}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.reached.max\endcsname{39.0}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.median_s\endcsname{636}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.median_s.min\endcsname{636}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.median_s.max\endcsname{636}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.p90_s\endcsname{5947}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.p90_s.min\endcsname{5947}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.p90_s.max\endcsname{5947}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.dollars_median\endcsname{0.02}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.dollars_median.min\endcsname{0.02}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.dollars_median.max\endcsname{0.02}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.reached\endcsname{0.7}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.reached.max\endcsname{2.0}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@all.rag-b2r.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@all.rag-b2r.m7.blast_radius\endcsname{0.18}
\expandafter\def\csname val@all.rag-b2r.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m7.blast_radius.max\endcsname{0.50}
\expandafter\def\csname val@all.rag-b2r.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.rag-b2r.m7.out_of_scope_actions\endcsname{3}
\expandafter\def\csname val@all.rag-b2r.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m7.out_of_scope_actions.max\endcsname{7}
\expandafter\def\csname val@all.rag-b2r.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@all.rag-b2r.m7.no_target_actions\endcsname{13}
\expandafter\def\csname val@all.rag-b2r.m7.no_target_actions.min\endcsname{2}
\expandafter\def\csname val@all.rag-b2r.m7.no_target_actions.max\endcsname{23}
\expandafter\def\csname val@all.rag-b2r.m7.executed_mutating_actions\endcsname{73}
\expandafter\def\csname val@all.rag-b2r.m7.executed_mutating_actions.min\endcsname{2}
\expandafter\def\csname val@all.rag-b2r.m7.executed_mutating_actions.max\endcsname{152}
\expandafter\def\csname val@all.rag-b2r.m7.claim_calls\endcsname{1634}
\expandafter\def\csname val@all.rag-b2r.m7.claim_calls.min\endcsname{648}
\expandafter\def\csname val@all.rag-b2r.m7.claim_calls.max\endcsname{2221}
\expandafter\def\csname val@all.rag-b2r.m7.max_mutations_per_tick\endcsname{9.33}
\expandafter\def\csname val@all.rag-b2r.m7.max_mutations_per_tick.min\endcsname{3.00}
\expandafter\def\csname val@all.rag-b2r.m7.max_mutations_per_tick.max\endcsname{17.00}
\expandafter\def\csname val@all.rag-b2r.m7.refused_actions\endcsname{20}
\expandafter\def\csname val@all.rag-b2r.m7.refused_actions.min\endcsname{5}
\expandafter\def\csname val@all.rag-b2r.m7.refused_actions.max\endcsname{31}
\expandafter\def\csname val@all.rag-b2r.m7.unlinked_citations\endcsname{31.67}
\expandafter\def\csname val@all.rag-b2r.m7.unlinked_citations.min\endcsname{14.00}
\expandafter\def\csname val@all.rag-b2r.m7.unlinked_citations.max\endcsname{60.00}
\expandafter\def\csname val@all.opensre-x3.m1.f1\endcsname{0.20}
\expandafter\def\csname val@all.opensre-x3.m1.f1.min\endcsname{0.05}
\expandafter\def\csname val@all.opensre-x3.m1.f1.max\endcsname{0.36}
\expandafter\def\csname val@all.opensre-x3.m1.precision\endcsname{0.15}
\expandafter\def\csname val@all.opensre-x3.m1.precision.min\endcsname{0.02}
\expandafter\def\csname val@all.opensre-x3.m1.precision.max\endcsname{0.27}
\expandafter\def\csname val@all.opensre-x3.m1.recall\endcsname{0.77}
\expandafter\def\csname val@all.opensre-x3.m1.recall.min\endcsname{0.54}
\expandafter\def\csname val@all.opensre-x3.m1.recall.max\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m1.nrr\endcsname{0.94}
\expandafter\def\csname val@all.opensre-x3.m1.nrr.min\endcsname{0.90}
\expandafter\def\csname val@all.opensre-x3.m1.nrr.max\endcsname{0.99}
\expandafter\def\csname val@all.opensre-x3.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@all.opensre-x3.m1.alerts_in_denominator.min\endcsname{60}
\expandafter\def\csname val@all.opensre-x3.m1.alerts_in_denominator.max\endcsname{85}
\expandafter\def\csname val@all.opensre-x3.m1.incidents_declared\endcsname{4}
\expandafter\def\csname val@all.opensre-x3.m1.incidents_declared.min\endcsname{1}
\expandafter\def\csname val@all.opensre-x3.m1.incidents_declared.max\endcsname{6}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_excluded\endcsname{60}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_excluded.min\endcsname{54}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_excluded.max\endcsname{67}
\expandafter\def\csname val@all.opensre-x3.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_share\endcsname{0.46}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_share.min\endcsname{0.39}
\expandafter\def\csname val@all.opensre-x3.m1.ambiguous_share.max\endcsname{0.53}
\expandafter\def\csname val@all.opensre-x3.m1.f1_overlap\endcsname{0.27}
\expandafter\def\csname val@all.opensre-x3.m1.f1_overlap.min\endcsname{0.14}
\expandafter\def\csname val@all.opensre-x3.m1.f1_overlap.max\endcsname{0.39}
\expandafter\def\csname val@all.opensre-x3.m1.detection_recall\endcsname{0.97}
\expandafter\def\csname val@all.opensre-x3.m1.detection_recall.min\endcsname{0.93}
\expandafter\def\csname val@all.opensre-x3.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m1.incident_precision\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m1.incident_precision.min\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m2.mean_credit\endcsname{0.31}
\expandafter\def\csname val@all.opensre-x3.m2.mean_credit.min\endcsname{0.29}
\expandafter\def\csname val@all.opensre-x3.m2.mean_credit.max\endcsname{0.33}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_1.min\endcsname{0.09}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_1.max\endcsname{0.19}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_3\endcsname{0.16}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_3.min\endcsname{0.09}
\expandafter\def\csname val@all.opensre-x3.m2.acc_at_3.max\endcsname{0.22}
\expandafter\def\csname val@all.opensre-x3.m2.services_overlap_mean\endcsname{0.90}
\expandafter\def\csname val@all.opensre-x3.m2.services_overlap_mean.min\endcsname{0.85}
\expandafter\def\csname val@all.opensre-x3.m2.services_overlap_mean.max\endcsname{0.95}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.category\endcsname{0.34}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.category.min\endcsname{0.27}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.category.max\endcsname{0.40}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.services\endcsname{0.40}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.services.min\endcsname{0.40}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.services.max\endcsname{0.41}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.artifact\endcsname{0.22}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.artifact.min\endcsname{0.13}
\expandafter\def\csname val@all.opensre-x3.m2.component_rates.artifact.max\endcsname{0.32}
\expandafter\def\csname val@all.opensre-x3.m2.false_diagnoses\endcsname{30}
\expandafter\def\csname val@all.opensre-x3.m2.false_diagnoses.min\endcsname{29}
\expandafter\def\csname val@all.opensre-x3.m2.false_diagnoses.max\endcsname{31}
\expandafter\def\csname val@all.opensre-x3.m2.loc_at_1\endcsname{0.22}
\expandafter\def\csname val@all.opensre-x3.m2.loc_at_1.min\endcsname{0.13}
\expandafter\def\csname val@all.opensre-x3.m2.loc_at_1.max\endcsname{0.32}
\expandafter\def\csname val@all.opensre-x3.m2.committed_claims\endcsname{72.50}
\expandafter\def\csname val@all.opensre-x3.m2.committed_claims.min\endcsname{70.00}
\expandafter\def\csname val@all.opensre-x3.m2.committed_claims.max\endcsname{75.00}
\expandafter\def\csname val@all.opensre-x3.m2.claim_precision\endcsname{0.59}
\expandafter\def\csname val@all.opensre-x3.m2.claim_precision.min\endcsname{0.59}
\expandafter\def\csname val@all.opensre-x3.m2.claim_precision.max\endcsname{0.59}
\expandafter\def\csname val@all.opensre-x3.m3.fsr\endcsname{0.24}
\expandafter\def\csname val@all.opensre-x3.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@all.opensre-x3.m3.fsr.max\endcsname{0.41}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_symptomatic\endcsname{0.13}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_symptomatic.max\endcsname{0.20}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate\endcsname{0.38}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate.max\endcsname{0.62}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate_symptomatic\endcsname{0.23}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@all.opensre-x3.m3.mitigated_rate_symptomatic.max\endcsname{0.36}
\expandafter\def\csname val@all.opensre-x3.m3.agent_attributed_rate\endcsname{0.06}
\expandafter\def\csname val@all.opensre-x3.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.agent_attributed_rate.max\endcsname{0.12}
\expandafter\def\csname val@all.opensre-x3.m3.root_fixed_rate\endcsname{0.10}
\expandafter\def\csname val@all.opensre-x3.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.root_fixed_rate.max\endcsname{0.20}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@all.opensre-x3.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@all.opensre-x3.m3.repairable_count\endcsname{21.50}
\expandafter\def\csname val@all.opensre-x3.m3.repairable_count.min\endcsname{13.00}
\expandafter\def\csname val@all.opensre-x3.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@all.opensre-x3.m4.regret\endcsname{0.98}
\expandafter\def\csname val@all.opensre-x3.m4.regret.min\endcsname{0.97}
\expandafter\def\csname val@all.opensre-x3.m4.regret.max\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m4.regret_raw\endcsname{1.20}
\expandafter\def\csname val@all.opensre-x3.m4.regret_raw.min\endcsname{0.97}
\expandafter\def\csname val@all.opensre-x3.m4.regret_raw.max\endcsname{1.44}
\expandafter\def\csname val@all.opensre-x3.m4.uim\endcsname{4798}
\expandafter\def\csname val@all.opensre-x3.m4.uim.min\endcsname{1793}
\expandafter\def\csname val@all.opensre-x3.m4.uim.max\endcsname{7804}
\expandafter\def\csname val@all.opensre-x3.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@all.opensre-x3.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@all.opensre-x3.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@all.opensre-x3.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m4.offered_requests\endcsname{9003.38}
\expandafter\def\csname val@all.opensre-x3.m4.offered_requests.min\endcsname{2332.84}
\expandafter\def\csname val@all.opensre-x3.m4.offered_requests.max\endcsname{15673.90}
\expandafter\def\csname val@all.opensre-x3.m4.load_live_share\endcsname{0.68}
\expandafter\def\csname val@all.opensre-x3.m4.load_live_share.min\endcsname{0.36}
\expandafter\def\csname val@all.opensre-x3.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.opensre-x3.m5.median_s\endcsname{172}
\expandafter\def\csname val@all.opensre-x3.m5.median_s.min\endcsname{152}
\expandafter\def\csname val@all.opensre-x3.m5.median_s.max\endcsname{193}
\expandafter\def\csname val@all.opensre-x3.m5.p90_s\endcsname{766}
\expandafter\def\csname val@all.opensre-x3.m5.p90_s.min\endcsname{306}
\expandafter\def\csname val@all.opensre-x3.m5.p90_s.max\endcsname{1225}
\expandafter\def\csname val@all.opensre-x3.m5.dollars_median\endcsname{0.55}
\expandafter\def\csname val@all.opensre-x3.m5.dollars_median.min\endcsname{0.47}
\expandafter\def\csname val@all.opensre-x3.m5.dollars_median.max\endcsname{0.64}
\expandafter\def\csname val@all.opensre-x3.m5.reached\endcsname{8.5}
\expandafter\def\csname val@all.opensre-x3.m5.reached.min\endcsname{5.0}
\expandafter\def\csname val@all.opensre-x3.m5.reached.max\endcsname{12.0}
\expandafter\def\csname val@all.opensre-x3.m5.injected\endcsname{57}
\expandafter\def\csname val@all.opensre-x3.m5.injected.min\endcsname{55}
\expandafter\def\csname val@all.opensre-x3.m5.injected.max\endcsname{59}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.median_s\endcsname{322}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.median_s.min\endcsname{243}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.median_s.max\endcsname{402}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.p90_s\endcsname{1987}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.p90_s.min\endcsname{490}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.p90_s.max\endcsname{3483}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.dollars_median\endcsname{1.65}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.dollars_median.min\endcsname{1.54}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.dollars_median.max\endcsname{1.76}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.reached\endcsname{21.0}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.reached.max\endcsname{34.0}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.injected\endcsname{57}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.injected.min\endcsname{55}
\expandafter\def\csname val@all.opensre-x3.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.median_s\endcsname{196}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.median_s.min\endcsname{196}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.median_s.max\endcsname{196}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.p90_s\endcsname{4950}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.p90_s.min\endcsname{4950}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.p90_s.max\endcsname{4950}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.dollars_median\endcsname{1.14}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.dollars_median.min\endcsname{1.14}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.dollars_median.max\endcsname{1.14}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.reached\endcsname{5.5}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.reached.max\endcsname{11.0}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.injected\endcsname{57}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.injected.min\endcsname{55}
\expandafter\def\csname val@all.opensre-x3.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@all.opensre-x3.m7.blast_radius\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.blast_radius.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.blast_radius.max\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.executed_mutating_actions\endcsname{11}
\expandafter\def\csname val@all.opensre-x3.m7.executed_mutating_actions.min\endcsname{7}
\expandafter\def\csname val@all.opensre-x3.m7.executed_mutating_actions.max\endcsname{15}
\expandafter\def\csname val@all.opensre-x3.m7.claim_calls\endcsname{546}
\expandafter\def\csname val@all.opensre-x3.m7.claim_calls.min\endcsname{545}
\expandafter\def\csname val@all.opensre-x3.m7.claim_calls.max\endcsname{546}
\expandafter\def\csname val@all.opensre-x3.m7.max_mutations_per_tick\endcsname{3.00}
\expandafter\def\csname val@all.opensre-x3.m7.max_mutations_per_tick.min\endcsname{2.00}
\expandafter\def\csname val@all.opensre-x3.m7.max_mutations_per_tick.max\endcsname{4.00}
\expandafter\def\csname val@all.opensre-x3.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@all.opensre-x3.m7.unlinked_citations\endcsname{4.00}
\expandafter\def\csname val@all.opensre-x3.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@all.opensre-x3.m7.unlinked_citations.max\endcsname{8.00}
\expandafter\def\csname val@all.orbit-0.m1.f1\endcsname{0.05}
\expandafter\def\csname val@all.orbit-0.m1.f1.min\endcsname{0.03}
\expandafter\def\csname val@all.orbit-0.m1.f1.max\endcsname{0.06}
\expandafter\def\csname val@all.orbit-0.m1.precision\endcsname{0.71}
\expandafter\def\csname val@all.orbit-0.m1.precision.min\endcsname{0.43}
\expandafter\def\csname val@all.orbit-0.m1.precision.max\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m1.recall\endcsname{0.02}
\expandafter\def\csname val@all.orbit-0.m1.recall.min\endcsname{0.02}
\expandafter\def\csname val@all.orbit-0.m1.recall.max\endcsname{0.03}
\expandafter\def\csname val@all.orbit-0.m1.nrr\endcsname{-0.69}
\expandafter\def\csname val@all.orbit-0.m1.nrr.min\endcsname{-0.89}
\expandafter\def\csname val@all.orbit-0.m1.nrr.max\endcsname{-0.49}
\expandafter\def\csname val@all.orbit-0.m1.alerts_in_denominator\endcsname{72}
\expandafter\def\csname val@all.orbit-0.m1.alerts_in_denominator.min\endcsname{54}
\expandafter\def\csname val@all.orbit-0.m1.alerts_in_denominator.max\endcsname{90}
\expandafter\def\csname val@all.orbit-0.m1.incidents_declared\endcsname{118}
\expandafter\def\csname val@all.orbit-0.m1.incidents_declared.min\endcsname{102}
\expandafter\def\csname val@all.orbit-0.m1.incidents_declared.max\endcsname{134}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_excluded\endcsname{51}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_excluded.min\endcsname{48}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_excluded.max\endcsname{54}
\expandafter\def\csname val@all.orbit-0.m1.agent_authored_excluded\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m1.agent_authored_excluded.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m1.agent_authored_excluded.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_share\endcsname{0.42}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_share.min\endcsname{0.38}
\expandafter\def\csname val@all.orbit-0.m1.ambiguous_share.max\endcsname{0.47}
\expandafter\def\csname val@all.orbit-0.m1.f1_overlap\endcsname{0.22}
\expandafter\def\csname val@all.orbit-0.m1.f1_overlap.min\endcsname{0.16}
\expandafter\def\csname val@all.orbit-0.m1.f1_overlap.max\endcsname{0.28}
\expandafter\def\csname val@all.orbit-0.m1.detection_recall\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m1.detection_recall.min\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m1.detection_recall.max\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m1.incident_precision\endcsname{0.96}
\expandafter\def\csname val@all.orbit-0.m1.incident_precision.min\endcsname{0.91}
\expandafter\def\csname val@all.orbit-0.m1.incident_precision.max\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m2.mean_credit\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.mean_credit.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.mean_credit.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_3\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_3.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.acc_at_3.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.category\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.category.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.category.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.services\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.services.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.services.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.artifact\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.artifact.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.component_rates.artifact.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.false_diagnoses\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m2.false_diagnoses.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m2.false_diagnoses.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m2.loc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.loc_at_1.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.loc_at_1.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.committed_claims\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.committed_claims.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m2.committed_claims.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.fsr\endcsname{0.21}
\expandafter\def\csname val@all.orbit-0.m3.fsr.min\endcsname{0.07}
\expandafter\def\csname val@all.orbit-0.m3.fsr.max\endcsname{0.35}
\expandafter\def\csname val@all.orbit-0.m3.fsr_symptomatic\endcsname{0.17}
\expandafter\def\csname val@all.orbit-0.m3.fsr_symptomatic.min\endcsname{0.05}
\expandafter\def\csname val@all.orbit-0.m3.fsr_symptomatic.max\endcsname{0.30}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate\endcsname{0.42}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate.min\endcsname{0.14}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate.max\endcsname{0.71}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate_symptomatic\endcsname{0.35}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate_symptomatic.min\endcsname{0.10}
\expandafter\def\csname val@all.orbit-0.m3.mitigated_rate_symptomatic.max\endcsname{0.59}
\expandafter\def\csname val@all.orbit-0.m3.agent_attributed_rate\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.agent_attributed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.agent_attributed_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.root_fixed_rate\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.root_fixed_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.root_fixed_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.fsr_agent\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.fsr_agent.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.fsr_agent.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.repaired_rate\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.repaired_rate.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.repaired_rate.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m3.cleared_without_agent_count\endcsname{2.00}
\expandafter\def\csname val@all.orbit-0.m3.cleared_without_agent_count.min\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m3.cleared_without_agent_count.max\endcsname{3.00}
\expandafter\def\csname val@all.orbit-0.m3.repairable_count\endcsname{21.00}
\expandafter\def\csname val@all.orbit-0.m3.repairable_count.min\endcsname{12.00}
\expandafter\def\csname val@all.orbit-0.m3.repairable_count.max\endcsname{30.00}
\expandafter\def\csname val@all.orbit-0.m4.regret\endcsname{0.94}
\expandafter\def\csname val@all.orbit-0.m4.regret.min\endcsname{0.93}
\expandafter\def\csname val@all.orbit-0.m4.regret.max\endcsname{0.96}
\expandafter\def\csname val@all.orbit-0.m4.regret_raw\endcsname{0.94}
\expandafter\def\csname val@all.orbit-0.m4.regret_raw.min\endcsname{0.93}
\expandafter\def\csname val@all.orbit-0.m4.regret_raw.max\endcsname{0.96}
\expandafter\def\csname val@all.orbit-0.m4.uim\endcsname{4335}
\expandafter\def\csname val@all.orbit-0.m4.uim.min\endcsname{1192}
\expandafter\def\csname val@all.orbit-0.m4.uim.max\endcsname{7478}
\expandafter\def\csname val@all.orbit-0.m4.uim_null\endcsname{4653}
\expandafter\def\csname val@all.orbit-0.m4.uim_null.min\endcsname{1244}
\expandafter\def\csname val@all.orbit-0.m4.uim_null.max\endcsname{8062}
\expandafter\def\csname val@all.orbit-0.m4.uim_oracle\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m4.uim_oracle.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m4.uim_oracle.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m4.offered_requests\endcsname{8129.78}
\expandafter\def\csname val@all.orbit-0.m4.offered_requests.min\endcsname{1525.92}
\expandafter\def\csname val@all.orbit-0.m4.offered_requests.max\endcsname{14733.60}
\expandafter\def\csname val@all.orbit-0.m4.load_live_share\endcsname{0.73}
\expandafter\def\csname val@all.orbit-0.m4.load_live_share.min\endcsname{0.45}
\expandafter\def\csname val@all.orbit-0.m4.load_live_share.max\endcsname{1.00}
\expandafter\def\csname val@all.orbit-0.m5.reached\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m5.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m5.reached.max\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m5.injected\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m5.injected.min\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m5.injected.max\endcsname{59}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.median_s\endcsname{345}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.median_s.min\endcsname{250}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.median_s.max\endcsname{441}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.p90_s\endcsname{912}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.p90_s.min\endcsname{493}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.p90_s.max\endcsname{1331}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.dollars_median\endcsname{0.86}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.dollars_median.min\endcsname{0.59}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.dollars_median.max\endcsname{1.13}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.reached\endcsname{24.5}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.reached.min\endcsname{8.0}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.reached.max\endcsname{41.0}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.injected\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.injected.min\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m6.mitigated.injected.max\endcsname{59}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.reached\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.reached.min\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.reached.max\endcsname{0.0}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.injected\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.injected.min\endcsname{58}
\expandafter\def\csname val@all.orbit-0.m6.root_fixed.injected.max\endcsname{59}
\expandafter\def\csname val@all.orbit-0.m7.violations\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.violations.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.violations.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.out_of_scope_actions\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.out_of_scope_actions.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.out_of_scope_actions.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.unscoped_actions\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.unscoped_actions.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.unscoped_actions.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.no_target_actions\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.no_target_actions.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.no_target_actions.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.executed_mutating_actions\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.executed_mutating_actions.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.executed_mutating_actions.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.claim_calls\endcsname{4148}
\expandafter\def\csname val@all.orbit-0.m7.claim_calls.min\endcsname{4036}
\expandafter\def\csname val@all.orbit-0.m7.claim_calls.max\endcsname{4260}
\expandafter\def\csname val@all.orbit-0.m7.max_mutations_per_tick\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.max_mutations_per_tick.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.max_mutations_per_tick.max\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.refused_actions\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.refused_actions.min\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.refused_actions.max\endcsname{0}
\expandafter\def\csname val@all.orbit-0.m7.unlinked_citations\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.unlinked_citations.min\endcsname{0.00}
\expandafter\def\csname val@all.orbit-0.m7.unlinked_citations.max\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.smash_score\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.smash_lo_r1\endcsname{0.42}
\expandafter\def\csname val@all.b0-null.smash_hi_r0\endcsname{28.42}
\expandafter\def\csname val@all.b0-null.dollars\endcsname{0.00}
\expandafter\def\csname val@all.b0-null.llm_calls\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.smash_score\endcsname{6.57}
\expandafter\def\csname val@all.b1-runbook.smash_lo_r1\endcsname{6.57}
\expandafter\def\csname val@all.b1-runbook.smash_hi_r0\endcsname{6.57}
\expandafter\def\csname val@all.b1-runbook.dollars\endcsname{0.00}
\expandafter\def\csname val@all.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@all.b1-runbook.rank\endcsname{2}
\expandafter\def\csname val@all.react-b2.smash_score\endcsname{20.23}
\expandafter\def\csname val@all.react-b2.smash_lo_r1\endcsname{20.23}
\expandafter\def\csname val@all.react-b2.smash_hi_r0\endcsname{20.23}
\expandafter\def\csname val@all.react-b2.dollars\endcsname{2.19}
\expandafter\def\csname val@all.react-b2.llm_calls\endcsname{222}
\expandafter\def\csname val@all.react-b2.rank\endcsname{1}
\expandafter\def\csname val@all.rag-b2r.smash_score\endcsname{0.97}
\expandafter\def\csname val@all.rag-b2r.smash_lo_r1\endcsname{0.97}
\expandafter\def\csname val@all.rag-b2r.smash_hi_r0\endcsname{0.97}
\expandafter\def\csname val@all.rag-b2r.dollars\endcsname{0.72}
\expandafter\def\csname val@all.rag-b2r.llm_calls\endcsname{38}
\expandafter\def\csname val@all.rag-b2r.rank\endcsname{4}
\expandafter\def\csname val@all.opensre-x3.smash_score\endcsname{-0.64}
\expandafter\def\csname val@all.opensre-x3.smash_lo_r1\endcsname{-0.64}
\expandafter\def\csname val@all.opensre-x3.smash_hi_r0\endcsname{-0.64}
\expandafter\def\csname val@all.opensre-x3.dollars\endcsname{4.37}
\expandafter\def\csname val@all.opensre-x3.llm_calls\endcsname{292}
\expandafter\def\csname val@all.opensre-x3.rank\endcsname{5}
\expandafter\def\csname val@all.orbit-0.smash_score\endcsname{2.69}
\expandafter\def\csname val@all.orbit-0.smash_lo_r1\endcsname{2.69}
\expandafter\def\csname val@all.orbit-0.smash_hi_r0\endcsname{2.69}
\expandafter\def\csname val@all.orbit-0.dollars\endcsname{3.35}
\expandafter\def\csname val@all.orbit-0.llm_calls\endcsname{124}
\expandafter\def\csname val@all.orbit-0.rank\endcsname{3}
\expandafter\def\csname val@short.astro-episode1.repaired\endcsname{2}
\expandafter\def\csname val@short.astro-episode1.parallel_ticks\endcsname{1}
\expandafter\def\csname val@short.astro-episode1.uim_null\endcsname{1009}
\expandafter\def\csname val@nullclass.astro-episode1.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode1.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode1.probe never reacted\endcsname{2}
\expandafter\def\csname val@nullclass.astro-episode1.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode1.unrepaired in both\endcsname{3}
\expandafter\def\csname val@nullclass.astro-episode1.no reference\endcsname{0}
\expandafter\def\csname val@short.astro-episode2.repaired\endcsname{3}
\expandafter\def\csname val@short.astro-episode2.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.astro-episode2.uim_null\endcsname{173}
\expandafter\def\csname val@nullclass.astro-episode2.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode2.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode2.probe never reacted\endcsname{3}
\expandafter\def\csname val@nullclass.astro-episode2.recovered in null too\endcsname{2}
\expandafter\def\csname val@nullclass.astro-episode2.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode2.no reference\endcsname{0}
\expandafter\def\csname val@short.ob-episode1.repaired\endcsname{4}
\expandafter\def\csname val@short.ob-episode1.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.ob-episode1.uim_null\endcsname{106}
\expandafter\def\csname val@nullclass.ob-episode1.agent recovered it\endcsname{2}
\expandafter\def\csname val@nullclass.ob-episode1.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode1.probe never reacted\endcsname{3}
\expandafter\def\csname val@nullclass.ob-episode1.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode1.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode1.no reference\endcsname{0}
\expandafter\def\csname val@short.ob-episode2.repaired\endcsname{5}
\expandafter\def\csname val@short.ob-episode2.parallel_ticks\endcsname{1}
\expandafter\def\csname val@short.ob-episode2.uim_null\endcsname{2508}
\expandafter\def\csname val@nullclass.ob-episode2.agent recovered it\endcsname{5}
\expandafter\def\csname val@nullclass.ob-episode2.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode2.probe never reacted\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode2.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode2.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode2.no reference\endcsname{0}
\expandafter\def\csname val@short.tt-episode1.repaired\endcsname{5}
\expandafter\def\csname val@short.tt-episode1.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.tt-episode1.uim_null\endcsname{3419}
\expandafter\def\csname val@nullclass.tt-episode1.agent recovered it\endcsname{2}
\expandafter\def\csname val@nullclass.tt-episode1.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode1.probe never reacted\endcsname{3}
\expandafter\def\csname val@nullclass.tt-episode1.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode1.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode1.no reference\endcsname{0}
\expandafter\def\csname val@short.tt-episode2.repaired\endcsname{5}
\expandafter\def\csname val@short.tt-episode2.parallel_ticks\endcsname{1}
\expandafter\def\csname val@short.tt-episode2.uim_null\endcsname{4108}
\expandafter\def\csname val@nullclass.tt-episode2.agent recovered it\endcsname{4}
\expandafter\def\csname val@nullclass.tt-episode2.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode2.probe never reacted\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode2.recovered in null too\endcsname{1}
\expandafter\def\csname val@nullclass.tt-episode2.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode2.no reference\endcsname{0}
\expandafter\def\csname val@short.ob-episode3.repaired\endcsname{0}
\expandafter\def\csname val@short.ob-episode3.parallel_ticks\endcsname{4}
\expandafter\def\csname val@short.ob-episode3.uim_null\endcsname{4542}
\expandafter\def\csname val@nullclass.ob-episode3.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode3.less severe with the agent\endcsname{10}
\expandafter\def\csname val@nullclass.ob-episode3.probe never reacted\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode3.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode3.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode3.no reference\endcsname{0}
\expandafter\def\csname val@short.ob-episode4.repaired\endcsname{0}
\expandafter\def\csname val@short.ob-episode4.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.ob-episode4.uim_null\endcsname{4144}
\expandafter\def\csname val@nullclass.ob-episode4.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode4.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode4.probe never reacted\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode4.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.ob-episode4.unrepaired in both\endcsname{10}
\expandafter\def\csname val@nullclass.ob-episode4.no reference\endcsname{0}
\expandafter\def\csname val@short.tt-episode3.repaired\endcsname{10}
\expandafter\def\csname val@short.tt-episode3.parallel_ticks\endcsname{1}
\expandafter\def\csname val@short.tt-episode3.uim_null\endcsname{16714}
\expandafter\def\csname val@nullclass.tt-episode3.agent recovered it\endcsname{9}
\expandafter\def\csname val@nullclass.tt-episode3.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode3.probe never reacted\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode3.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode3.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode3.no reference\endcsname{1}
\expandafter\def\csname val@short.tt-episode4.repaired\endcsname{4}
\expandafter\def\csname val@short.tt-episode4.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.tt-episode4.uim_null\endcsname{3240}
\expandafter\def\csname val@nullclass.tt-episode4.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode4.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode4.probe never reacted\endcsname{5}
\expandafter\def\csname val@nullclass.tt-episode4.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.tt-episode4.unrepaired in both\endcsname{5}
\expandafter\def\csname val@nullclass.tt-episode4.no reference\endcsname{0}
\expandafter\def\csname val@short.astro-episode3.repaired\endcsname{1}
\expandafter\def\csname val@short.astro-episode3.parallel_ticks\endcsname{1}
\expandafter\def\csname val@short.astro-episode3.uim_null\endcsname{477}
\expandafter\def\csname val@nullclass.astro-episode3.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode3.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode3.probe never reacted\endcsname{4}
\expandafter\def\csname val@nullclass.astro-episode3.recovered in null too\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode3.unrepaired in both\endcsname{5}
\expandafter\def\csname val@nullclass.astro-episode3.no reference\endcsname{0}
\expandafter\def\csname val@short.astro-episode4.repaired\endcsname{3}
\expandafter\def\csname val@short.astro-episode4.parallel_ticks\endcsname{2}
\expandafter\def\csname val@short.astro-episode4.uim_null\endcsname{38}
\expandafter\def\csname val@nullclass.astro-episode4.agent recovered it\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode4.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode4.probe never reacted\endcsname{8}
\expandafter\def\csname val@nullclass.astro-episode4.recovered in null too\endcsname{2}
\expandafter\def\csname val@nullclass.astro-episode4.unrepaired in both\endcsname{0}
\expandafter\def\csname val@nullclass.astro-episode4.no reference\endcsname{0}
\expandafter\def\csname val@fail.long.b1-runbook.A2_per100calls\endcsname{0.2}
\expandafter\def\csname val@fail.long.b1-runbook.A2.stale_pod_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.b1-runbook.A2.invented_path_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.b1-runbook.A2.query_syntax_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.b1-runbook.A2.vocabulary_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.b1-runbook.A1_per_mutation\endcsname{0.01}
\expandafter\def\csname val@fail.long.b1-runbook.A1+_per_mutation\endcsname{0.00}
\expandafter\def\csname val@fail.long.b1-runbook.A5_per_mutation\endcsname{0.52}
\expandafter\def\csname val@fail.long.b1-runbook.A6_per_mutation\endcsname{0.25}
\expandafter\def\csname val@fail.long.b1-runbook.T4_per_llm_call\endcsname{---}
\expandafter\def\csname val@fail.long.b1-runbook.status_per_llm_call\endcsname{---}
\expandafter\def\csname val@fail.long.b1-runbook.incidents_per_occurrence\endcsname{1.07}
\expandafter\def\csname val@fail.long.b1-runbook.T1_count\endcsname{30}
\expandafter\def\csname val@fail.long.b1-runbook.T3_count\endcsname{0}
\expandafter\def\csname val@fail.long.b1-runbook.T4_count\endcsname{0}
\expandafter\def\csname val@fail.long.b1-runbook.T6a_count\endcsname{0}
\expandafter\def\csname val@fail.long.b1-runbook.T6b_count\endcsname{85}
\expandafter\def\csname val@fail.long.b1-runbook.executed_mutations\endcsname{179}
\expandafter\def\csname val@fail.long.b1-runbook.audit_calls\endcsname{1565}
\expandafter\def\csname val@fail.long.b1-runbook.llm_calls\endcsname{0}
\expandafter\def\csname val@fail.long.b1-runbook.status_claims\endcsname{832}
\expandafter\def\csname val@fail.long.b1-runbook.rca_claims\endcsname{182}
\expandafter\def\csname val@fail.long.react-b2.A2_per100calls\endcsname{7.4}
\expandafter\def\csname val@fail.long.react-b2.A2.stale_pod_per100calls\endcsname{5.2}
\expandafter\def\csname val@fail.long.react-b2.A2.invented_path_per100calls\endcsname{0.3}
\expandafter\def\csname val@fail.long.react-b2.A2.query_syntax_per100calls\endcsname{0.8}
\expandafter\def\csname val@fail.long.react-b2.A2.vocabulary_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.react-b2.A1_per_mutation\endcsname{0.26}
\expandafter\def\csname val@fail.long.react-b2.A1+_per_mutation\endcsname{0.00}
\expandafter\def\csname val@fail.long.react-b2.A5_per_mutation\endcsname{0.11}
\expandafter\def\csname val@fail.long.react-b2.A6_per_mutation\endcsname{0.00}
\expandafter\def\csname val@fail.long.react-b2.T4_per_llm_call\endcsname{0.00}
\expandafter\def\csname val@fail.long.react-b2.status_per_llm_call\endcsname{3.2}
\expandafter\def\csname val@fail.long.react-b2.incidents_per_occurrence\endcsname{0.84}
\expandafter\def\csname val@fail.long.react-b2.T1_count\endcsname{9}
\expandafter\def\csname val@fail.long.react-b2.T3_count\endcsname{0}
\expandafter\def\csname val@fail.long.react-b2.T4_count\endcsname{0}
\expandafter\def\csname val@fail.long.react-b2.T6a_count\endcsname{9}
\expandafter\def\csname val@fail.long.react-b2.T6b_count\endcsname{6}
\expandafter\def\csname val@fail.long.react-b2.executed_mutations\endcsname{46}
\expandafter\def\csname val@fail.long.react-b2.audit_calls\endcsname{5147}
\expandafter\def\csname val@fail.long.react-b2.llm_calls\endcsname{896}
\expandafter\def\csname val@fail.long.react-b2.status_claims\endcsname{2907}
\expandafter\def\csname val@fail.long.react-b2.rca_claims\endcsname{107}
\expandafter\def\csname val@fail.long.rag-b2r.A2_per100calls\endcsname{4.0}
\expandafter\def\csname val@fail.long.rag-b2r.A2.stale_pod_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.rag-b2r.A2.invented_path_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.rag-b2r.A2.query_syntax_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.rag-b2r.A2.vocabulary_per100calls\endcsname{0.5}
\expandafter\def\csname val@fail.long.rag-b2r.A1_per_mutation\endcsname{0.88}
\expandafter\def\csname val@fail.long.rag-b2r.A1+_per_mutation\endcsname{0.31}
\expandafter\def\csname val@fail.long.rag-b2r.A5_per_mutation\endcsname{0.63}
\expandafter\def\csname val@fail.long.rag-b2r.A6_per_mutation\endcsname{0.35}
\expandafter\def\csname val@fail.long.rag-b2r.T4_per_llm_call\endcsname{0.17}
\expandafter\def\csname val@fail.long.rag-b2r.status_per_llm_call\endcsname{28.6}
\expandafter\def\csname val@fail.long.rag-b2r.incidents_per_occurrence\endcsname{0.51}
\expandafter\def\csname val@fail.long.rag-b2r.T1_count\endcsname{36}
\expandafter\def\csname val@fail.long.rag-b2r.T3_count\endcsname{0}
\expandafter\def\csname val@fail.long.rag-b2r.T4_count\endcsname{19}
\expandafter\def\csname val@fail.long.rag-b2r.T6a_count\endcsname{0}
\expandafter\def\csname val@fail.long.rag-b2r.T6b_count\endcsname{14}
\expandafter\def\csname val@fail.long.rag-b2r.executed_mutations\endcsname{220}
\expandafter\def\csname val@fail.long.rag-b2r.audit_calls\endcsname{6470}
\expandafter\def\csname val@fail.long.rag-b2r.llm_calls\endcsname{114}
\expandafter\def\csname val@fail.long.rag-b2r.status_claims\endcsname{3260}
\expandafter\def\csname val@fail.long.rag-b2r.rca_claims\endcsname{1441}
\expandafter\def\csname val@fail.long.opensre-x3.A2_per100calls\endcsname{5.7}
\expandafter\def\csname val@fail.long.opensre-x3.A2.stale_pod_per100calls\endcsname{4.6}
\expandafter\def\csname val@fail.long.opensre-x3.A2.invented_path_per100calls\endcsname{0.2}
\expandafter\def\csname val@fail.long.opensre-x3.A2.query_syntax_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.opensre-x3.A2.vocabulary_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.opensre-x3.A1_per_mutation\endcsname{0.23}
\expandafter\def\csname val@fail.long.opensre-x3.A1+_per_mutation\endcsname{0.05}
\expandafter\def\csname val@fail.long.opensre-x3.A5_per_mutation\endcsname{0.23}
\expandafter\def\csname val@fail.long.opensre-x3.A6_per_mutation\endcsname{0.05}
\expandafter\def\csname val@fail.long.opensre-x3.T4_per_llm_call\endcsname{0.00}
\expandafter\def\csname val@fail.long.opensre-x3.status_per_llm_call\endcsname{1.3}
\expandafter\def\csname val@fail.long.opensre-x3.incidents_per_occurrence\endcsname{0.06}
\expandafter\def\csname val@fail.long.opensre-x3.T1_count\endcsname{9}
\expandafter\def\csname val@fail.long.opensre-x3.T3_count\endcsname{0}
\expandafter\def\csname val@fail.long.opensre-x3.T4_count\endcsname{0}
\expandafter\def\csname val@fail.long.opensre-x3.T6a_count\endcsname{35}
\expandafter\def\csname val@fail.long.opensre-x3.T6b_count\endcsname{5}
\expandafter\def\csname val@fail.long.opensre-x3.executed_mutations\endcsname{22}
\expandafter\def\csname val@fail.long.opensre-x3.audit_calls\endcsname{2108}
\expandafter\def\csname val@fail.long.opensre-x3.llm_calls\endcsname{584}
\expandafter\def\csname val@fail.long.opensre-x3.status_claims\endcsname{771}
\expandafter\def\csname val@fail.long.opensre-x3.rca_claims\endcsname{156}
\expandafter\def\csname val@fail.long.orbit-0.A2_per100calls\endcsname{0.1}
\expandafter\def\csname val@fail.long.orbit-0.A2.stale_pod_per100calls\endcsname{0.1}
\expandafter\def\csname val@fail.long.orbit-0.A2.invented_path_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.orbit-0.A2.query_syntax_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.orbit-0.A2.vocabulary_per100calls\endcsname{0.0}
\expandafter\def\csname val@fail.long.orbit-0.A1_per_mutation\endcsname{---}
\expandafter\def\csname val@fail.long.orbit-0.A1+_per_mutation\endcsname{---}
\expandafter\def\csname val@fail.long.orbit-0.A5_per_mutation\endcsname{---}
\expandafter\def\csname val@fail.long.orbit-0.A6_per_mutation\endcsname{---}
\expandafter\def\csname val@fail.long.orbit-0.T4_per_llm_call\endcsname{0.60}
\expandafter\def\csname val@fail.long.orbit-0.status_per_llm_call\endcsname{25.0}
\expandafter\def\csname val@fail.long.orbit-0.incidents_per_occurrence\endcsname{2.02}
\expandafter\def\csname val@fail.long.orbit-0.T1_count\endcsname{31}
\expandafter\def\csname val@fail.long.orbit-0.T3_count\endcsname{38}
\expandafter\def\csname val@fail.long.orbit-0.T4_count\endcsname{149}
\expandafter\def\csname val@fail.long.orbit-0.T6a_count\endcsname{0}
\expandafter\def\csname val@fail.long.orbit-0.T6b_count\endcsname{0}
\expandafter\def\csname val@fail.long.orbit-0.executed_mutations\endcsname{0}
\expandafter\def\csname val@fail.long.orbit-0.audit_calls\endcsname{8466}
\expandafter\def\csname val@fail.long.orbit-0.llm_calls\endcsname{247}
\expandafter\def\csname val@fail.long.orbit-0.status_claims\endcsname{6179}
\expandafter\def\csname val@fail.long.orbit-0.rca_claims\endcsname{1939}
\expandafter\def\csname val@fail.short.react-b2.A2_per100calls\endcsname{11.9}
\expandafter\def\csname val@fail.short.react-b2.A2.stale_pod_per100calls\endcsname{7.1}
\expandafter\def\csname val@fail.short.react-b2.A2.invented_path_per100calls\endcsname{1.3}
\expandafter\def\csname val@fail.short.react-b2.A2.query_syntax_per100calls\endcsname{1.1}
\expandafter\def\csname val@fail.short.react-b2.A2.vocabulary_per100calls\endcsname{0.1}
\expandafter\def\csname val@fail.short.react-b2.A1_per_mutation\endcsname{0.00}
\expandafter\def\csname val@fail.short.react-b2.A1+_per_mutation\endcsname{0.00}
\expandafter\def\csname val@fail.short.react-b2.A5_per_mutation\endcsname{0.25}
\expandafter\def\csname val@fail.short.react-b2.A6_per_mutation\endcsname{0.01}
\expandafter\def\csname val@fail.short.react-b2.T4_per_llm_call\endcsname{0.00}
\expandafter\def\csname val@fail.short.react-b2.status_per_llm_call\endcsname{0.5}
\expandafter\def\csname val@fail.short.react-b2.incidents_per_occurrence\endcsname{1.75}
\expandafter\def\csname val@fail.short.react-b2.T1_count\endcsname{3}
\expandafter\def\csname val@fail.short.react-b2.T3_count\endcsname{0}
\expandafter\def\csname val@fail.short.react-b2.T4_count\endcsname{0}
\expandafter\def\csname val@fail.short.react-b2.T6a_count\endcsname{40}
\expandafter\def\csname val@fail.short.react-b2.T6b_count\endcsname{22}
\expandafter\def\csname val@fail.short.react-b2.executed_mutations\endcsname{111}
\expandafter\def\csname val@fail.short.react-b2.audit_calls\endcsname{6383}
\expandafter\def\csname val@fail.short.react-b2.llm_calls\endcsname{2441}
\expandafter\def\csname val@fail.short.react-b2.status_claims\endcsname{1220}
\expandafter\def\csname val@fail.short.react-b2.rca_claims\endcsname{200}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.credit\endcsname{0.33}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.mitigated_symptomatic\endcsname{0.07}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.agent_attributed\endcsname{0.13}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.claimed_share\endcsname{0.53}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.acted_share\endcsname{0.53}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.reacted_share\endcsname{0.53}
\expandafter\def\csname val@dim.b1-runbook.phase.Q1.reaction_median_s\endcsname{155}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.credit\endcsname{0.28}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.claimed_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.acted_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.reacted_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.phase.Q2.reaction_median_s\endcsname{158}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.credit\endcsname{0.37}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.mitigated_symptomatic\endcsname{0.12}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.claimed_share\endcsname{0.64}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.acted_share\endcsname{0.61}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.reacted_share\endcsname{0.61}
\expandafter\def\csname val@dim.b1-runbook.phase.Q3.reaction_median_s\endcsname{261}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.credit\endcsname{0.34}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.claimed_share\endcsname{0.49}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.acted_share\endcsname{0.49}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.reacted_share\endcsname{0.49}
\expandafter\def\csname val@dim.b1-runbook.phase.Q4.reaction_median_s\endcsname{209}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.credit\endcsname{0.32}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.mitigated_symptomatic\endcsname{0.18}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.agent_attributed\endcsname{0.20}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.claimed_share\endcsname{0.65}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.acted_share\endcsname{0.65}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.reacted_share\endcsname{0.65}
\expandafter\def\csname val@dim.b1-runbook.concurrency.0-2.reaction_median_s\endcsname{168}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.credit\endcsname{0.36}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.agent_attributed\endcsname{0.03}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.claimed_share\endcsname{0.56}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.acted_share\endcsname{0.55}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.reacted_share\endcsname{0.55}
\expandafter\def\csname val@dim.b1-runbook.concurrency.3-5.reaction_median_s\endcsname{159}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.credit\endcsname{0.32}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.mitigated_symptomatic\endcsname{0.10}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.agent_attributed\endcsname{0.03}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.claimed_share\endcsname{0.48}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.acted_share\endcsname{0.48}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.reacted_share\endcsname{0.48}
\expandafter\def\csname val@dim.b1-runbook.concurrency.6+.reaction_median_s\endcsname{189}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.credit\endcsname{0.34}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.mitigated_symptomatic\endcsname{0.27}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.agent_attributed\endcsname{0.15}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.claimed_share\endcsname{0.54}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.acted_share\endcsname{0.54}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.reacted_share\endcsname{0.54}
\expandafter\def\csname val@dim.b1-runbook.family_nth.1st.reaction_median_s\endcsname{147}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.credit\endcsname{0.28}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.claimed_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.acted_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.reacted_share\endcsname{0.47}
\expandafter\def\csname val@dim.b1-runbook.family_nth.2nd-3rd.reaction_median_s\endcsname{158}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.credit\endcsname{0.36}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.acc_at_1\endcsname{0.01}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.mitigated_symptomatic\endcsname{0.04}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.agent_attributed\endcsname{0.01}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.claimed_share\endcsname{0.57}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.acted_share\endcsname{0.56}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.reacted_share\endcsname{0.56}
\expandafter\def\csname val@dim.b1-runbook.family_nth.4th+.reaction_median_s\endcsname{210}
\expandafter\def\csname val@dim.react-b2.phase.Q1.credit\endcsname{0.29}
\expandafter\def\csname val@dim.react-b2.phase.Q1.acc_at_1\endcsname{0.16}
\expandafter\def\csname val@dim.react-b2.phase.Q1.mitigated_symptomatic\endcsname{0.04}
\expandafter\def\csname val@dim.react-b2.phase.Q1.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@dim.react-b2.phase.Q1.claimed_share\endcsname{0.40}
\expandafter\def\csname val@dim.react-b2.phase.Q1.acted_share\endcsname{0.51}
\expandafter\def\csname val@dim.react-b2.phase.Q1.reacted_share\endcsname{0.76}
\expandafter\def\csname val@dim.react-b2.phase.Q1.reaction_median_s\endcsname{132}
\expandafter\def\csname val@dim.react-b2.phase.Q2.credit\endcsname{0.13}
\expandafter\def\csname val@dim.react-b2.phase.Q2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@dim.react-b2.phase.Q2.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@dim.react-b2.phase.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.react-b2.phase.Q2.claimed_share\endcsname{0.27}
\expandafter\def\csname val@dim.react-b2.phase.Q2.acted_share\endcsname{0.10}
\expandafter\def\csname val@dim.react-b2.phase.Q2.reacted_share\endcsname{0.77}
\expandafter\def\csname val@dim.react-b2.phase.Q2.reaction_median_s\endcsname{48}
\expandafter\def\csname val@dim.react-b2.phase.Q3.credit\endcsname{0.10}
\expandafter\def\csname val@dim.react-b2.phase.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.react-b2.phase.Q3.mitigated_symptomatic\endcsname{0.23}
\expandafter\def\csname val@dim.react-b2.phase.Q3.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@dim.react-b2.phase.Q3.claimed_share\endcsname{0.17}
\expandafter\def\csname val@dim.react-b2.phase.Q3.acted_share\endcsname{0.23}
\expandafter\def\csname val@dim.react-b2.phase.Q3.reacted_share\endcsname{0.81}
\expandafter\def\csname val@dim.react-b2.phase.Q3.reaction_median_s\endcsname{154}
\expandafter\def\csname val@dim.react-b2.phase.Q4.credit\endcsname{0.09}
\expandafter\def\csname val@dim.react-b2.phase.Q4.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@dim.react-b2.phase.Q4.mitigated_symptomatic\endcsname{0.16}
\expandafter\def\csname val@dim.react-b2.phase.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.react-b2.phase.Q4.claimed_share\endcsname{0.11}
\expandafter\def\csname val@dim.react-b2.phase.Q4.acted_share\endcsname{0.07}
\expandafter\def\csname val@dim.react-b2.phase.Q4.reacted_share\endcsname{0.78}
\expandafter\def\csname val@dim.react-b2.phase.Q4.reaction_median_s\endcsname{43}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.credit\endcsname{0.25}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.acc_at_1\endcsname{0.12}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.mitigated_symptomatic\endcsname{0.12}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.agent_attributed\endcsname{0.06}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.claimed_share\endcsname{0.41}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.acted_share\endcsname{0.35}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.reacted_share\endcsname{0.88}
\expandafter\def\csname val@dim.react-b2.concurrency.0-2.reaction_median_s\endcsname{130}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.credit\endcsname{0.16}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.mitigated_symptomatic\endcsname{0.17}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.agent_attributed\endcsname{0.01}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.claimed_share\endcsname{0.24}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.acted_share\endcsname{0.29}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.reacted_share\endcsname{0.79}
\expandafter\def\csname val@dim.react-b2.concurrency.3-5.reaction_median_s\endcsname{131}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.credit\endcsname{0.12}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.mitigated_symptomatic\endcsname{0.12}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.agent_attributed\endcsname{0.03}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.claimed_share\endcsname{0.17}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.acted_share\endcsname{0.15}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.reacted_share\endcsname{0.75}
\expandafter\def\csname val@dim.react-b2.concurrency.6+.reaction_median_s\endcsname{134}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.credit\endcsname{0.31}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.acc_at_1\endcsname{0.13}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.mitigated_symptomatic\endcsname{0.24}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.agent_attributed\endcsname{0.05}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.claimed_share\endcsname{0.46}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.acted_share\endcsname{0.41}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.reacted_share\endcsname{0.69}
\expandafter\def\csname val@dim.react-b2.family_nth.1st.reaction_median_s\endcsname{132}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.credit\endcsname{0.12}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.mitigated_symptomatic\endcsname{0.18}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.claimed_share\endcsname{0.20}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.acted_share\endcsname{0.24}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.reacted_share\endcsname{0.80}
\expandafter\def\csname val@dim.react-b2.family_nth.2nd-3rd.reaction_median_s\endcsname{116}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.credit\endcsname{0.10}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.acc_at_1\endcsname{0.04}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.mitigated_symptomatic\endcsname{0.08}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.claimed_share\endcsname{0.14}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.acted_share\endcsname{0.15}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.reacted_share\endcsname{0.81}
\expandafter\def\csname val@dim.react-b2.family_nth.4th+.reaction_median_s\endcsname{145}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.credit\endcsname{0.38}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.mitigated_symptomatic\endcsname{0.07}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.claimed_share\endcsname{0.68}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.acted_share\endcsname{0.27}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.reacted_share\endcsname{0.77}
\expandafter\def\csname val@dim.rag-b2r.phase.Q1.reaction_median_s\endcsname{133}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.credit\endcsname{0.46}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.mitigated_symptomatic\endcsname{0.10}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.claimed_share\endcsname{0.90}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.acted_share\endcsname{0.37}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.reacted_share\endcsname{0.90}
\expandafter\def\csname val@dim.rag-b2r.phase.Q2.reaction_median_s\endcsname{41}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.credit\endcsname{0.51}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.acc_at_1\endcsname{0.04}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.mitigated_symptomatic\endcsname{0.08}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.claimed_share\endcsname{0.89}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.acted_share\endcsname{0.43}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.reacted_share\endcsname{0.98}
\expandafter\def\csname val@dim.rag-b2r.phase.Q3.reaction_median_s\endcsname{65}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.credit\endcsname{0.50}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.acc_at_1\endcsname{0.13}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.claimed_share\endcsname{0.76}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.acted_share\endcsname{0.33}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.reacted_share\endcsname{0.93}
\expandafter\def\csname val@dim.rag-b2r.phase.Q4.reaction_median_s\endcsname{79}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.credit\endcsname{0.37}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.mitigated_symptomatic\endcsname{0.20}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.claimed_share\endcsname{0.76}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.acted_share\endcsname{0.35}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.reacted_share\endcsname{0.76}
\expandafter\def\csname val@dim.rag-b2r.concurrency.0-2.reaction_median_s\endcsname{104}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.credit\endcsname{0.53}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.acc_at_1\endcsname{0.09}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.mitigated_symptomatic\endcsname{0.07}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.claimed_share\endcsname{0.88}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.acted_share\endcsname{0.36}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.reacted_share\endcsname{0.93}
\expandafter\def\csname val@dim.rag-b2r.concurrency.3-5.reaction_median_s\endcsname{65}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.credit\endcsname{0.42}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.claimed_share\endcsname{0.73}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.acted_share\endcsname{0.34}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.reacted_share\endcsname{0.90}
\expandafter\def\csname val@dim.rag-b2r.concurrency.6+.reaction_median_s\endcsname{77}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.credit\endcsname{0.25}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.mitigated_symptomatic\endcsname{0.29}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.claimed_share\endcsname{0.56}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.acted_share\endcsname{0.18}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.reacted_share\endcsname{0.69}
\expandafter\def\csname val@dim.rag-b2r.family_nth.1st.reaction_median_s\endcsname{123}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.credit\endcsname{0.52}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.claimed_share\endcsname{0.91}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.acted_share\endcsname{0.38}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.reacted_share\endcsname{0.98}
\expandafter\def\csname val@dim.rag-b2r.family_nth.2nd-3rd.reaction_median_s\endcsname{59}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.credit\endcsname{0.53}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.acc_at_1\endcsname{0.10}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.mitigated_symptomatic\endcsname{0.03}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.claimed_share\endcsname{0.85}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.acted_share\endcsname{0.41}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.reacted_share\endcsname{0.95}
\expandafter\def\csname val@dim.rag-b2r.family_nth.4th+.reaction_median_s\endcsname{67}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.credit\endcsname{0.49}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.acc_at_1\endcsname{0.40}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.agent_attributed\endcsname{0.10}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.claimed_share\endcsname{0.60}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.acted_share\endcsname{0.33}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.reacted_share\endcsname{0.70}
\expandafter\def\csname val@dim.opensre-x3.phase.Q1.reaction_median_s\endcsname{147}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.credit\endcsname{0.41}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.acc_at_1\endcsname{0.11}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.mitigated_symptomatic\endcsname{0.22}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.claimed_share\endcsname{0.58}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.acted_share\endcsname{0.16}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.reacted_share\endcsname{0.74}
\expandafter\def\csname val@dim.opensre-x3.phase.Q2.reaction_median_s\endcsname{35}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.credit\endcsname{0.13}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.mitigated_symptomatic\endcsname{0.33}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.claimed_share\endcsname{0.30}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.acted_share\endcsname{0.03}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.reacted_share\endcsname{0.87}
\expandafter\def\csname val@dim.opensre-x3.phase.Q3.reaction_median_s\endcsname{98}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.credit\endcsname{0.26}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.acc_at_1\endcsname{0.06}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.mitigated_symptomatic\endcsname{0.14}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.agent_attributed\endcsname{0.03}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.claimed_share\endcsname{0.43}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.acted_share\endcsname{0.06}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.reacted_share\endcsname{0.91}
\expandafter\def\csname val@dim.opensre-x3.phase.Q4.reaction_median_s\endcsname{54}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.credit\endcsname{0.29}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.acc_at_1\endcsname{0.08}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.mitigated_symptomatic\endcsname{0.33}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.agent_attributed\endcsname{0.08}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.claimed_share\endcsname{0.54}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.acted_share\endcsname{0.38}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.reacted_share\endcsname{0.85}
\expandafter\def\csname val@dim.opensre-x3.concurrency.0-2.reaction_median_s\endcsname{177}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.credit\endcsname{0.31}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.acc_at_1\endcsname{0.18}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.mitigated_symptomatic\endcsname{0.21}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.agent_attributed\endcsname{0.06}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.claimed_share\endcsname{0.41}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.acted_share\endcsname{0.18}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.reacted_share\endcsname{0.80}
\expandafter\def\csname val@dim.opensre-x3.concurrency.3-5.reaction_median_s\endcsname{138}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.credit\endcsname{0.32}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.acc_at_1\endcsname{0.12}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.mitigated_symptomatic\endcsname{0.15}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.claimed_share\endcsname{0.50}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.acted_share\endcsname{0.04}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.reacted_share\endcsname{0.82}
\expandafter\def\csname val@dim.opensre-x3.concurrency.6+.reaction_median_s\endcsname{52}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.credit\endcsname{0.31}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.acc_at_1\endcsname{0.13}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.mitigated_symptomatic\endcsname{0.28}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.agent_attributed\endcsname{0.06}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.claimed_share\endcsname{0.52}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.acted_share\endcsname{0.29}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.reacted_share\endcsname{0.65}
\expandafter\def\csname val@dim.opensre-x3.family_nth.1st.reaction_median_s\endcsname{147}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.credit\endcsname{0.48}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.acc_at_1\endcsname{0.33}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.mitigated_symptomatic\endcsname{0.26}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.claimed_share\endcsname{0.56}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.acted_share\endcsname{0.19}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.reacted_share\endcsname{0.85}
\expandafter\def\csname val@dim.opensre-x3.family_nth.2nd-3rd.reaction_median_s\endcsname{138}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.credit\endcsname{0.23}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.claimed_share\endcsname{0.39}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.acted_share\endcsname{0.04}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.reacted_share\endcsname{0.89}
\expandafter\def\csname val@dim.opensre-x3.family_nth.4th+.reaction_median_s\endcsname{54}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.mitigated_symptomatic\endcsname{0.17}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.reacted_share\endcsname{0.13}
\expandafter\def\csname val@dim.orbit-0.phase.Q1.reaction_median_s\endcsname{180}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.mitigated_symptomatic\endcsname{0.22}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.reacted_share\endcsname{0.05}
\expandafter\def\csname val@dim.orbit-0.phase.Q2.reaction_median_s\endcsname{76}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.mitigated_symptomatic\endcsname{0.35}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.reacted_share\endcsname{0.03}
\expandafter\def\csname val@dim.orbit-0.phase.Q3.reaction_median_s\endcsname{19}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.mitigated_symptomatic\endcsname{0.25}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.reacted_share\endcsname{0.06}
\expandafter\def\csname val@dim.orbit-0.phase.Q4.reaction_median_s\endcsname{729}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.mitigated_symptomatic\endcsname{0.25}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.reacted_share\endcsname{0.36}
\expandafter\def\csname val@dim.orbit-0.concurrency.0-2.reaction_median_s\endcsname{179}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.mitigated_symptomatic\endcsname{0.28}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.reacted_share\endcsname{0.04}
\expandafter\def\csname val@dim.orbit-0.concurrency.3-5.reaction_median_s\endcsname{582}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.mitigated_symptomatic\endcsname{0.24}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.reacted_share\endcsname{0.04}
\expandafter\def\csname val@dim.orbit-0.concurrency.6+.reaction_median_s\endcsname{232}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.mitigated_symptomatic\endcsname{0.35}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.reacted_share\endcsname{0.16}
\expandafter\def\csname val@dim.orbit-0.family_nth.1st.reaction_median_s\endcsname{151}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.mitigated_symptomatic\endcsname{0.35}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.reacted_share\endcsname{0.03}
\expandafter\def\csname val@dim.orbit-0.family_nth.2nd-3rd.reaction_median_s\endcsname{1146}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.credit\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.mitigated_symptomatic\endcsname{0.15}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.claimed_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.acted_share\endcsname{0.00}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.reacted_share\endcsname{0.04}
\expandafter\def\csname val@dim.orbit-0.family_nth.4th+.reaction_median_s\endcsname{165}
\expandafter\def\csname val@lifecycle.b0-null.Q1.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q1.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q1.mitigated_symptomatic\endcsname{0.04}
\expandafter\def\csname val@lifecycle.b0-null.Q1.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q1.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q2.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q2.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@lifecycle.b0-null.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q2.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q3.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q3.mitigated_symptomatic\endcsname{0.21}
\expandafter\def\csname val@lifecycle.b0-null.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q3.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q4.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q4.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q4.mitigated_symptomatic\endcsname{0.24}
\expandafter\def\csname val@lifecycle.b0-null.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b0-null.Q4.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.credit\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.mitigated_symptomatic\endcsname{0.16}
\expandafter\def\csname val@all.long.b0-null.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.acted_share\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.reacted_share\endcsname{0.00}
\expandafter\def\csname val@all.long.b0-null.n\endcsname{177}
\expandafter\def\csname val@lifecycle.b1-runbook.Q1.credit\endcsname{0.33}
\expandafter\def\csname val@lifecycle.b1-runbook.Q1.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@lifecycle.b1-runbook.Q1.mitigated_symptomatic\endcsname{0.07}
\expandafter\def\csname val@lifecycle.b1-runbook.Q1.agent_attributed\endcsname{0.13}
\expandafter\def\csname val@lifecycle.b1-runbook.Q1.claimed_share\endcsname{0.53}
\expandafter\def\csname val@lifecycle.b1-runbook.Q2.credit\endcsname{0.28}
\expandafter\def\csname val@lifecycle.b1-runbook.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b1-runbook.Q2.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@lifecycle.b1-runbook.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b1-runbook.Q2.claimed_share\endcsname{0.47}
\expandafter\def\csname val@lifecycle.b1-runbook.Q3.credit\endcsname{0.37}
\expandafter\def\csname val@lifecycle.b1-runbook.Q3.acc_at_1\endcsname{0.02}
\expandafter\def\csname val@lifecycle.b1-runbook.Q3.mitigated_symptomatic\endcsname{0.12}
\expandafter\def\csname val@lifecycle.b1-runbook.Q3.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@lifecycle.b1-runbook.Q3.claimed_share\endcsname{0.64}
\expandafter\def\csname val@lifecycle.b1-runbook.Q4.credit\endcsname{0.34}
\expandafter\def\csname val@lifecycle.b1-runbook.Q4.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.b1-runbook.Q4.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@lifecycle.b1-runbook.Q4.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@lifecycle.b1-runbook.Q4.claimed_share\endcsname{0.49}
\expandafter\def\csname val@all.long.b1-runbook.credit\endcsname{0.34}
\expandafter\def\csname val@all.long.b1-runbook.acc_at_1\endcsname{0.01}
\expandafter\def\csname val@all.long.b1-runbook.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@all.long.b1-runbook.agent_attributed\endcsname{0.05}
\expandafter\def\csname val@all.long.b1-runbook.claimed_share\endcsname{0.53}
\expandafter\def\csname val@all.long.b1-runbook.acted_share\endcsname{0.53}
\expandafter\def\csname val@all.long.b1-runbook.reacted_share\endcsname{0.53}
\expandafter\def\csname val@all.long.b1-runbook.n\endcsname{172}
\expandafter\def\csname val@lifecycle.react-b2.Q1.credit\endcsname{0.29}
\expandafter\def\csname val@lifecycle.react-b2.Q1.acc_at_1\endcsname{0.16}
\expandafter\def\csname val@lifecycle.react-b2.Q1.mitigated_symptomatic\endcsname{0.04}
\expandafter\def\csname val@lifecycle.react-b2.Q1.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@lifecycle.react-b2.Q1.claimed_share\endcsname{0.40}
\expandafter\def\csname val@lifecycle.react-b2.Q2.credit\endcsname{0.13}
\expandafter\def\csname val@lifecycle.react-b2.Q2.acc_at_1\endcsname{0.03}
\expandafter\def\csname val@lifecycle.react-b2.Q2.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@lifecycle.react-b2.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.react-b2.Q2.claimed_share\endcsname{0.27}
\expandafter\def\csname val@lifecycle.react-b2.Q3.credit\endcsname{0.10}
\expandafter\def\csname val@lifecycle.react-b2.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.react-b2.Q3.mitigated_symptomatic\endcsname{0.23}
\expandafter\def\csname val@lifecycle.react-b2.Q3.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@lifecycle.react-b2.Q3.claimed_share\endcsname{0.17}
\expandafter\def\csname val@lifecycle.react-b2.Q4.credit\endcsname{0.09}
\expandafter\def\csname val@lifecycle.react-b2.Q4.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@lifecycle.react-b2.Q4.mitigated_symptomatic\endcsname{0.16}
\expandafter\def\csname val@lifecycle.react-b2.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.react-b2.Q4.claimed_share\endcsname{0.11}
\expandafter\def\csname val@all.long.react-b2.credit\endcsname{0.15}
\expandafter\def\csname val@all.long.react-b2.acc_at_1\endcsname{0.07}
\expandafter\def\csname val@all.long.react-b2.mitigated_symptomatic\endcsname{0.14}
\expandafter\def\csname val@all.long.react-b2.agent_attributed\endcsname{0.02}
\expandafter\def\csname val@all.long.react-b2.claimed_share\endcsname{0.23}
\expandafter\def\csname val@all.long.react-b2.acted_share\endcsname{0.23}
\expandafter\def\csname val@all.long.react-b2.reacted_share\endcsname{0.78}
\expandafter\def\csname val@all.long.react-b2.n\endcsname{177}
\expandafter\def\csname val@lifecycle.rag-b2r.Q1.credit\endcsname{0.38}
\expandafter\def\csname val@lifecycle.rag-b2r.Q1.acc_at_1\endcsname{0.05}
\expandafter\def\csname val@lifecycle.rag-b2r.Q1.mitigated_symptomatic\endcsname{0.07}
\expandafter\def\csname val@lifecycle.rag-b2r.Q1.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.rag-b2r.Q1.claimed_share\endcsname{0.68}
\expandafter\def\csname val@lifecycle.rag-b2r.Q2.credit\endcsname{0.46}
\expandafter\def\csname val@lifecycle.rag-b2r.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.rag-b2r.Q2.mitigated_symptomatic\endcsname{0.10}
\expandafter\def\csname val@lifecycle.rag-b2r.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.rag-b2r.Q2.claimed_share\endcsname{0.90}
\expandafter\def\csname val@lifecycle.rag-b2r.Q3.credit\endcsname{0.51}
\expandafter\def\csname val@lifecycle.rag-b2r.Q3.acc_at_1\endcsname{0.04}
\expandafter\def\csname val@lifecycle.rag-b2r.Q3.mitigated_symptomatic\endcsname{0.08}
\expandafter\def\csname val@lifecycle.rag-b2r.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.rag-b2r.Q3.claimed_share\endcsname{0.89}
\expandafter\def\csname val@lifecycle.rag-b2r.Q4.credit\endcsname{0.50}
\expandafter\def\csname val@lifecycle.rag-b2r.Q4.acc_at_1\endcsname{0.13}
\expandafter\def\csname val@lifecycle.rag-b2r.Q4.mitigated_symptomatic\endcsname{0.11}
\expandafter\def\csname val@lifecycle.rag-b2r.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.rag-b2r.Q4.claimed_share\endcsname{0.76}
\expandafter\def\csname val@all.long.rag-b2r.credit\endcsname{0.47}
\expandafter\def\csname val@all.long.rag-b2r.acc_at_1\endcsname{0.06}
\expandafter\def\csname val@all.long.rag-b2r.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@all.long.rag-b2r.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.long.rag-b2r.claimed_share\endcsname{0.80}
\expandafter\def\csname val@all.long.rag-b2r.acted_share\endcsname{0.35}
\expandafter\def\csname val@all.long.rag-b2r.reacted_share\endcsname{0.90}
\expandafter\def\csname val@all.long.rag-b2r.n\endcsname{175}
\expandafter\def\csname val@lifecycle.opensre-x3.Q1.credit\endcsname{0.49}
\expandafter\def\csname val@lifecycle.opensre-x3.Q1.acc_at_1\endcsname{0.40}
\expandafter\def\csname val@lifecycle.opensre-x3.Q1.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@lifecycle.opensre-x3.Q1.agent_attributed\endcsname{0.10}
\expandafter\def\csname val@lifecycle.opensre-x3.Q1.claimed_share\endcsname{0.60}
\expandafter\def\csname val@lifecycle.opensre-x3.Q2.credit\endcsname{0.41}
\expandafter\def\csname val@lifecycle.opensre-x3.Q2.acc_at_1\endcsname{0.11}
\expandafter\def\csname val@lifecycle.opensre-x3.Q2.mitigated_symptomatic\endcsname{0.22}
\expandafter\def\csname val@lifecycle.opensre-x3.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.opensre-x3.Q2.claimed_share\endcsname{0.58}
\expandafter\def\csname val@lifecycle.opensre-x3.Q3.credit\endcsname{0.13}
\expandafter\def\csname val@lifecycle.opensre-x3.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.opensre-x3.Q3.mitigated_symptomatic\endcsname{0.33}
\expandafter\def\csname val@lifecycle.opensre-x3.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.opensre-x3.Q3.claimed_share\endcsname{0.30}
\expandafter\def\csname val@lifecycle.opensre-x3.Q4.credit\endcsname{0.26}
\expandafter\def\csname val@lifecycle.opensre-x3.Q4.acc_at_1\endcsname{0.06}
\expandafter\def\csname val@lifecycle.opensre-x3.Q4.mitigated_symptomatic\endcsname{0.14}
\expandafter\def\csname val@lifecycle.opensre-x3.Q4.agent_attributed\endcsname{0.03}
\expandafter\def\csname val@lifecycle.opensre-x3.Q4.claimed_share\endcsname{0.43}
\expandafter\def\csname val@all.long.opensre-x3.credit\endcsname{0.31}
\expandafter\def\csname val@all.long.opensre-x3.acc_at_1\endcsname{0.14}
\expandafter\def\csname val@all.long.opensre-x3.mitigated_symptomatic\endcsname{0.19}
\expandafter\def\csname val@all.long.opensre-x3.agent_attributed\endcsname{0.04}
\expandafter\def\csname val@all.long.opensre-x3.claimed_share\endcsname{0.46}
\expandafter\def\csname val@all.long.opensre-x3.acted_share\endcsname{0.14}
\expandafter\def\csname val@all.long.opensre-x3.reacted_share\endcsname{0.82}
\expandafter\def\csname val@all.long.opensre-x3.n\endcsname{114}
\expandafter\def\csname val@lifecycle.orbit-0.Q1.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q1.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q1.mitigated_symptomatic\endcsname{0.17}
\expandafter\def\csname val@lifecycle.orbit-0.Q1.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q1.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q2.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q2.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q2.mitigated_symptomatic\endcsname{0.22}
\expandafter\def\csname val@lifecycle.orbit-0.Q2.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q2.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q3.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q3.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q3.mitigated_symptomatic\endcsname{0.35}
\expandafter\def\csname val@lifecycle.orbit-0.Q3.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q3.claimed_share\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q4.credit\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q4.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q4.mitigated_symptomatic\endcsname{0.25}
\expandafter\def\csname val@lifecycle.orbit-0.Q4.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@lifecycle.orbit-0.Q4.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.credit\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.mitigated_symptomatic\endcsname{0.26}
\expandafter\def\csname val@all.long.orbit-0.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.acted_share\endcsname{0.00}
\expandafter\def\csname val@all.long.orbit-0.reacted_share\endcsname{0.07}
\expandafter\def\csname val@all.long.orbit-0.n\endcsname{117}
\expandafter\def\csname val@all.short.b0-null.credit\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.mitigated_symptomatic\endcsname{0.09}
\expandafter\def\csname val@all.short.b0-null.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.acted_share\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.reacted_share\endcsname{0.00}
\expandafter\def\csname val@all.short.b0-null.n\endcsname{88}
\expandafter\def\csname val@all.short.react-b2.credit\endcsname{0.39}
\expandafter\def\csname val@all.short.react-b2.acc_at_1\endcsname{0.20}
\expandafter\def\csname val@all.short.react-b2.mitigated_symptomatic\endcsname{0.53}
\expandafter\def\csname val@all.short.react-b2.agent_attributed\endcsname{0.20}
\expandafter\def\csname val@all.short.react-b2.claimed_share\endcsname{0.65}
\expandafter\def\csname val@all.short.react-b2.acted_share\endcsname{0.80}
\expandafter\def\csname val@all.short.react-b2.reacted_share\endcsname{0.93}
\expandafter\def\csname val@all.short.react-b2.n\endcsname{89}
\expandafter\def\csname val@all.short5.b0-null.credit\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.mitigated_symptomatic\endcsname{0.17}
\expandafter\def\csname val@all.short5.b0-null.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.acted_share\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.reacted_share\endcsname{0.00}
\expandafter\def\csname val@all.short5.b0-null.n\endcsname{30}
\expandafter\def\csname val@all.short5.react-b2.credit\endcsname{0.36}
\expandafter\def\csname val@all.short5.react-b2.acc_at_1\endcsname{0.17}
\expandafter\def\csname val@all.short5.react-b2.mitigated_symptomatic\endcsname{0.94}
\expandafter\def\csname val@all.short5.react-b2.agent_attributed\endcsname{0.43}
\expandafter\def\csname val@all.short5.react-b2.claimed_share\endcsname{0.67}
\expandafter\def\csname val@all.short5.react-b2.acted_share\endcsname{0.90}
\expandafter\def\csname val@all.short5.react-b2.reacted_share\endcsname{0.97}
\expandafter\def\csname val@all.short5.react-b2.n\endcsname{30}
\expandafter\def\csname val@all.short10.b0-null.credit\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.acc_at_1\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.mitigated_symptomatic\endcsname{0.06}
\expandafter\def\csname val@all.short10.b0-null.agent_attributed\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.claimed_share\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.acted_share\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.reacted_share\endcsname{0.00}
\expandafter\def\csname val@all.short10.b0-null.n\endcsname{58}
\expandafter\def\csname val@all.short10.react-b2.credit\endcsname{0.41}
\expandafter\def\csname val@all.short10.react-b2.acc_at_1\endcsname{0.22}
\expandafter\def\csname val@all.short10.react-b2.mitigated_symptomatic\endcsname{0.34}
\expandafter\def\csname val@all.short10.react-b2.agent_attributed\endcsname{0.08}
\expandafter\def\csname val@all.short10.react-b2.claimed_share\endcsname{0.64}
\expandafter\def\csname val@all.short10.react-b2.acted_share\endcsname{0.75}
\expandafter\def\csname val@all.short10.react-b2.reacted_share\endcsname{0.92}
\expandafter\def\csname val@all.short10.react-b2.n\endcsname{59}
\expandafter\def\csname val@act.b0-null.0-15.mean_active_faults\endcsname{5.12}
\expandafter\def\csname val@act.b0-null.0-15.mean_probes_bad\endcsname{1.50}
\expandafter\def\csname val@act.b0-null.0-15.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.0-15.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.0-15.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.0-15.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b0-null.15-30.mean_active_faults\endcsname{6.33}
\expandafter\def\csname val@act.b0-null.15-30.mean_probes_bad\endcsname{4.10}
\expandafter\def\csname val@act.b0-null.15-30.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.15-30.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.15-30.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.15-30.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b0-null.30-45.mean_active_faults\endcsname{5.17}
\expandafter\def\csname val@act.b0-null.30-45.mean_probes_bad\endcsname{2.75}
\expandafter\def\csname val@act.b0-null.30-45.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.30-45.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.30-45.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.30-45.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b0-null.45-60.mean_active_faults\endcsname{7.29}
\expandafter\def\csname val@act.b0-null.45-60.mean_probes_bad\endcsname{4.76}
\expandafter\def\csname val@act.b0-null.45-60.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.45-60.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.45-60.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.45-60.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b0-null.60-90.mean_active_faults\endcsname{5.20}
\expandafter\def\csname val@act.b0-null.60-90.mean_probes_bad\endcsname{2.11}
\expandafter\def\csname val@act.b0-null.60-90.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.60-90.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.60-90.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.60-90.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b0-null.90-∞.mean_active_faults\endcsname{1.88}
\expandafter\def\csname val@act.b0-null.90-∞.mean_probes_bad\endcsname{0.65}
\expandafter\def\csname val@act.b0-null.90-∞.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls_read\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls_claim\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_claims_status\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b0-null.90-∞.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_incidents_open\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.b0-null.90-∞.failed_call_share\endcsname{---}
\expandafter\def\csname val@act.b0-null.90-∞.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_active_faults\endcsname{5.21}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_probes_bad\endcsname{1.54}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_mutations_ok\endcsname{1.17}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_mutations_failed\endcsname{0.04}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls_failed\endcsname{0.04}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls\endcsname{8.46}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls_read\endcsname{0.83}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls_claim\endcsname{6.42}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls_act\endcsname{0.71}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_calls_guarded\endcsname{0.50}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_claims_rca_committed\endcsname{1.21}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_claims_status\endcsname{3.92}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_turns_failed\endcsname{0.12}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_incidents_open\endcsname{4.67}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_mutations_attempted\endcsname{1.21}
\expandafter\def\csname val@act.b1-runbook.0-15.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.0-15.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_active_faults\endcsname{6.29}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_probes_bad\endcsname{3.86}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_mutations_ok\endcsname{1.67}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls\endcsname{10.43}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls_read\endcsname{0.76}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls_claim\endcsname{8.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls_act\endcsname{1.19}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_calls_guarded\endcsname{0.48}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_claims_rca_committed\endcsname{1.67}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_claims_status\endcsname{5.05}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_turns_failed\endcsname{0.19}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_incidents_open\endcsname{10.05}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_mutations_attempted\endcsname{1.67}
\expandafter\def\csname val@act.b1-runbook.15-30.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.15-30.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_active_faults\endcsname{5.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_probes_bad\endcsname{2.71}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_mutations_ok\endcsname{0.67}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls\endcsname{7.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls_read\endcsname{0.75}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls_claim\endcsname{5.58}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls_act\endcsname{0.54}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_calls_guarded\endcsname{0.12}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_claims_rca_committed\endcsname{0.67}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_claims_status\endcsname{3.58}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_turns_failed\endcsname{0.21}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_incidents_open\endcsname{9.54}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_mutations_attempted\endcsname{0.67}
\expandafter\def\csname val@act.b1-runbook.30-45.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.30-45.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_active_faults\endcsname{7.10}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_probes_bad\endcsname{3.90}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_mutations_ok\endcsname{2.33}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_mutations_failed\endcsname{0.10}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls_failed\endcsname{0.10}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls\endcsname{12.24}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls_read\endcsname{0.57}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls_claim\endcsname{9.24}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls_act\endcsname{1.33}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_calls_guarded\endcsname{1.10}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_claims_rca_committed\endcsname{2.43}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_claims_status\endcsname{5.81}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_turns_failed\endcsname{0.14}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_incidents_open\endcsname{11.57}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_mutations_attempted\endcsname{2.43}
\expandafter\def\csname val@act.b1-runbook.45-60.failed_call_share\endcsname{0.01}
\expandafter\def\csname val@act.b1-runbook.45-60.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_active_faults\endcsname{4.40}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_probes_bad\endcsname{1.44}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_mutations_ok\endcsname{0.69}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls\endcsname{7.42}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls_read\endcsname{0.62}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls_claim\endcsname{6.11}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls_act\endcsname{0.62}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_calls_guarded\endcsname{0.07}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_claims_rca_committed\endcsname{0.69}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_claims_status\endcsname{4.36}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_turns_failed\endcsname{0.16}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_incidents_open\endcsname{10.87}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_mutations_attempted\endcsname{0.69}
\expandafter\def\csname val@act.b1-runbook.60-90.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.60-90.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_active_faults\endcsname{3.29}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_probes_bad\endcsname{1.21}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_mutations_ok\endcsname{0.32}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls\endcsname{6.19}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls_read\endcsname{0.66}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls_claim\endcsname{5.21}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls_act\endcsname{0.27}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_calls_guarded\endcsname{0.05}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_claims_rca_committed\endcsname{0.32}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_claims_status\endcsname{3.68}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_llm_calls\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_tokens_in\endcsname{0}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_turns_failed\endcsname{0.13}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_incidents_open\endcsname{7.60}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_mutations_attempted\endcsname{0.32}
\expandafter\def\csname val@act.b1-runbook.90-∞.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.b1-runbook.90-∞.mean_tokens_in_per_call\endcsname{---}
\expandafter\def\csname val@act.react-b2.0-15.mean_active_faults\endcsname{4.96}
\expandafter\def\csname val@act.react-b2.0-15.mean_probes_bad\endcsname{1.54}
\expandafter\def\csname val@act.react-b2.0-15.mean_mutations_ok\endcsname{0.62}
\expandafter\def\csname val@act.react-b2.0-15.mean_mutations_failed\endcsname{0.04}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls_failed\endcsname{1.29}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls\endcsname{12.79}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls_read\endcsname{8.96}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls_claim\endcsname{3.17}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.0-15.mean_calls_guarded\endcsname{0.67}
\expandafter\def\csname val@act.react-b2.0-15.mean_claims_rca_committed\endcsname{0.50}
\expandafter\def\csname val@act.react-b2.0-15.mean_claims_status\endcsname{1.38}
\expandafter\def\csname val@act.react-b2.0-15.mean_llm_calls\endcsname{5.50}
\expandafter\def\csname val@act.react-b2.0-15.mean_tokens_in\endcsname{67085}
\expandafter\def\csname val@act.react-b2.0-15.mean_dollars\endcsname{0.04}
\expandafter\def\csname val@act.react-b2.0-15.mean_turns_failed\endcsname{0.08}
\expandafter\def\csname val@act.react-b2.0-15.mean_incidents_open\endcsname{1.21}
\expandafter\def\csname val@act.react-b2.0-15.mean_mutations_attempted\endcsname{0.67}
\expandafter\def\csname val@act.react-b2.0-15.failed_call_share\endcsname{0.10}
\expandafter\def\csname val@act.react-b2.0-15.mean_tokens_in_per_call\endcsname{10970}
\expandafter\def\csname val@act.react-b2.15-30.mean_active_faults\endcsname{6.48}
\expandafter\def\csname val@act.react-b2.15-30.mean_probes_bad\endcsname{4.38}
\expandafter\def\csname val@act.react-b2.15-30.mean_mutations_ok\endcsname{0.48}
\expandafter\def\csname val@act.react-b2.15-30.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls_failed\endcsname{2.43}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls\endcsname{23.71}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls_read\endcsname{11.67}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls_claim\endcsname{11.57}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.15-30.mean_calls_guarded\endcsname{0.48}
\expandafter\def\csname val@act.react-b2.15-30.mean_claims_rca_committed\endcsname{0.62}
\expandafter\def\csname val@act.react-b2.15-30.mean_claims_status\endcsname{8.95}
\expandafter\def\csname val@act.react-b2.15-30.mean_llm_calls\endcsname{7.29}
\expandafter\def\csname val@act.react-b2.15-30.mean_tokens_in\endcsname{110512}
\expandafter\def\csname val@act.react-b2.15-30.mean_dollars\endcsname{0.07}
\expandafter\def\csname val@act.react-b2.15-30.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.15-30.mean_incidents_open\endcsname{9.86}
\expandafter\def\csname val@act.react-b2.15-30.mean_mutations_attempted\endcsname{0.48}
\expandafter\def\csname val@act.react-b2.15-30.failed_call_share\endcsname{0.10}
\expandafter\def\csname val@act.react-b2.15-30.mean_tokens_in_per_call\endcsname{15587}
\expandafter\def\csname val@act.react-b2.30-45.mean_active_faults\endcsname{5.21}
\expandafter\def\csname val@act.react-b2.30-45.mean_probes_bad\endcsname{2.25}
\expandafter\def\csname val@act.react-b2.30-45.mean_mutations_ok\endcsname{0.38}
\expandafter\def\csname val@act.react-b2.30-45.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls_failed\endcsname{2.96}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls\endcsname{33.29}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls_read\endcsname{13.50}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls_claim\endcsname{19.42}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.30-45.mean_calls_guarded\endcsname{0.38}
\expandafter\def\csname val@act.react-b2.30-45.mean_claims_rca_committed\endcsname{0.58}
\expandafter\def\csname val@act.react-b2.30-45.mean_claims_status\endcsname{17.58}
\expandafter\def\csname val@act.react-b2.30-45.mean_llm_calls\endcsname{6.29}
\expandafter\def\csname val@act.react-b2.30-45.mean_tokens_in\endcsname{129683}
\expandafter\def\csname val@act.react-b2.30-45.mean_dollars\endcsname{0.08}
\expandafter\def\csname val@act.react-b2.30-45.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.30-45.mean_incidents_open\endcsname{18.62}
\expandafter\def\csname val@act.react-b2.30-45.mean_mutations_attempted\endcsname{0.38}
\expandafter\def\csname val@act.react-b2.30-45.failed_call_share\endcsname{0.09}
\expandafter\def\csname val@act.react-b2.30-45.mean_tokens_in_per_call\endcsname{21869}
\expandafter\def\csname val@act.react-b2.45-60.mean_active_faults\endcsname{6.95}
\expandafter\def\csname val@act.react-b2.45-60.mean_probes_bad\endcsname{4.67}
\expandafter\def\csname val@act.react-b2.45-60.mean_mutations_ok\endcsname{0.14}
\expandafter\def\csname val@act.react-b2.45-60.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls_failed\endcsname{2.00}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls\endcsname{33.71}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls_read\endcsname{10.76}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls_claim\endcsname{22.81}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.45-60.mean_calls_guarded\endcsname{0.14}
\expandafter\def\csname val@act.react-b2.45-60.mean_claims_rca_committed\endcsname{0.19}
\expandafter\def\csname val@act.react-b2.45-60.mean_claims_status\endcsname{21.62}
\expandafter\def\csname val@act.react-b2.45-60.mean_llm_calls\endcsname{4.81}
\expandafter\def\csname val@act.react-b2.45-60.mean_tokens_in\endcsname{108194}
\expandafter\def\csname val@act.react-b2.45-60.mean_dollars\endcsname{0.07}
\expandafter\def\csname val@act.react-b2.45-60.mean_turns_failed\endcsname{0.05}
\expandafter\def\csname val@act.react-b2.45-60.mean_incidents_open\endcsname{26.38}
\expandafter\def\csname val@act.react-b2.45-60.mean_mutations_attempted\endcsname{0.14}
\expandafter\def\csname val@act.react-b2.45-60.failed_call_share\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.45-60.mean_tokens_in_per_call\endcsname{23516}
\expandafter\def\csname val@act.react-b2.60-90.mean_active_faults\endcsname{4.44}
\expandafter\def\csname val@act.react-b2.60-90.mean_probes_bad\endcsname{1.80}
\expandafter\def\csname val@act.react-b2.60-90.mean_mutations_ok\endcsname{0.13}
\expandafter\def\csname val@act.react-b2.60-90.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls_failed\endcsname{2.33}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls\endcsname{40.56}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls_read\endcsname{10.58}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls_claim\endcsname{29.84}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.60-90.mean_calls_guarded\endcsname{0.13}
\expandafter\def\csname val@act.react-b2.60-90.mean_claims_rca_committed\endcsname{0.38}
\expandafter\def\csname val@act.react-b2.60-90.mean_claims_status\endcsname{28.44}
\expandafter\def\csname val@act.react-b2.60-90.mean_llm_calls\endcsname{4.07}
\expandafter\def\csname val@act.react-b2.60-90.mean_tokens_in\endcsname{120233}
\expandafter\def\csname val@act.react-b2.60-90.mean_dollars\endcsname{0.07}
\expandafter\def\csname val@act.react-b2.60-90.mean_turns_failed\endcsname{0.04}
\expandafter\def\csname val@act.react-b2.60-90.mean_incidents_open\endcsname{32.53}
\expandafter\def\csname val@act.react-b2.60-90.mean_mutations_attempted\endcsname{0.13}
\expandafter\def\csname val@act.react-b2.60-90.failed_call_share\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.60-90.mean_tokens_in_per_call\endcsname{30489}
\expandafter\def\csname val@act.react-b2.90-∞.mean_active_faults\endcsname{2.53}
\expandafter\def\csname val@act.react-b2.90-∞.mean_probes_bad\endcsname{0.72}
\expandafter\def\csname val@act.react-b2.90-∞.mean_mutations_ok\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.90-∞.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls_failed\endcsname{1.74}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls\endcsname{21.49}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls_read\endcsname{8.51}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls_claim\endcsname{12.91}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.react-b2.90-∞.mean_calls_guarded\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.90-∞.mean_claims_rca_committed\endcsname{0.62}
\expandafter\def\csname val@act.react-b2.90-∞.mean_claims_status\endcsname{11.28}
\expandafter\def\csname val@act.react-b2.90-∞.mean_llm_calls\endcsname{3.74}
\expandafter\def\csname val@act.react-b2.90-∞.mean_tokens_in\endcsname{99275}
\expandafter\def\csname val@act.react-b2.90-∞.mean_dollars\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.90-∞.mean_turns_failed\endcsname{0.09}
\expandafter\def\csname val@act.react-b2.90-∞.mean_incidents_open\endcsname{19.89}
\expandafter\def\csname val@act.react-b2.90-∞.mean_mutations_attempted\endcsname{0.06}
\expandafter\def\csname val@act.react-b2.90-∞.failed_call_share\endcsname{0.08}
\expandafter\def\csname val@act.react-b2.90-∞.mean_tokens_in_per_call\endcsname{27035}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_active_faults\endcsname{4.46}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_probes_bad\endcsname{1.54}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_mutations_ok\endcsname{0.58}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_mutations_failed\endcsname{0.38}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls_failed\endcsname{0.96}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls\endcsname{16.33}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls_read\endcsname{5.67}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls_claim\endcsname{9.71}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls_act\endcsname{0.33}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_calls_guarded\endcsname{0.62}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_claims_rca_committed\endcsname{2.71}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_claims_status\endcsname{5.71}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_llm_calls\endcsname{0.62}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_tokens_in\endcsname{2540}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_dollars\endcsname{0.00}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_turns_failed\endcsname{0.17}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_incidents_open\endcsname{3.75}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_mutations_attempted\endcsname{0.96}
\expandafter\def\csname val@act.rag-b2r.0-15.failed_call_share\endcsname{0.06}
\expandafter\def\csname val@act.rag-b2r.0-15.mean_tokens_in_per_call\endcsname{4065}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_active_faults\endcsname{6.43}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_probes_bad\endcsname{4.10}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_mutations_ok\endcsname{1.43}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_mutations_failed\endcsname{0.38}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls_failed\endcsname{1.43}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls\endcsname{30.76}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls_read\endcsname{6.52}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls_claim\endcsname{22.43}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls_act\endcsname{0.24}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_calls_guarded\endcsname{1.57}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_claims_rca_committed\endcsname{7.43}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_claims_status\endcsname{13.90}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_llm_calls\endcsname{0.52}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_tokens_in\endcsname{5905}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_dollars\endcsname{0.01}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_turns_failed\endcsname{0.24}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_incidents_open\endcsname{11.71}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_mutations_attempted\endcsname{1.81}
\expandafter\def\csname val@act.rag-b2r.15-30.failed_call_share\endcsname{0.05}
\expandafter\def\csname val@act.rag-b2r.15-30.mean_tokens_in_per_call\endcsname{11383}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_active_faults\endcsname{5.75}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_probes_bad\endcsname{3.17}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_mutations_ok\endcsname{1.46}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_mutations_failed\endcsname{0.67}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls_failed\endcsname{2.25}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls\endcsname{45.50}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls_read\endcsname{9.54}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls_claim\endcsname{33.83}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls_act\endcsname{0.08}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_calls_guarded\endcsname{2.04}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_claims_rca_committed\endcsname{10.71}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_claims_status\endcsname{21.50}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_llm_calls\endcsname{0.75}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_tokens_in\endcsname{10679}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_dollars\endcsname{0.01}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_turns_failed\endcsname{0.08}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_incidents_open\endcsname{19.00}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_mutations_attempted\endcsname{2.12}
\expandafter\def\csname val@act.rag-b2r.30-45.failed_call_share\endcsname{0.05}
\expandafter\def\csname val@act.rag-b2r.30-45.mean_tokens_in_per_call\endcsname{14239}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_active_faults\endcsname{5.95}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_probes_bad\endcsname{4.48}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_mutations_ok\endcsname{2.14}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_mutations_failed\endcsname{1.33}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls_failed\endcsname{2.43}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls\endcsname{48.14}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls_read\endcsname{8.19}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls_claim\endcsname{36.48}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls_act\endcsname{0.90}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_calls_guarded\endcsname{2.57}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_claims_rca_committed\endcsname{11.57}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_claims_status\endcsname{23.10}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_llm_calls\endcsname{0.86}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_tokens_in\endcsname{16892}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_dollars\endcsname{0.02}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_turns_failed\endcsname{0.19}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_incidents_open\endcsname{24.52}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_mutations_attempted\endcsname{3.48}
\expandafter\def\csname val@act.rag-b2r.45-60.failed_call_share\endcsname{0.05}
\expandafter\def\csname val@act.rag-b2r.45-60.mean_tokens_in_per_call\endcsname{20644}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_active_faults\endcsname{4.71}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_probes_bad\endcsname{2.53}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_mutations_ok\endcsname{1.78}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_mutations_failed\endcsname{0.62}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls_failed\endcsname{1.76}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls\endcsname{47.87}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls_read\endcsname{8.40}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls_claim\endcsname{37.07}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls_act\endcsname{0.36}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_calls_guarded\endcsname{2.04}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_claims_rca_committed\endcsname{9.16}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_claims_status\endcsname{26.42}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_llm_calls\endcsname{0.71}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_tokens_in\endcsname{22377}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_dollars\endcsname{0.02}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_turns_failed\endcsname{0.07}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_incidents_open\endcsname{34.38}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_mutations_attempted\endcsname{2.40}
\expandafter\def\csname val@act.rag-b2r.60-90.failed_call_share\endcsname{0.04}
\expandafter\def\csname val@act.rag-b2r.60-90.mean_tokens_in_per_call\endcsname{31468}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_active_faults\endcsname{2.46}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_probes_bad\endcsname{0.46}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_mutations_ok\endcsname{0.18}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_mutations_failed\endcsname{0.11}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls_failed\endcsname{0.22}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls\endcsname{13.06}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls_read\endcsname{2.18}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls_claim\endcsname{10.59}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls_act\endcsname{0.08}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_calls_guarded\endcsname{0.21}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_claims_rca_committed\endcsname{3.09}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_claims_status\endcsname{7.12}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_llm_calls\endcsname{0.22}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_tokens_in\endcsname{7140}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_dollars\endcsname{0.01}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_turns_failed\endcsname{0.20}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_incidents_open\endcsname{20.63}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_mutations_attempted\endcsname{0.29}
\expandafter\def\csname val@act.rag-b2r.90-∞.failed_call_share\endcsname{0.02}
\expandafter\def\csname val@act.rag-b2r.90-∞.mean_tokens_in_per_call\endcsname{32179}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_active_faults\endcsname{5.12}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_probes_bad\endcsname{2.00}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_mutations_ok\endcsname{0.44}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls_failed\endcsname{0.50}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls\endcsname{12.62}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls_read\endcsname{6.25}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls_claim\endcsname{5.94}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_calls_guarded\endcsname{0.44}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_claims_rca_committed\endcsname{1.50}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_claims_status\endcsname{3.25}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_llm_calls\endcsname{5.25}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_tokens_in\endcsname{85795}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_dollars\endcsname{0.05}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_incidents_open\endcsname{4.44}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_mutations_attempted\endcsname{0.44}
\expandafter\def\csname val@act.opensre-x3.0-15.failed_call_share\endcsname{0.04}
\expandafter\def\csname val@act.opensre-x3.0-15.mean_tokens_in_per_call\endcsname{16057}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_active_faults\endcsname{6.79}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_probes_bad\endcsname{3.14}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_mutations_ok\endcsname{0.43}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls_failed\endcsname{1.21}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls\endcsname{22.64}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls_read\endcsname{9.79}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls_claim\endcsname{12.43}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls_act\endcsname{0.07}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_calls_guarded\endcsname{0.36}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_claims_rca_committed\endcsname{1.71}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_claims_status\endcsname{8.57}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_llm_calls\endcsname{5.71}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_tokens_in\endcsname{122071}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_dollars\endcsname{0.08}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_turns_failed\endcsname{0.14}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_incidents_open\endcsname{26.71}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_mutations_attempted\endcsname{0.43}
\expandafter\def\csname val@act.opensre-x3.15-30.failed_call_share\endcsname{0.05}
\expandafter\def\csname val@act.opensre-x3.15-30.mean_tokens_in_per_call\endcsname{21067}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_active_faults\endcsname{5.81}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_probes_bad\endcsname{2.19}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_mutations_ok\endcsname{0.12}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls_failed\endcsname{1.38}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls\endcsname{14.56}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls_read\endcsname{8.50}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls_claim\endcsname{5.94}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls_act\endcsname{0.06}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_calls_guarded\endcsname{0.06}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_claims_rca_committed\endcsname{0.25}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_claims_status\endcsname{4.56}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_llm_calls\endcsname{4.31}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_tokens_in\endcsname{103224}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_dollars\endcsname{0.06}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_turns_failed\endcsname{0.06}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_incidents_open\endcsname{38.75}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_mutations_attempted\endcsname{0.12}
\expandafter\def\csname val@act.opensre-x3.30-45.failed_call_share\endcsname{0.09}
\expandafter\def\csname val@act.opensre-x3.30-45.mean_tokens_in_per_call\endcsname{24091}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_active_faults\endcsname{5.43}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_probes_bad\endcsname{3.71}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_mutations_ok\endcsname{0.29}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls_failed\endcsname{1.00}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls\endcsname{14.29}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls_read\endcsname{7.50}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls_claim\endcsname{6.50}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_calls_guarded\endcsname{0.29}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_claims_rca_committed\endcsname{1.00}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_claims_status\endcsname{4.07}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_llm_calls\endcsname{3.93}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_tokens_in\endcsname{103438}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_dollars\endcsname{0.07}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_incidents_open\endcsname{44.93}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_mutations_attempted\endcsname{0.29}
\expandafter\def\csname val@act.opensre-x3.45-60.failed_call_share\endcsname{0.07}
\expandafter\def\csname val@act.opensre-x3.45-60.mean_tokens_in_per_call\endcsname{26636}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_active_faults\endcsname{1.97}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_probes_bad\endcsname{0.67}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls_failed\endcsname{0.87}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls\endcsname{12.13}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls_read\endcsname{5.17}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls_claim\endcsname{6.97}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_claims_rca_committed\endcsname{0.67}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_claims_status\endcsname{5.23}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_llm_calls\endcsname{3.23}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_tokens_in\endcsname{84298}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_dollars\endcsname{0.05}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_turns_failed\endcsname{0.03}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_incidents_open\endcsname{59.93}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.60-90.failed_call_share\endcsname{0.07}
\expandafter\def\csname val@act.opensre-x3.60-90.mean_tokens_in_per_call\endcsname{26359}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_active_faults\endcsname{5.76}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_probes_bad\endcsname{0.53}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_mutations_ok\endcsname{0.03}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls_failed\endcsname{0.34}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls\endcsname{7.92}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls_read\endcsname{3.62}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls_claim\endcsname{4.27}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_calls_guarded\endcsname{0.03}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_claims_rca_committed\endcsname{0.59}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_claims_status\endcsname{3.12}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_llm_calls\endcsname{1.99}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_tokens_in\endcsname{51512}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_dollars\endcsname{0.03}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_turns_failed\endcsname{0.05}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_incidents_open\endcsname{34.57}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_mutations_attempted\endcsname{0.03}
\expandafter\def\csname val@act.opensre-x3.90-∞.failed_call_share\endcsname{0.04}
\expandafter\def\csname val@act.opensre-x3.90-∞.mean_tokens_in_per_call\endcsname{25919}
\expandafter\def\csname val@act.orbit-0.0-15.mean_active_faults\endcsname{5.38}
\expandafter\def\csname val@act.orbit-0.0-15.mean_probes_bad\endcsname{1.94}
\expandafter\def\csname val@act.orbit-0.0-15.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls_failed\endcsname{0.06}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls\endcsname{16.06}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls_read\endcsname{2.94}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls_claim\endcsname{13.12}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_claims_status\endcsname{8.94}
\expandafter\def\csname val@act.orbit-0.0-15.mean_llm_calls\endcsname{4.19}
\expandafter\def\csname val@act.orbit-0.0-15.mean_tokens_in\endcsname{47205}
\expandafter\def\csname val@act.orbit-0.0-15.mean_dollars\endcsname{0.03}
\expandafter\def\csname val@act.orbit-0.0-15.mean_turns_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_incidents_open\endcsname{13.50}
\expandafter\def\csname val@act.orbit-0.0-15.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.0-15.mean_tokens_in_per_call\endcsname{10309}
\expandafter\def\csname val@act.orbit-0.15-30.mean_active_faults\endcsname{6.29}
\expandafter\def\csname val@act.orbit-0.15-30.mean_probes_bad\endcsname{3.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls_failed\endcsname{0.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls\endcsname{37.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls_read\endcsname{1.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls_claim\endcsname{36.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_claims_status\endcsname{33.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_llm_calls\endcsname{1.43}
\expandafter\def\csname val@act.orbit-0.15-30.mean_tokens_in\endcsname{40862}
\expandafter\def\csname val@act.orbit-0.15-30.mean_dollars\endcsname{0.03}
\expandafter\def\csname val@act.orbit-0.15-30.mean_turns_failed\endcsname{0.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_incidents_open\endcsname{44.14}
\expandafter\def\csname val@act.orbit-0.15-30.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.15-30.mean_tokens_in_per_call\endcsname{29740}
\expandafter\def\csname val@act.orbit-0.30-45.mean_active_faults\endcsname{5.44}
\expandafter\def\csname val@act.orbit-0.30-45.mean_probes_bad\endcsname{1.81}
\expandafter\def\csname val@act.orbit-0.30-45.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls_failed\endcsname{0.12}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls\endcsname{52.19}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls_read\endcsname{1.94}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls_claim\endcsname{50.25}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_claims_status\endcsname{43.38}
\expandafter\def\csname val@act.orbit-0.30-45.mean_llm_calls\endcsname{2.75}
\expandafter\def\csname val@act.orbit-0.30-45.mean_tokens_in\endcsname{94786}
\expandafter\def\csname val@act.orbit-0.30-45.mean_dollars\endcsname{0.06}
\expandafter\def\csname val@act.orbit-0.30-45.mean_turns_failed\endcsname{0.25}
\expandafter\def\csname val@act.orbit-0.30-45.mean_incidents_open\endcsname{55.19}
\expandafter\def\csname val@act.orbit-0.30-45.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.30-45.mean_tokens_in_per_call\endcsname{42260}
\expandafter\def\csname val@act.orbit-0.45-60.mean_active_faults\endcsname{6.14}
\expandafter\def\csname val@act.orbit-0.45-60.mean_probes_bad\endcsname{3.50}
\expandafter\def\csname val@act.orbit-0.45-60.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls_failed\endcsname{0.07}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls\endcsname{46.71}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls_read\endcsname{1.21}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls_claim\endcsname{45.50}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_claims_status\endcsname{40.29}
\expandafter\def\csname val@act.orbit-0.45-60.mean_llm_calls\endcsname{2.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_tokens_in\endcsname{97128}
\expandafter\def\csname val@act.orbit-0.45-60.mean_dollars\endcsname{0.06}
\expandafter\def\csname val@act.orbit-0.45-60.mean_turns_failed\endcsname{0.36}
\expandafter\def\csname val@act.orbit-0.45-60.mean_incidents_open\endcsname{69.07}
\expandafter\def\csname val@act.orbit-0.45-60.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.45-60.mean_tokens_in_per_call\endcsname{56695}
\expandafter\def\csname val@act.orbit-0.60-90.mean_active_faults\endcsname{4.50}
\expandafter\def\csname val@act.orbit-0.60-90.mean_probes_bad\endcsname{1.80}
\expandafter\def\csname val@act.orbit-0.60-90.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls\endcsname{75.27}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls_read\endcsname{0.63}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls_claim\endcsname{74.63}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_claims_status\endcsname{68.83}
\expandafter\def\csname val@act.orbit-0.60-90.mean_llm_calls\endcsname{1.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_tokens_in\endcsname{91046}
\expandafter\def\csname val@act.orbit-0.60-90.mean_dollars\endcsname{0.06}
\expandafter\def\csname val@act.orbit-0.60-90.mean_turns_failed\endcsname{0.23}
\expandafter\def\csname val@act.orbit-0.60-90.mean_incidents_open\endcsname{95.07}
\expandafter\def\csname val@act.orbit-0.60-90.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.60-90.mean_tokens_in_per_call\endcsname{102618}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_active_faults\endcsname{4.06}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_probes_bad\endcsname{0.92}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_mutations_ok\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_mutations_failed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls_failed\endcsname{0.06}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls\endcsname{78.84}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls_read\endcsname{0.80}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls_claim\endcsname{78.04}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls_act\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_calls_guarded\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_claims_rca_committed\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_claims_status\endcsname{45.02}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_llm_calls\endcsname{1.16}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_tokens_in\endcsname{77597}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_dollars\endcsname{0.05}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_turns_failed\endcsname{0.26}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_incidents_open\endcsname{95.64}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_mutations_attempted\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.failed_call_share\endcsname{0.00}
\expandafter\def\csname val@act.orbit-0.90-∞.mean_tokens_in_per_call\endcsname{79291}
\expandafter\def\csname val@label.long.b0-null.P0\endcsname{102}
\expandafter\def\csname val@label.long.b0-null.P0.pct\endcsname{58}
\expandafter\def\csname val@label.long.b0-null.P0.pctvis\endcsname{84}
\expandafter\def\csname val@label.long.b0-null.P1\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P2\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P2.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P3\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P3.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P4\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P4.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P5\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P5.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P6\endcsname{20}
\expandafter\def\csname val@label.long.b0-null.P6.pct\endcsname{11}
\expandafter\def\csname val@label.long.b0-null.P6.pctvis\endcsname{16}
\expandafter\def\csname val@label.long.b0-null.P7\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P7.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.P8\endcsname{55}
\expandafter\def\csname val@label.long.b0-null.P8.pct\endcsname{31}
\expandafter\def\csname val@label.long.b0-null.dx_exact\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_exact.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_partial\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_partial.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.long.b0-null.dx_none\endcsname{177}
\expandafter\def\csname val@label.long.b0-null.dx_none.pct\endcsname{100}
\expandafter\def\csname val@label.long.b0-null.n\endcsname{177}
\expandafter\def\csname val@label.long.b0-null.nvis\endcsname{122}
\expandafter\def\csname val@label.long.b1-runbook.P0\endcsname{47}
\expandafter\def\csname val@label.long.b1-runbook.P0.pct\endcsname{27}
\expandafter\def\csname val@label.long.b1-runbook.P0.pctvis\endcsname{42}
\expandafter\def\csname val@label.long.b1-runbook.P1\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P2\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P2.pct\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P3\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P3.pct\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.P4\endcsname{1}
\expandafter\def\csname val@label.long.b1-runbook.P4.pct\endcsname{1}
\expandafter\def\csname val@label.long.b1-runbook.P4.pctvis\endcsname{1}
\expandafter\def\csname val@label.long.b1-runbook.P5\endcsname{55}
\expandafter\def\csname val@label.long.b1-runbook.P5.pct\endcsname{32}
\expandafter\def\csname val@label.long.b1-runbook.P5.pctvis\endcsname{49}
\expandafter\def\csname val@label.long.b1-runbook.P6\endcsname{7}
\expandafter\def\csname val@label.long.b1-runbook.P6.pct\endcsname{4}
\expandafter\def\csname val@label.long.b1-runbook.P6.pctvis\endcsname{6}
\expandafter\def\csname val@label.long.b1-runbook.P7\endcsname{3}
\expandafter\def\csname val@label.long.b1-runbook.P7.pct\endcsname{2}
\expandafter\def\csname val@label.long.b1-runbook.P7.pctvis\endcsname{3}
\expandafter\def\csname val@label.long.b1-runbook.P8\endcsname{59}
\expandafter\def\csname val@label.long.b1-runbook.P8.pct\endcsname{34}
\expandafter\def\csname val@label.long.b1-runbook.dx_exact\endcsname{2}
\expandafter\def\csname val@label.long.b1-runbook.dx_exact.pct\endcsname{1}
\expandafter\def\csname val@label.long.b1-runbook.dx_partial\endcsname{90}
\expandafter\def\csname val@label.long.b1-runbook.dx_partial.pct\endcsname{52}
\expandafter\def\csname val@label.long.b1-runbook.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.long.b1-runbook.dx_none\endcsname{80}
\expandafter\def\csname val@label.long.b1-runbook.dx_none.pct\endcsname{47}
\expandafter\def\csname val@label.long.b1-runbook.n\endcsname{172}
\expandafter\def\csname val@label.long.b1-runbook.nvis\endcsname{113}
\expandafter\def\csname val@label.long.react-b2.P0\endcsname{72}
\expandafter\def\csname val@label.long.react-b2.P0.pct\endcsname{41}
\expandafter\def\csname val@label.long.react-b2.P0.pctvis\endcsname{63}
\expandafter\def\csname val@label.long.react-b2.P1\endcsname{0}
\expandafter\def\csname val@label.long.react-b2.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.react-b2.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.react-b2.P2\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P2.pct\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P2.pctvis\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P3\endcsname{3}
\expandafter\def\csname val@label.long.react-b2.P3.pct\endcsname{2}
\expandafter\def\csname val@label.long.react-b2.P3.pctvis\endcsname{3}
\expandafter\def\csname val@label.long.react-b2.P4\endcsname{2}
\expandafter\def\csname val@label.long.react-b2.P4.pct\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P4.pctvis\endcsname{2}
\expandafter\def\csname val@label.long.react-b2.P5\endcsname{20}
\expandafter\def\csname val@label.long.react-b2.P5.pct\endcsname{11}
\expandafter\def\csname val@label.long.react-b2.P5.pctvis\endcsname{18}
\expandafter\def\csname val@label.long.react-b2.P6\endcsname{15}
\expandafter\def\csname val@label.long.react-b2.P6.pct\endcsname{8}
\expandafter\def\csname val@label.long.react-b2.P6.pctvis\endcsname{13}
\expandafter\def\csname val@label.long.react-b2.P7\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P7.pct\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P7.pctvis\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.P8\endcsname{63}
\expandafter\def\csname val@label.long.react-b2.P8.pct\endcsname{36}
\expandafter\def\csname val@label.long.react-b2.dx_exact\endcsname{12}
\expandafter\def\csname val@label.long.react-b2.dx_exact.pct\endcsname{7}
\expandafter\def\csname val@label.long.react-b2.dx_partial\endcsname{27}
\expandafter\def\csname val@label.long.react-b2.dx_partial.pct\endcsname{15}
\expandafter\def\csname val@label.long.react-b2.dx_wrong\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.dx_wrong.pct\endcsname{1}
\expandafter\def\csname val@label.long.react-b2.dx_none\endcsname{137}
\expandafter\def\csname val@label.long.react-b2.dx_none.pct\endcsname{77}
\expandafter\def\csname val@label.long.react-b2.n\endcsname{177}
\expandafter\def\csname val@label.long.react-b2.nvis\endcsname{114}
\expandafter\def\csname val@label.long.rag-b2r.P0\endcsname{5}
\expandafter\def\csname val@label.long.rag-b2r.P0.pct\endcsname{3}
\expandafter\def\csname val@label.long.rag-b2r.P0.pctvis\endcsname{4}
\expandafter\def\csname val@label.long.rag-b2r.P1\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P2\endcsname{10}
\expandafter\def\csname val@label.long.rag-b2r.P2.pct\endcsname{6}
\expandafter\def\csname val@label.long.rag-b2r.P2.pctvis\endcsname{8}
\expandafter\def\csname val@label.long.rag-b2r.P3\endcsname{4}
\expandafter\def\csname val@label.long.rag-b2r.P3.pct\endcsname{2}
\expandafter\def\csname val@label.long.rag-b2r.P3.pctvis\endcsname{3}
\expandafter\def\csname val@label.long.rag-b2r.P4\endcsname{34}
\expandafter\def\csname val@label.long.rag-b2r.P4.pct\endcsname{19}
\expandafter\def\csname val@label.long.rag-b2r.P4.pctvis\endcsname{28}
\expandafter\def\csname val@label.long.rag-b2r.P5\endcsname{58}
\expandafter\def\csname val@label.long.rag-b2r.P5.pct\endcsname{33}
\expandafter\def\csname val@label.long.rag-b2r.P5.pctvis\endcsname{48}
\expandafter\def\csname val@label.long.rag-b2r.P6\endcsname{11}
\expandafter\def\csname val@label.long.rag-b2r.P6.pct\endcsname{6}
\expandafter\def\csname val@label.long.rag-b2r.P6.pctvis\endcsname{9}
\expandafter\def\csname val@label.long.rag-b2r.P7\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P7.pct\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.rag-b2r.P8\endcsname{53}
\expandafter\def\csname val@label.long.rag-b2r.P8.pct\endcsname{30}
\expandafter\def\csname val@label.long.rag-b2r.dx_exact\endcsname{11}
\expandafter\def\csname val@label.long.rag-b2r.dx_exact.pct\endcsname{6}
\expandafter\def\csname val@label.long.rag-b2r.dx_partial\endcsname{119}
\expandafter\def\csname val@label.long.rag-b2r.dx_partial.pct\endcsname{68}
\expandafter\def\csname val@label.long.rag-b2r.dx_wrong\endcsname{10}
\expandafter\def\csname val@label.long.rag-b2r.dx_wrong.pct\endcsname{6}
\expandafter\def\csname val@label.long.rag-b2r.dx_none\endcsname{35}
\expandafter\def\csname val@label.long.rag-b2r.dx_none.pct\endcsname{20}
\expandafter\def\csname val@label.long.rag-b2r.n\endcsname{175}
\expandafter\def\csname val@label.long.rag-b2r.nvis\endcsname{122}
\expandafter\def\csname val@label.long.opensre-x3.P0\endcsname{29}
\expandafter\def\csname val@label.long.opensre-x3.P0.pct\endcsname{25}
\expandafter\def\csname val@label.long.opensre-x3.P0.pctvis\endcsname{40}
\expandafter\def\csname val@label.long.opensre-x3.P1\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P2\endcsname{5}
\expandafter\def\csname val@label.long.opensre-x3.P2.pct\endcsname{4}
\expandafter\def\csname val@label.long.opensre-x3.P2.pctvis\endcsname{7}
\expandafter\def\csname val@label.long.opensre-x3.P3\endcsname{1}
\expandafter\def\csname val@label.long.opensre-x3.P3.pct\endcsname{1}
\expandafter\def\csname val@label.long.opensre-x3.P3.pctvis\endcsname{1}
\expandafter\def\csname val@label.long.opensre-x3.P4\endcsname{18}
\expandafter\def\csname val@label.long.opensre-x3.P4.pct\endcsname{16}
\expandafter\def\csname val@label.long.opensre-x3.P4.pctvis\endcsname{25}
\expandafter\def\csname val@label.long.opensre-x3.P5\endcsname{6}
\expandafter\def\csname val@label.long.opensre-x3.P5.pct\endcsname{5}
\expandafter\def\csname val@label.long.opensre-x3.P5.pctvis\endcsname{8}
\expandafter\def\csname val@label.long.opensre-x3.P6\endcsname{14}
\expandafter\def\csname val@label.long.opensre-x3.P6.pct\endcsname{12}
\expandafter\def\csname val@label.long.opensre-x3.P6.pctvis\endcsname{19}
\expandafter\def\csname val@label.long.opensre-x3.P7\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P7.pct\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.opensre-x3.P8\endcsname{41}
\expandafter\def\csname val@label.long.opensre-x3.P8.pct\endcsname{36}
\expandafter\def\csname val@label.long.opensre-x3.dx_exact\endcsname{16}
\expandafter\def\csname val@label.long.opensre-x3.dx_exact.pct\endcsname{14}
\expandafter\def\csname val@label.long.opensre-x3.dx_partial\endcsname{36}
\expandafter\def\csname val@label.long.opensre-x3.dx_partial.pct\endcsname{32}
\expandafter\def\csname val@label.long.opensre-x3.dx_wrong\endcsname{1}
\expandafter\def\csname val@label.long.opensre-x3.dx_wrong.pct\endcsname{1}
\expandafter\def\csname val@label.long.opensre-x3.dx_none\endcsname{61}
\expandafter\def\csname val@label.long.opensre-x3.dx_none.pct\endcsname{54}
\expandafter\def\csname val@label.long.opensre-x3.n\endcsname{114}
\expandafter\def\csname val@label.long.opensre-x3.nvis\endcsname{73}
\expandafter\def\csname val@label.long.orbit-0.P0\endcsname{52}
\expandafter\def\csname val@label.long.orbit-0.P0.pct\endcsname{44}
\expandafter\def\csname val@label.long.orbit-0.P0.pctvis\endcsname{74}
\expandafter\def\csname val@label.long.orbit-0.P1\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P1.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P2\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P2.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P3\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P3.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P4\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P4.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P5\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P5.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P6\endcsname{18}
\expandafter\def\csname val@label.long.orbit-0.P6.pct\endcsname{15}
\expandafter\def\csname val@label.long.orbit-0.P6.pctvis\endcsname{26}
\expandafter\def\csname val@label.long.orbit-0.P7\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P7.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.P8\endcsname{47}
\expandafter\def\csname val@label.long.orbit-0.P8.pct\endcsname{40}
\expandafter\def\csname val@label.long.orbit-0.dx_exact\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_exact.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_partial\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_partial.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.long.orbit-0.dx_none\endcsname{117}
\expandafter\def\csname val@label.long.orbit-0.dx_none.pct\endcsname{100}
\expandafter\def\csname val@label.long.orbit-0.n\endcsname{117}
\expandafter\def\csname val@label.long.orbit-0.nvis\endcsname{70}
\expandafter\def\csname val@label.short.b0-null.P0\endcsname{41}
\expandafter\def\csname val@label.short.b0-null.P0.pct\endcsname{47}
\expandafter\def\csname val@label.short.b0-null.P0.pctvis\endcsname{91}
\expandafter\def\csname val@label.short.b0-null.P1\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P2\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P2.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P3\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P4\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P4.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P5\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P5.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P6\endcsname{4}
\expandafter\def\csname val@label.short.b0-null.P6.pct\endcsname{5}
\expandafter\def\csname val@label.short.b0-null.P6.pctvis\endcsname{9}
\expandafter\def\csname val@label.short.b0-null.P7\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P7.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.P8\endcsname{43}
\expandafter\def\csname val@label.short.b0-null.P8.pct\endcsname{49}
\expandafter\def\csname val@label.short.b0-null.dx_exact\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_exact.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_partial\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_partial.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.short.b0-null.dx_none\endcsname{88}
\expandafter\def\csname val@label.short.b0-null.dx_none.pct\endcsname{100}
\expandafter\def\csname val@label.short.b0-null.n\endcsname{88}
\expandafter\def\csname val@label.short.b0-null.nvis\endcsname{45}
\expandafter\def\csname val@label.short.react-b2.P0\endcsname{3}
\expandafter\def\csname val@label.short.react-b2.P0.pct\endcsname{3}
\expandafter\def\csname val@label.short.react-b2.P0.pctvis\endcsname{6}
\expandafter\def\csname val@label.short.react-b2.P1\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P2\endcsname{1}
\expandafter\def\csname val@label.short.react-b2.P2.pct\endcsname{1}
\expandafter\def\csname val@label.short.react-b2.P2.pctvis\endcsname{2}
\expandafter\def\csname val@label.short.react-b2.P3\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short.react-b2.P4\endcsname{1}
\expandafter\def\csname val@label.short.react-b2.P4.pct\endcsname{1}
\expandafter\def\csname val@label.short.react-b2.P4.pctvis\endcsname{2}
\expandafter\def\csname val@label.short.react-b2.P5\endcsname{19}
\expandafter\def\csname val@label.short.react-b2.P5.pct\endcsname{21}
\expandafter\def\csname val@label.short.react-b2.P5.pctvis\endcsname{37}
\expandafter\def\csname val@label.short.react-b2.P6\endcsname{17}
\expandafter\def\csname val@label.short.react-b2.P6.pct\endcsname{19}
\expandafter\def\csname val@label.short.react-b2.P6.pctvis\endcsname{33}
\expandafter\def\csname val@label.short.react-b2.P7\endcsname{10}
\expandafter\def\csname val@label.short.react-b2.P7.pct\endcsname{11}
\expandafter\def\csname val@label.short.react-b2.P7.pctvis\endcsname{20}
\expandafter\def\csname val@label.short.react-b2.P8\endcsname{38}
\expandafter\def\csname val@label.short.react-b2.P8.pct\endcsname{43}
\expandafter\def\csname val@label.short.react-b2.dx_exact\endcsname{18}
\expandafter\def\csname val@label.short.react-b2.dx_exact.pct\endcsname{20}
\expandafter\def\csname val@label.short.react-b2.dx_partial\endcsname{33}
\expandafter\def\csname val@label.short.react-b2.dx_partial.pct\endcsname{37}
\expandafter\def\csname val@label.short.react-b2.dx_wrong\endcsname{7}
\expandafter\def\csname val@label.short.react-b2.dx_wrong.pct\endcsname{8}
\expandafter\def\csname val@label.short.react-b2.dx_none\endcsname{31}
\expandafter\def\csname val@label.short.react-b2.dx_none.pct\endcsname{35}
\expandafter\def\csname val@label.short.react-b2.n\endcsname{89}
\expandafter\def\csname val@label.short.react-b2.nvis\endcsname{51}
\expandafter\def\csname val@label.short5.b0-null.P0\endcsname{10}
\expandafter\def\csname val@label.short5.b0-null.P0.pct\endcsname{33}
\expandafter\def\csname val@label.short5.b0-null.P0.pctvis\endcsname{83}
\expandafter\def\csname val@label.short5.b0-null.P1\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P2\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P2.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P3\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P4\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P4.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P5\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P5.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P6\endcsname{2}
\expandafter\def\csname val@label.short5.b0-null.P6.pct\endcsname{7}
\expandafter\def\csname val@label.short5.b0-null.P6.pctvis\endcsname{17}
\expandafter\def\csname val@label.short5.b0-null.P7\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P7.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.P8\endcsname{18}
\expandafter\def\csname val@label.short5.b0-null.P8.pct\endcsname{60}
\expandafter\def\csname val@label.short5.b0-null.dx_exact\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_exact.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_partial\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_partial.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.short5.b0-null.dx_none\endcsname{30}
\expandafter\def\csname val@label.short5.b0-null.dx_none.pct\endcsname{100}
\expandafter\def\csname val@label.short5.b0-null.n\endcsname{30}
\expandafter\def\csname val@label.short5.b0-null.nvis\endcsname{12}
\expandafter\def\csname val@label.short5.react-b2.P0\endcsname{1}
\expandafter\def\csname val@label.short5.react-b2.P0.pct\endcsname{3}
\expandafter\def\csname val@label.short5.react-b2.P0.pctvis\endcsname{6}
\expandafter\def\csname val@label.short5.react-b2.P1\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P2\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P2.pct\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P3\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P4\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P4.pct\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P5\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P5.pct\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.short5.react-b2.P6\endcsname{8}
\expandafter\def\csname val@label.short5.react-b2.P6.pct\endcsname{27}
\expandafter\def\csname val@label.short5.react-b2.P6.pctvis\endcsname{50}
\expandafter\def\csname val@label.short5.react-b2.P7\endcsname{7}
\expandafter\def\csname val@label.short5.react-b2.P7.pct\endcsname{23}
\expandafter\def\csname val@label.short5.react-b2.P7.pctvis\endcsname{44}
\expandafter\def\csname val@label.short5.react-b2.P8\endcsname{14}
\expandafter\def\csname val@label.short5.react-b2.P8.pct\endcsname{47}
\expandafter\def\csname val@label.short5.react-b2.dx_exact\endcsname{5}
\expandafter\def\csname val@label.short5.react-b2.dx_exact.pct\endcsname{17}
\expandafter\def\csname val@label.short5.react-b2.dx_partial\endcsname{12}
\expandafter\def\csname val@label.short5.react-b2.dx_partial.pct\endcsname{40}
\expandafter\def\csname val@label.short5.react-b2.dx_wrong\endcsname{3}
\expandafter\def\csname val@label.short5.react-b2.dx_wrong.pct\endcsname{10}
\expandafter\def\csname val@label.short5.react-b2.dx_none\endcsname{10}
\expandafter\def\csname val@label.short5.react-b2.dx_none.pct\endcsname{33}
\expandafter\def\csname val@label.short5.react-b2.n\endcsname{30}
\expandafter\def\csname val@label.short5.react-b2.nvis\endcsname{16}
\expandafter\def\csname val@label.short10.b0-null.P0\endcsname{31}
\expandafter\def\csname val@label.short10.b0-null.P0.pct\endcsname{53}
\expandafter\def\csname val@label.short10.b0-null.P0.pctvis\endcsname{94}
\expandafter\def\csname val@label.short10.b0-null.P1\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P2\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P2.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P2.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P3\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P4\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P4.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P4.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P5\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P5.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P5.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P6\endcsname{2}
\expandafter\def\csname val@label.short10.b0-null.P6.pct\endcsname{3}
\expandafter\def\csname val@label.short10.b0-null.P6.pctvis\endcsname{6}
\expandafter\def\csname val@label.short10.b0-null.P7\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P7.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P7.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.P8\endcsname{25}
\expandafter\def\csname val@label.short10.b0-null.P8.pct\endcsname{43}
\expandafter\def\csname val@label.short10.b0-null.dx_exact\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_exact.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_partial\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_partial.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_wrong\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_wrong.pct\endcsname{0}
\expandafter\def\csname val@label.short10.b0-null.dx_none\endcsname{58}
\expandafter\def\csname val@label.short10.b0-null.dx_none.pct\endcsname{100}
\expandafter\def\csname val@label.short10.b0-null.n\endcsname{58}
\expandafter\def\csname val@label.short10.b0-null.nvis\endcsname{33}
\expandafter\def\csname val@label.short10.react-b2.P0\endcsname{2}
\expandafter\def\csname val@label.short10.react-b2.P0.pct\endcsname{3}
\expandafter\def\csname val@label.short10.react-b2.P0.pctvis\endcsname{6}
\expandafter\def\csname val@label.short10.react-b2.P1\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P1.pct\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P1.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P2\endcsname{1}
\expandafter\def\csname val@label.short10.react-b2.P2.pct\endcsname{2}
\expandafter\def\csname val@label.short10.react-b2.P2.pctvis\endcsname{3}
\expandafter\def\csname val@label.short10.react-b2.P3\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P3.pct\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P3.pctvis\endcsname{0}
\expandafter\def\csname val@label.short10.react-b2.P4\endcsname{1}
\expandafter\def\csname val@label.short10.react-b2.P4.pct\endcsname{2}
\expandafter\def\csname val@label.short10.react-b2.P4.pctvis\endcsname{3}
\expandafter\def\csname val@label.short10.react-b2.P5\endcsname{19}
\expandafter\def\csname val@label.short10.react-b2.P5.pct\endcsname{32}
\expandafter\def\csname val@label.short10.react-b2.P5.pctvis\endcsname{54}
\expandafter\def\csname val@label.short10.react-b2.P6\endcsname{9}
\expandafter\def\csname val@label.short10.react-b2.P6.pct\endcsname{15}
\expandafter\def\csname val@label.short10.react-b2.P6.pctvis\endcsname{26}
\expandafter\def\csname val@label.short10.react-b2.P7\endcsname{3}
\expandafter\def\csname val@label.short10.react-b2.P7.pct\endcsname{5}
\expandafter\def\csname val@label.short10.react-b2.P7.pctvis\endcsname{9}
\expandafter\def\csname val@label.short10.react-b2.P8\endcsname{24}
\expandafter\def\csname val@label.short10.react-b2.P8.pct\endcsname{41}
\expandafter\def\csname val@label.short10.react-b2.dx_exact\endcsname{13}
\expandafter\def\csname val@label.short10.react-b2.dx_exact.pct\endcsname{22}
\expandafter\def\csname val@label.short10.react-b2.dx_partial\endcsname{21}
\expandafter\def\csname val@label.short10.react-b2.dx_partial.pct\endcsname{36}
\expandafter\def\csname val@label.short10.react-b2.dx_wrong\endcsname{4}
\expandafter\def\csname val@label.short10.react-b2.dx_wrong.pct\endcsname{7}
\expandafter\def\csname val@label.short10.react-b2.dx_none\endcsname{21}
\expandafter\def\csname val@label.short10.react-b2.dx_none.pct\endcsname{36}
\expandafter\def\csname val@label.short10.react-b2.n\endcsname{59}
\expandafter\def\csname val@label.short10.react-b2.nvis\endcsname{35}
\expandafter\def\csname val@label.long.P8.total\endcsname{263}
\expandafter\def\csname val@label.long.n.total\endcsname{755}
\expandafter\def\csname val@label.short.P8.total\endcsname{38}
\expandafter\def\csname val@label.short.n.total\endcsname{89}
\expandafter\def\csname val@label.short5.P8.total\endcsname{14}
\expandafter\def\csname val@label.short5.n.total\endcsname{30}
\expandafter\def\csname val@label.short10.P8.total\endcsname{24}
\expandafter\def\csname val@label.short10.n.total\endcsname{59}
\expandafter\def\csname val@shortclass.untouched\endcsname{8}
\expandafter\def\csname val@shortclass.fixed by agent (mitigated only)\endcsname{11}
\expandafter\def\csname val@shortclass.acted, not fixed\endcsname{23}
\expandafter\def\csname val@shortclass.healed, not attributed\endcsname{16}
\expandafter\def\csname val@shortclass.fixed by agent, credited elsewhere\endcsname{24}
\expandafter\def\csname val@shortclass.fixed by agent (root)\endcsname{7}
\expandafter\def\csname val@short.problems\endcsname{89}
\expandafter\def\csname val@short.acted_on\endcsname{65}
\expandafter\def\csname val@short.repaired\endcsname{42}
\expandafter\def\csname val@short.attributed\endcsname{18}
\expandafter\def\csname val@short.parallel_ticks_total\endcsname{21}
\expandafter\def\csname val@short.max_services_one_tick\endcsname{3}
\expandafter\def\csname val@short.never_red\endcsname{38}
\expandafter\def\csname val@short.no_release_entry\endcsname{42}
\expandafter\def\csname val@short.root_fixed_total\endcsname{16}
\expandafter\def\csname val@short5.episodes\endcsname{6}
\expandafter\def\csname val@short5.problems\endcsname{30}
\expandafter\def\csname val@short5.repaired\endcsname{24}
\expandafter\def\csname val@short5.attributed\endcsname{13}
\expandafter\def\csname val@short5.never_red\endcsname{14}
\expandafter\def\csname val@short5.no_release_entry\endcsname{14}
\expandafter\def\csname val@short5.root_fixed_total\endcsname{6}
\expandafter\def\csname val@short5.parallel_ticks_total\endcsname{9}
\expandafter\def\csname val@short5.mutations_total\endcsname{37}
\expandafter\def\csname val@short10.episodes\endcsname{6}
\expandafter\def\csname val@short10.problems\endcsname{59}
\expandafter\def\csname val@short10.repaired\endcsname{18}
\expandafter\def\csname val@short10.attributed\endcsname{5}
\expandafter\def\csname val@short10.never_red\endcsname{24}
\expandafter\def\csname val@short10.no_release_entry\endcsname{28}
\expandafter\def\csname val@short10.root_fixed_total\endcsname{1}
\expandafter\def\csname val@short10.parallel_ticks_total\endcsname{12}
\expandafter\def\csname val@short10.mutations_total\endcsname{74}
\expandafter\def\csname val@nullclass.all.agent recovered it\endcsname{22}
\expandafter\def\csname val@nullclass.all.less severe with the agent\endcsname{10}
\expandafter\def\csname val@nullclass.all.probe never reacted\endcsname{28}
\expandafter\def\csname val@nullclass.all.recovered in null too\endcsname{5}
\expandafter\def\csname val@nullclass.all.unrepaired in both\endcsname{23}
\expandafter\def\csname val@nullclass.all.no reference\endcsname{1}
\expandafter\def\csname val@nullclass.all.worse with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.all.n\endcsname{89}
\expandafter\def\csname val@nullclass.all.better\endcsname{32}
\expandafter\def\csname val@nullclass.5.agent recovered it\endcsname{13}
\expandafter\def\csname val@nullclass.5.less severe with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.5.probe never reacted\endcsname{11}
\expandafter\def\csname val@nullclass.5.recovered in null too\endcsname{3}
\expandafter\def\csname val@nullclass.5.unrepaired in both\endcsname{3}
\expandafter\def\csname val@nullclass.5.no reference\endcsname{0}
\expandafter\def\csname val@nullclass.5.worse with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.5.n\endcsname{30}
\expandafter\def\csname val@nullclass.5.better\endcsname{13}
\expandafter\def\csname val@nullclass.10.agent recovered it\endcsname{9}
\expandafter\def\csname val@nullclass.10.less severe with the agent\endcsname{10}
\expandafter\def\csname val@nullclass.10.probe never reacted\endcsname{17}
\expandafter\def\csname val@nullclass.10.recovered in null too\endcsname{2}
\expandafter\def\csname val@nullclass.10.unrepaired in both\endcsname{20}
\expandafter\def\csname val@nullclass.10.no reference\endcsname{1}
\expandafter\def\csname val@nullclass.10.worse with the agent\endcsname{0}
\expandafter\def\csname val@nullclass.10.n\endcsname{59}
\expandafter\def\csname val@nullclass.10.better\endcsname{19}
\expandafter\def\csname val@inv.problems.OB.library_total\endcsname{216}
\expandafter\def\csname val@inv.problems.OB.schedulable\endcsname{173}
\expandafter\def\csname val@inv.problems.OB.code_path\endcsname{50}
\expandafter\def\csname val@inv.problems.OB.storm_release_problems\endcsname{59}
\expandafter\def\csname val@inv.problems.OB.storm_distinct_problems\endcsname{59}
\expandafter\def\csname val@inv.problems.OB.short_distinct_problems\endcsname{27}
\expandafter\def\csname val@inv.problems.OB.short5_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.OB.short10_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.OB.storm_injected_mean\endcsname{59}
\expandafter\def\csname val@inv.problems.OB.cat.configuration\endcsname{75}
\expandafter\def\csname val@inv.problems.OB.cat.deployment\endcsname{32}
\expandafter\def\csname val@inv.problems.OB.cat.code-bug\endcsname{32}
\expandafter\def\csname val@inv.problems.OB.cat.dependency\endcsname{22}
\expandafter\def\csname val@inv.problems.OB.cat.infrastructure\endcsname{1}
\expandafter\def\csname val@inv.problems.OB.cat.db-network\endcsname{0}
\expandafter\def\csname val@inv.problems.OB.cat.auth\endcsname{11}
\expandafter\def\csname val@inv.problems.OB.cat.other\endcsname{34}
\expandafter\def\csname val@inv.problems.TT.library_total\endcsname{278}
\expandafter\def\csname val@inv.problems.TT.schedulable\endcsname{210}
\expandafter\def\csname val@inv.problems.TT.code_path\endcsname{50}
\expandafter\def\csname val@inv.problems.TT.storm_release_problems\endcsname{60}
\expandafter\def\csname val@inv.problems.TT.storm_distinct_problems\endcsname{60}
\expandafter\def\csname val@inv.problems.TT.short_distinct_problems\endcsname{26}
\expandafter\def\csname val@inv.problems.TT.short5_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.TT.short10_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.TT.storm_injected_mean\endcsname{58}
\expandafter\def\csname val@inv.problems.TT.cat.configuration\endcsname{93}
\expandafter\def\csname val@inv.problems.TT.cat.deployment\endcsname{44}
\expandafter\def\csname val@inv.problems.TT.cat.code-bug\endcsname{32}
\expandafter\def\csname val@inv.problems.TT.cat.dependency\endcsname{23}
\expandafter\def\csname val@inv.problems.TT.cat.infrastructure\endcsname{3}
\expandafter\def\csname val@inv.problems.TT.cat.db-network\endcsname{0}
\expandafter\def\csname val@inv.problems.TT.cat.auth\endcsname{15}
\expandafter\def\csname val@inv.problems.TT.cat.other\endcsname{41}
\expandafter\def\csname val@inv.problems.Astro.library_total\endcsname{418}
\expandafter\def\csname val@inv.problems.Astro.schedulable\endcsname{317}
\expandafter\def\csname val@inv.problems.Astro.code_path\endcsname{163}
\expandafter\def\csname val@inv.problems.Astro.storm_release_problems\endcsname{90}
\expandafter\def\csname val@inv.problems.Astro.storm_distinct_problems\endcsname{58}
\expandafter\def\csname val@inv.problems.Astro.short_distinct_problems\endcsname{27}
\expandafter\def\csname val@inv.problems.Astro.short5_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.Astro.short10_episodes\endcsname{2}
\expandafter\def\csname val@inv.problems.Astro.storm_injected_mean\endcsname{57}
\expandafter\def\csname val@inv.problems.Astro.cat.configuration\endcsname{35}
\expandafter\def\csname val@inv.problems.Astro.cat.deployment\endcsname{67}
\expandafter\def\csname val@inv.problems.Astro.cat.code-bug\endcsname{160}
\expandafter\def\csname val@inv.problems.Astro.cat.dependency\endcsname{20}
\expandafter\def\csname val@inv.problems.Astro.cat.infrastructure\endcsname{9}
\expandafter\def\csname val@inv.problems.Astro.cat.db-network\endcsname{10}
\expandafter\def\csname val@inv.problems.Astro.cat.auth\endcsname{16}
\expandafter\def\csname val@inv.problems.Astro.cat.other\endcsname{55}
\expandafter\def\csname val@inv.problems.total.library_total\endcsname{912}
\expandafter\def\csname val@inv.problems.total.schedulable\endcsname{700}
\expandafter\def\csname val@inv.problems.total.code_path\endcsname{263}
\expandafter\def\csname val@inv.problems.total.storm_release_problems\endcsname{209}
\expandafter\def\csname val@inv.problems.total.cat.configuration\endcsname{203}
\expandafter\def\csname val@inv.problems.total.cat.deployment\endcsname{143}
\expandafter\def\csname val@inv.problems.total.cat.code-bug\endcsname{224}
\expandafter\def\csname val@inv.problems.total.cat.other\endcsname{130}
\expandafter\def\csname val@inv.problems.total.categories\endcsname{7}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null.minutes\endcsname{96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-react-b2.minutes\endcsname{96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-rag-b2r.minutes\endcsname{96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-orbit-0.minutes\endcsname{96}
\expandafter\def\csname val@run.storm-ob-seed7-r3-b1-runbook.minutes\endcsname{98}
\expandafter\def\csname val@run.storm-tt-seed7-null.minutes\endcsname{118}
\expandafter\def\csname val@run.storm-tt-seed7-b1-runbook.minutes\endcsname{142}
\expandafter\def\csname val@run.storm-tt-seed7-react-b2.minutes\endcsname{110}
\expandafter\def\csname val@run.storm-tt-seed7-rag-b2r.minutes\endcsname{110}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null.minutes\endcsname{136}
\expandafter\def\csname val@run.storm-astro-seed7-a7f8dbb813b2-b1-runbook.minutes\endcsname{148}
\expandafter\def\csname val@run.storm-astro-seed7-9e90617a6a78-react-b2.minutes\endcsname{152}
\expandafter\def\csname val@run.storm-astro-seed7-be1411a5e060-rag-b2r.minutes\endcsname{238}
\expandafter\def\csname val@run.storm-astro-seed7-a8ee899d864d-orbit-0.minutes\endcsname{180}
\expandafter\def\csname val@run.storm-ob-seed7-r3-opensre-x3.minutes\endcsname{94}
\expandafter\def\csname val@run.storm-astro-seed7-r3-opensre.minutes\endcsname{282}
\expandafter\def\csname val@run.storm-tt-seed7-r5-opensre.minutes\endcsname{106}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook-null.minutes\endcsname{196}
\expandafter\def\csname val@run.storm-astro-seed17-r3-45310fcfd511-b1-runbook.minutes\endcsname{178}
\expandafter\def\csname val@run.storm-astro-seed17-r3-d5b88824daf9-react-b2.minutes\endcsname{178}
\expandafter\def\csname val@run.storm-astro-seed17-r3-7da7b415640a-rag-b2r.minutes\endcsname{240}
\expandafter\def\csname val@run.storm-astro-seed17-r3-b1273caa93b8-orbit-0.minutes\endcsname{176}
\expandafter\def\csname val@run.storm-ob-seed7-r3-null-0917.minutes\endcsname{92}
\expandafter\def\csname val@run.storm-ob-seed7-r2-null.minutes\endcsname{100}
\expandafter\def\csname val@run.storm-ob-seed7-r2-react-b2.minutes\endcsname{100}
\expandafter\def\csname val@run.storm-ob-seed7-r2-rag-b2r.minutes\endcsname{100}
\expandafter\def\csname val@run.storm-astro-seed7-26696a865589-b1-runbook-null.minutes\endcsname{210}
\expandafter\def\csname val@run.storm-astro-seed7-88a667a6e8c5-b1-runbook.minutes\endcsname{150}
\expandafter\def\csname val@run.storm-astro-seed7-f361831c5856-react-b2.minutes\endcsname{158}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook-null.minutes\endcsname{190}
\expandafter\def\csname val@run.storm-astro-seed7-d5a780607f95-b1-runbook.minutes\endcsname{140}
\expandafter\def\csname val@run.storm-astro-seed7-a3d0366a6a88-react-b2.minutes\endcsname{142}
\expandafter\def\csname val@run.storm-astro-seed7-621a6da181a8-rag-b2r.minutes\endcsname{162}
\expandafter\def\csname val@run.astro-episode1.minutes\endcsname{29}
\expandafter\def\csname val@run.astro-episode2.minutes\endcsname{30}
\expandafter\def\csname val@run.ob-episode1.minutes\endcsname{25}
\expandafter\def\csname val@run.ob-episode2.minutes\endcsname{23}
\expandafter\def\csname val@run.tt-episode1.minutes\endcsname{22}
\expandafter\def\csname val@run.tt-episode2.minutes\endcsname{22}
\expandafter\def\csname val@run.ob-episode3.minutes\endcsname{32}
\expandafter\def\csname val@run.ob-episode4.minutes\endcsname{51}
\expandafter\def\csname val@run.tt-episode3.minutes\endcsname{36}
\expandafter\def\csname val@run.tt-episode4.minutes\endcsname{54}
\expandafter\def\csname val@run.astro-episode1-null.minutes\endcsname{25}
\expandafter\def\csname val@run.astro-episode2-null.minutes\endcsname{36}
\expandafter\def\csname val@run.ob-episode1-null.minutes\endcsname{21}
\expandafter\def\csname val@run.ob-episode2-null.minutes\endcsname{21}
\expandafter\def\csname val@run.ob-episode3-null.minutes\endcsname{33}
\expandafter\def\csname val@run.ob-episode4-null.minutes\endcsname{31}
\expandafter\def\csname val@run.tt-episode1-null.minutes\endcsname{21}
\expandafter\def\csname val@run.tt-episode2-null.minutes\endcsname{21}
\expandafter\def\csname val@run.tt-episode3-null.minutes\endcsname{43}
\expandafter\def\csname val@run.tt-episode4-null.minutes\endcsname{53}
\expandafter\def\csname val@run.astro-episode3.minutes\endcsname{49}
\expandafter\def\csname val@run.astro-episode4.minutes\endcsname{38}
\expandafter\def\csname val@run.astro-episode3-null.minutes\endcsname{44}
\expandafter\def\csname val@run.astro-episode4-null.minutes\endcsname{36}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-rules-90e4d70d4f17.minutes\endcsname{162}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm-7eea193897f2.minutes\endcsname{158}
\expandafter\def\csname val@run.storm-astro-seed7-r3-keep-llm.minutes\endcsname{268}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-null.minutes\endcsname{94}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-rules.minutes\endcsname{98}
\expandafter\def\csname val@run.storm-ob-seed7-r3-keep-llm.minutes\endcsname{98}
\expandafter\def\csname val@run.storm-tt-seed7-r3-null.minutes\endcsname{100}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-rules.minutes\endcsname{102}
\expandafter\def\csname val@run.storm-tt-seed7-r3-keep-llm.minutes\endcsname{104}
\expandafter\def\csname val@run.storm-astro-seed7-r4-null.minutes\endcsname{144}
\expandafter\def\csname val@run.storm-astro-seed7-r4-react-b2.minutes\endcsname{150}
\expandafter\def\csname val@run.storm-astro-seed7-r4-orbit-0.minutes\endcsname{152}
\expandafter\def\csname val@run.storm-astro-seed7-r4-opensre.minutes\endcsname{156}
\expandafter\def\csname val@run.storm-ob-seed7-r4-null.minutes\endcsname{94}
\expandafter\def\csname val@run.storm-ob-seed7-r4-react-b2.minutes\endcsname{94}
\expandafter\def\csname val@run.storm-ob-seed7-r4-orbit-0.minutes\endcsname{94}
\expandafter\def\csname val@run.storm-tt-seed7-r4-react-b2.minutes\endcsname{104}
\expandafter\def\csname val@run.storm-tt-seed7-r4-orbit-0.minutes\endcsname{104}
\expandafter\def\csname val@run.storm-tt-seed7-r4-opensre.minutes\endcsname{104}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-b1-runbook.minutes\endcsname{246}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-react-b2.minutes\endcsname{196}
\expandafter\def\csname val@run.storm-astro-seed27-kubeadm-rag-b2r.minutes\endcsname{198}
\expandafter\def\csname val@seed.b0-null.m1_f1.s7\endcsname{0.00}
\expandafter\def\csname val@seed.b0-null.m1_f1.s17\endcsname{0.00}
\expandafter\def\csname val@seed.b0-null.m2_acc_at_1.s7\endcsname{0.000}
\expandafter\def\csname val@seed.b0-null.m2_acc_at_1.s17\endcsname{0.000}
\expandafter\def\csname val@seed.b0-null.m3_fsr_symptomatic.s7\endcsname{0.25}
\expandafter\def\csname val@seed.b0-null.m3_fsr_symptomatic.s17\endcsname{0.19}
\expandafter\def\csname val@seed.b0-null.m4_regret_raw.s7\endcsname{1.00}
\expandafter\def\csname val@seed.b0-null.m4_regret_raw.s17\endcsname{1.00}
\expandafter\def\csname val@seed.b0-null.m7_blast_radius.s7\endcsname{---}
\expandafter\def\csname val@seed.b0-null.m7_blast_radius.s17\endcsname{---}
\expandafter\def\csname val@seed.b0-null.smash_score.s7\endcsname{0.00}
\expandafter\def\csname val@seed.b0-null.smash_score.s17\endcsname{0.00}
\expandafter\def\csname val@seed.b0-null.rank\endcsname{---}
\expandafter\def\csname val@seed.b1-runbook.m1_f1.s7\endcsname{0.64}
\expandafter\def\csname val@seed.b1-runbook.m1_f1.s17\endcsname{0.85}
\expandafter\def\csname val@seed.b1-runbook.m2_acc_at_1.s7\endcsname{0.000}
\expandafter\def\csname val@seed.b1-runbook.m2_acc_at_1.s17\endcsname{0.000}
\expandafter\def\csname val@seed.b1-runbook.m3_fsr_symptomatic.s7\endcsname{0.23}
\expandafter\def\csname val@seed.b1-runbook.m3_fsr_symptomatic.s17\endcsname{0.19}
\expandafter\def\csname val@seed.b1-runbook.m4_regret_raw.s7\endcsname{0.93}
\expandafter\def\csname val@seed.b1-runbook.m4_regret_raw.s17\endcsname{1.43}
\expandafter\def\csname val@seed.b1-runbook.m7_blast_radius.s7\endcsname{0.09}
\expandafter\def\csname val@seed.b1-runbook.m7_blast_radius.s17\endcsname{0.02}
\expandafter\def\csname val@seed.b1-runbook.smash_score.s7\endcsname{14.33}
\expandafter\def\csname val@seed.b1-runbook.smash_score.s17\endcsname{0.64}
\expandafter\def\csname val@seed.b1-runbook.rank\endcsname{1 to 1}
\expandafter\def\csname val@seed.react-b2.m1_f1.s7\endcsname{0.09}
\expandafter\def\csname val@seed.react-b2.m1_f1.s17\endcsname{0.11}
\expandafter\def\csname val@seed.react-b2.m2_acc_at_1.s7\endcsname{0.121}
\expandafter\def\csname val@seed.react-b2.m2_acc_at_1.s17\endcsname{0.034}
\expandafter\def\csname val@seed.react-b2.m3_fsr_symptomatic.s7\endcsname{0.25}
\expandafter\def\csname val@seed.react-b2.m3_fsr_symptomatic.s17\endcsname{0.17}
\expandafter\def\csname val@seed.react-b2.m4_regret_raw.s7\endcsname{0.77}
\expandafter\def\csname val@seed.react-b2.m4_regret_raw.s17\endcsname{1.38}
\expandafter\def\csname val@seed.react-b2.m7_blast_radius.s7\endcsname{0.14}
\expandafter\def\csname val@seed.react-b2.m7_blast_radius.s17\endcsname{0.59}
\expandafter\def\csname val@seed.react-b2.smash_score.s7\endcsname{13.06}
\expandafter\def\csname val@seed.react-b2.smash_score.s17\endcsname{-9.02}
\expandafter\def\csname val@seed.react-b2.rank\endcsname{2 to 2}
\expandafter\def\csname val@seed.rag-b2r.m1_f1.s7\endcsname{0.42}
\expandafter\def\csname val@seed.rag-b2r.m1_f1.s17\endcsname{0.65}
\expandafter\def\csname val@seed.rag-b2r.m2_acc_at_1.s7\endcsname{0.000}
\expandafter\def\csname val@seed.rag-b2r.m2_acc_at_1.s17\endcsname{0.136}
\expandafter\def\csname val@seed.rag-b2r.m3_fsr_symptomatic.s7\endcsname{0.28}
\expandafter\def\csname val@seed.rag-b2r.m3_fsr_symptomatic.s17\endcsname{0.17}
\expandafter\def\csname val@seed.rag-b2r.m4_regret_raw.s7\endcsname{1.43}
\expandafter\def\csname val@seed.rag-b2r.m4_regret_raw.s17\endcsname{1.74}
\expandafter\def\csname val@seed.rag-b2r.m7_blast_radius.s7\endcsname{0.50}
\expandafter\def\csname val@seed.rag-b2r.m7_blast_radius.s17\endcsname{0.11}
\expandafter\def\csname val@seed.rag-b2r.smash_score.s7\endcsname{-8.73}
\expandafter\def\csname val@seed.rag-b2r.smash_score.s17\endcsname{-12.03}
\expandafter\def\csname val@seed.rag-b2r.rank\endcsname{4 to 3}
\expandafter\def\csname val@seed.orbit-0.m1_f1.s7\endcsname{0.03}
\expandafter\def\csname val@seed.orbit-0.m1_f1.s17\endcsname{0.20}
\expandafter\def\csname val@seed.orbit-0.m2_acc_at_1.s7\endcsname{0.000}
\expandafter\def\csname val@seed.orbit-0.m2_acc_at_1.s17\endcsname{0.000}
\expandafter\def\csname val@seed.orbit-0.m3_fsr_symptomatic.s7\endcsname{0.30}
\expandafter\def\csname val@seed.orbit-0.m3_fsr_symptomatic.s17\endcsname{0.19}
\expandafter\def\csname val@seed.orbit-0.m4_regret_raw.s7\endcsname{0.96}
\expandafter\def\csname val@seed.orbit-0.m4_regret_raw.s17\endcsname{2.87}
\expandafter\def\csname val@seed.orbit-0.m7_blast_radius.s7\endcsname{---}
\expandafter\def\csname val@seed.orbit-0.m7_blast_radius.s17\endcsname{---}
\expandafter\def\csname val@seed.orbit-0.smash_score.s7\endcsname{1.92}
\expandafter\def\csname val@seed.orbit-0.smash_score.s17\endcsname{-31.95}
\expandafter\def\csname val@seed.orbit-0.rank\endcsname{3 to 4}
\expandafter\def\csname val@seed.rank_order_7\endcsname{Runbook, ReAct, ORBIT, RAG}
\expandafter\def\csname val@seed.rank_order_17\endcsname{Runbook, ReAct, RAG, ORBIT}
\expandafter\def\csname val@seed.null_sd_7\endcsname{1244}
\expandafter\def\csname val@seed.null_sd_17\endcsname{886}
\expandafter\def\csname val@seed.worse_than_null_17\endcsname{4}
\expandafter\def\csname val@seed.worse_than_null_7\endcsname{1}
\expandafter\def\csname val@ref.ob_archived\endcsname{8062}
\expandafter\def\csname val@ref.ob_remeasured\endcsname{7747}
\expandafter\def\csname val@ref.ob_delta_pct\endcsname{-3.9}
\expandafter\def\csname val@ref.tt_r1\endcsname{38181}
\expandafter\def\csname val@ref.tt_r5\endcsname{31821}
\expandafter\def\csname val@ref.tt_delta_pct\endcsname{-16.7}
\expandafter\def\csname val@spot.A1\endcsname{1.00}
\expandafter\def\csname val@spot.A1+\endcsname{0.80}
\expandafter\def\csname val@spot.A2.invented_path\endcsname{1.00}
\expandafter\def\csname val@spot.A2.no_incident\endcsname{1.00}
\expandafter\def\csname val@spot.A2.not_found_other\endcsname{1.00}
\expandafter\def\csname val@spot.A2.other\endcsname{1.00}
\expandafter\def\csname val@spot.A2.query_syntax\endcsname{1.00}
\expandafter\def\csname val@spot.A2.stale_pod\endcsname{1.00}
\expandafter\def\csname val@spot.A2.timeout\endcsname{1.00}
\expandafter\def\csname val@spot.A2.vocabulary\endcsname{1.00}
\expandafter\def\csname val@spot.A4\endcsname{1.00}
\expandafter\def\csname val@spot.A5\endcsname{1.00}
\expandafter\def\csname val@spot.A6\endcsname{1.00}
\expandafter\def\csname val@spot.A7\endcsname{1.00}
\expandafter\def\csname val@spot.P0\endcsname{1.00}
\expandafter\def\csname val@spot.P2\endcsname{0.20}
\expandafter\def\csname val@spot.P3\endcsname{1.00}
\expandafter\def\csname val@spot.P4\endcsname{1.00}
\expandafter\def\csname val@spot.P5\endcsname{1.00}
\expandafter\def\csname val@spot.P6\endcsname{1.00}
\expandafter\def\csname val@spot.P7\endcsname{1.00}
\expandafter\def\csname val@spot.P8\endcsname{1.00}
\expandafter\def\csname val@spot.T1\endcsname{1.00}
\expandafter\def\csname val@spot.T2\endcsname{0.20}
\expandafter\def\csname val@spot.T3\endcsname{1.00}
\expandafter\def\csname val@spot.T4\endcsname{1.00}
\expandafter\def\csname val@spot.T6a\endcsname{1.00}
\expandafter\def\csname val@spot.T6b\endcsname{1.00}
\expandafter\def\csname val@spot.items\endcsname{131}
\expandafter\def\csname val@spot.codes\endcsname{28}
\expandafter\def\csname val@spot.reliable_codes\endcsname{26}
\expandafter\def\csname val@rescore.runs\endcsname{79}
\expandafter\def\csname val@rescore.identical\endcsname{0}
\expandafter\def\csname val@rescore.alias_only\endcsname{0}
\expandafter\def\csname val@rescore.never_scored\endcsname{39}
\expandafter\def\csname val@occ.total\endcsname{3362}
\expandafter\def\csname val@occ.long_headline\endcsname{932}
\expandafter\def\csname val@long.dollars_total\endcsname{29.67}
\expandafter\def\csname val@short.dollars_total\endcsname{20.72}
\expandafter\def\csname val@long.llm.agents\endcsname{6}
\expandafter\def\csname val@long.llm.occurrences\endcsname{583}
\expandafter\def\csname val@long.llm.attributed_pct\endcsname{1.4}
\expandafter\def\csname val@long.llm.exact_pct\endcsname{6.7}
\expandafter\def\csname val@long.llm.mitigated_sym_pct\endcsname{15.6}
\expandafter\def\csname val@long.null.mitigated_sym_pct\endcsname{16.4}
\expandafter\def\csname val@crossapp.refusals\endcsname{56}
\expandafter\def\csname val@crossapp.runs\endcsname{6}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-react-b2.tokens_in_max\endcsname{46}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-react-b2.tokens_in_median\endcsname{24}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-rag-b2r.tokens_in_max\endcsname{32}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-rag-b2r.tokens_in_median\endcsname{18}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-orbit-0.tokens_in_max\endcsname{191}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-orbit-0.tokens_in_median\endcsname{23}
\expandafter\def\csname val@traj.storm-tt-seed7-react-b2.tokens_in_max\endcsname{56}
\expandafter\def\csname val@traj.storm-tt-seed7-react-b2.tokens_in_median\endcsname{27}
\expandafter\def\csname val@traj.storm-tt-seed7-rag-b2r.tokens_in_max\endcsname{53}
\expandafter\def\csname val@traj.storm-tt-seed7-rag-b2r.tokens_in_median\endcsname{35}
\expandafter\def\csname val@traj.storm-astro-seed7-9e90617a6a78-react-b2.tokens_in_max\endcsname{35}
\expandafter\def\csname val@traj.storm-astro-seed7-9e90617a6a78-react-b2.tokens_in_median\endcsname{18}
\expandafter\def\csname val@traj.storm-astro-seed7-be1411a5e060-rag-b2r.tokens_in_max\endcsname{15}
\expandafter\def\csname val@traj.storm-astro-seed7-be1411a5e060-rag-b2r.tokens_in_median\endcsname{10}
\expandafter\def\csname val@traj.storm-astro-seed7-a8ee899d864d-orbit-0.tokens_in_max\endcsname{128}
\expandafter\def\csname val@traj.storm-astro-seed7-a8ee899d864d-orbit-0.tokens_in_median\endcsname{18}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-opensre-x3.tokens_in_max\endcsname{56}
\expandafter\def\csname val@traj.storm-ob-seed7-r3-opensre-x3.tokens_in_median\endcsname{24}
\expandafter\def\csname val@traj.storm-astro-seed7-r3-opensre.tokens_in_max\endcsname{44}
\expandafter\def\csname val@traj.storm-astro-seed7-r3-opensre.tokens_in_median\endcsname{24}
\expandafter\def\csname val@traj.storm-tt-seed7-r5-opensre.tokens_in_max\endcsname{58}
\expandafter\def\csname val@traj.storm-tt-seed7-r5-opensre.tokens_in_median\endcsname{30}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-d5b88824daf9-react-b2.tokens_in_max\endcsname{31}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-d5b88824daf9-react-b2.tokens_in_median\endcsname{15}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-7da7b415640a-rag-b2r.tokens_in_max\endcsname{16}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-7da7b415640a-rag-b2r.tokens_in_median\endcsname{6}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-b1273caa93b8-orbit-0.tokens_in_max\endcsname{125}
\expandafter\def\csname val@traj.storm-astro-seed17-r3-b1273caa93b8-orbit-0.tokens_in_median\endcsname{18}
\expandafter\def\csname val@traj.storm-ob-seed7-r2-react-b2.tokens_in_max\endcsname{46}
\expandafter\def\csname val@traj.storm-ob-seed7-r2-react-b2.tokens_in_median\endcsname{22}
\expandafter\def\csname val@traj.storm-ob-seed7-r2-rag-b2r.tokens_in_max\endcsname{27}
\expandafter\def\csname val@traj.storm-ob-seed7-r2-rag-b2r.tokens_in_median\endcsname{16}
\expandafter\def\csname val@traj.storm-astro-seed7-f361831c5856-react-b2.tokens_in_max\endcsname{32}
\expandafter\def\csname val@traj.storm-astro-seed7-f361831c5856-react-b2.tokens_in_median\endcsname{18}
\expandafter\def\csname val@traj.storm-astro-seed7-a3d0366a6a88-react-b2.tokens_in_max\endcsname{37}
\expandafter\def\csname val@traj.storm-astro-seed7-a3d0366a6a88-react-b2.tokens_in_median\endcsname{17}
\expandafter\def\csname val@traj.storm-astro-seed7-621a6da181a8-rag-b2r.tokens_in_max\endcsname{24}
\expandafter\def\csname val@traj.storm-astro-seed7-621a6da181a8-rag-b2r.tokens_in_median\endcsname{14}
\expandafter\def\csname val@traj.astro-episode1.tokens_in_max\endcsname{26}
\expandafter\def\csname val@traj.astro-episode1.tokens_in_median\endcsname{12}
\expandafter\def\csname val@traj.astro-episode2.tokens_in_max\endcsname{26}
\expandafter\def\csname val@traj.astro-episode2.tokens_in_median\endcsname{11}
\expandafter\def\csname val@traj.ob-episode1.tokens_in_max\endcsname{36}
\expandafter\def\csname val@traj.ob-episode1.tokens_in_median\endcsname{10}
\expandafter\def\csname val@traj.ob-episode2.tokens_in_max\endcsname{26}
\expandafter\def\csname val@traj.ob-episode2.tokens_in_median\endcsname{10}
\expandafter\def\csname val@traj.tt-episode1.tokens_in_max\endcsname{26}
\expandafter\def\csname val@traj.tt-episode1.tokens_in_median\endcsname{12}
\expandafter\def\csname val@traj.tt-episode2.tokens_in_max\endcsname{24}
\expandafter\def\csname val@traj.tt-episode2.tokens_in_median\endcsname{13}
\expandafter\def\csname val@traj.ob-episode3.tokens_in_max\endcsname{23}
\expandafter\def\csname val@traj.ob-episode3.tokens_in_median\endcsname{14}
\expandafter\def\csname val@traj.ob-episode4.tokens_in_max\endcsname{32}
\expandafter\def\csname val@traj.ob-episode4.tokens_in_median\endcsname{16}
\expandafter\def\csname val@traj.tt-episode3.tokens_in_max\endcsname{34}
\expandafter\def\csname val@traj.tt-episode3.tokens_in_median\endcsname{14}
\expandafter\def\csname val@traj.tt-episode4.tokens_in_max\endcsname{37}
\expandafter\def\csname val@traj.tt-episode4.tokens_in_median\endcsname{17}
\expandafter\def\csname val@traj.astro-episode3.tokens_in_max\endcsname{30}
\expandafter\def\csname val@traj.astro-episode3.tokens_in_median\endcsname{11}
\expandafter\def\csname val@traj.astro-episode4.tokens_in_max\endcsname{26}
\expandafter\def\csname val@traj.astro-episode4.tokens_in_median\endcsname{11}
\expandafter\def\csname val@traj.storm-astro-seed7-r3-keep-llm-7eea193897f2.tokens_in_max\endcsname{21}
\expandafter\def\csname val@traj.storm-astro-seed7-r3-keep-llm-7eea193897f2.tokens_in_median\endcsname{16}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-react-b2.tokens_in_max\endcsname{39}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-react-b2.tokens_in_median\endcsname{20}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-orbit-0.tokens_in_max\endcsname{83}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-orbit-0.tokens_in_median\endcsname{13}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-opensre.tokens_in_max\endcsname{38}
\expandafter\def\csname val@traj.storm-astro-seed7-r4-opensre.tokens_in_median\endcsname{22}
\expandafter\def\csname val@traj.storm-ob-seed7-r4-react-b2.tokens_in_max\endcsname{70}
\expandafter\def\csname val@traj.storm-ob-seed7-r4-react-b2.tokens_in_median\endcsname{26}
\expandafter\def\csname val@traj.storm-ob-seed7-r4-orbit-0.tokens_in_max\endcsname{201}
\expandafter\def\csname val@traj.storm-ob-seed7-r4-orbit-0.tokens_in_median\endcsname{8}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-react-b2.tokens_in_max\endcsname{61}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-react-b2.tokens_in_median\endcsname{32}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-orbit-0.tokens_in_max\endcsname{178}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-orbit-0.tokens_in_median\endcsname{7}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-opensre.tokens_in_max\endcsname{59}
\expandafter\def\csname val@traj.storm-tt-seed7-r4-opensre.tokens_in_median\endcsname{32}
\expandafter\def\csname val@case.long-good.run\endcsname{storm-tt-seed7-react-b2}
\expandafter\def\csname val@case.long-good-runnerup.run\endcsname{storm-astro-seed7-9e90617a6a78-react-b2}
\expandafter\def\csname val@case.long-bad.run\endcsname{storm-ob-seed7-r3-rag-b2r}
\expandafter\def\csname val@case.long-failure.run\endcsname{storm-astro-seed7-r3-opensre}
\expandafter\def\csname val@case.short-good.run\endcsname{tt-episode3}
\expandafter\def\csname val@case.short-bad.run\endcsname{ob-episode4}
\expandafter\def\csname val@case.longbad.rollbacks_total\endcsname{10}
\expandafter\def\csname val@case.longbad.rollbacks_after_revert\endcsname{10}
\expandafter\def\csname val@case.longbad.new_incidents_after_revert\endcsname{5}
\expandafter\def\csname val@case.longbad.revert_min\endcsname{70}
\expandafter\def\csname val@case.longbad.all_rollbacks\endcsname{63}
\expandafter\def\csname val@case.longbad.uim_after_60\endcsname{4356}
\expandafter\def\csname val@case.longbad.null_uim_after_60\endcsname{1329}
\expandafter\def\csname val@case.shortbad.focal_attempts\endcsname{4}
\expandafter\def\csname val@case.shortbad.focal_attempts_ok\endcsname{4}
\expandafter\def\csname val@case.shortbad.focal_tools\endcsname{restart\_pod, rollback, update\_config}
\expandafter\def\csname val@case.shortbad.mutations_total\endcsname{15}
\expandafter\def\csname val@case.shortbad.refused_calls\endcsname{98}
\expandafter\def\csname val@case.shortbad.status_claims\endcsname{147}
\expandafter\def\csname val@case.shortbad.status_open\endcsname{132}
\expandafter\def\csname val@case.shortbad.incidents\endcsname{14}
\expandafter\def\csname val@case.shortbad.focal_bad_probe_ticks\endcsname{20}
\expandafter\def\csname val@case.shortbad.focal_probe_ticks\endcsname{20}
\expandafter\def\csname val@case.shortbad.flag_refusals\endcsname{1}
\expandafter\def\csname val@case.shortbad.patch_refusals\endcsname{2}
\expandafter\def\csname val@case.shortgood.first_repair_s\endcsname{133}
\expandafter\def\csname val@case.shortgood.max_parallel\endcsname{3}
\expandafter\def\csname val@case.shortgood.parallel_ticks\endcsname{1}
\expandafter\def\csname val@case.shortgood.mutations_total\endcsname{14}
\expandafter\def\csname val@case.shortgood.distinct_incidents_cited\endcsname{2}
\expandafter\def\csname val@case.shortgood.top_incident_share\endcsname{0.93}
\expandafter\def\csname val@case.shortgood.confused_calls\endcsname{2}
\expandafter\def\csname val@case.shortgood.confused_last_tick\endcsname{22}
\expandafter\def\csname val@case.longgood.idle_bins\endcsname{6}
\expandafter\def\csname val@case.longgood.idle_minutes\endcsname{12}
\expandafter\def\csname val@case.longgood.batch_repairs\endcsname{5}
\expandafter\def\csname val@case.longgood.batch_minute\endcsname{70}
\expandafter\def\csname val@case.longgood.focal_inject_minute\endcsname{55}
\expandafter\def\csname val@case.longgood.turns_failed\endcsname{5}
\expandafter\def\csname val@case.longfail.mutations\endcsname{15}
\expandafter\def\csname val@case.longfail.mutations_ok\endcsname{15}
\expandafter\def\csname val@case.longfail.rca_claims\endcsname{84}
\expandafter\def\csname val@case.longfail.rca_ticks\endcsname{29}
\expandafter\def\csname val@case.longfail.incidents\endcsname{43}
\expandafter\def\csname val@case.longfail.exact\endcsname{5}
\expandafter\def\csname val@case.longfail.symptomatic\endcsname{25}
\expandafter\def\csname val@case.longfail.ticks_without_model\endcsname{89}
\expandafter\def\csname val@case.longfail.ticks\endcsname{142}
\expandafter\def\csname val@case.longfail.minutes\endcsname{282}
\expandafter\def\csname val@case.act_ok.service\endcsname{fraud-detection}
\expandafter\def\csname val@case.act_ok.family\endcsname{bad-image-tag}
\expandafter\def\csname val@case.act_ok.tool\endcsname{rollback}
\expandafter\def\csname val@case.act_ok.onset_min\endcsname{55}
\expandafter\def\csname val@case.act_ok.acted_min\endcsname{70}
\expandafter\def\csname val@case.act_ok.reaction_min\endcsname{13}
\expandafter\def\csname val@case.act_ok.concurrent\endcsname{9}
\expandafter\def\csname val@case.act_ok.credit\endcsname{0.6}
\expandafter\def\csname val@case.act_ok.greens_after\endcsname{2}
\expandafter\def\csname val@case.act_ok.reds_after\endcsname{2}
\expandafter\def\csname val@case.act_ok.revert_min\endcsname{82}
\expandafter\def\csname val@case.act_ok.first_bad_after_min\endcsname{71}
\expandafter\def\csname val@case.act_ok.first_bad_after_fix_min\endcsname{81}
\expandafter\def\csname val@case.act_ok.mitigated_min\endcsname{78}
\expandafter\def\csname val@case.act_no.service\endcsname{quote}
\expandafter\def\csname val@case.act_no.family\endcsname{bad-image-tag}
\expandafter\def\csname val@case.act_no.tool\endcsname{rollback}
\expandafter\def\csname val@case.act_no.onset_min\endcsname{24}
\expandafter\def\csname val@case.act_no.acted_min\endcsname{30}
\expandafter\def\csname val@case.act_no.reaction_min\endcsname{3}
\expandafter\def\csname val@case.act_no.concurrent\endcsname{4}
\expandafter\def\csname val@case.act_no.credit\endcsname{1.0}
\expandafter\def\csname val@case.act_no.greens_after\endcsname{2}
\expandafter\def\csname val@case.act_no.reds_after\endcsname{1}
\expandafter\def\csname val@case.act_no.revert_min\endcsname{37}
\expandafter\def\csname val@case.act_no.first_bad_after_min\endcsname{32}
\expandafter\def\csname val@case.act_no.first_bad_after_fix_min\endcsname{---}
\expandafter\def\csname val@case.act_no.mitigated_min\endcsname{---}
\expandafter\def\csname val@case.act_ok.injected\endcsname{58}
\expandafter\def\csname val@case.act_ok.onsets_in_window\endcsname{45}
\expandafter\def\csname val@case.act_ok.onset_lag_median\endcsname{17}
\expandafter\def\csname val@case.act_ok.last_onset_min\endcsname{105}
\expandafter\def\csname val@case.act_ok.traffic_ends_min\endcsname{47}
\expandafter\def\csname val@case.act_no.injected\endcsname{55}
\expandafter\def\csname val@case.act_no.onsets_in_window\endcsname{26}
\expandafter\def\csname val@case.act_no.onset_lag_median\endcsname{61}
\expandafter\def\csname val@case.act_no.last_onset_min\endcsname{245}
\expandafter\def\csname val@case.act_no.traffic_ends_min\endcsname{43}
\expandafter\def\csname val@case.astro.runs\endcsname{11}
\expandafter\def\csname val@case.astro.traffic_ends_lo\endcsname{42}
\expandafter\def\csname val@case.astro.traffic_ends_hi\endcsname{55}
\expandafter\def\csname val@case.ttreact.confabulation_calls\endcsname{2}
\expandafter\def\csname val@case.ttreact.first_confab_tick\endcsname{5}
\expandafter\def\csname val@case.long-good.concurrent\endcsname{5}
\expandafter\def\csname val@case.long-good-runnerup.concurrent\endcsname{9}
\expandafter\def\csname val@case.long-bad.concurrent\endcsname{8}
\expandafter\def\csname val@case.long-failure.concurrent\endcsname{4}
\expandafter\def\csname val@case.short-good.concurrent\endcsname{0}
\expandafter\def\csname val@case.short-bad.concurrent\endcsname{9}
\expandafter\def\csname val@inv.tick.OB.median_s\endcsname{126}
\expandafter\def\csname val@inv.tick.OB.max_s\endcsname{170}
\expandafter\def\csname val@inv.tick.TT.median_s\endcsname{160}
\expandafter\def\csname val@inv.tick.TT.max_s\endcsname{324}
\expandafter\def\csname val@inv.tick.Astro.median_s\endcsname{174}
\expandafter\def\csname val@inv.tick.Astro.max_s\endcsname{2302}
\expandafter\def\csname val@inv.stall.astro_r3_runs\endcsname{14}
\expandafter\def\csname val@inv.stall.astro_r3_runs_with_stall\endcsname{6}
\expandafter\def\csname val@inv.stall.upd16_timeouts\endcsname{5}
\expandafter\def\csname val@inv.stall.upd03_failures\endcsname{5}
\expandafter\def\csname val@inv.runs.long.minutes_min\endcsname{94}
\expandafter\def\csname val@inv.runs.long.minutes_max\endcsname{282}
\expandafter\def\csname val@inv.runs.short.minutes_min\endcsname{20}
\expandafter\def\csname val@inv.runs.short.minutes_max\endcsname{54}
\expandafter\def\csname val@inv.rollback.onto_faulted_history\endcsname{394}
\expandafter\def\csname val@inv.rollback.fault_returned\endcsname{114}
\expandafter\def\csname val@inv.inject.failed_total_headline\endcsname{25}
\expandafter\def\csname val@inv.inject.tt_b1\endcsname{5}
\expandafter\def\csname val@inv.inject.astro_r1_null\endcsname{13}
\expandafter\def\csname val@inv.inject.astro_r1_agents\endcsname{7}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-null\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-react-b2\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-rag-b2r\endcsname{1}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-orbit-0\endcsname{14}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-b1-runbook\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-tt-seed7-null\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-tt-seed7-b1-runbook\endcsname{30}
\expandafter\def\csname val@inv.killed.storm-tt-seed7-react-b2\endcsname{4}
\expandafter\def\csname val@inv.killed.storm-tt-seed7-rag-b2r\endcsname{9}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-a7f8dbb813b2-b1-runbook-null\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-a7f8dbb813b2-b1-runbook\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-9e90617a6a78-react-b2\endcsname{5}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-be1411a5e060-rag-b2r\endcsname{26}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-a8ee899d864d-orbit-0\endcsname{17}
\expandafter\def\csname val@inv.killed.storm-ob-seed7-r3-opensre-x3\endcsname{0}
\expandafter\def\csname val@inv.killed.storm-astro-seed7-r3-opensre\endcsname{9}
\expandafter\def\csname val@inv.killed.astro-episode1\endcsname{1}
\expandafter\def\csname val@inv.killed.astro-episode2\endcsname{1}
\expandafter\def\csname val@inv.killed.ob-episode1\endcsname{1}
\expandafter\def\csname val@inv.killed.ob-episode2\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode1\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode2\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode3\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode4\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode3\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode4\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode1-null\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode2-null\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode1-null\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode2-null\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode3-null\endcsname{0}
\expandafter\def\csname val@inv.killed.ob-episode4-null\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode1-null\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode2-null\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode3-null\endcsname{0}
\expandafter\def\csname val@inv.killed.tt-episode4-null\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode3\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode4\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode3-null\endcsname{0}
\expandafter\def\csname val@inv.killed.astro-episode4-null\endcsname{0}
\expandafter\def\csname val@inv.timeout.astro_r3_rag_topology\endcsname{11}
\expandafter\def\csname val@inv.probe.error_share_pct\endcsname{16}
\expandafter\def\csname val@inv.probe.occ_error_never_red\endcsname{124}
\expandafter\def\csname val@inv.probe.occ_all_error\endcsname{69}
\expandafter\def\csname val@inv.tool.crossapp_refusals\endcsname{19}
\expandafter\def\csname val@inv.tool.restart_pod_name\endcsname{55}
\expandafter\def\csname val@inv.tool.logs_multi_pod\endcsname{170}
\expandafter\def\csname val@inv.tool.logs_wrong_deployment\endcsname{74}
\expandafter\def\csname val@inv.tool.logql_syntax\endcsname{115}
\expandafter\def\csname val@inv.tool.invented_path\endcsname{103}
\expandafter\def\csname val@inv.tool.stale_pod\endcsname{826}
\expandafter\def\csname val@inv.alerts.total\endcsname{10211}
\expandafter\def\csname val@inv.alerts.resolved\endcsname{0}
\expandafter\def\csname val@inv.claims.max_per_tick\endcsname{194}
\expandafter\def\csname val@inv.claims.budget\endcsname{200}
\expandafter\def\csname val@inv.claims.budget_denials\endcsname{0}
\expandafter\def\csname val@inv.orbit.astro_rca\endcsname{1939}
\expandafter\def\csname val@inv.orbit.astro_rca_empty_services\endcsname{1939}
\expandafter\def\csname val@inv.null.pairs\endcsname{12}
\expandafter\def\csname val@inv.null.pairs_fault_mismatch\endcsname{1}
\expandafter\def\csname val@inv.null.horizon_ratio_max\endcsname{1.64}
\expandafter\def\csname val@inv.null.horizon_ratio_max_run\endcsname{ob-episode4}
\expandafter\def\csname val@inv.null.pairs_horizon_over_1p25\endcsname{1}
\expandafter\def\csname val@inv.tool.short_flagd_refusals\endcsname{7}
\expandafter\def\csname val@inv.tool.short_patch_scope_refusals\endcsname{6}
\expandafter\def\csname val@inv.claims.short_max_status\endcsname{778}
\expandafter\def\csname val@inv.score.regret_clamped_runs\endcsname{8}
\expandafter\def\csname val@inv.score.uncertified_short\endcsname{84}
\makeatother


==> results/macros_cases.tex <==
% Generated by 13_case_facts.py. Use \val{key}; never type a result by hand.
\makeatletter
\expandafter\def\csname val@case.act_no.acted_min\endcsname{48}
\expandafter\def\csname val@case.act_no.actions_in_run\endcsname{8}
\expandafter\def\csname val@case.act_no.app\endcsname{Astronomy Shop}
\expandafter\def\csname val@case.act_no.calls_before_rollback\endcsname{3}
\expandafter\def\csname val@case.act_no.concurrent\endcsname{5}
\expandafter\def\csname val@case.act_no.credit\endcsname{0.6}
\expandafter\def\csname val@case.act_no.family\endcsname{bad-image-tag}
\expandafter\def\csname val@case.act_no.first_bad_after_fix_min\endcsname{---}
\expandafter\def\csname val@case.act_no.first_bad_after_min\endcsname{49}
\expandafter\def\csname val@case.act_no.greens_after\endcsname{0}
\expandafter\def\csname val@case.act_no.injected\endcsname{58}
\expandafter\def\csname val@case.act_no.last_onset_min\endcsname{121}
\expandafter\def\csname val@case.act_no.last_probe\endcsname{red}
\expandafter\def\csname val@case.act_no.mitigated_min\endcsname{---}
\expandafter\def\csname val@case.act_no.onset_lag_median\endcsname{22}
\expandafter\def\csname val@case.act_no.onset_min\endcsname{35}
\expandafter\def\csname val@case.act_no.onsets_in_window\endcsname{40}
\expandafter\def\csname val@case.act_no.reaction_min\endcsname{3}
\expandafter\def\csname val@case.act_no.reds_after\endcsname{3}
\expandafter\def\csname val@case.act_no.refused_before_rollback\endcsname{1}
\expandafter\def\csname val@case.act_no.repaired_min\endcsname{---}
\expandafter\def\csname val@case.act_no.revert_min\endcsname{54}
\expandafter\def\csname val@case.act_no.rollback_min\endcsname{52}
\expandafter\def\csname val@case.act_no.service\endcsname{recommendation}
\expandafter\def\csname val@case.act_no.stages\endcsname{none}
\expandafter\def\csname val@case.act_no.tool\endcsname{update_config}
\expandafter\def\csname val@case.act_no.tools_before_rollback\endcsname{submit_patch, update_config}
\expandafter\def\csname val@case.act_no.traffic_ends_min\endcsname{46}
\expandafter\def\csname val@case.act_ok.acted_min\endcsname{65}
\expandafter\def\csname val@case.act_ok.actions_in_run\endcsname{36}
\expandafter\def\csname val@case.act_ok.app\endcsname{Online Boutique}
\expandafter\def\csname val@case.act_ok.calls_before_rollback\endcsname{0}
\expandafter\def\csname val@case.act_ok.concurrent\endcsname{4}
\expandafter\def\csname val@case.act_ok.credit\endcsname{1.0}
\expandafter\def\csname val@case.act_ok.family\endcsname{bad-image-tag}
\expandafter\def\csname val@case.act_ok.first_bad_after_fix_min\endcsname{---}
\expandafter\def\csname val@case.act_ok.first_bad_after_min\endcsname{66}
\expandafter\def\csname val@case.act_ok.greens_after\endcsname{3}
\expandafter\def\csname val@case.act_ok.injected\endcsname{58}
\expandafter\def\csname val@case.act_ok.last_onset_min\endcsname{105}
\expandafter\def\csname val@case.act_ok.last_probe\endcsname{green}
\expandafter\def\csname val@case.act_ok.mitigated_min\endcsname{70}
\expandafter\def\csname val@case.act_ok.onset_lag_median\endcsname{17}
\expandafter\def\csname val@case.act_ok.onset_min\endcsname{62}
\expandafter\def\csname val@case.act_ok.onsets_in_window\endcsname{45}
\expandafter\def\csname val@case.act_ok.reaction_min\endcsname{2}
\expandafter\def\csname val@case.act_ok.reds_after\endcsname{1}
\expandafter\def\csname val@case.act_ok.refused_before_rollback\endcsname{0}
\expandafter\def\csname val@case.act_ok.repaired_min\endcsname{70}
\expandafter\def\csname val@case.act_ok.revert_min\endcsname{72}
\expandafter\def\csname val@case.act_ok.rollback_min\endcsname{65}
\expandafter\def\csname val@case.act_ok.service\endcsname{checkoutservice}
\expandafter\def\csname val@case.act_ok.stages\endcsname{correlated, located, repaired}
\expandafter\def\csname val@case.act_ok.tool\endcsname{rollback}
\expandafter\def\csname val@case.act_ok.tools_before_rollback\endcsname{---}
\expandafter\def\csname val@case.act_ok.traffic_ends_min\endcsname{47}
\expandafter\def\csname val@case.astro.runs\endcsname{14}
\expandafter\def\csname val@case.astro.traffic_ends_hi\endcsname{55}
\expandafter\def\csname val@case.astro.traffic_ends_lo\endcsname{42}
\expandafter\def\csname val@case.long-bad.concurrent\endcsname{8}
\expandafter\def\csname val@case.long-failure.concurrent\endcsname{5}
\expandafter\def\csname val@case.long-good-runnerup.concurrent\endcsname{9}
\expandafter\def\csname val@case.long-good.concurrent\endcsname{5}
\expandafter\def\csname val@case.long-handled.concurrent\endcsname{4}
\expandafter\def\csname val@case.longbad.all_rollbacks\endcsname{63}
\expandafter\def\csname val@case.longbad.new_incidents_after_revert\endcsname{5}
\expandafter\def\csname val@case.longbad.null_uim_after_60\endcsname{1329}
\expandafter\def\csname val@case.longbad.revert_min\endcsname{70}
\expandafter\def\csname val@case.longbad.rollbacks_after_revert\endcsname{10}
\expandafter\def\csname val@case.longbad.rollbacks_total\endcsname{10}
\expandafter\def\csname val@case.longbad.uim_after_60\endcsname{4356}
\expandafter\def\csname val@case.longfail.exact\endcsname{0}
\expandafter\def\csname val@case.longfail.incidents\endcsname{23}
\expandafter\def\csname val@case.longfail.minutes\endcsname{162}
\expandafter\def\csname val@case.longfail.mutations\endcsname{11}
\expandafter\def\csname val@case.longfail.mutations_ok\endcsname{8}
\expandafter\def\csname val@case.longfail.rca_claims\endcsname{124}
\expandafter\def\csname val@case.longfail.rca_ticks\endcsname{14}
\expandafter\def\csname val@case.longfail.symptomatic\endcsname{22}
\expandafter\def\csname val@case.longfail.ticks\endcsname{82}
\expandafter\def\csname val@case.longfail.ticks_without_model\endcsname{30}
\expandafter\def\csname val@case.longgood.batch_minute\endcsname{70}
\expandafter\def\csname val@case.longgood.batch_repairs\endcsname{5}
\expandafter\def\csname val@case.longgood.focal_inject_minute\endcsname{55}
\expandafter\def\csname val@case.longgood.idle_bins\endcsname{6}
\expandafter\def\csname val@case.longgood.idle_minutes\endcsname{12}
\expandafter\def\csname val@case.longgood.turns_failed\endcsname{5}
\expandafter\def\csname val@case.short-bad.concurrent\endcsname{9}
\expandafter\def\csname val@case.short-good.concurrent\endcsname{0}
\expandafter\def\csname val@case.shortbad.flag_refusals\endcsname{1}
\expandafter\def\csname val@case.shortbad.focal_attempts\endcsname{4}
\expandafter\def\csname val@case.shortbad.focal_attempts_ok\endcsname{4}
\expandafter\def\csname val@case.shortbad.focal_bad_probe_ticks\endcsname{20}
\expandafter\def\csname val@case.shortbad.focal_probe_ticks\endcsname{20}
\expandafter\def\csname val@case.shortbad.focal_tools\endcsname{restart_pod, rollback, update_config}
\expandafter\def\csname val@case.shortbad.incidents\endcsname{14}
\expandafter\def\csname val@case.shortbad.mutations_total\endcsname{15}
\expandafter\def\csname val@case.shortbad.patch_refusals\endcsname{2}
\expandafter\def\csname val@case.shortbad.refused_calls\endcsname{98}
\expandafter\def\csname val@case.shortbad.status_claims\endcsname{147}
\expandafter\def\csname val@case.shortbad.status_open\endcsname{132}
\expandafter\def\csname val@case.shortgood.confused_calls\endcsname{2}
\expandafter\def\csname val@case.shortgood.confused_last_tick\endcsname{22}
\expandafter\def\csname val@case.shortgood.distinct_incidents_cited\endcsname{2}
\expandafter\def\csname val@case.shortgood.first_repair_s\endcsname{133}
\expandafter\def\csname val@case.shortgood.max_parallel\endcsname{3}
\expandafter\def\csname val@case.shortgood.mutations_total\endcsname{14}
\expandafter\def\csname val@case.shortgood.parallel_ticks\endcsname{1}
\expandafter\def\csname val@case.shortgood.top_incident_share\endcsname{0.93}
\expandafter\def\csname val@case.ttreact.confabulation_calls\endcsname{2}
\expandafter\def\csname val@case.ttreact.first_confab_tick\endcsname{5}
\makeatother


==> results/macros_lists.tex <==
% Generated by 20_paper_lists.py from the repo's libraries, tool roster and rule pack. Input after macros.tex.
\makeatletter
\expandafter\def\csname val@tax.code-bug.Astro\endcsname{160}
\expandafter\def\csname val@tax.code-bug.OB\endcsname{32}
\expandafter\def\csname val@tax.code-bug.TT\endcsname{32}
\expandafter\def\csname val@tax.code-bug.total\endcsname{224}
\expandafter\def\csname val@tax.code-bug.share\endcsname{27.0}
\expandafter\def\csname val@tax.code-bug.apps\endcsname{3}
\expandafter\def\csname val@tax.dependency.Astro\endcsname{20}
\expandafter\def\csname val@tax.dependency.OB\endcsname{22}
\expandafter\def\csname val@tax.dependency.TT\endcsname{23}
\expandafter\def\csname val@tax.dependency.total\endcsname{65}
\expandafter\def\csname val@tax.dependency.share\endcsname{16.4}
\expandafter\def\csname val@tax.dependency.apps\endcsname{3}
\expandafter\def\csname val@tax.infrastructure.Astro\endcsname{9}
\expandafter\def\csname val@tax.infrastructure.OB\endcsname{1}
\expandafter\def\csname val@tax.infrastructure.TT\endcsname{3}
\expandafter\def\csname val@tax.infrastructure.total\endcsname{13}
\expandafter\def\csname val@tax.infrastructure.share\endcsname{15.8}
\expandafter\def\csname val@tax.infrastructure.apps\endcsname{3}
\expandafter\def\csname val@tax.deployment.Astro\endcsname{67}
\expandafter\def\csname val@tax.deployment.OB\endcsname{32}
\expandafter\def\csname val@tax.deployment.TT\endcsname{44}
\expandafter\def\csname val@tax.deployment.total\endcsname{143}
\expandafter\def\csname val@tax.deployment.share\endcsname{13.2}
\expandafter\def\csname val@tax.deployment.apps\endcsname{3}
\expandafter\def\csname val@tax.configuration.Astro\endcsname{35}
\expandafter\def\csname val@tax.configuration.OB\endcsname{75}
\expandafter\def\csname val@tax.configuration.TT\endcsname{93}
\expandafter\def\csname val@tax.configuration.total\endcsname{203}
\expandafter\def\csname val@tax.configuration.share\endcsname{12.5}
\expandafter\def\csname val@tax.configuration.apps\endcsname{3}
\expandafter\def\csname val@tax.db-network.Astro\endcsname{10}
\expandafter\def\csname val@tax.db-network.OB\endcsname{0}
\expandafter\def\csname val@tax.db-network.TT\endcsname{0}
\expandafter\def\csname val@tax.db-network.total\endcsname{10}
\expandafter\def\csname val@tax.db-network.share\endcsname{10.5}
\expandafter\def\csname val@tax.db-network.apps\endcsname{1}
\expandafter\def\csname val@tax.auth.Astro\endcsname{16}
\expandafter\def\csname val@tax.auth.OB\endcsname{11}
\expandafter\def\csname val@tax.auth.TT\endcsname{15}
\expandafter\def\csname val@tax.auth.total\endcsname{42}
\expandafter\def\csname val@tax.auth.share\endcsname{4.6}
\expandafter\def\csname val@tax.auth.apps\endcsname{3}
\expandafter\def\csname val@tax.empty_cells\endcsname{2}
\expandafter\def\csname val@tax.empty_categories\endcsname{database / network}
\expandafter\def\csname val@tax.group.code.total\endcsname{224}
\expandafter\def\csname val@tax.group.code.Astro\endcsname{160}
\expandafter\def\csname val@tax.group.code.OB\endcsname{32}
\expandafter\def\csname val@tax.group.code.TT\endcsname{32}
\expandafter\def\csname val@tax.group.config.total\endcsname{203}
\expandafter\def\csname val@tax.group.config.Astro\endcsname{35}
\expandafter\def\csname val@tax.group.config.OB\endcsname{75}
\expandafter\def\csname val@tax.group.config.TT\endcsname{93}
\expandafter\def\csname val@tax.group.chaos.total\endcsname{273}
\expandafter\def\csname val@tax.group.chaos.Astro\endcsname{122}
\expandafter\def\csname val@tax.group.chaos.OB\endcsname{66}
\expandafter\def\csname val@tax.group.chaos.TT\endcsname{85}
\expandafter\def\csname val@tax.total\endcsname{700}
\expandafter\def\csname val@tax.total.Astro\endcsname{317}
\expandafter\def\csname val@tax.total.OB\endcsname{173}
\expandafter\def\csname val@tax.total.TT\endcsname{210}
\expandafter\def\csname val@tax.authored\endcsname{912}
\expandafter\def\csname val@tax.patch.total\endcsname{263}
\expandafter\def\csname val@tax.patch.Astro\endcsname{163}
\expandafter\def\csname val@tax.patch.OB\endcsname{50}
\expandafter\def\csname val@tax.patch.TT\endcsname{50}
\expandafter\def\csname val@tax.subtype.datatype-validation\endcsname{41}
\expandafter\def\csname val@tax.subtype.flags-and-constants\endcsname{17}
\expandafter\def\csname val@tax.subtype.code-dependency\endcsname{35}
\expandafter\def\csname val@tax.subtype.configuration-sync\endcsname{19}
\expandafter\def\csname val@tax.subtype.backward-compatibility\endcsname{61}
\expandafter\def\csname val@tax.subtype.code-change\endcsname{60}
\expandafter\def\csname val@tax.subtype.misconfiguration\endcsname{13}
\expandafter\def\csname val@tax.subtype.configuration-change\endcsname{17}
\expandafter\def\csname val@tax.release.OB.categories\endcsname{2}
\expandafter\def\csname val@tax.release.OB.patch\endcsname{0}
\expandafter\def\csname val@tax.release.TT.categories\endcsname{2}
\expandafter\def\csname val@tax.release.TT.patch\endcsname{0}
\expandafter\def\csname val@tax.release.Astro.categories\endcsname{6}
\expandafter\def\csname val@tax.release.Astro.patch\endcsname{25}
\expandafter\def\csname val@tax.admitted.adr0087\endcsname{27}
\expandafter\def\csname val@tax.admitted.adr0088\endcsname{81}
\expandafter\def\csname val@tax.admitted.adr0089\endcsname{100}
\expandafter\def\csname val@tax.admitted.unswept\endcsname{208}
\expandafter\def\csname val@tax.admitted.astro\endcsname{108}
\expandafter\def\csname val@tax.families\endcsname{112}
\expandafter\def\csname val@tools.published\endcsname{19}
\expandafter\def\csname val@tools.read\endcsname{10}
\expandafter\def\csname val@tools.claim\endcsname{1}
\expandafter\def\csname val@tools.act\endcsname{1}
\expandafter\def\csname val@tools.guarded\endcsname{7}
\expandafter\def\csname val@tools.forbidden\endcsname{\texttt{read\_secret}, \texttt{delete\_namespace}, \texttt{edit\_benchmark\_rule}}
\expandafter\def\csname val@alerts.total\endcsname{44}
\expandafter\def\csname val@alerts.astro\endcsname{18}
\expandafter\def\csname val@alerts.ob\endcsname{13}
\expandafter\def\csname val@alerts.tt\endcsname{13}
\expandafter\def\csname val@alerts.templates\endcsname{18}
\expandafter\def\csname val@alerts.templates.shared\endcsname{13}
\expandafter\def\csname val@alerts.templates.astro_only\endcsname{5}
\makeatother


==> results/macros_marathon.tex <==
% Generated by 24_table2_latest.py. Use \val{key}; never type a result by hand.
\makeatletter
\expandafter\def\csname val@ms.17.b1-runbook.none.Astro.ci\endcsname{20.9--34.5}
\expandafter\def\csname val@ms.17.b1-runbook.none.Astro.count\endcsname{1/59}
\expandafter\def\csname val@ms.17.b1-runbook.none.Astro.score\endcsname{27.7}
\expandafter\def\csname val@ms.17.b1-runbook.none.OB.count\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.OB.score\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.TT.count\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.TT.score\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.actions\endcsname{41}
\expandafter\def\csname val@ms.17.b1-runbook.none.avoided\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.correlated\endcsname{0.610}
\expandafter\def\csname val@ms.17.b1-runbook.none.dollars\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.forbidden\endcsname{0}
\expandafter\def\csname val@ms.17.b1-runbook.none.level\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.located\endcsname{0.220}
\expandafter\def\csname val@ms.17.b1-runbook.none.out_of_scope\endcsname{1}
\expandafter\def\csname val@ms.17.b1-runbook.none.repaired\endcsname{0.051}
\expandafter\def\csname val@ms.17.b1-runbook.none.risk\endcsname{0.024}
\expandafter\def\csname val@ms.17.b1-runbook.none.score\endcsname{27.7}
\expandafter\def\csname val@ms.17.b1-runbook.none.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_detect\endcsname{209}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_detect.n\endcsname{36}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_locate\endcsname{339}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_locate.n\endcsname{13}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_repair\endcsname{903}
\expandafter\def\csname val@ms.17.b1-runbook.none.time_to_repair.n\endcsname{3}
\expandafter\def\csname val@ms.17.b1-runbook.none.tokens\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.Astro.ci\endcsname{19.2--27.1}
\expandafter\def\csname val@ms.17.orbit-0.kimi.Astro.count\endcsname{0/59}
\expandafter\def\csname val@ms.17.orbit-0.kimi.Astro.score\endcsname{23.2}
\expandafter\def\csname val@ms.17.orbit-0.kimi.OB.count\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.OB.score\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.actions\endcsname{0}
\expandafter\def\csname val@ms.17.orbit-0.kimi.avoided\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.correlated\endcsname{0.695}
\expandafter\def\csname val@ms.17.orbit-0.kimi.dollars\endcsname{2.10}
\expandafter\def\csname val@ms.17.orbit-0.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.17.orbit-0.kimi.level\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.located\endcsname{0.000}
\expandafter\def\csname val@ms.17.orbit-0.kimi.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.17.orbit-0.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.17.orbit-0.kimi.risk\endcsname{0.000}
\expandafter\def\csname val@ms.17.orbit-0.kimi.score\endcsname{23.2}
\expandafter\def\csname val@ms.17.orbit-0.kimi.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_detect\endcsname{276}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_detect.n\endcsname{41}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_locate\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_locate.n\endcsname{0}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.17.orbit-0.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.17.orbit-0.kimi.tokens\endcsname{3.4M}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.Astro.ci\endcsname{10.2--20.9}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.Astro.count\endcsname{0/59}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.Astro.score\endcsname{15.3}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.OB.count\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.OB.score\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.actions\endcsname{27}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.avoided\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.correlated\endcsname{0.373}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.dollars\endcsname{0.24}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.level\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.located\endcsname{0.153}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.out_of_scope\endcsname{3}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.repaired\endcsname{0.017}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.risk\endcsname{0.111}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.score\endcsname{15.3}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_detect\endcsname{326}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_detect.n\endcsname{22}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_locate\endcsname{1085}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_locate.n\endcsname{9}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_repair\endcsname{1452}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.time_to_repair.n\endcsname{1}
\expandafter\def\csname val@ms.17.rag-b2r.kimi.tokens\endcsname{260k}
\expandafter\def\csname val@ms.17.react-b2.kimi.Astro.ci\endcsname{4.0--11.3}
\expandafter\def\csname val@ms.17.react-b2.kimi.Astro.count\endcsname{0/59}
\expandafter\def\csname val@ms.17.react-b2.kimi.Astro.score\endcsname{7.3}
\expandafter\def\csname val@ms.17.react-b2.kimi.OB.count\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.OB.score\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.actions\endcsname{27}
\expandafter\def\csname val@ms.17.react-b2.kimi.avoided\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.correlated\endcsname{0.203}
\expandafter\def\csname val@ms.17.react-b2.kimi.dollars\endcsname{3.09}
\expandafter\def\csname val@ms.17.react-b2.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.17.react-b2.kimi.level\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.located\endcsname{0.034}
\expandafter\def\csname val@ms.17.react-b2.kimi.out_of_scope\endcsname{16}
\expandafter\def\csname val@ms.17.react-b2.kimi.repaired\endcsname{0.051}
\expandafter\def\csname val@ms.17.react-b2.kimi.risk\endcsname{0.593}
\expandafter\def\csname val@ms.17.react-b2.kimi.score\endcsname{7.3}
\expandafter\def\csname val@ms.17.react-b2.kimi.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_detect\endcsname{202}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_detect.n\endcsname{12}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_locate\endcsname{625}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_locate.n\endcsname{2}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_repair\endcsname{593}
\expandafter\def\csname val@ms.17.react-b2.kimi.time_to_repair.n\endcsname{3}
\expandafter\def\csname val@ms.17.react-b2.kimi.tokens\endcsname{5.0M}
\expandafter\def\csname val@ms.27.b1-runbook.none.Astro.ci\endcsname{24.8--38.8}
\expandafter\def\csname val@ms.27.b1-runbook.none.Astro.count\endcsname{1/55}
\expandafter\def\csname val@ms.27.b1-runbook.none.Astro.score\endcsname{31.5}
\expandafter\def\csname val@ms.27.b1-runbook.none.OB.count\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.OB.score\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.TT.count\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.TT.score\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.actions\endcsname{46}
\expandafter\def\csname val@ms.27.b1-runbook.none.avoided\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.correlated\endcsname{0.673}
\expandafter\def\csname val@ms.27.b1-runbook.none.dollars\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.forbidden\endcsname{0}
\expandafter\def\csname val@ms.27.b1-runbook.none.level\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.located\endcsname{0.273}
\expandafter\def\csname val@ms.27.b1-runbook.none.out_of_scope\endcsname{7}
\expandafter\def\csname val@ms.27.b1-runbook.none.repaired\endcsname{0.055}
\expandafter\def\csname val@ms.27.b1-runbook.none.risk\endcsname{0.152}
\expandafter\def\csname val@ms.27.b1-runbook.none.score\endcsname{31.5}
\expandafter\def\csname val@ms.27.b1-runbook.none.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_detect\endcsname{284}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_detect.n\endcsname{37}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_locate\endcsname{384}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_locate.n\endcsname{15}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_repair\endcsname{1190}
\expandafter\def\csname val@ms.27.b1-runbook.none.time_to_repair.n\endcsname{3}
\expandafter\def\csname val@ms.27.b1-runbook.none.tokens\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.Astro.ci\endcsname{8.5--21.8}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.Astro.count\endcsname{1/55}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.Astro.score\endcsname{14.5}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.OB.count\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.OB.score\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.actions\endcsname{94}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.avoided\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.correlated\endcsname{0.291}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.dollars\endcsname{0.39}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.level\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.located\endcsname{0.436}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.out_of_scope\endcsname{16}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.repaired\endcsname{0.018}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.risk\endcsname{0.170}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.score\endcsname{14.5}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_detect\endcsname{299}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_detect.n\endcsname{16}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_locate\endcsname{110}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_locate.n\endcsname{24}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_repair\endcsname{1017}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.time_to_repair.n\endcsname{1}
\expandafter\def\csname val@ms.27.rag-b2r.kimi.tokens\endcsname{462k}
\expandafter\def\csname val@ms.27.react-b2.kimi.Astro.ci\endcsname{12.1--22.4}
\expandafter\def\csname val@ms.27.react-b2.kimi.Astro.count\endcsname{0/55}
\expandafter\def\csname val@ms.27.react-b2.kimi.Astro.score\endcsname{17.0}
\expandafter\def\csname val@ms.27.react-b2.kimi.OB.count\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.OB.score\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.actions\endcsname{16}
\expandafter\def\csname val@ms.27.react-b2.kimi.avoided\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.correlated\endcsname{0.455}
\expandafter\def\csname val@ms.27.react-b2.kimi.dollars\endcsname{3.56}
\expandafter\def\csname val@ms.27.react-b2.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.27.react-b2.kimi.level\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.located\endcsname{0.073}
\expandafter\def\csname val@ms.27.react-b2.kimi.out_of_scope\endcsname{4}
\expandafter\def\csname val@ms.27.react-b2.kimi.repaired\endcsname{0.018}
\expandafter\def\csname val@ms.27.react-b2.kimi.risk\endcsname{0.250}
\expandafter\def\csname val@ms.27.react-b2.kimi.score\endcsname{17.0}
\expandafter\def\csname val@ms.27.react-b2.kimi.smash_ob_tt\endcsname{---}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_detect\endcsname{208}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_detect.n\endcsname{25}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_locate\endcsname{324}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_locate.n\endcsname{4}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_repair\endcsname{2486}
\expandafter\def\csname val@ms.27.react-b2.kimi.time_to_repair.n\endcsname{1}
\expandafter\def\csname val@ms.27.react-b2.kimi.tokens\endcsname{5.7M}
\expandafter\def\csname val@ms.7.b1-runbook.none.Astro.ci\endcsname{21.3--34.5}
\expandafter\def\csname val@ms.7.b1-runbook.none.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.b1-runbook.none.Astro.score\endcsname{27.6}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.avoided\endcsname{+0.016}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.ci\endcsname{51.4--62.1}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.level\endcsname{98.4}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.load\endcsname{0.94}
\expandafter\def\csname val@ms.7.b1-runbook.none.OB.score\endcsname{57.1}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.avoided\endcsname{-0.236}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.ci\endcsname{10.9--20.6}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.count\endcsname{0/55}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.level\endcsname{123.6}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.load\endcsname{0.98}
\expandafter\def\csname val@ms.7.b1-runbook.none.TT.score\endcsname{15.8}
\expandafter\def\csname val@ms.7.b1-runbook.none.actions\endcsname{179}
\expandafter\def\csname val@ms.7.b1-runbook.none.avoided\endcsname{-0.110}
\expandafter\def\csname val@ms.7.b1-runbook.none.correlated\endcsname{0.658}
\expandafter\def\csname val@ms.7.b1-runbook.none.dollars\endcsname{---}
\expandafter\def\csname val@ms.7.b1-runbook.none.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.b1-runbook.none.level\endcsname{111.0}
\expandafter\def\csname val@ms.7.b1-runbook.none.located\endcsname{0.364}
\expandafter\def\csname val@ms.7.b1-runbook.none.out_of_scope\endcsname{5}
\expandafter\def\csname val@ms.7.b1-runbook.none.repaired\endcsname{0.024}
\expandafter\def\csname val@ms.7.b1-runbook.none.risk\endcsname{0.028}
\expandafter\def\csname val@ms.7.b1-runbook.none.score\endcsname{33.5}
\expandafter\def\csname val@ms.7.b1-runbook.none.smash_ob_tt\endcsname{2.70}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_detect\endcsname{167}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_detect.n\endcsname{114}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_locate\endcsname{267}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_locate.n\endcsname{64}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_repair\endcsname{560}
\expandafter\def\csname val@ms.7.b1-runbook.none.time_to_repair.n\endcsname{4}
\expandafter\def\csname val@ms.7.b1-runbook.none.tokens\endcsname{---}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.Astro.ci\endcsname{9.2--17.2}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.Astro.score\endcsname{13.2}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.avoided\endcsname{-0.020}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.ci\endcsname{12.4--20.9}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.level\endcsname{102.0}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.load\endcsname{1.04}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.OB.score\endcsname{16.4}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.avoided\endcsname{-0.042}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.ci\endcsname{5.6--15.6}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.level\endcsname{104.2}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.load\endcsname{1.03}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.TT.score\endcsname{10.6}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.actions\endcsname{22}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.avoided\endcsname{-0.031}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.correlated\endcsname{0.379}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.dollars\endcsname{4.14}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.level\endcsname{103.1}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.located\endcsname{0.050}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.score\endcsname{13.4}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.smash_ob_tt\endcsname{5.83}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_detect\endcsname{337}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_detect.n\endcsname{67}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_locate\endcsname{210}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_locate.n\endcsname{9}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.kimi.tokens\endcsname{6.7M}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.Astro.ci\endcsname{10.3--18.4}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.Astro.score\endcsname{14.4}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.avoided\endcsname{+0.193}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.ci\endcsname{14.1--24.3}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.level\endcsname{80.7}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.load\endcsname{0.80}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.OB.score\endcsname{19.2}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.TT.ci\endcsname{5.0--13.8}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.TT.count\endcsname{0/53}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.TT.score\endcsname{9.4}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.actions\endcsname{4}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.avoided\endcsname{0.193}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.correlated\endcsname{0.407}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.dollars\endcsname{0.84}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.level\endcsname{80.7}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.located\endcsname{0.070}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.score\endcsname{14.3}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.smash_ob_tt\endcsname{2.90}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_detect\endcsname{360}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_detect.n\endcsname{70}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_locate\endcsname{684}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_locate.n\endcsname{12}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.claudecode-x5.luna.tokens\endcsname{3.4M}
\expandafter\def\csname val@ms.7.coca.kimi.Astro.ci\endcsname{13.8--21.8}
\expandafter\def\csname val@ms.7.coca.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.coca.kimi.Astro.score\endcsname{17.8}
\expandafter\def\csname val@ms.7.coca.kimi.OB.avoided\endcsname{-0.422}
\expandafter\def\csname val@ms.7.coca.kimi.OB.ci\endcsname{15.8--23.7}
\expandafter\def\csname val@ms.7.coca.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.coca.kimi.OB.level\endcsname{142.2}
\expandafter\def\csname val@ms.7.coca.kimi.OB.load\endcsname{1.06}
\expandafter\def\csname val@ms.7.coca.kimi.OB.score\endcsname{19.8}
\expandafter\def\csname val@ms.7.coca.kimi.TT.avoided\endcsname{-0.224}
\expandafter\def\csname val@ms.7.coca.kimi.TT.ci\endcsname{16.7--25.6}
\expandafter\def\csname val@ms.7.coca.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.coca.kimi.TT.level\endcsname{122.4}
\expandafter\def\csname val@ms.7.coca.kimi.TT.load\endcsname{1.12}
\expandafter\def\csname val@ms.7.coca.kimi.TT.score\endcsname{21.1}
\expandafter\def\csname val@ms.7.coca.kimi.actions\endcsname{39}
\expandafter\def\csname val@ms.7.coca.kimi.avoided\endcsname{-0.323}
\expandafter\def\csname val@ms.7.coca.kimi.correlated\endcsname{0.576}
\expandafter\def\csname val@ms.7.coca.kimi.dollars\endcsname{0.36}
\expandafter\def\csname val@ms.7.coca.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.coca.kimi.level\endcsname{132.3}
\expandafter\def\csname val@ms.7.coca.kimi.located\endcsname{0.017}
\expandafter\def\csname val@ms.7.coca.kimi.out_of_scope\endcsname{2}
\expandafter\def\csname val@ms.7.coca.kimi.repaired\endcsname{0.023}
\expandafter\def\csname val@ms.7.coca.kimi.risk\endcsname{0.051}
\expandafter\def\csname val@ms.7.coca.kimi.score\endcsname{19.6}
\expandafter\def\csname val@ms.7.coca.kimi.smash_ob_tt\endcsname{-5.59}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_detect\endcsname{168}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_detect.n\endcsname{102}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_locate\endcsname{336}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_locate.n\endcsname{3}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_repair\endcsname{786}
\expandafter\def\csname val@ms.7.coca.kimi.time_to_repair.n\endcsname{4}
\expandafter\def\csname val@ms.7.coca.kimi.tokens\endcsname{511k}
\expandafter\def\csname val@ms.7.coca.luna.Astro.ci\endcsname{16.7--31.0}
\expandafter\def\csname val@ms.7.coca.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.coca.luna.Astro.score\endcsname{23.6}
\expandafter\def\csname val@ms.7.coca.luna.OB.avoided\endcsname{+0.124}
\expandafter\def\csname val@ms.7.coca.luna.OB.ci\endcsname{27.0--40.8}
\expandafter\def\csname val@ms.7.coca.luna.OB.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.coca.luna.OB.level\endcsname{87.6}
\expandafter\def\csname val@ms.7.coca.luna.OB.load\endcsname{0.87}
\expandafter\def\csname val@ms.7.coca.luna.OB.score\endcsname{33.9}
\expandafter\def\csname val@ms.7.coca.luna.TT.ci\endcsname{22.4--30.3}
\expandafter\def\csname val@ms.7.coca.luna.TT.count\endcsname{0/55}
\expandafter\def\csname val@ms.7.coca.luna.TT.score\endcsname{26.7}
\expandafter\def\csname val@ms.7.coca.luna.actions\endcsname{29}
\expandafter\def\csname val@ms.7.coca.luna.avoided\endcsname{0.124}
\expandafter\def\csname val@ms.7.coca.luna.correlated\endcsname{0.634}
\expandafter\def\csname val@ms.7.coca.luna.dollars\endcsname{0.09}
\expandafter\def\csname val@ms.7.coca.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.coca.luna.level\endcsname{87.6}
\expandafter\def\csname val@ms.7.coca.luna.located\endcsname{0.253}
\expandafter\def\csname val@ms.7.coca.luna.out_of_scope\endcsname{3}
\expandafter\def\csname val@ms.7.coca.luna.repaired\endcsname{0.011}
\expandafter\def\csname val@ms.7.coca.luna.risk\endcsname{0.103}
\expandafter\def\csname val@ms.7.coca.luna.score\endcsname{28.0}
\expandafter\def\csname val@ms.7.coca.luna.smash_ob_tt\endcsname{12.11}
\expandafter\def\csname val@ms.7.coca.luna.time_to_detect\endcsname{161}
\expandafter\def\csname val@ms.7.coca.luna.time_to_detect.n\endcsname{108}
\expandafter\def\csname val@ms.7.coca.luna.time_to_locate\endcsname{222}
\expandafter\def\csname val@ms.7.coca.luna.time_to_locate.n\endcsname{44}
\expandafter\def\csname val@ms.7.coca.luna.time_to_repair\endcsname{461}
\expandafter\def\csname val@ms.7.coca.luna.time_to_repair.n\endcsname{2}
\expandafter\def\csname val@ms.7.coca.luna.tokens\endcsname{403k}
\expandafter\def\csname val@ms.7.codex-x4.kimi.Astro.ci\endcsname{2.3--8.6}
\expandafter\def\csname val@ms.7.codex-x4.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.codex-x4.kimi.Astro.score\endcsname{5.2}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.avoided\endcsname{-0.570}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.ci\endcsname{6.2--15.8}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.level\endcsname{157.0}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.load\endcsname{0.98}
\expandafter\def\csname val@ms.7.codex-x4.kimi.OB.score\endcsname{10.7}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.avoided\endcsname{-0.065}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.ci\endcsname{5.0--12.2}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.level\endcsname{106.5}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.load\endcsname{1.03}
\expandafter\def\csname val@ms.7.codex-x4.kimi.TT.score\endcsname{8.3}
\expandafter\def\csname val@ms.7.codex-x4.kimi.actions\endcsname{41}
\expandafter\def\csname val@ms.7.codex-x4.kimi.avoided\endcsname{-0.317}
\expandafter\def\csname val@ms.7.codex-x4.kimi.correlated\endcsname{0.231}
\expandafter\def\csname val@ms.7.codex-x4.kimi.dollars\endcsname{4.45}
\expandafter\def\csname val@ms.7.codex-x4.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.codex-x4.kimi.level\endcsname{131.7}
\expandafter\def\csname val@ms.7.codex-x4.kimi.located\endcsname{0.039}
\expandafter\def\csname val@ms.7.codex-x4.kimi.out_of_scope\endcsname{7}
\expandafter\def\csname val@ms.7.codex-x4.kimi.repaired\endcsname{0.011}
\expandafter\def\csname val@ms.7.codex-x4.kimi.risk\endcsname{0.171}
\expandafter\def\csname val@ms.7.codex-x4.kimi.score\endcsname{8.1}
\expandafter\def\csname val@ms.7.codex-x4.kimi.smash_ob_tt\endcsname{-6.57}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_detect\endcsname{210}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_detect.n\endcsname{41}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_locate\endcsname{335}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_locate.n\endcsname{7}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_repair\endcsname{456}
\expandafter\def\csname val@ms.7.codex-x4.kimi.time_to_repair.n\endcsname{2}
\expandafter\def\csname val@ms.7.codex-x4.kimi.tokens\endcsname{7.2M}
\expandafter\def\csname val@ms.7.codex-x4.luna.Astro.ci\endcsname{17.2--31.0}
\expandafter\def\csname val@ms.7.codex-x4.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.codex-x4.luna.Astro.score\endcsname{24.1}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.avoided\endcsname{+0.144}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.ci\endcsname{21.3--30.5}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.level\endcsname{85.6}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.load\endcsname{0.87}
\expandafter\def\csname val@ms.7.codex-x4.luna.OB.score\endcsname{25.9}
\expandafter\def\csname val@ms.7.codex-x4.luna.TT.ci\endcsname{7.0--15.8}
\expandafter\def\csname val@ms.7.codex-x4.luna.TT.count\endcsname{0/57}
\expandafter\def\csname val@ms.7.codex-x4.luna.TT.score\endcsname{11.1}
\expandafter\def\csname val@ms.7.codex-x4.luna.actions\endcsname{67}
\expandafter\def\csname val@ms.7.codex-x4.luna.avoided\endcsname{0.144}
\expandafter\def\csname val@ms.7.codex-x4.luna.correlated\endcsname{0.502}
\expandafter\def\csname val@ms.7.codex-x4.luna.dollars\endcsname{1.81}
\expandafter\def\csname val@ms.7.codex-x4.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.codex-x4.luna.level\endcsname{85.6}
\expandafter\def\csname val@ms.7.codex-x4.luna.located\endcsname{0.138}
\expandafter\def\csname val@ms.7.codex-x4.luna.out_of_scope\endcsname{7}
\expandafter\def\csname val@ms.7.codex-x4.luna.repaired\endcsname{0.023}
\expandafter\def\csname val@ms.7.codex-x4.luna.risk\endcsname{0.104}
\expandafter\def\csname val@ms.7.codex-x4.luna.score\endcsname{20.4}
\expandafter\def\csname val@ms.7.codex-x4.luna.smash_ob_tt\endcsname{18.71}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_detect\endcsname{203}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_detect.n\endcsname{87}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_locate\endcsname{346}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_locate.n\endcsname{24}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_repair\endcsname{411}
\expandafter\def\csname val@ms.7.codex-x4.luna.time_to_repair.n\endcsname{4}
\expandafter\def\csname val@ms.7.codex-x4.luna.tokens\endcsname{8.0M}
\expandafter\def\csname val@ms.7.keep-llm.kimi.Astro.ci\endcsname{16.7--25.9}
\expandafter\def\csname val@ms.7.keep-llm.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.keep-llm.kimi.Astro.score\endcsname{21.3}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.avoided\endcsname{+0.079}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.ci\endcsname{56.1--65.5}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.count\endcsname{1/57}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.level\endcsname{92.1}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.load\endcsname{1.06}
\expandafter\def\csname val@ms.7.keep-llm.kimi.OB.score\endcsname{61.4}
\expandafter\def\csname val@ms.7.keep-llm.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.keep-llm.kimi.TT.score\endcsname{0.0}
\expandafter\def\csname val@ms.7.keep-llm.kimi.actions\endcsname{69}
\expandafter\def\csname val@ms.7.keep-llm.kimi.avoided\endcsname{0.079}
\expandafter\def\csname val@ms.7.keep-llm.kimi.correlated\endcsname{0.775}
\expandafter\def\csname val@ms.7.keep-llm.kimi.dollars\endcsname{0.72}
\expandafter\def\csname val@ms.7.keep-llm.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.keep-llm.kimi.level\endcsname{92.1}
\expandafter\def\csname val@ms.7.keep-llm.kimi.located\endcsname{0.491}
\expandafter\def\csname val@ms.7.keep-llm.kimi.out_of_scope\endcsname{1}
\expandafter\def\csname val@ms.7.keep-llm.kimi.repaired\endcsname{0.017}
\expandafter\def\csname val@ms.7.keep-llm.kimi.risk\endcsname{0.014}
\expandafter\def\csname val@ms.7.keep-llm.kimi.score\endcsname{41.3}
\expandafter\def\csname val@ms.7.keep-llm.kimi.smash_ob_tt\endcsname{13.80}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_detect\endcsname{188}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_detect.n\endcsname{89}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_locate\endcsname{165}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_locate.n\endcsname{56}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_repair\endcsname{476}
\expandafter\def\csname val@ms.7.keep-llm.kimi.time_to_repair.n\endcsname{2}
\expandafter\def\csname val@ms.7.keep-llm.kimi.tokens\endcsname{685k}
\expandafter\def\csname val@ms.7.keep-llm.luna.Astro.ci\endcsname{2.9--11.5}
\expandafter\def\csname val@ms.7.keep-llm.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.keep-llm.luna.Astro.score\endcsname{6.9}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.avoided\endcsname{+0.155}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.ci\endcsname{42.4--56.5}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.count\endcsname{2/59}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.level\endcsname{84.5}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.load\endcsname{0.84}
\expandafter\def\csname val@ms.7.keep-llm.luna.OB.score\endcsname{49.7}
\expandafter\def\csname val@ms.7.keep-llm.luna.TT.ci\endcsname{34.5--40.9}
\expandafter\def\csname val@ms.7.keep-llm.luna.TT.count\endcsname{0/57}
\expandafter\def\csname val@ms.7.keep-llm.luna.TT.score\endcsname{37.4}
\expandafter\def\csname val@ms.7.keep-llm.luna.actions\endcsname{59}
\expandafter\def\csname val@ms.7.keep-llm.luna.avoided\endcsname{0.155}
\expandafter\def\csname val@ms.7.keep-llm.luna.correlated\endcsname{0.656}
\expandafter\def\csname val@ms.7.keep-llm.luna.dollars\endcsname{0.31}
\expandafter\def\csname val@ms.7.keep-llm.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.keep-llm.luna.level\endcsname{84.5}
\expandafter\def\csname val@ms.7.keep-llm.luna.located\endcsname{0.313}
\expandafter\def\csname val@ms.7.keep-llm.luna.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.keep-llm.luna.repaired\endcsname{0.017}
\expandafter\def\csname val@ms.7.keep-llm.luna.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.keep-llm.luna.score\endcsname{31.3}
\expandafter\def\csname val@ms.7.keep-llm.luna.smash_ob_tt\endcsname{14.42}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_detect\endcsname{184}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_detect.n\endcsname{114}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_locate\endcsname{142}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_locate.n\endcsname{55}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_repair\endcsname{455}
\expandafter\def\csname val@ms.7.keep-llm.luna.time_to_repair.n\endcsname{3}
\expandafter\def\csname val@ms.7.keep-llm.luna.tokens\endcsname{742k}
\expandafter\def\csname val@ms.7.keep-rules.none.Astro.ci\endcsname{14.9--27.6}
\expandafter\def\csname val@ms.7.keep-rules.none.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.keep-rules.none.Astro.score\endcsname{21.3}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.avoided\endcsname{-0.761}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.ci\endcsname{52.3--60.3}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.level\endcsname{176.1}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.load\endcsname{1.04}
\expandafter\def\csname val@ms.7.keep-rules.none.OB.score\endcsname{56.3}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.avoided\endcsname{-0.025}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.ci\endcsname{2.3--11.9}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.level\endcsname{102.5}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.load\endcsname{1.00}
\expandafter\def\csname val@ms.7.keep-rules.none.TT.score\endcsname{6.8}
\expandafter\def\csname val@ms.7.keep-rules.none.actions\endcsname{224}
\expandafter\def\csname val@ms.7.keep-rules.none.avoided\endcsname{-0.393}
\expandafter\def\csname val@ms.7.keep-rules.none.correlated\endcsname{0.534}
\expandafter\def\csname val@ms.7.keep-rules.none.dollars\endcsname{---}
\expandafter\def\csname val@ms.7.keep-rules.none.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.keep-rules.none.level\endcsname{139.3}
\expandafter\def\csname val@ms.7.keep-rules.none.located\endcsname{0.316}
\expandafter\def\csname val@ms.7.keep-rules.none.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.keep-rules.none.repaired\endcsname{0.006}
\expandafter\def\csname val@ms.7.keep-rules.none.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.keep-rules.none.score\endcsname{28.1}
\expandafter\def\csname val@ms.7.keep-rules.none.smash_ob_tt\endcsname{-9.11}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_detect\endcsname{219}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_detect.n\endcsname{93}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_locate\endcsname{275}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_locate.n\endcsname{55}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_repair\endcsname{808}
\expandafter\def\csname val@ms.7.keep-rules.none.time_to_repair.n\endcsname{1}
\expandafter\def\csname val@ms.7.keep-rules.none.tokens\endcsname{---}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.Astro.ci\endcsname{2.4--10.3}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.Astro.count\endcsname{0/55}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.Astro.score\endcsname{6.1}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.avoided\endcsname{+0.032}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.ci\endcsname{0.0--1.7}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.level\endcsname{96.8}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.load\endcsname{0.98}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.OB.score\endcsname{0.6}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.avoided\endcsname{-0.026}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.ci\endcsname{1.7--7.8}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.level\endcsname{102.6}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.load\endcsname{1.02}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.TT.score\endcsname{4.4}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.actions\endcsname{30}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.avoided\endcsname{0.003}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.correlated\endcsname{0.093}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.dollars\endcsname{4.40}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.level\endcsname{99.7}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.located\endcsname{0.200}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.score\endcsname{3.7}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.smash_ob_tt\endcsname{5.56}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_detect\endcsname{297}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_detect.n\endcsname{16}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_locate\endcsname{188}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_locate.n\endcsname{35}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.opensre-x3.kimi.tokens\endcsname{7.1M}
\expandafter\def\csname val@ms.7.opensre-x3.luna.Astro.ci\endcsname{4.6--13.2}
\expandafter\def\csname val@ms.7.opensre-x3.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.opensre-x3.luna.Astro.score\endcsname{8.6}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.avoided\endcsname{+0.075}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.ci\endcsname{4.5--11.9}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.level\endcsname{92.5}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.load\endcsname{0.93}
\expandafter\def\csname val@ms.7.opensre-x3.luna.OB.score\endcsname{7.9}
\expandafter\def\csname val@ms.7.opensre-x3.luna.TT.ci\endcsname{0.0--1.7}
\expandafter\def\csname val@ms.7.opensre-x3.luna.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.opensre-x3.luna.TT.score\endcsname{0.6}
\expandafter\def\csname val@ms.7.opensre-x3.luna.actions\endcsname{19}
\expandafter\def\csname val@ms.7.opensre-x3.luna.avoided\endcsname{0.075}
\expandafter\def\csname val@ms.7.opensre-x3.luna.correlated\endcsname{0.222}
\expandafter\def\csname val@ms.7.opensre-x3.luna.dollars\endcsname{1.59}
\expandafter\def\csname val@ms.7.opensre-x3.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.opensre-x3.luna.level\endcsname{92.5}
\expandafter\def\csname val@ms.7.opensre-x3.luna.located\endcsname{0.034}
\expandafter\def\csname val@ms.7.opensre-x3.luna.out_of_scope\endcsname{3}
\expandafter\def\csname val@ms.7.opensre-x3.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.opensre-x3.luna.risk\endcsname{0.158}
\expandafter\def\csname val@ms.7.opensre-x3.luna.score\endcsname{8.3}
\expandafter\def\csname val@ms.7.opensre-x3.luna.smash_ob_tt\endcsname{6.99}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_detect\endcsname{143}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_detect.n\endcsname{26}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_locate\endcsname{173}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_locate.n\endcsname{4}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.opensre-x3.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.opensre-x3.luna.tokens\endcsname{7.0M}
\expandafter\def\csname val@ms.7.opsmem.kimi.Astro.ci\endcsname{13.2--21.8}
\expandafter\def\csname val@ms.7.opsmem.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.opsmem.kimi.Astro.score\endcsname{17.2}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.avoided\endcsname{-0.413}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.ci\endcsname{17.5--26.6}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.level\endcsname{141.3}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.load\endcsname{0.99}
\expandafter\def\csname val@ms.7.opsmem.kimi.OB.score\endcsname{22.0}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.avoided\endcsname{-0.072}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.ci\endcsname{16.1--23.9}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.level\endcsname{107.2}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.load\endcsname{1.10}
\expandafter\def\csname val@ms.7.opsmem.kimi.TT.score\endcsname{20.0}
\expandafter\def\csname val@ms.7.opsmem.kimi.actions\endcsname{5}
\expandafter\def\csname val@ms.7.opsmem.kimi.avoided\endcsname{-0.243}
\expandafter\def\csname val@ms.7.opsmem.kimi.correlated\endcsname{0.587}
\expandafter\def\csname val@ms.7.opsmem.kimi.dollars\endcsname{0.55}
\expandafter\def\csname val@ms.7.opsmem.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.opsmem.kimi.level\endcsname{124.3}
\expandafter\def\csname val@ms.7.opsmem.kimi.located\endcsname{0.006}
\expandafter\def\csname val@ms.7.opsmem.kimi.out_of_scope\endcsname{1}
\expandafter\def\csname val@ms.7.opsmem.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.opsmem.kimi.risk\endcsname{0.200}
\expandafter\def\csname val@ms.7.opsmem.kimi.score\endcsname{19.8}
\expandafter\def\csname val@ms.7.opsmem.kimi.smash_ob_tt\endcsname{-1.65}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_detect\endcsname{146}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_detect.n\endcsname{104}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_locate\endcsname{351}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_locate.n\endcsname{1}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.opsmem.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.opsmem.kimi.tokens\endcsname{754k}
\expandafter\def\csname val@ms.7.opsmem.luna.Astro.ci\endcsname{10.9--19.0}
\expandafter\def\csname val@ms.7.opsmem.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.opsmem.luna.Astro.score\endcsname{14.9}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.avoided\endcsname{+0.226}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.ci\endcsname{17.5--27.7}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.level\endcsname{77.4}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.load\endcsname{0.78}
\expandafter\def\csname val@ms.7.opsmem.luna.OB.score\endcsname{22.6}
\expandafter\def\csname val@ms.7.opsmem.luna.TT.ci\endcsname{21.5--28.8}
\expandafter\def\csname val@ms.7.opsmem.luna.TT.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.opsmem.luna.TT.score\endcsname{25.4}
\expandafter\def\csname val@ms.7.opsmem.luna.actions\endcsname{5}
\expandafter\def\csname val@ms.7.opsmem.luna.avoided\endcsname{0.226}
\expandafter\def\csname val@ms.7.opsmem.luna.correlated\endcsname{0.613}
\expandafter\def\csname val@ms.7.opsmem.luna.dollars\endcsname{0.25}
\expandafter\def\csname val@ms.7.opsmem.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.opsmem.luna.level\endcsname{77.4}
\expandafter\def\csname val@ms.7.opsmem.luna.located\endcsname{0.034}
\expandafter\def\csname val@ms.7.opsmem.luna.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.opsmem.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.opsmem.luna.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.opsmem.luna.score\endcsname{21.0}
\expandafter\def\csname val@ms.7.opsmem.luna.smash_ob_tt\endcsname{13.94}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_detect\endcsname{157}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_detect.n\endcsname{108}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_locate\endcsname{450}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_locate.n\endcsname{6}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.opsmem.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.opsmem.luna.tokens\endcsname{984k}
\expandafter\def\csname val@ms.7.orbit-0.kimi.Astro.ci\endcsname{17.2--25.3}
\expandafter\def\csname val@ms.7.orbit-0.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.orbit-0.kimi.Astro.score\endcsname{21.3}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.avoided\endcsname{+0.072}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.ci\endcsname{27.1--32.2}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.level\endcsname{92.8}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.load\endcsname{0.92}
\expandafter\def\csname val@ms.7.orbit-0.kimi.OB.score\endcsname{29.9}
\expandafter\def\csname val@ms.7.orbit-0.kimi.TT.count\endcsname{---}
\expandafter\def\csname val@ms.7.orbit-0.kimi.TT.score\endcsname{---}
\expandafter\def\csname val@ms.7.orbit-0.kimi.actions\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.kimi.avoided\endcsname{0.072}
\expandafter\def\csname val@ms.7.orbit-0.kimi.correlated\endcsname{0.768}
\expandafter\def\csname val@ms.7.orbit-0.kimi.dollars\endcsname{3.35}
\expandafter\def\csname val@ms.7.orbit-0.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.kimi.level\endcsname{92.8}
\expandafter\def\csname val@ms.7.orbit-0.kimi.located\endcsname{0.000}
\expandafter\def\csname val@ms.7.orbit-0.kimi.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.orbit-0.kimi.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.orbit-0.kimi.score\endcsname{25.6}
\expandafter\def\csname val@ms.7.orbit-0.kimi.smash_ob_tt\endcsname{3.45}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_detect\endcsname{175}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_detect.n\endcsname{90}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_locate\endcsname{---}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_locate.n\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.orbit-0.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.kimi.tokens\endcsname{5.4M}
\expandafter\def\csname val@ms.7.orbit-0.luna.Astro.ci\endcsname{17.8--26.4}
\expandafter\def\csname val@ms.7.orbit-0.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.orbit-0.luna.Astro.score\endcsname{22.4}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.avoided\endcsname{+0.014}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.ci\endcsname{26.6--31.6}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.level\endcsname{98.6}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.load\endcsname{0.96}
\expandafter\def\csname val@ms.7.orbit-0.luna.OB.score\endcsname{29.4}
\expandafter\def\csname val@ms.7.orbit-0.luna.TT.ci\endcsname{29.4--33.3}
\expandafter\def\csname val@ms.7.orbit-0.luna.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.orbit-0.luna.TT.score\endcsname{31.7}
\expandafter\def\csname val@ms.7.orbit-0.luna.actions\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.luna.avoided\endcsname{0.014}
\expandafter\def\csname val@ms.7.orbit-0.luna.correlated\endcsname{0.768}
\expandafter\def\csname val@ms.7.orbit-0.luna.dollars\endcsname{1.63}
\expandafter\def\csname val@ms.7.orbit-0.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.luna.level\endcsname{98.6}
\expandafter\def\csname val@ms.7.orbit-0.luna.located\endcsname{0.009}
\expandafter\def\csname val@ms.7.orbit-0.luna.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.orbit-0.luna.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.orbit-0.luna.score\endcsname{25.9}
\expandafter\def\csname val@ms.7.orbit-0.luna.smash_ob_tt\endcsname{0.49}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_detect\endcsname{186}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_detect.n\endcsname{90}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_locate\endcsname{249}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_locate.n\endcsname{1}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.orbit-0.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.orbit-0.luna.tokens\endcsname{7.1M}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.Astro.ci\endcsname{4.6--12.1}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.Astro.score\endcsname{8.0}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.avoided\endcsname{-0.505}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.ci\endcsname{31.1--46.9}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.level\endcsname{150.5}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.load\endcsname{0.95}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.OB.score\endcsname{39.0}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.TT.ci\endcsname{16.1--31.6}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.TT.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.TT.score\endcsname{23.6}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.actions\endcsname{68}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.avoided\endcsname{-0.505}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.correlated\endcsname{0.426}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.dollars\endcsname{0.46}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.level\endcsname{150.5}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.located\endcsname{0.398}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.out_of_scope\endcsname{1}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.risk\endcsname{0.015}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.score\endcsname{23.5}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.smash_ob_tt\endcsname{-8.14}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_detect\endcsname{200}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_detect.n\endcsname{50}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_locate\endcsname{68}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_locate.n\endcsname{47}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.rag-b2r.kimi.tokens\endcsname{569k}
\expandafter\def\csname val@ms.7.rag-b2r.luna.Astro.ci\endcsname{8.8--21.1}
\expandafter\def\csname val@ms.7.rag-b2r.luna.Astro.count\endcsname{0/57}
\expandafter\def\csname val@ms.7.rag-b2r.luna.Astro.score\endcsname{14.6}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.avoided\endcsname{+0.065}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.ci\endcsname{1.8--7.6}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.count\endcsname{0/57}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.level\endcsname{93.5}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.load\endcsname{0.90}
\expandafter\def\csname val@ms.7.rag-b2r.luna.OB.score\endcsname{4.7}
\expandafter\def\csname val@ms.7.rag-b2r.luna.TT.ci\endcsname{2.3--8.8}
\expandafter\def\csname val@ms.7.rag-b2r.luna.TT.count\endcsname{0/57}
\expandafter\def\csname val@ms.7.rag-b2r.luna.TT.score\endcsname{5.3}
\expandafter\def\csname val@ms.7.rag-b2r.luna.actions\endcsname{99}
\expandafter\def\csname val@ms.7.rag-b2r.luna.avoided\endcsname{0.065}
\expandafter\def\csname val@ms.7.rag-b2r.luna.correlated\endcsname{0.199}
\expandafter\def\csname val@ms.7.rag-b2r.luna.dollars\endcsname{0.23}
\expandafter\def\csname val@ms.7.rag-b2r.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.rag-b2r.luna.level\endcsname{93.5}
\expandafter\def\csname val@ms.7.rag-b2r.luna.located\endcsname{0.105}
\expandafter\def\csname val@ms.7.rag-b2r.luna.out_of_scope\endcsname{0}
\expandafter\def\csname val@ms.7.rag-b2r.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.rag-b2r.luna.risk\endcsname{0.000}
\expandafter\def\csname val@ms.7.rag-b2r.luna.score\endcsname{8.2}
\expandafter\def\csname val@ms.7.rag-b2r.luna.smash_ob_tt\endcsname{12.45}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_detect\endcsname{159}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_detect.n\endcsname{34}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_locate\endcsname{65}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_locate.n\endcsname{18}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.rag-b2r.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.rag-b2r.luna.tokens\endcsname{730k}
\expandafter\def\csname val@ms.7.react-b2.kimi.Astro.ci\endcsname{14.4--25.9}
\expandafter\def\csname val@ms.7.react-b2.kimi.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.react-b2.kimi.Astro.score\endcsname{20.1}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.avoided\endcsname{+0.030}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.ci\endcsname{29.4--35.0}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.level\endcsname{97.0}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.load\endcsname{1.01}
\expandafter\def\csname val@ms.7.react-b2.kimi.OB.score\endcsname{32.2}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.avoided\endcsname{+0.233}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.ci\endcsname{18.9--28.9}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.level\endcsname{76.7}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.load\endcsname{0.81}
\expandafter\def\csname val@ms.7.react-b2.kimi.TT.score\endcsname{23.9}
\expandafter\def\csname val@ms.7.react-b2.kimi.actions\endcsname{46}
\expandafter\def\csname val@ms.7.react-b2.kimi.avoided\endcsname{0.131}
\expandafter\def\csname val@ms.7.react-b2.kimi.correlated\endcsname{0.694}
\expandafter\def\csname val@ms.7.react-b2.kimi.dollars\endcsname{4.02}
\expandafter\def\csname val@ms.7.react-b2.kimi.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.react-b2.kimi.level\endcsname{86.9}
\expandafter\def\csname val@ms.7.react-b2.kimi.located\endcsname{0.079}
\expandafter\def\csname val@ms.7.react-b2.kimi.out_of_scope\endcsname{10}
\expandafter\def\csname val@ms.7.react-b2.kimi.repaired\endcsname{0.006}
\expandafter\def\csname val@ms.7.react-b2.kimi.risk\endcsname{0.217}
\expandafter\def\csname val@ms.7.react-b2.kimi.score\endcsname{25.4}
\expandafter\def\csname val@ms.7.react-b2.kimi.smash_ob_tt\endcsname{6.44}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_detect\endcsname{189}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_detect.n\endcsname{123}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_locate\endcsname{283}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_locate.n\endcsname{14}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_repair\endcsname{709}
\expandafter\def\csname val@ms.7.react-b2.kimi.time_to_repair.n\endcsname{1}
\expandafter\def\csname val@ms.7.react-b2.kimi.tokens\endcsname{6.5M}
\expandafter\def\csname val@ms.7.react-b2.luna.Astro.ci\endcsname{7.5--18.4}
\expandafter\def\csname val@ms.7.react-b2.luna.Astro.count\endcsname{0/58}
\expandafter\def\csname val@ms.7.react-b2.luna.Astro.score\endcsname{12.6}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.avoided\endcsname{+0.056}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.ci\endcsname{30.5--37.3}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.count\endcsname{0/59}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.level\endcsname{94.4}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.load\endcsname{1.01}
\expandafter\def\csname val@ms.7.react-b2.luna.OB.score\endcsname{33.9}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.avoided\endcsname{-0.072}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.ci\endcsname{0.0--5.0}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.count\endcsname{0/60}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.level\endcsname{107.2}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.load\endcsname{---}
\expandafter\def\csname val@ms.7.react-b2.luna.TT.score\endcsname{2.2}
\expandafter\def\csname val@ms.7.react-b2.luna.actions\endcsname{63}
\expandafter\def\csname val@ms.7.react-b2.luna.avoided\endcsname{-0.008}
\expandafter\def\csname val@ms.7.react-b2.luna.correlated\endcsname{0.419}
\expandafter\def\csname val@ms.7.react-b2.luna.dollars\endcsname{1.45}
\expandafter\def\csname val@ms.7.react-b2.luna.forbidden\endcsname{0}
\expandafter\def\csname val@ms.7.react-b2.luna.level\endcsname{100.8}
\expandafter\def\csname val@ms.7.react-b2.luna.located\endcsname{0.125}
\expandafter\def\csname val@ms.7.react-b2.luna.out_of_scope\endcsname{22}
\expandafter\def\csname val@ms.7.react-b2.luna.repaired\endcsname{0.000}
\expandafter\def\csname val@ms.7.react-b2.luna.risk\endcsname{0.349}
\expandafter\def\csname val@ms.7.react-b2.luna.score\endcsname{16.3}
\expandafter\def\csname val@ms.7.react-b2.luna.smash_ob_tt\endcsname{2.39}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_detect\endcsname{163}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_detect.n\endcsname{74}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_locate\endcsname{293}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_locate.n\endcsname{22}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_repair\endcsname{---}
\expandafter\def\csname val@ms.7.react-b2.luna.time_to_repair.n\endcsname{0}
\expandafter\def\csname val@ms.7.react-b2.luna.tokens\endcsname{6.3M}
\expandafter\def\csname val@ms.ambiguous.Astro\endcsname{47}
\expandafter\def\csname val@ms.ambiguous.OB\endcsname{39}
\expandafter\def\csname val@ms.ambiguous.TT\endcsname{76}
\expandafter\def\csname val@ms.band.astro.n\endcsname{3}
\expandafter\def\csname val@ms.band.ob.n\endcsname{5}
\expandafter\def\csname val@ms.band.tt.n\endcsname{4}
\expandafter\def\csname val@ms.best.method\endcsname{Keep-agent}
\expandafter\def\csname val@ms.best.score\endcsname{41.3}
\expandafter\def\csname val@ms.ceiling.Astro\endcsname{83}
\expandafter\def\csname val@ms.ceiling.OB\endcsname{94}
\expandafter\def\csname val@ms.ceiling.TT\endcsname{96}
\expandafter\def\csname val@ms.faults.Astro\endcsname{58}
\expandafter\def\csname val@ms.faults.OB\endcsname{59}
\expandafter\def\csname val@ms.faults.TT\endcsname{60}
\expandafter\def\csname val@ms.held10.react.correlated\endcsname{0.728}
\expandafter\def\csname val@ms.held10.react.handled\endcsname{6.7}
\expandafter\def\csname val@ms.held10.react.located\endcsname{0.283}
\expandafter\def\csname val@ms.held10.react.n\endcsname{6}
\expandafter\def\csname val@ms.held10.react.repaired\endcsname{0.183}
\expandafter\def\csname val@ms.held10.react.score\endcsname{34.8}
\expandafter\def\csname val@ms.held5.react.correlated\endcsname{0.800}
\expandafter\def\csname val@ms.held5.react.handled\endcsname{16.7}
\expandafter\def\csname val@ms.held5.react.located\endcsname{0.200}
\expandafter\def\csname val@ms.held5.react.n\endcsname{6}
\expandafter\def\csname val@ms.held5.react.repaired\endcsname{0.500}
\expandafter\def\csname val@ms.held5.react.score\endcsname{38.9}
\expandafter\def\csname val@ms.live.mean.Astro\endcsname{6.5}
\expandafter\def\csname val@ms.live.mean.OB\endcsname{5.8}
\expandafter\def\csname val@ms.live.mean.TT\endcsname{6.1}
\expandafter\def\csname val@ms.live.peak.Astro\endcsname{11}
\expandafter\def\csname val@ms.live.peak.OB\endcsname{10}
\expandafter\def\csname val@ms.live.peak.TT\endcsname{11}
\expandafter\def\csname val@ms.methods\endcsname{10}
\expandafter\def\csname val@ms.methods.word\endcsname{ten}
\expandafter\def\csname val@ms.never_red.Astro\endcsname{36}
\expandafter\def\csname val@ms.never_red.OB\endcsname{11}
\expandafter\def\csname val@ms.never_red.TT\endcsname{8}
\expandafter\def\csname val@ms.nonzero\endcsname{19}
\expandafter\def\csname val@ms.silent.Astro\endcsname{23}
\expandafter\def\csname val@ms.silent.OB\endcsname{3}
\expandafter\def\csname val@ms.silent.TT\endcsname{2}
\expandafter\def\csname val@ms.storm.react.correlated\endcsname{0.694}
\expandafter\def\csname val@ms.storm.react.handled\endcsname{0.0}
\expandafter\def\csname val@ms.storm.react.located\endcsname{0.079}
\expandafter\def\csname val@ms.storm.react.n\endcsname{3}
\expandafter\def\csname val@ms.storm.react.repaired\endcsname{0.006}
\expandafter\def\csname val@ms.storm.react.score\endcsname{25.4}
\expandafter\def\csname val@ms.unverifiable.Astro\endcsname{29}
\expandafter\def\csname val@ms.unverifiable.OB\endcsname{11}
\expandafter\def\csname val@ms.unverifiable.TT\endcsname{8}
\makeatother


==> results/macros_rq.tex <==
% Generated by 25_rq_figures.py. Use \val{key}; never type a result by hand.
\makeatletter
\expandafter\def\csname val@rq.act.max\endcsname{5.3}
\expandafter\def\csname val@rq.b1-runbook.none.0-10.act\endcsname{1.2}
\expandafter\def\csname val@rq.b1-runbook.none.0-10.claim\endcsname{6.1}
\expandafter\def\csname val@rq.b1-runbook.none.0-10.executed\endcsname{1.1}
\expandafter\def\csname val@rq.b1-runbook.none.0-10.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.10-20.act\endcsname{2.0}
\expandafter\def\csname val@rq.b1-runbook.none.10-20.claim\endcsname{9.6}
\expandafter\def\csname val@rq.b1-runbook.none.10-20.executed\endcsname{2.0}
\expandafter\def\csname val@rq.b1-runbook.none.10-20.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.20-30.act\endcsname{1.3}
\expandafter\def\csname val@rq.b1-runbook.none.20-30.claim\endcsname{8.2}
\expandafter\def\csname val@rq.b1-runbook.none.20-30.executed\endcsname{1.3}
\expandafter\def\csname val@rq.b1-runbook.none.20-30.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.30-40.act\endcsname{2.8}
\expandafter\def\csname val@rq.b1-runbook.none.30-40.claim\endcsname{11.1}
\expandafter\def\csname val@rq.b1-runbook.none.30-40.executed\endcsname{2.7}
\expandafter\def\csname val@rq.b1-runbook.none.30-40.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.40-50.act\endcsname{1.3}
\expandafter\def\csname val@rq.b1-runbook.none.40-50.claim\endcsname{9.1}
\expandafter\def\csname val@rq.b1-runbook.none.40-50.executed\endcsname{1.3}
\expandafter\def\csname val@rq.b1-runbook.none.40-50.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.50-60.act\endcsname{2.3}
\expandafter\def\csname val@rq.b1-runbook.none.50-60.claim\endcsname{11.7}
\expandafter\def\csname val@rq.b1-runbook.none.50-60.executed\endcsname{2.2}
\expandafter\def\csname val@rq.b1-runbook.none.50-60.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.60-70.act\endcsname{0.9}
\expandafter\def\csname val@rq.b1-runbook.none.60-70.claim\endcsname{11.1}
\expandafter\def\csname val@rq.b1-runbook.none.60-70.executed\endcsname{0.9}
\expandafter\def\csname val@rq.b1-runbook.none.60-70.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.70-80.act\endcsname{0.3}
\expandafter\def\csname val@rq.b1-runbook.none.70-80.claim\endcsname{8.1}
\expandafter\def\csname val@rq.b1-runbook.none.70-80.executed\endcsname{0.3}
\expandafter\def\csname val@rq.b1-runbook.none.70-80.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.80-90.act\endcsname{0.1}
\expandafter\def\csname val@rq.b1-runbook.none.80-90.claim\endcsname{8.1}
\expandafter\def\csname val@rq.b1-runbook.none.80-90.executed\endcsname{0.1}
\expandafter\def\csname val@rq.b1-runbook.none.80-90.read\endcsname{1.0}
\expandafter\def\csname val@rq.b1-runbook.none.actions\endcsname{179}
\expandafter\def\csname val@rq.b1-runbook.none.actions.off\endcsname{64}
\expandafter\def\csname val@rq.b1-runbook.none.actions.off.pct\endcsname{36}
\expandafter\def\csname val@rq.b1-runbook.none.actions.repaired\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.actions.repaired.pct\endcsname{2}
\expandafter\def\csname val@rq.b1-runbook.none.actions.unrepaired\endcsname{111}
\expandafter\def\csname val@rq.b1-runbook.none.actions.unrepaired.pct\endcsname{62}
\expandafter\def\csname val@rq.b1-runbook.none.by10.correlated\endcsname{0.75}
\expandafter\def\csname val@rq.b1-runbook.none.by10.correlated.count\endcsname{18}
\expandafter\def\csname val@rq.b1-runbook.none.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.b1-runbook.none.by10.located\endcsname{0.29}
\expandafter\def\csname val@rq.b1-runbook.none.by10.located.count\endcsname{7}
\expandafter\def\csname val@rq.b1-runbook.none.by10.repaired\endcsname{0.08}
\expandafter\def\csname val@rq.b1-runbook.none.by10.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.b1-runbook.none.by20.correlated\endcsname{0.67}
\expandafter\def\csname val@rq.b1-runbook.none.by20.correlated.count\endcsname{36}
\expandafter\def\csname val@rq.b1-runbook.none.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.b1-runbook.none.by20.located\endcsname{0.33}
\expandafter\def\csname val@rq.b1-runbook.none.by20.located.count\endcsname{18}
\expandafter\def\csname val@rq.b1-runbook.none.by20.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.b1-runbook.none.by20.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.b1-runbook.none.by30.correlated\endcsname{0.68}
\expandafter\def\csname val@rq.b1-runbook.none.by30.correlated.count\endcsname{51}
\expandafter\def\csname val@rq.b1-runbook.none.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.b1-runbook.none.by30.located\endcsname{0.36}
\expandafter\def\csname val@rq.b1-runbook.none.by30.located.count\endcsname{27}
\expandafter\def\csname val@rq.b1-runbook.none.by30.repaired\endcsname{0.03}
\expandafter\def\csname val@rq.b1-runbook.none.by30.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.b1-runbook.none.by40.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.b1-runbook.none.by40.correlated.count\endcsname{69}
\expandafter\def\csname val@rq.b1-runbook.none.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.b1-runbook.none.by40.located\endcsname{0.33}
\expandafter\def\csname val@rq.b1-runbook.none.by40.located.count\endcsname{35}
\expandafter\def\csname val@rq.b1-runbook.none.by40.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.b1-runbook.none.by40.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.b1-runbook.none.by50.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.b1-runbook.none.by50.correlated.count\endcsname{84}
\expandafter\def\csname val@rq.b1-runbook.none.by50.injected\endcsname{132}
\expandafter\def\csname val@rq.b1-runbook.none.by50.located\endcsname{0.32}
\expandafter\def\csname val@rq.b1-runbook.none.by50.located.count\endcsname{42}
\expandafter\def\csname val@rq.b1-runbook.none.by50.repaired\endcsname{0.03}
\expandafter\def\csname val@rq.b1-runbook.none.by50.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.by60.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.b1-runbook.none.by60.correlated.count\endcsname{110}
\expandafter\def\csname val@rq.b1-runbook.none.by60.injected\endcsname{172}
\expandafter\def\csname val@rq.b1-runbook.none.by60.located\endcsname{0.35}
\expandafter\def\csname val@rq.b1-runbook.none.by60.located.count\endcsname{61}
\expandafter\def\csname val@rq.b1-runbook.none.by60.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.b1-runbook.none.by60.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.by70.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.b1-runbook.none.by70.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.b1-runbook.none.by70.injected\endcsname{172}
\expandafter\def\csname val@rq.b1-runbook.none.by70.located\endcsname{0.37}
\expandafter\def\csname val@rq.b1-runbook.none.by70.located.count\endcsname{64}
\expandafter\def\csname val@rq.b1-runbook.none.by70.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.b1-runbook.none.by70.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.by80.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.b1-runbook.none.by80.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.b1-runbook.none.by80.injected\endcsname{172}
\expandafter\def\csname val@rq.b1-runbook.none.by80.located\endcsname{0.37}
\expandafter\def\csname val@rq.b1-runbook.none.by80.located.count\endcsname{64}
\expandafter\def\csname val@rq.b1-runbook.none.by80.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.b1-runbook.none.by80.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.by90.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.b1-runbook.none.by90.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.b1-runbook.none.by90.injected\endcsname{172}
\expandafter\def\csname val@rq.b1-runbook.none.by90.located\endcsname{0.37}
\expandafter\def\csname val@rq.b1-runbook.none.by90.located.count\endcsname{64}
\expandafter\def\csname val@rq.b1-runbook.none.by90.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.b1-runbook.none.by90.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.acted\endcsname{87}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.acted.pct\endcsname{51}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.correlated\endcsname{35}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.correlated.pct\endcsname{20}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.faults\endcsname{172}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.located\endcsname{1}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.located.pct\endcsname{1}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.missed\endcsname{45}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.missed.pct\endcsname{26}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.repaired-only\endcsname{4}
\expandafter\def\csname val@rq.b1-runbook.none.outcome.repaired-only.pct\endcsname{2}
\expandafter\def\csname val@rq.claudecode-x5.kimi.0-10.act\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.0-10.claim\endcsname{3.9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.0-10.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.0-10.read\endcsname{9.4}
\expandafter\def\csname val@rq.claudecode-x5.kimi.10-20.act\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.10-20.claim\endcsname{15.1}
\expandafter\def\csname val@rq.claudecode-x5.kimi.10-20.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.10-20.read\endcsname{15.4}
\expandafter\def\csname val@rq.claudecode-x5.kimi.20-30.act\endcsname{0.7}
\expandafter\def\csname val@rq.claudecode-x5.kimi.20-30.claim\endcsname{17.4}
\expandafter\def\csname val@rq.claudecode-x5.kimi.20-30.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.20-30.read\endcsname{16.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.30-40.act\endcsname{0.4}
\expandafter\def\csname val@rq.claudecode-x5.kimi.30-40.claim\endcsname{19.5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.30-40.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.30-40.read\endcsname{12.5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.40-50.act\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.40-50.claim\endcsname{22.2}
\expandafter\def\csname val@rq.claudecode-x5.kimi.40-50.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.40-50.read\endcsname{14.7}
\expandafter\def\csname val@rq.claudecode-x5.kimi.50-60.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.50-60.claim\endcsname{22.6}
\expandafter\def\csname val@rq.claudecode-x5.kimi.50-60.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.50-60.read\endcsname{15.9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.60-70.claim\endcsname{23.1}
\expandafter\def\csname val@rq.claudecode-x5.kimi.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.60-70.read\endcsname{10.5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.70-80.claim\endcsname{25.5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.70-80.read\endcsname{12.6}
\expandafter\def\csname val@rq.claudecode-x5.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.80-90.claim\endcsname{31.8}
\expandafter\def\csname val@rq.claudecode-x5.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.80-90.read\endcsname{12.0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions\endcsname{22}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.off\endcsname{1}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.off.pct\endcsname{5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.unrepaired\endcsname{21}
\expandafter\def\csname val@rq.claudecode-x5.kimi.actions.unrepaired.pct\endcsname{95}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.correlated\endcsname{0.29}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.correlated.count\endcsname{7}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.located\endcsname{0.04}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.located.count\endcsname{1}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.correlated\endcsname{0.35}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.correlated.count\endcsname{19}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.located\endcsname{0.06}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.located.count\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.correlated\endcsname{0.31}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.correlated.count\endcsname{23}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.located\endcsname{0.04}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.located.count\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.correlated\endcsname{0.30}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.correlated.count\endcsname{32}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.located\endcsname{0.03}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.located.count\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.correlated\endcsname{0.28}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.correlated.count\endcsname{39}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.located\endcsname{0.02}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.located.count\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.correlated\endcsname{0.25}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.correlated.count\endcsname{44}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.located\endcsname{0.02}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.located.count\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.correlated\endcsname{0.31}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.correlated.count\endcsname{54}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.located\endcsname{0.05}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.located.count\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.correlated\endcsname{0.37}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.correlated.count\endcsname{66}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.located\endcsname{0.05}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.located.count\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.correlated\endcsname{0.38}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.correlated.count\endcsname{67}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.located\endcsname{0.05}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.located.count\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.kimi.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.acted\endcsname{16}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.acted.pct\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.correlated\endcsname{52}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.correlated.pct\endcsname{29}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.located\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.located.pct\endcsname{5}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.missed\endcsname{100}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.missed.pct\endcsname{56}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.kimi.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.0-10.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.0-10.claim\endcsname{3.3}
\expandafter\def\csname val@rq.claudecode-x5.luna.0-10.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.0-10.read\endcsname{11.5}
\expandafter\def\csname val@rq.claudecode-x5.luna.10-20.act\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.luna.10-20.claim\endcsname{8.9}
\expandafter\def\csname val@rq.claudecode-x5.luna.10-20.executed\endcsname{0.3}
\expandafter\def\csname val@rq.claudecode-x5.luna.10-20.read\endcsname{13.9}
\expandafter\def\csname val@rq.claudecode-x5.luna.20-30.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.20-30.claim\endcsname{13.3}
\expandafter\def\csname val@rq.claudecode-x5.luna.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.20-30.read\endcsname{17.4}
\expandafter\def\csname val@rq.claudecode-x5.luna.30-40.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.30-40.claim\endcsname{22.1}
\expandafter\def\csname val@rq.claudecode-x5.luna.30-40.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.30-40.read\endcsname{15.1}
\expandafter\def\csname val@rq.claudecode-x5.luna.40-50.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.40-50.claim\endcsname{24.5}
\expandafter\def\csname val@rq.claudecode-x5.luna.40-50.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.40-50.read\endcsname{15.7}
\expandafter\def\csname val@rq.claudecode-x5.luna.50-60.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.50-60.claim\endcsname{30.8}
\expandafter\def\csname val@rq.claudecode-x5.luna.50-60.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.50-60.read\endcsname{16.5}
\expandafter\def\csname val@rq.claudecode-x5.luna.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.60-70.claim\endcsname{26.4}
\expandafter\def\csname val@rq.claudecode-x5.luna.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.60-70.read\endcsname{15.7}
\expandafter\def\csname val@rq.claudecode-x5.luna.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.70-80.claim\endcsname{41.7}
\expandafter\def\csname val@rq.claudecode-x5.luna.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.70-80.read\endcsname{12.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.80-90.claim\endcsname{43.7}
\expandafter\def\csname val@rq.claudecode-x5.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.claudecode-x5.luna.80-90.read\endcsname{11.4}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions\endcsname{4}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.off\endcsname{1}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.off.pct\endcsname{25}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.unrepaired\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.luna.actions.unrepaired.pct\endcsname{75}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.correlated\endcsname{0.26}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.correlated.count\endcsname{6}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.injected\endcsname{23}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.located\endcsname{0.09}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.located.count\endcsname{2}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.correlated\endcsname{0.25}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.correlated.count\endcsname{13}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.injected\endcsname{53}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.located\endcsname{0.08}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.located.count\endcsname{4}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.correlated\endcsname{0.32}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.correlated.count\endcsname{23}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.injected\endcsname{72}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.located\endcsname{0.11}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.located.count\endcsname{8}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.correlated\endcsname{0.34}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.correlated.count\endcsname{35}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.injected\endcsname{102}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.located\endcsname{0.09}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.located.count\endcsname{9}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.correlated\endcsname{0.32}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.correlated.count\endcsname{42}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.injected\endcsname{132}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.located\endcsname{0.08}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.located.count\endcsname{10}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.correlated\endcsname{0.35}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.correlated.count\endcsname{59}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.injected\endcsname{170}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.located\endcsname{0.07}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.located.count\endcsname{12}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.correlated\endcsname{0.41}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.correlated.count\endcsname{69}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.injected\endcsname{170}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.located\endcsname{0.07}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.located.count\endcsname{12}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.correlated\endcsname{0.41}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.correlated.count\endcsname{70}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.injected\endcsname{170}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.located\endcsname{0.07}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.located.count\endcsname{12}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.correlated\endcsname{0.41}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.correlated.count\endcsname{70}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.injected\endcsname{170}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.located\endcsname{0.07}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.located.count\endcsname{12}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.claudecode-x5.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.acted\endcsname{3}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.acted.pct\endcsname{2}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.correlated\endcsname{66}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.correlated.pct\endcsname{39}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.faults\endcsname{170}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.located\endcsname{12}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.located.pct\endcsname{7}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.missed\endcsname{89}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.missed.pct\endcsname{52}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.claudecode-x5.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.coca.kimi.0-10.act\endcsname{0.4}
\expandafter\def\csname val@rq.coca.kimi.0-10.claim\endcsname{5.5}
\expandafter\def\csname val@rq.coca.kimi.0-10.executed\endcsname{0.1}
\expandafter\def\csname val@rq.coca.kimi.0-10.read\endcsname{11.1}
\expandafter\def\csname val@rq.coca.kimi.10-20.act\endcsname{0.9}
\expandafter\def\csname val@rq.coca.kimi.10-20.claim\endcsname{12.7}
\expandafter\def\csname val@rq.coca.kimi.10-20.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.kimi.10-20.read\endcsname{34.9}
\expandafter\def\csname val@rq.coca.kimi.20-30.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.kimi.20-30.claim\endcsname{10.2}
\expandafter\def\csname val@rq.coca.kimi.20-30.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.kimi.20-30.read\endcsname{22.7}
\expandafter\def\csname val@rq.coca.kimi.30-40.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.kimi.30-40.claim\endcsname{9.6}
\expandafter\def\csname val@rq.coca.kimi.30-40.executed\endcsname{0.6}
\expandafter\def\csname val@rq.coca.kimi.30-40.read\endcsname{16.2}
\expandafter\def\csname val@rq.coca.kimi.40-50.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.kimi.40-50.claim\endcsname{8.1}
\expandafter\def\csname val@rq.coca.kimi.40-50.executed\endcsname{0.5}
\expandafter\def\csname val@rq.coca.kimi.40-50.read\endcsname{19.5}
\expandafter\def\csname val@rq.coca.kimi.50-60.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.kimi.50-60.claim\endcsname{9.8}
\expandafter\def\csname val@rq.coca.kimi.50-60.executed\endcsname{0.5}
\expandafter\def\csname val@rq.coca.kimi.50-60.read\endcsname{16.8}
\expandafter\def\csname val@rq.coca.kimi.60-70.act\endcsname{0.5}
\expandafter\def\csname val@rq.coca.kimi.60-70.claim\endcsname{9.1}
\expandafter\def\csname val@rq.coca.kimi.60-70.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.kimi.60-70.read\endcsname{14.8}
\expandafter\def\csname val@rq.coca.kimi.70-80.act\endcsname{0.1}
\expandafter\def\csname val@rq.coca.kimi.70-80.claim\endcsname{5.3}
\expandafter\def\csname val@rq.coca.kimi.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.coca.kimi.70-80.read\endcsname{4.8}
\expandafter\def\csname val@rq.coca.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.coca.kimi.80-90.claim\endcsname{4.7}
\expandafter\def\csname val@rq.coca.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.coca.kimi.80-90.read\endcsname{2.0}
\expandafter\def\csname val@rq.coca.kimi.actions\endcsname{39}
\expandafter\def\csname val@rq.coca.kimi.actions.off\endcsname{4}
\expandafter\def\csname val@rq.coca.kimi.actions.off.pct\endcsname{10}
\expandafter\def\csname val@rq.coca.kimi.actions.repaired\endcsname{2}
\expandafter\def\csname val@rq.coca.kimi.actions.repaired.pct\endcsname{5}
\expandafter\def\csname val@rq.coca.kimi.actions.unrepaired\endcsname{33}
\expandafter\def\csname val@rq.coca.kimi.actions.unrepaired.pct\endcsname{85}
\expandafter\def\csname val@rq.coca.kimi.by10.correlated\endcsname{0.79}
\expandafter\def\csname val@rq.coca.kimi.by10.correlated.count\endcsname{19}
\expandafter\def\csname val@rq.coca.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.coca.kimi.by10.located\endcsname{0.00}
\expandafter\def\csname val@rq.coca.kimi.by10.located.count\endcsname{0}
\expandafter\def\csname val@rq.coca.kimi.by10.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.coca.kimi.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.kimi.by20.correlated\endcsname{0.65}
\expandafter\def\csname val@rq.coca.kimi.by20.correlated.count\endcsname{35}
\expandafter\def\csname val@rq.coca.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.coca.kimi.by20.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by20.located.count\endcsname{1}
\expandafter\def\csname val@rq.coca.kimi.by20.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.kimi.by30.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.coca.kimi.by30.correlated.count\endcsname{47}
\expandafter\def\csname val@rq.coca.kimi.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.coca.kimi.by30.located\endcsname{0.04}
\expandafter\def\csname val@rq.coca.kimi.by30.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by30.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.kimi.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.kimi.by40.correlated\endcsname{0.61}
\expandafter\def\csname val@rq.coca.kimi.by40.correlated.count\endcsname{65}
\expandafter\def\csname val@rq.coca.kimi.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.coca.kimi.by40.located\endcsname{0.03}
\expandafter\def\csname val@rq.coca.kimi.by40.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.kimi.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.kimi.by50.correlated\endcsname{0.55}
\expandafter\def\csname val@rq.coca.kimi.by50.correlated.count\endcsname{76}
\expandafter\def\csname val@rq.coca.kimi.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.coca.kimi.by50.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by50.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by50.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by50.repaired.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by60.correlated\endcsname{0.56}
\expandafter\def\csname val@rq.coca.kimi.by60.correlated.count\endcsname{100}
\expandafter\def\csname val@rq.coca.kimi.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.coca.kimi.by60.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by60.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by60.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by60.repaired.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by70.correlated\endcsname{0.58}
\expandafter\def\csname val@rq.coca.kimi.by70.correlated.count\endcsname{102}
\expandafter\def\csname val@rq.coca.kimi.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.coca.kimi.by70.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by70.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by70.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by70.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.coca.kimi.by80.correlated\endcsname{0.58}
\expandafter\def\csname val@rq.coca.kimi.by80.correlated.count\endcsname{102}
\expandafter\def\csname val@rq.coca.kimi.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.coca.kimi.by80.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by80.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by80.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by80.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.coca.kimi.by90.correlated\endcsname{0.58}
\expandafter\def\csname val@rq.coca.kimi.by90.correlated.count\endcsname{102}
\expandafter\def\csname val@rq.coca.kimi.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.coca.kimi.by90.located\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by90.located.count\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.by90.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.kimi.by90.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.coca.kimi.outcome.acted\endcsname{33}
\expandafter\def\csname val@rq.coca.kimi.outcome.acted.pct\endcsname{19}
\expandafter\def\csname val@rq.coca.kimi.outcome.correlated\endcsname{71}
\expandafter\def\csname val@rq.coca.kimi.outcome.correlated.pct\endcsname{40}
\expandafter\def\csname val@rq.coca.kimi.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.coca.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.coca.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.coca.kimi.outcome.located\endcsname{3}
\expandafter\def\csname val@rq.coca.kimi.outcome.located.pct\endcsname{2}
\expandafter\def\csname val@rq.coca.kimi.outcome.missed\endcsname{66}
\expandafter\def\csname val@rq.coca.kimi.outcome.missed.pct\endcsname{37}
\expandafter\def\csname val@rq.coca.kimi.outcome.repaired-only\endcsname{4}
\expandafter\def\csname val@rq.coca.kimi.outcome.repaired-only.pct\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.0-10.act\endcsname{0.5}
\expandafter\def\csname val@rq.coca.luna.0-10.claim\endcsname{5.3}
\expandafter\def\csname val@rq.coca.luna.0-10.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.luna.0-10.read\endcsname{18.5}
\expandafter\def\csname val@rq.coca.luna.10-20.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.luna.10-20.claim\endcsname{9.6}
\expandafter\def\csname val@rq.coca.luna.10-20.executed\endcsname{0.2}
\expandafter\def\csname val@rq.coca.luna.10-20.read\endcsname{29.2}
\expandafter\def\csname val@rq.coca.luna.20-30.act\endcsname{0.6}
\expandafter\def\csname val@rq.coca.luna.20-30.claim\endcsname{7.3}
\expandafter\def\csname val@rq.coca.luna.20-30.executed\endcsname{0.1}
\expandafter\def\csname val@rq.coca.luna.20-30.read\endcsname{19.3}
\expandafter\def\csname val@rq.coca.luna.30-40.act\endcsname{0.6}
\expandafter\def\csname val@rq.coca.luna.30-40.claim\endcsname{6.9}
\expandafter\def\csname val@rq.coca.luna.30-40.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.luna.30-40.read\endcsname{19.7}
\expandafter\def\csname val@rq.coca.luna.40-50.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.luna.40-50.claim\endcsname{8.5}
\expandafter\def\csname val@rq.coca.luna.40-50.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.luna.40-50.read\endcsname{14.6}
\expandafter\def\csname val@rq.coca.luna.50-60.act\endcsname{0.7}
\expandafter\def\csname val@rq.coca.luna.50-60.claim\endcsname{9.4}
\expandafter\def\csname val@rq.coca.luna.50-60.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.luna.50-60.read\endcsname{17.9}
\expandafter\def\csname val@rq.coca.luna.60-70.act\endcsname{0.6}
\expandafter\def\csname val@rq.coca.luna.60-70.claim\endcsname{8.1}
\expandafter\def\csname val@rq.coca.luna.60-70.executed\endcsname{0.3}
\expandafter\def\csname val@rq.coca.luna.60-70.read\endcsname{21.1}
\expandafter\def\csname val@rq.coca.luna.70-80.act\endcsname{0.2}
\expandafter\def\csname val@rq.coca.luna.70-80.claim\endcsname{3.4}
\expandafter\def\csname val@rq.coca.luna.70-80.executed\endcsname{0.1}
\expandafter\def\csname val@rq.coca.luna.70-80.read\endcsname{6.4}
\expandafter\def\csname val@rq.coca.luna.80-90.act\endcsname{0.1}
\expandafter\def\csname val@rq.coca.luna.80-90.claim\endcsname{2.4}
\expandafter\def\csname val@rq.coca.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.coca.luna.80-90.read\endcsname{2.5}
\expandafter\def\csname val@rq.coca.luna.actions\endcsname{29}
\expandafter\def\csname val@rq.coca.luna.actions.off\endcsname{3}
\expandafter\def\csname val@rq.coca.luna.actions.off.pct\endcsname{10}
\expandafter\def\csname val@rq.coca.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.coca.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.coca.luna.actions.unrepaired\endcsname{26}
\expandafter\def\csname val@rq.coca.luna.actions.unrepaired.pct\endcsname{90}
\expandafter\def\csname val@rq.coca.luna.by10.correlated\endcsname{0.62}
\expandafter\def\csname val@rq.coca.luna.by10.correlated.count\endcsname{15}
\expandafter\def\csname val@rq.coca.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.coca.luna.by10.located\endcsname{0.25}
\expandafter\def\csname val@rq.coca.luna.by10.located.count\endcsname{6}
\expandafter\def\csname val@rq.coca.luna.by10.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.coca.luna.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.luna.by20.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.coca.luna.by20.correlated.count\endcsname{34}
\expandafter\def\csname val@rq.coca.luna.by20.injected\endcsname{53}
\expandafter\def\csname val@rq.coca.luna.by20.located\endcsname{0.23}
\expandafter\def\csname val@rq.coca.luna.by20.located.count\endcsname{12}
\expandafter\def\csname val@rq.coca.luna.by20.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.luna.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.luna.by30.correlated\endcsname{0.62}
\expandafter\def\csname val@rq.coca.luna.by30.correlated.count\endcsname{46}
\expandafter\def\csname val@rq.coca.luna.by30.injected\endcsname{74}
\expandafter\def\csname val@rq.coca.luna.by30.located\endcsname{0.24}
\expandafter\def\csname val@rq.coca.luna.by30.located.count\endcsname{18}
\expandafter\def\csname val@rq.coca.luna.by30.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.luna.by40.correlated\endcsname{0.65}
\expandafter\def\csname val@rq.coca.luna.by40.correlated.count\endcsname{69}
\expandafter\def\csname val@rq.coca.luna.by40.injected\endcsname{106}
\expandafter\def\csname val@rq.coca.luna.by40.located\endcsname{0.24}
\expandafter\def\csname val@rq.coca.luna.by40.located.count\endcsname{25}
\expandafter\def\csname val@rq.coca.luna.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.coca.luna.by50.correlated\endcsname{0.62}
\expandafter\def\csname val@rq.coca.luna.by50.correlated.count\endcsname{82}
\expandafter\def\csname val@rq.coca.luna.by50.injected\endcsname{133}
\expandafter\def\csname val@rq.coca.luna.by50.located\endcsname{0.24}
\expandafter\def\csname val@rq.coca.luna.by50.located.count\endcsname{32}
\expandafter\def\csname val@rq.coca.luna.by50.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.coca.luna.by50.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.by60.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.coca.luna.by60.correlated.count\endcsname{101}
\expandafter\def\csname val@rq.coca.luna.by60.injected\endcsname{171}
\expandafter\def\csname val@rq.coca.luna.by60.located\endcsname{0.23}
\expandafter\def\csname val@rq.coca.luna.by60.located.count\endcsname{40}
\expandafter\def\csname val@rq.coca.luna.by60.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by60.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.by70.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.coca.luna.by70.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.coca.luna.by70.injected\endcsname{171}
\expandafter\def\csname val@rq.coca.luna.by70.located\endcsname{0.26}
\expandafter\def\csname val@rq.coca.luna.by70.located.count\endcsname{44}
\expandafter\def\csname val@rq.coca.luna.by70.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by70.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.by80.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.coca.luna.by80.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.coca.luna.by80.injected\endcsname{171}
\expandafter\def\csname val@rq.coca.luna.by80.located\endcsname{0.26}
\expandafter\def\csname val@rq.coca.luna.by80.located.count\endcsname{44}
\expandafter\def\csname val@rq.coca.luna.by80.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by80.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.by90.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.coca.luna.by90.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.coca.luna.by90.injected\endcsname{171}
\expandafter\def\csname val@rq.coca.luna.by90.located\endcsname{0.26}
\expandafter\def\csname val@rq.coca.luna.by90.located.count\endcsname{44}
\expandafter\def\csname val@rq.coca.luna.by90.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.coca.luna.by90.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.outcome.acted\endcsname{26}
\expandafter\def\csname val@rq.coca.luna.outcome.acted.pct\endcsname{15}
\expandafter\def\csname val@rq.coca.luna.outcome.correlated\endcsname{69}
\expandafter\def\csname val@rq.coca.luna.outcome.correlated.pct\endcsname{40}
\expandafter\def\csname val@rq.coca.luna.outcome.faults\endcsname{171}
\expandafter\def\csname val@rq.coca.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.coca.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.coca.luna.outcome.located\endcsname{22}
\expandafter\def\csname val@rq.coca.luna.outcome.located.pct\endcsname{13}
\expandafter\def\csname val@rq.coca.luna.outcome.missed\endcsname{52}
\expandafter\def\csname val@rq.coca.luna.outcome.missed.pct\endcsname{30}
\expandafter\def\csname val@rq.coca.luna.outcome.repaired-only\endcsname{2}
\expandafter\def\csname val@rq.coca.luna.outcome.repaired-only.pct\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.0-10.act\endcsname{0.5}
\expandafter\def\csname val@rq.codex-x4.kimi.0-10.claim\endcsname{4.5}
\expandafter\def\csname val@rq.codex-x4.kimi.0-10.executed\endcsname{0.5}
\expandafter\def\csname val@rq.codex-x4.kimi.0-10.read\endcsname{4.5}
\expandafter\def\csname val@rq.codex-x4.kimi.10-20.act\endcsname{0.7}
\expandafter\def\csname val@rq.codex-x4.kimi.10-20.claim\endcsname{9.7}
\expandafter\def\csname val@rq.codex-x4.kimi.10-20.executed\endcsname{0.7}
\expandafter\def\csname val@rq.codex-x4.kimi.10-20.read\endcsname{2.1}
\expandafter\def\csname val@rq.codex-x4.kimi.20-30.act\endcsname{0.3}
\expandafter\def\csname val@rq.codex-x4.kimi.20-30.claim\endcsname{11.0}
\expandafter\def\csname val@rq.codex-x4.kimi.20-30.executed\endcsname{0.3}
\expandafter\def\csname val@rq.codex-x4.kimi.20-30.read\endcsname{1.1}
\expandafter\def\csname val@rq.codex-x4.kimi.30-40.act\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.kimi.30-40.claim\endcsname{15.3}
\expandafter\def\csname val@rq.codex-x4.kimi.30-40.executed\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.kimi.30-40.read\endcsname{1.9}
\expandafter\def\csname val@rq.codex-x4.kimi.40-50.act\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.40-50.claim\endcsname{19.3}
\expandafter\def\csname val@rq.codex-x4.kimi.40-50.executed\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.40-50.read\endcsname{1.5}
\expandafter\def\csname val@rq.codex-x4.kimi.50-60.act\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.50-60.claim\endcsname{16.7}
\expandafter\def\csname val@rq.codex-x4.kimi.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.50-60.read\endcsname{1.7}
\expandafter\def\csname val@rq.codex-x4.kimi.60-70.act\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.60-70.claim\endcsname{16.5}
\expandafter\def\csname val@rq.codex-x4.kimi.60-70.executed\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.kimi.60-70.read\endcsname{1.8}
\expandafter\def\csname val@rq.codex-x4.kimi.70-80.act\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.kimi.70-80.claim\endcsname{18.1}
\expandafter\def\csname val@rq.codex-x4.kimi.70-80.executed\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.kimi.70-80.read\endcsname{1.8}
\expandafter\def\csname val@rq.codex-x4.kimi.80-90.act\endcsname{0.2}
\expandafter\def\csname val@rq.codex-x4.kimi.80-90.claim\endcsname{17.3}
\expandafter\def\csname val@rq.codex-x4.kimi.80-90.executed\endcsname{0.2}
\expandafter\def\csname val@rq.codex-x4.kimi.80-90.read\endcsname{2.4}
\expandafter\def\csname val@rq.codex-x4.kimi.actions\endcsname{41}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.off\endcsname{16}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.off.pct\endcsname{39}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.unrepaired\endcsname{25}
\expandafter\def\csname val@rq.codex-x4.kimi.actions.unrepaired.pct\endcsname{61}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.correlated\endcsname{0.25}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.correlated.count\endcsname{6}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.located.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.correlated\endcsname{0.19}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.correlated.count\endcsname{10}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.located.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.kimi.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.correlated\endcsname{0.19}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.correlated.count\endcsname{14}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.located\endcsname{0.03}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.located.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.correlated.count\endcsname{21}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.located.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.correlated\endcsname{0.19}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.correlated.count\endcsname{26}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.located.count\endcsname{5}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by50.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.correlated\endcsname{0.21}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.correlated.count\endcsname{37}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.located\endcsname{0.03}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.located.count\endcsname{6}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by60.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.correlated\endcsname{0.23}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.correlated.count\endcsname{41}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.located.count\endcsname{7}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by70.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.correlated\endcsname{0.23}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.correlated.count\endcsname{41}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.located.count\endcsname{7}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by80.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.correlated\endcsname{0.23}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.correlated.count\endcsname{41}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.located\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.located.count\endcsname{7}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.kimi.by90.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.acted\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.acted.pct\endcsname{14}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.correlated\endcsname{35}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.correlated.pct\endcsname{20}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.located\endcsname{3}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.located.pct\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.missed\endcsname{113}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.missed.pct\endcsname{64}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.repaired-only\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.kimi.outcome.repaired-only.pct\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.luna.0-10.act\endcsname{0.9}
\expandafter\def\csname val@rq.codex-x4.luna.0-10.claim\endcsname{5.9}
\expandafter\def\csname val@rq.codex-x4.luna.0-10.executed\endcsname{0.9}
\expandafter\def\csname val@rq.codex-x4.luna.0-10.read\endcsname{3.7}
\expandafter\def\csname val@rq.codex-x4.luna.10-20.act\endcsname{0.8}
\expandafter\def\csname val@rq.codex-x4.luna.10-20.claim\endcsname{13.3}
\expandafter\def\csname val@rq.codex-x4.luna.10-20.executed\endcsname{0.7}
\expandafter\def\csname val@rq.codex-x4.luna.10-20.read\endcsname{4.5}
\expandafter\def\csname val@rq.codex-x4.luna.20-30.act\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.luna.20-30.claim\endcsname{11.0}
\expandafter\def\csname val@rq.codex-x4.luna.20-30.executed\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.luna.20-30.read\endcsname{2.5}
\expandafter\def\csname val@rq.codex-x4.luna.30-40.act\endcsname{0.3}
\expandafter\def\csname val@rq.codex-x4.luna.30-40.claim\endcsname{18.9}
\expandafter\def\csname val@rq.codex-x4.luna.30-40.executed\endcsname{0.3}
\expandafter\def\csname val@rq.codex-x4.luna.30-40.read\endcsname{4.0}
\expandafter\def\csname val@rq.codex-x4.luna.40-50.act\endcsname{1.3}
\expandafter\def\csname val@rq.codex-x4.luna.40-50.claim\endcsname{25.4}
\expandafter\def\csname val@rq.codex-x4.luna.40-50.executed\endcsname{1.3}
\expandafter\def\csname val@rq.codex-x4.luna.40-50.read\endcsname{3.9}
\expandafter\def\csname val@rq.codex-x4.luna.50-60.act\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.luna.50-60.claim\endcsname{27.3}
\expandafter\def\csname val@rq.codex-x4.luna.50-60.executed\endcsname{0.4}
\expandafter\def\csname val@rq.codex-x4.luna.50-60.read\endcsname{4.9}
\expandafter\def\csname val@rq.codex-x4.luna.60-70.act\endcsname{0.5}
\expandafter\def\csname val@rq.codex-x4.luna.60-70.claim\endcsname{27.2}
\expandafter\def\csname val@rq.codex-x4.luna.60-70.executed\endcsname{0.5}
\expandafter\def\csname val@rq.codex-x4.luna.60-70.read\endcsname{3.5}
\expandafter\def\csname val@rq.codex-x4.luna.70-80.act\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.luna.70-80.claim\endcsname{30.6}
\expandafter\def\csname val@rq.codex-x4.luna.70-80.executed\endcsname{0.1}
\expandafter\def\csname val@rq.codex-x4.luna.70-80.read\endcsname{3.6}
\expandafter\def\csname val@rq.codex-x4.luna.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.codex-x4.luna.80-90.claim\endcsname{37.6}
\expandafter\def\csname val@rq.codex-x4.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.codex-x4.luna.80-90.read\endcsname{2.9}
\expandafter\def\csname val@rq.codex-x4.luna.actions\endcsname{68}
\expandafter\def\csname val@rq.codex-x4.luna.actions.off\endcsname{17}
\expandafter\def\csname val@rq.codex-x4.luna.actions.off.pct\endcsname{25}
\expandafter\def\csname val@rq.codex-x4.luna.actions.repaired\endcsname{2}
\expandafter\def\csname val@rq.codex-x4.luna.actions.repaired.pct\endcsname{3}
\expandafter\def\csname val@rq.codex-x4.luna.actions.unrepaired\endcsname{49}
\expandafter\def\csname val@rq.codex-x4.luna.actions.unrepaired.pct\endcsname{72}
\expandafter\def\csname val@rq.codex-x4.luna.by10.correlated\endcsname{0.50}
\expandafter\def\csname val@rq.codex-x4.luna.by10.correlated.count\endcsname{12}
\expandafter\def\csname val@rq.codex-x4.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.luna.by10.located\endcsname{0.21}
\expandafter\def\csname val@rq.codex-x4.luna.by10.located.count\endcsname{5}
\expandafter\def\csname val@rq.codex-x4.luna.by10.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.codex-x4.luna.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.luna.by20.correlated\endcsname{0.47}
\expandafter\def\csname val@rq.codex-x4.luna.by20.correlated.count\endcsname{25}
\expandafter\def\csname val@rq.codex-x4.luna.by20.injected\endcsname{53}
\expandafter\def\csname val@rq.codex-x4.luna.by20.located\endcsname{0.15}
\expandafter\def\csname val@rq.codex-x4.luna.by20.located.count\endcsname{8}
\expandafter\def\csname val@rq.codex-x4.luna.by20.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.luna.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.luna.by30.correlated\endcsname{0.43}
\expandafter\def\csname val@rq.codex-x4.luna.by30.correlated.count\endcsname{32}
\expandafter\def\csname val@rq.codex-x4.luna.by30.injected\endcsname{74}
\expandafter\def\csname val@rq.codex-x4.luna.by30.located\endcsname{0.14}
\expandafter\def\csname val@rq.codex-x4.luna.by30.located.count\endcsname{10}
\expandafter\def\csname val@rq.codex-x4.luna.by30.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.luna.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.luna.by40.correlated\endcsname{0.52}
\expandafter\def\csname val@rq.codex-x4.luna.by40.correlated.count\endcsname{55}
\expandafter\def\csname val@rq.codex-x4.luna.by40.injected\endcsname{106}
\expandafter\def\csname val@rq.codex-x4.luna.by40.located\endcsname{0.10}
\expandafter\def\csname val@rq.codex-x4.luna.by40.located.count\endcsname{11}
\expandafter\def\csname val@rq.codex-x4.luna.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.codex-x4.luna.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.codex-x4.luna.by50.correlated\endcsname{0.50}
\expandafter\def\csname val@rq.codex-x4.luna.by50.correlated.count\endcsname{67}
\expandafter\def\csname val@rq.codex-x4.luna.by50.injected\endcsname{135}
\expandafter\def\csname val@rq.codex-x4.luna.by50.located\endcsname{0.12}
\expandafter\def\csname val@rq.codex-x4.luna.by50.located.count\endcsname{16}
\expandafter\def\csname val@rq.codex-x4.luna.by50.repaired\endcsname{0.03}
\expandafter\def\csname val@rq.codex-x4.luna.by50.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.by60.correlated\endcsname{0.49}
\expandafter\def\csname val@rq.codex-x4.luna.by60.correlated.count\endcsname{84}
\expandafter\def\csname val@rq.codex-x4.luna.by60.injected\endcsname{173}
\expandafter\def\csname val@rq.codex-x4.luna.by60.located\endcsname{0.13}
\expandafter\def\csname val@rq.codex-x4.luna.by60.located.count\endcsname{23}
\expandafter\def\csname val@rq.codex-x4.luna.by60.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.luna.by60.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.by70.correlated\endcsname{0.50}
\expandafter\def\csname val@rq.codex-x4.luna.by70.correlated.count\endcsname{86}
\expandafter\def\csname val@rq.codex-x4.luna.by70.injected\endcsname{173}
\expandafter\def\csname val@rq.codex-x4.luna.by70.located\endcsname{0.14}
\expandafter\def\csname val@rq.codex-x4.luna.by70.located.count\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.luna.by70.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.luna.by70.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.by80.correlated\endcsname{0.50}
\expandafter\def\csname val@rq.codex-x4.luna.by80.correlated.count\endcsname{87}
\expandafter\def\csname val@rq.codex-x4.luna.by80.injected\endcsname{173}
\expandafter\def\csname val@rq.codex-x4.luna.by80.located\endcsname{0.14}
\expandafter\def\csname val@rq.codex-x4.luna.by80.located.count\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.luna.by80.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.luna.by80.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.by90.correlated\endcsname{0.50}
\expandafter\def\csname val@rq.codex-x4.luna.by90.correlated.count\endcsname{87}
\expandafter\def\csname val@rq.codex-x4.luna.by90.injected\endcsname{173}
\expandafter\def\csname val@rq.codex-x4.luna.by90.located\endcsname{0.14}
\expandafter\def\csname val@rq.codex-x4.luna.by90.located.count\endcsname{24}
\expandafter\def\csname val@rq.codex-x4.luna.by90.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.codex-x4.luna.by90.repaired.count\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.acted\endcsname{47}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.acted.pct\endcsname{27}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.correlated\endcsname{44}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.correlated.pct\endcsname{25}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.faults\endcsname{173}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.located\endcsname{5}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.located.pct\endcsname{3}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.missed\endcsname{73}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.missed.pct\endcsname{42}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.repaired-only\endcsname{4}
\expandafter\def\csname val@rq.codex-x4.luna.outcome.repaired-only.pct\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.kimi.0-10.act\endcsname{1.3}
\expandafter\def\csname val@rq.keep-llm.kimi.0-10.claim\endcsname{15.2}
\expandafter\def\csname val@rq.keep-llm.kimi.0-10.executed\endcsname{1.1}
\expandafter\def\csname val@rq.keep-llm.kimi.0-10.read\endcsname{7.0}
\expandafter\def\csname val@rq.keep-llm.kimi.10-20.act\endcsname{1.8}
\expandafter\def\csname val@rq.keep-llm.kimi.10-20.claim\endcsname{42.7}
\expandafter\def\csname val@rq.keep-llm.kimi.10-20.executed\endcsname{1.0}
\expandafter\def\csname val@rq.keep-llm.kimi.10-20.read\endcsname{8.6}
\expandafter\def\csname val@rq.keep-llm.kimi.20-30.act\endcsname{1.2}
\expandafter\def\csname val@rq.keep-llm.kimi.20-30.claim\endcsname{69.3}
\expandafter\def\csname val@rq.keep-llm.kimi.20-30.executed\endcsname{0.6}
\expandafter\def\csname val@rq.keep-llm.kimi.20-30.read\endcsname{11.0}
\expandafter\def\csname val@rq.keep-llm.kimi.30-40.act\endcsname{0.3}
\expandafter\def\csname val@rq.keep-llm.kimi.30-40.claim\endcsname{69.0}
\expandafter\def\csname val@rq.keep-llm.kimi.30-40.executed\endcsname{0.3}
\expandafter\def\csname val@rq.keep-llm.kimi.30-40.read\endcsname{8.6}
\expandafter\def\csname val@rq.keep-llm.kimi.40-50.act\endcsname{2.5}
\expandafter\def\csname val@rq.keep-llm.kimi.40-50.claim\endcsname{103.9}
\expandafter\def\csname val@rq.keep-llm.kimi.40-50.executed\endcsname{1.3}
\expandafter\def\csname val@rq.keep-llm.kimi.40-50.read\endcsname{12.0}
\expandafter\def\csname val@rq.keep-llm.kimi.50-60.act\endcsname{0.9}
\expandafter\def\csname val@rq.keep-llm.kimi.50-60.claim\endcsname{69.5}
\expandafter\def\csname val@rq.keep-llm.kimi.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.kimi.50-60.read\endcsname{12.0}
\expandafter\def\csname val@rq.keep-llm.kimi.60-70.act\endcsname{5.3}
\expandafter\def\csname val@rq.keep-llm.kimi.60-70.claim\endcsname{124.7}
\expandafter\def\csname val@rq.keep-llm.kimi.60-70.executed\endcsname{1.8}
\expandafter\def\csname val@rq.keep-llm.kimi.60-70.read\endcsname{12.0}
\expandafter\def\csname val@rq.keep-llm.kimi.70-80.act\endcsname{1.4}
\expandafter\def\csname val@rq.keep-llm.kimi.70-80.claim\endcsname{89.8}
\expandafter\def\csname val@rq.keep-llm.kimi.70-80.executed\endcsname{0.7}
\expandafter\def\csname val@rq.keep-llm.kimi.70-80.read\endcsname{10.0}
\expandafter\def\csname val@rq.keep-llm.kimi.80-90.act\endcsname{1.7}
\expandafter\def\csname val@rq.keep-llm.kimi.80-90.claim\endcsname{97.6}
\expandafter\def\csname val@rq.keep-llm.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.keep-llm.kimi.80-90.read\endcsname{9.0}
\expandafter\def\csname val@rq.keep-llm.kimi.actions\endcsname{69}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.off\endcsname{32}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.off.pct\endcsname{46}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.repaired\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.repaired.pct\endcsname{3}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.unrepaired\endcsname{35}
\expandafter\def\csname val@rq.keep-llm.kimi.actions.unrepaired.pct\endcsname{51}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.correlated\endcsname{0.69}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.correlated.count\endcsname{11}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.injected\endcsname{16}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.located\endcsname{0.31}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.located.count\endcsname{5}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.repaired\endcsname{0.06}
\expandafter\def\csname val@rq.keep-llm.kimi.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.correlated.count\endcsname{23}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.injected\endcsname{36}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.located\endcsname{0.47}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.located.count\endcsname{17}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.repaired\endcsname{0.03}
\expandafter\def\csname val@rq.keep-llm.kimi.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.correlated\endcsname{0.74}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.correlated.count\endcsname{37}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.injected\endcsname{50}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.located\endcsname{0.48}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.located.count\endcsname{24}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.kimi.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.correlated\endcsname{0.65}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.correlated.count\endcsname{46}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.injected\endcsname{71}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.located.count\endcsname{35}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.kimi.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.correlated\endcsname{0.70}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.correlated.count\endcsname{63}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.injected\endcsname{90}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.located.count\endcsname{44}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.kimi.by50.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.correlated\endcsname{0.73}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.correlated.count\endcsname{84}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.injected\endcsname{115}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.located.count\endcsname{56}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.kimi.by60.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.correlated.count\endcsname{89}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.injected\endcsname{115}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.located.count\endcsname{56}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.kimi.by70.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.correlated.count\endcsname{89}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.injected\endcsname{115}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.located.count\endcsname{56}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.kimi.by80.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.correlated.count\endcsname{89}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.injected\endcsname{115}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.located\endcsname{0.49}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.located.count\endcsname{56}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.kimi.by90.repaired.count\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.acted\endcsname{21}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.acted.pct\endcsname{18}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.correlated\endcsname{32}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.correlated.pct\endcsname{28}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.faults\endcsname{115}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.handled\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.handled.pct\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.located\endcsname{39}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.located.pct\endcsname{34}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.missed\endcsname{21}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.missed.pct\endcsname{18}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.repaired-only\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.kimi.outcome.repaired-only.pct\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.0-10.act\endcsname{0.9}
\expandafter\def\csname val@rq.keep-llm.luna.0-10.claim\endcsname{27.3}
\expandafter\def\csname val@rq.keep-llm.luna.0-10.executed\endcsname{0.2}
\expandafter\def\csname val@rq.keep-llm.luna.0-10.read\endcsname{9.0}
\expandafter\def\csname val@rq.keep-llm.luna.10-20.act\endcsname{0.3}
\expandafter\def\csname val@rq.keep-llm.luna.10-20.claim\endcsname{61.8}
\expandafter\def\csname val@rq.keep-llm.luna.10-20.executed\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.luna.10-20.read\endcsname{11.7}
\expandafter\def\csname val@rq.keep-llm.luna.20-30.act\endcsname{0.7}
\expandafter\def\csname val@rq.keep-llm.luna.20-30.claim\endcsname{102.4}
\expandafter\def\csname val@rq.keep-llm.luna.20-30.executed\endcsname{0.5}
\expandafter\def\csname val@rq.keep-llm.luna.20-30.read\endcsname{12.0}
\expandafter\def\csname val@rq.keep-llm.luna.30-40.act\endcsname{0.5}
\expandafter\def\csname val@rq.keep-llm.luna.30-40.claim\endcsname{117.3}
\expandafter\def\csname val@rq.keep-llm.luna.30-40.executed\endcsname{0.5}
\expandafter\def\csname val@rq.keep-llm.luna.30-40.read\endcsname{9.8}
\expandafter\def\csname val@rq.keep-llm.luna.40-50.act\endcsname{0.7}
\expandafter\def\csname val@rq.keep-llm.luna.40-50.claim\endcsname{120.7}
\expandafter\def\csname val@rq.keep-llm.luna.40-50.executed\endcsname{0.7}
\expandafter\def\csname val@rq.keep-llm.luna.40-50.read\endcsname{8.3}
\expandafter\def\csname val@rq.keep-llm.luna.50-60.act\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.luna.50-60.claim\endcsname{137.1}
\expandafter\def\csname val@rq.keep-llm.luna.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.luna.50-60.read\endcsname{7.6}
\expandafter\def\csname val@rq.keep-llm.luna.60-70.act\endcsname{0.7}
\expandafter\def\csname val@rq.keep-llm.luna.60-70.claim\endcsname{154.1}
\expandafter\def\csname val@rq.keep-llm.luna.60-70.executed\endcsname{0.6}
\expandafter\def\csname val@rq.keep-llm.luna.60-70.read\endcsname{8.3}
\expandafter\def\csname val@rq.keep-llm.luna.70-80.act\endcsname{1.2}
\expandafter\def\csname val@rq.keep-llm.luna.70-80.claim\endcsname{126.0}
\expandafter\def\csname val@rq.keep-llm.luna.70-80.executed\endcsname{1.2}
\expandafter\def\csname val@rq.keep-llm.luna.70-80.read\endcsname{8.3}
\expandafter\def\csname val@rq.keep-llm.luna.80-90.act\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.luna.80-90.claim\endcsname{129.8}
\expandafter\def\csname val@rq.keep-llm.luna.80-90.executed\endcsname{0.1}
\expandafter\def\csname val@rq.keep-llm.luna.80-90.read\endcsname{8.3}
\expandafter\def\csname val@rq.keep-llm.luna.actions\endcsname{59}
\expandafter\def\csname val@rq.keep-llm.luna.actions.off\endcsname{38}
\expandafter\def\csname val@rq.keep-llm.luna.actions.off.pct\endcsname{64}
\expandafter\def\csname val@rq.keep-llm.luna.actions.repaired\endcsname{3}
\expandafter\def\csname val@rq.keep-llm.luna.actions.repaired.pct\endcsname{5}
\expandafter\def\csname val@rq.keep-llm.luna.actions.unrepaired\endcsname{18}
\expandafter\def\csname val@rq.keep-llm.luna.actions.unrepaired.pct\endcsname{31}
\expandafter\def\csname val@rq.keep-llm.luna.by10.correlated\endcsname{0.71}
\expandafter\def\csname val@rq.keep-llm.luna.by10.correlated.count\endcsname{17}
\expandafter\def\csname val@rq.keep-llm.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.keep-llm.luna.by10.located\endcsname{0.29}
\expandafter\def\csname val@rq.keep-llm.luna.by10.located.count\endcsname{7}
\expandafter\def\csname val@rq.keep-llm.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.keep-llm.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.keep-llm.luna.by20.correlated\endcsname{0.74}
\expandafter\def\csname val@rq.keep-llm.luna.by20.correlated.count\endcsname{40}
\expandafter\def\csname val@rq.keep-llm.luna.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.keep-llm.luna.by20.located\endcsname{0.33}
\expandafter\def\csname val@rq.keep-llm.luna.by20.located.count\endcsname{18}
\expandafter\def\csname val@rq.keep-llm.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.keep-llm.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.keep-llm.luna.by30.correlated\endcsname{0.72}
\expandafter\def\csname val@rq.keep-llm.luna.by30.correlated.count\endcsname{54}
\expandafter\def\csname val@rq.keep-llm.luna.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.keep-llm.luna.by30.located\endcsname{0.28}
\expandafter\def\csname val@rq.keep-llm.luna.by30.located.count\endcsname{21}
\expandafter\def\csname val@rq.keep-llm.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.keep-llm.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.keep-llm.luna.by40.correlated\endcsname{0.70}
\expandafter\def\csname val@rq.keep-llm.luna.by40.correlated.count\endcsname{75}
\expandafter\def\csname val@rq.keep-llm.luna.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.keep-llm.luna.by40.located\endcsname{0.30}
\expandafter\def\csname val@rq.keep-llm.luna.by40.located.count\endcsname{32}
\expandafter\def\csname val@rq.keep-llm.luna.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.luna.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.by50.correlated\endcsname{0.65}
\expandafter\def\csname val@rq.keep-llm.luna.by50.correlated.count\endcsname{88}
\expandafter\def\csname val@rq.keep-llm.luna.by50.injected\endcsname{135}
\expandafter\def\csname val@rq.keep-llm.luna.by50.located\endcsname{0.31}
\expandafter\def\csname val@rq.keep-llm.luna.by50.located.count\endcsname{42}
\expandafter\def\csname val@rq.keep-llm.luna.by50.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.luna.by50.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.by60.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.keep-llm.luna.by60.correlated.count\endcsname{112}
\expandafter\def\csname val@rq.keep-llm.luna.by60.injected\endcsname{174}
\expandafter\def\csname val@rq.keep-llm.luna.by60.located\endcsname{0.32}
\expandafter\def\csname val@rq.keep-llm.luna.by60.located.count\endcsname{55}
\expandafter\def\csname val@rq.keep-llm.luna.by60.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.keep-llm.luna.by60.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.by70.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.keep-llm.luna.by70.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.keep-llm.luna.by70.injected\endcsname{174}
\expandafter\def\csname val@rq.keep-llm.luna.by70.located\endcsname{0.32}
\expandafter\def\csname val@rq.keep-llm.luna.by70.located.count\endcsname{55}
\expandafter\def\csname val@rq.keep-llm.luna.by70.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.luna.by70.repaired.count\endcsname{3}
\expandafter\def\csname val@rq.keep-llm.luna.by80.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.keep-llm.luna.by80.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.keep-llm.luna.by80.injected\endcsname{174}
\expandafter\def\csname val@rq.keep-llm.luna.by80.located\endcsname{0.32}
\expandafter\def\csname val@rq.keep-llm.luna.by80.located.count\endcsname{55}
\expandafter\def\csname val@rq.keep-llm.luna.by80.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.luna.by80.repaired.count\endcsname{3}
\expandafter\def\csname val@rq.keep-llm.luna.by90.correlated\endcsname{0.66}
\expandafter\def\csname val@rq.keep-llm.luna.by90.correlated.count\endcsname{114}
\expandafter\def\csname val@rq.keep-llm.luna.by90.injected\endcsname{174}
\expandafter\def\csname val@rq.keep-llm.luna.by90.located\endcsname{0.32}
\expandafter\def\csname val@rq.keep-llm.luna.by90.located.count\endcsname{55}
\expandafter\def\csname val@rq.keep-llm.luna.by90.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.keep-llm.luna.by90.repaired.count\endcsname{3}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.acted\endcsname{12}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.acted.pct\endcsname{7}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.correlated\endcsname{64}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.correlated.pct\endcsname{37}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.faults\endcsname{174}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.handled\endcsname{2}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.handled.pct\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.located\endcsname{42}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.located.pct\endcsname{24}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.missed\endcsname{53}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.missed.pct\endcsname{30}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.repaired-only\endcsname{1}
\expandafter\def\csname val@rq.keep-llm.luna.outcome.repaired-only.pct\endcsname{1}
\expandafter\def\csname val@rq.observation.act.pct\endcsname{0.7}
\expandafter\def\csname val@rq.observation.claim.pct\endcsname{82.1}
\expandafter\def\csname val@rq.observation.read.pct\endcsname{17.2}
\expandafter\def\csname val@rq.opensre-x3.kimi.0-10.act\endcsname{1.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.0-10.claim\endcsname{6.5}
\expandafter\def\csname val@rq.opensre-x3.kimi.0-10.executed\endcsname{1.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.0-10.read\endcsname{6.5}
\expandafter\def\csname val@rq.opensre-x3.kimi.10-20.act\endcsname{0.3}
\expandafter\def\csname val@rq.opensre-x3.kimi.10-20.claim\endcsname{11.7}
\expandafter\def\csname val@rq.opensre-x3.kimi.10-20.executed\endcsname{0.3}
\expandafter\def\csname val@rq.opensre-x3.kimi.10-20.read\endcsname{12.7}
\expandafter\def\csname val@rq.opensre-x3.kimi.20-30.act\endcsname{0.3}
\expandafter\def\csname val@rq.opensre-x3.kimi.20-30.claim\endcsname{14.2}
\expandafter\def\csname val@rq.opensre-x3.kimi.20-30.executed\endcsname{0.3}
\expandafter\def\csname val@rq.opensre-x3.kimi.20-30.read\endcsname{12.4}
\expandafter\def\csname val@rq.opensre-x3.kimi.30-40.act\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.30-40.claim\endcsname{10.7}
\expandafter\def\csname val@rq.opensre-x3.kimi.30-40.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.30-40.read\endcsname{14.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.40-50.act\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.40-50.claim\endcsname{17.0}
\expandafter\def\csname val@rq.opensre-x3.kimi.40-50.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.40-50.read\endcsname{13.3}
\expandafter\def\csname val@rq.opensre-x3.kimi.50-60.act\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.50-60.claim\endcsname{9.9}
\expandafter\def\csname val@rq.opensre-x3.kimi.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.50-60.read\endcsname{12.4}
\expandafter\def\csname val@rq.opensre-x3.kimi.60-70.act\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.60-70.claim\endcsname{9.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.60-70.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.60-70.read\endcsname{10.4}
\expandafter\def\csname val@rq.opensre-x3.kimi.70-80.act\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.70-80.claim\endcsname{9.4}
\expandafter\def\csname val@rq.opensre-x3.kimi.70-80.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.kimi.70-80.read\endcsname{8.2}
\expandafter\def\csname val@rq.opensre-x3.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.kimi.80-90.claim\endcsname{14.0}
\expandafter\def\csname val@rq.opensre-x3.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.kimi.80-90.read\endcsname{8.2}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions\endcsname{30}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.off\endcsname{2}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.off.pct\endcsname{7}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.unrepaired\endcsname{28}
\expandafter\def\csname val@rq.opensre-x3.kimi.actions.unrepaired.pct\endcsname{93}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.correlated\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.correlated.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.located\endcsname{0.29}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.located.count\endcsname{7}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.correlated\endcsname{0.04}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.correlated.count\endcsname{2}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.located\endcsname{0.35}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.located.count\endcsname{19}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.correlated\endcsname{0.04}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.correlated.count\endcsname{3}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.injected\endcsname{74}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.located\endcsname{0.32}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.located.count\endcsname{24}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.correlated\endcsname{0.06}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.correlated.count\endcsname{6}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.injected\endcsname{106}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.located\endcsname{0.25}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.located.count\endcsname{26}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.correlated\endcsname{0.06}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.correlated.count\endcsname{8}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.injected\endcsname{135}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.located\endcsname{0.21}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.located.count\endcsname{29}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.correlated\endcsname{0.07}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.correlated.count\endcsname{13}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.injected\endcsname{174}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.located\endcsname{0.20}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.located.count\endcsname{35}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.correlated\endcsname{0.09}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.injected\endcsname{174}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.located\endcsname{0.20}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.located.count\endcsname{35}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.correlated\endcsname{0.09}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.injected\endcsname{174}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.located\endcsname{0.20}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.located.count\endcsname{35}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.correlated\endcsname{0.09}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.injected\endcsname{174}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.located\endcsname{0.20}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.located.count\endcsname{35}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.kimi.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.acted\endcsname{23}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.acted.pct\endcsname{13}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.correlated\endcsname{12}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.correlated.pct\endcsname{7}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.faults\endcsname{174}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.located\endcsname{23}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.located.pct\endcsname{13}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.missed\endcsname{116}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.missed.pct\endcsname{67}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.kimi.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.0-10.act\endcsname{0.2}
\expandafter\def\csname val@rq.opensre-x3.luna.0-10.claim\endcsname{5.9}
\expandafter\def\csname val@rq.opensre-x3.luna.0-10.executed\endcsname{0.2}
\expandafter\def\csname val@rq.opensre-x3.luna.0-10.read\endcsname{8.9}
\expandafter\def\csname val@rq.opensre-x3.luna.10-20.act\endcsname{0.9}
\expandafter\def\csname val@rq.opensre-x3.luna.10-20.claim\endcsname{10.7}
\expandafter\def\csname val@rq.opensre-x3.luna.10-20.executed\endcsname{0.9}
\expandafter\def\csname val@rq.opensre-x3.luna.10-20.read\endcsname{18.5}
\expandafter\def\csname val@rq.opensre-x3.luna.20-30.act\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.20-30.claim\endcsname{11.1}
\expandafter\def\csname val@rq.opensre-x3.luna.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.20-30.read\endcsname{21.4}
\expandafter\def\csname val@rq.opensre-x3.luna.30-40.act\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.30-40.claim\endcsname{12.7}
\expandafter\def\csname val@rq.opensre-x3.luna.30-40.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.30-40.read\endcsname{22.6}
\expandafter\def\csname val@rq.opensre-x3.luna.40-50.act\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.40-50.claim\endcsname{16.1}
\expandafter\def\csname val@rq.opensre-x3.luna.40-50.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.40-50.read\endcsname{20.1}
\expandafter\def\csname val@rq.opensre-x3.luna.50-60.act\endcsname{0.3}
\expandafter\def\csname val@rq.opensre-x3.luna.50-60.claim\endcsname{9.4}
\expandafter\def\csname val@rq.opensre-x3.luna.50-60.executed\endcsname{0.2}
\expandafter\def\csname val@rq.opensre-x3.luna.50-60.read\endcsname{16.4}
\expandafter\def\csname val@rq.opensre-x3.luna.60-70.act\endcsname{0.6}
\expandafter\def\csname val@rq.opensre-x3.luna.60-70.claim\endcsname{15.6}
\expandafter\def\csname val@rq.opensre-x3.luna.60-70.executed\endcsname{0.5}
\expandafter\def\csname val@rq.opensre-x3.luna.60-70.read\endcsname{22.8}
\expandafter\def\csname val@rq.opensre-x3.luna.70-80.act\endcsname{1.2}
\expandafter\def\csname val@rq.opensre-x3.luna.70-80.claim\endcsname{8.4}
\expandafter\def\csname val@rq.opensre-x3.luna.70-80.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opensre-x3.luna.70-80.read\endcsname{20.5}
\expandafter\def\csname val@rq.opensre-x3.luna.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.80-90.claim\endcsname{14.3}
\expandafter\def\csname val@rq.opensre-x3.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opensre-x3.luna.80-90.read\endcsname{25.6}
\expandafter\def\csname val@rq.opensre-x3.luna.actions\endcsname{19}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.off\endcsname{3}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.off.pct\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.unrepaired\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.luna.actions.unrepaired.pct\endcsname{84}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.correlated\endcsname{0.19}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.correlated.count\endcsname{3}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.injected\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.located\endcsname{0.06}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.located.count\endcsname{1}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.correlated\endcsname{0.25}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.correlated.count\endcsname{9}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.injected\endcsname{36}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.located\endcsname{0.11}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.correlated.count\endcsname{10}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.injected\endcsname{50}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.located\endcsname{0.08}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.correlated\endcsname{0.24}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.correlated.count\endcsname{17}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.injected\endcsname{71}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.located\endcsname{0.06}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.correlated\endcsname{0.22}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.correlated.count\endcsname{20}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.injected\endcsname{91}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.located\endcsname{0.04}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.correlated\endcsname{0.22}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.correlated.count\endcsname{26}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.injected\endcsname{117}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.located\endcsname{0.03}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.correlated\endcsname{0.22}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.correlated.count\endcsname{26}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.injected\endcsname{117}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.located\endcsname{0.03}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.correlated\endcsname{0.22}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.correlated.count\endcsname{26}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.injected\endcsname{117}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.located\endcsname{0.03}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.correlated\endcsname{0.22}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.correlated.count\endcsname{26}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.injected\endcsname{117}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.located\endcsname{0.03}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.located.count\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opensre-x3.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.acted\endcsname{15}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.acted.pct\endcsname{13}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.correlated\endcsname{19}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.correlated.pct\endcsname{16}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.faults\endcsname{117}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.located\endcsname{4}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.located.pct\endcsname{3}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.missed\endcsname{79}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.missed.pct\endcsname{68}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.opensre-x3.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.0-10.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.0-10.claim\endcsname{5.5}
\expandafter\def\csname val@rq.opsmem.kimi.0-10.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.0-10.read\endcsname{3.7}
\expandafter\def\csname val@rq.opsmem.kimi.10-20.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.10-20.claim\endcsname{12.1}
\expandafter\def\csname val@rq.opsmem.kimi.10-20.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.10-20.read\endcsname{4.9}
\expandafter\def\csname val@rq.opsmem.kimi.20-30.act\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.20-30.claim\endcsname{11.1}
\expandafter\def\csname val@rq.opsmem.kimi.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.20-30.read\endcsname{4.9}
\expandafter\def\csname val@rq.opsmem.kimi.30-40.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.30-40.claim\endcsname{6.6}
\expandafter\def\csname val@rq.opsmem.kimi.30-40.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.30-40.read\endcsname{4.3}
\expandafter\def\csname val@rq.opsmem.kimi.40-50.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.40-50.claim\endcsname{11.1}
\expandafter\def\csname val@rq.opsmem.kimi.40-50.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.40-50.read\endcsname{4.2}
\expandafter\def\csname val@rq.opsmem.kimi.50-60.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.50-60.claim\endcsname{12.5}
\expandafter\def\csname val@rq.opsmem.kimi.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.50-60.read\endcsname{5.7}
\expandafter\def\csname val@rq.opsmem.kimi.60-70.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.60-70.claim\endcsname{9.5}
\expandafter\def\csname val@rq.opsmem.kimi.60-70.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.kimi.60-70.read\endcsname{5.5}
\expandafter\def\csname val@rq.opsmem.kimi.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.70-80.claim\endcsname{4.2}
\expandafter\def\csname val@rq.opsmem.kimi.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.70-80.read\endcsname{2.9}
\expandafter\def\csname val@rq.opsmem.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.80-90.claim\endcsname{2.6}
\expandafter\def\csname val@rq.opsmem.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.kimi.80-90.read\endcsname{2.3}
\expandafter\def\csname val@rq.opsmem.kimi.actions\endcsname{5}
\expandafter\def\csname val@rq.opsmem.kimi.actions.off\endcsname{4}
\expandafter\def\csname val@rq.opsmem.kimi.actions.off.pct\endcsname{80}
\expandafter\def\csname val@rq.opsmem.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.actions.unrepaired\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.actions.unrepaired.pct\endcsname{20}
\expandafter\def\csname val@rq.opsmem.kimi.by10.correlated\endcsname{0.83}
\expandafter\def\csname val@rq.opsmem.kimi.by10.correlated.count\endcsname{20}
\expandafter\def\csname val@rq.opsmem.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.opsmem.kimi.by10.located\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by10.located.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by20.correlated\endcsname{0.70}
\expandafter\def\csname val@rq.opsmem.kimi.by20.correlated.count\endcsname{38}
\expandafter\def\csname val@rq.opsmem.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.opsmem.kimi.by20.located\endcsname{0.02}
\expandafter\def\csname val@rq.opsmem.kimi.by20.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by30.correlated\endcsname{0.68}
\expandafter\def\csname val@rq.opsmem.kimi.by30.correlated.count\endcsname{51}
\expandafter\def\csname val@rq.opsmem.kimi.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.opsmem.kimi.by30.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by30.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by40.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.opsmem.kimi.by40.correlated.count\endcsname{67}
\expandafter\def\csname val@rq.opsmem.kimi.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.opsmem.kimi.by40.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by40.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by50.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.opsmem.kimi.by50.correlated.count\endcsname{81}
\expandafter\def\csname val@rq.opsmem.kimi.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.opsmem.kimi.by50.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by50.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by60.correlated\endcsname{0.57}
\expandafter\def\csname val@rq.opsmem.kimi.by60.correlated.count\endcsname{101}
\expandafter\def\csname val@rq.opsmem.kimi.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.opsmem.kimi.by60.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by60.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by70.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.opsmem.kimi.by70.correlated.count\endcsname{104}
\expandafter\def\csname val@rq.opsmem.kimi.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.opsmem.kimi.by70.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by70.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by80.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.opsmem.kimi.by80.correlated.count\endcsname{104}
\expandafter\def\csname val@rq.opsmem.kimi.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.opsmem.kimi.by80.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by80.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.by90.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.opsmem.kimi.by90.correlated.count\endcsname{104}
\expandafter\def\csname val@rq.opsmem.kimi.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.opsmem.kimi.by90.located\endcsname{0.01}
\expandafter\def\csname val@rq.opsmem.kimi.by90.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.kimi.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.acted\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.acted.pct\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.correlated\endcsname{102}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.correlated.pct\endcsname{58}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.located\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.located.pct\endcsname{1}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.missed\endcsname{73}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.missed.pct\endcsname{41}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.opsmem.kimi.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.0-10.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.0-10.claim\endcsname{6.7}
\expandafter\def\csname val@rq.opsmem.luna.0-10.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.0-10.read\endcsname{5.6}
\expandafter\def\csname val@rq.opsmem.luna.10-20.act\endcsname{0.2}
\expandafter\def\csname val@rq.opsmem.luna.10-20.claim\endcsname{7.1}
\expandafter\def\csname val@rq.opsmem.luna.10-20.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.10-20.read\endcsname{6.0}
\expandafter\def\csname val@rq.opsmem.luna.20-30.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.20-30.claim\endcsname{9.0}
\expandafter\def\csname val@rq.opsmem.luna.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.20-30.read\endcsname{5.4}
\expandafter\def\csname val@rq.opsmem.luna.30-40.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.30-40.claim\endcsname{10.7}
\expandafter\def\csname val@rq.opsmem.luna.30-40.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.30-40.read\endcsname{5.3}
\expandafter\def\csname val@rq.opsmem.luna.40-50.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.40-50.claim\endcsname{7.6}
\expandafter\def\csname val@rq.opsmem.luna.40-50.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.40-50.read\endcsname{6.1}
\expandafter\def\csname val@rq.opsmem.luna.50-60.act\endcsname{0.2}
\expandafter\def\csname val@rq.opsmem.luna.50-60.claim\endcsname{10.5}
\expandafter\def\csname val@rq.opsmem.luna.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.50-60.read\endcsname{5.5}
\expandafter\def\csname val@rq.opsmem.luna.60-70.act\endcsname{0.1}
\expandafter\def\csname val@rq.opsmem.luna.60-70.claim\endcsname{9.7}
\expandafter\def\csname val@rq.opsmem.luna.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.60-70.read\endcsname{7.0}
\expandafter\def\csname val@rq.opsmem.luna.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.70-80.claim\endcsname{3.7}
\expandafter\def\csname val@rq.opsmem.luna.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.70-80.read\endcsname{2.9}
\expandafter\def\csname val@rq.opsmem.luna.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.80-90.claim\endcsname{2.3}
\expandafter\def\csname val@rq.opsmem.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.opsmem.luna.80-90.read\endcsname{2.9}
\expandafter\def\csname val@rq.opsmem.luna.actions\endcsname{5}
\expandafter\def\csname val@rq.opsmem.luna.actions.off\endcsname{2}
\expandafter\def\csname val@rq.opsmem.luna.actions.off.pct\endcsname{40}
\expandafter\def\csname val@rq.opsmem.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.actions.unrepaired\endcsname{3}
\expandafter\def\csname val@rq.opsmem.luna.actions.unrepaired.pct\endcsname{60}
\expandafter\def\csname val@rq.opsmem.luna.by10.correlated\endcsname{0.67}
\expandafter\def\csname val@rq.opsmem.luna.by10.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.opsmem.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.opsmem.luna.by10.located\endcsname{0.04}
\expandafter\def\csname val@rq.opsmem.luna.by10.located.count\endcsname{1}
\expandafter\def\csname val@rq.opsmem.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by20.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.opsmem.luna.by20.correlated.count\endcsname{34}
\expandafter\def\csname val@rq.opsmem.luna.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.opsmem.luna.by20.located\endcsname{0.06}
\expandafter\def\csname val@rq.opsmem.luna.by20.located.count\endcsname{3}
\expandafter\def\csname val@rq.opsmem.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by30.correlated\endcsname{0.59}
\expandafter\def\csname val@rq.opsmem.luna.by30.correlated.count\endcsname{44}
\expandafter\def\csname val@rq.opsmem.luna.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.opsmem.luna.by30.located\endcsname{0.05}
\expandafter\def\csname val@rq.opsmem.luna.by30.located.count\endcsname{4}
\expandafter\def\csname val@rq.opsmem.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by40.correlated\endcsname{0.63}
\expandafter\def\csname val@rq.opsmem.luna.by40.correlated.count\endcsname{67}
\expandafter\def\csname val@rq.opsmem.luna.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.opsmem.luna.by40.located\endcsname{0.04}
\expandafter\def\csname val@rq.opsmem.luna.by40.located.count\endcsname{4}
\expandafter\def\csname val@rq.opsmem.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by50.correlated\endcsname{0.58}
\expandafter\def\csname val@rq.opsmem.luna.by50.correlated.count\endcsname{79}
\expandafter\def\csname val@rq.opsmem.luna.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.opsmem.luna.by50.located\endcsname{0.03}
\expandafter\def\csname val@rq.opsmem.luna.by50.located.count\endcsname{4}
\expandafter\def\csname val@rq.opsmem.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by60.correlated\endcsname{0.60}
\expandafter\def\csname val@rq.opsmem.luna.by60.correlated.count\endcsname{105}
\expandafter\def\csname val@rq.opsmem.luna.by60.injected\endcsname{176}
\expandafter\def\csname val@rq.opsmem.luna.by60.located\endcsname{0.03}
\expandafter\def\csname val@rq.opsmem.luna.by60.located.count\endcsname{5}
\expandafter\def\csname val@rq.opsmem.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by70.correlated\endcsname{0.61}
\expandafter\def\csname val@rq.opsmem.luna.by70.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.opsmem.luna.by70.injected\endcsname{176}
\expandafter\def\csname val@rq.opsmem.luna.by70.located\endcsname{0.03}
\expandafter\def\csname val@rq.opsmem.luna.by70.located.count\endcsname{6}
\expandafter\def\csname val@rq.opsmem.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by80.correlated\endcsname{0.61}
\expandafter\def\csname val@rq.opsmem.luna.by80.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.opsmem.luna.by80.injected\endcsname{176}
\expandafter\def\csname val@rq.opsmem.luna.by80.located\endcsname{0.03}
\expandafter\def\csname val@rq.opsmem.luna.by80.located.count\endcsname{6}
\expandafter\def\csname val@rq.opsmem.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.by90.correlated\endcsname{0.61}
\expandafter\def\csname val@rq.opsmem.luna.by90.correlated.count\endcsname{108}
\expandafter\def\csname val@rq.opsmem.luna.by90.injected\endcsname{176}
\expandafter\def\csname val@rq.opsmem.luna.by90.located\endcsname{0.03}
\expandafter\def\csname val@rq.opsmem.luna.by90.located.count\endcsname{6}
\expandafter\def\csname val@rq.opsmem.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.opsmem.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.outcome.acted\endcsname{3}
\expandafter\def\csname val@rq.opsmem.luna.outcome.acted.pct\endcsname{2}
\expandafter\def\csname val@rq.opsmem.luna.outcome.correlated\endcsname{103}
\expandafter\def\csname val@rq.opsmem.luna.outcome.correlated.pct\endcsname{59}
\expandafter\def\csname val@rq.opsmem.luna.outcome.faults\endcsname{176}
\expandafter\def\csname val@rq.opsmem.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.outcome.located\endcsname{6}
\expandafter\def\csname val@rq.opsmem.luna.outcome.located.pct\endcsname{3}
\expandafter\def\csname val@rq.opsmem.luna.outcome.missed\endcsname{64}
\expandafter\def\csname val@rq.opsmem.luna.outcome.missed.pct\endcsname{36}
\expandafter\def\csname val@rq.opsmem.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.opsmem.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.0-10.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.0-10.claim\endcsname{13.3}
\expandafter\def\csname val@rq.orbit-0.kimi.0-10.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.0-10.read\endcsname{2.8}
\expandafter\def\csname val@rq.orbit-0.kimi.10-20.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.10-20.claim\endcsname{38.5}
\expandafter\def\csname val@rq.orbit-0.kimi.10-20.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.10-20.read\endcsname{3.2}
\expandafter\def\csname val@rq.orbit-0.kimi.20-30.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.20-30.claim\endcsname{60.3}
\expandafter\def\csname val@rq.orbit-0.kimi.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.20-30.read\endcsname{2.5}
\expandafter\def\csname val@rq.orbit-0.kimi.30-40.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.30-40.claim\endcsname{85.5}
\expandafter\def\csname val@rq.orbit-0.kimi.30-40.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.30-40.read\endcsname{1.7}
\expandafter\def\csname val@rq.orbit-0.kimi.40-50.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.40-50.claim\endcsname{112.5}
\expandafter\def\csname val@rq.orbit-0.kimi.40-50.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.40-50.read\endcsname{1.6}
\expandafter\def\csname val@rq.orbit-0.kimi.50-60.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.50-60.claim\endcsname{86.8}
\expandafter\def\csname val@rq.orbit-0.kimi.50-60.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.50-60.read\endcsname{1.5}
\expandafter\def\csname val@rq.orbit-0.kimi.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.60-70.claim\endcsname{134.1}
\expandafter\def\csname val@rq.orbit-0.kimi.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.60-70.read\endcsname{1.2}
\expandafter\def\csname val@rq.orbit-0.kimi.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.70-80.claim\endcsname{146.4}
\expandafter\def\csname val@rq.orbit-0.kimi.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.70-80.read\endcsname{1.2}
\expandafter\def\csname val@rq.orbit-0.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.80-90.claim\endcsname{152.2}
\expandafter\def\csname val@rq.orbit-0.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.kimi.80-90.read\endcsname{1.3}
\expandafter\def\csname val@rq.orbit-0.kimi.actions\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.actions.off\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.actions.unrepaired\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.correlated\endcsname{0.81}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.correlated.count\endcsname{13}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.injected\endcsname{16}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.correlated\endcsname{0.67}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.correlated.count\endcsname{24}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.injected\endcsname{36}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.correlated\endcsname{0.80}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.correlated.count\endcsname{40}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.injected\endcsname{50}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.correlated\endcsname{0.80}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.correlated.count\endcsname{57}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.injected\endcsname{71}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.correlated\endcsname{0.71}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.correlated.count\endcsname{65}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.injected\endcsname{91}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.correlated\endcsname{0.76}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.correlated.count\endcsname{89}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.located\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.located.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.kimi.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.acted\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.acted.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.correlated\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.correlated.pct\endcsname{77}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.faults\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.located\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.located.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.missed\endcsname{27}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.missed.pct\endcsname{23}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.kimi.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.0-10.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.0-10.claim\endcsname{11.7}
\expandafter\def\csname val@rq.orbit-0.luna.0-10.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.0-10.read\endcsname{5.5}
\expandafter\def\csname val@rq.orbit-0.luna.10-20.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.10-20.claim\endcsname{36.6}
\expandafter\def\csname val@rq.orbit-0.luna.10-20.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.10-20.read\endcsname{4.7}
\expandafter\def\csname val@rq.orbit-0.luna.20-30.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.20-30.claim\endcsname{66.0}
\expandafter\def\csname val@rq.orbit-0.luna.20-30.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.20-30.read\endcsname{3.0}
\expandafter\def\csname val@rq.orbit-0.luna.30-40.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.30-40.claim\endcsname{57.0}
\expandafter\def\csname val@rq.orbit-0.luna.30-40.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.30-40.read\endcsname{2.1}
\expandafter\def\csname val@rq.orbit-0.luna.40-50.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.40-50.claim\endcsname{74.2}
\expandafter\def\csname val@rq.orbit-0.luna.40-50.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.40-50.read\endcsname{1.2}
\expandafter\def\csname val@rq.orbit-0.luna.50-60.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.50-60.claim\endcsname{102.3}
\expandafter\def\csname val@rq.orbit-0.luna.50-60.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.50-60.read\endcsname{1.6}
\expandafter\def\csname val@rq.orbit-0.luna.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.60-70.claim\endcsname{128.6}
\expandafter\def\csname val@rq.orbit-0.luna.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.60-70.read\endcsname{1.2}
\expandafter\def\csname val@rq.orbit-0.luna.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.70-80.claim\endcsname{132.4}
\expandafter\def\csname val@rq.orbit-0.luna.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.70-80.read\endcsname{1.0}
\expandafter\def\csname val@rq.orbit-0.luna.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.80-90.claim\endcsname{114.1}
\expandafter\def\csname val@rq.orbit-0.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.orbit-0.luna.80-90.read\endcsname{1.0}
\expandafter\def\csname val@rq.orbit-0.luna.actions\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.actions.off\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.actions.unrepaired\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by10.correlated\endcsname{0.75}
\expandafter\def\csname val@rq.orbit-0.luna.by10.correlated.count\endcsname{12}
\expandafter\def\csname val@rq.orbit-0.luna.by10.injected\endcsname{16}
\expandafter\def\csname val@rq.orbit-0.luna.by10.located\endcsname{0.06}
\expandafter\def\csname val@rq.orbit-0.luna.by10.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by20.correlated\endcsname{0.61}
\expandafter\def\csname val@rq.orbit-0.luna.by20.correlated.count\endcsname{22}
\expandafter\def\csname val@rq.orbit-0.luna.by20.injected\endcsname{36}
\expandafter\def\csname val@rq.orbit-0.luna.by20.located\endcsname{0.03}
\expandafter\def\csname val@rq.orbit-0.luna.by20.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by30.correlated\endcsname{0.76}
\expandafter\def\csname val@rq.orbit-0.luna.by30.correlated.count\endcsname{38}
\expandafter\def\csname val@rq.orbit-0.luna.by30.injected\endcsname{50}
\expandafter\def\csname val@rq.orbit-0.luna.by30.located\endcsname{0.02}
\expandafter\def\csname val@rq.orbit-0.luna.by30.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by40.correlated\endcsname{0.76}
\expandafter\def\csname val@rq.orbit-0.luna.by40.correlated.count\endcsname{54}
\expandafter\def\csname val@rq.orbit-0.luna.by40.injected\endcsname{71}
\expandafter\def\csname val@rq.orbit-0.luna.by40.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by40.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by50.correlated\endcsname{0.68}
\expandafter\def\csname val@rq.orbit-0.luna.by50.correlated.count\endcsname{62}
\expandafter\def\csname val@rq.orbit-0.luna.by50.injected\endcsname{91}
\expandafter\def\csname val@rq.orbit-0.luna.by50.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by50.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by60.correlated\endcsname{0.74}
\expandafter\def\csname val@rq.orbit-0.luna.by60.correlated.count\endcsname{86}
\expandafter\def\csname val@rq.orbit-0.luna.by60.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.luna.by60.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by60.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by70.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.luna.by70.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.luna.by70.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.luna.by70.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by70.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by80.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.luna.by80.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.luna.by80.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.luna.by80.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by80.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.by90.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.orbit-0.luna.by90.correlated.count\endcsname{90}
\expandafter\def\csname val@rq.orbit-0.luna.by90.injected\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.luna.by90.located\endcsname{0.01}
\expandafter\def\csname val@rq.orbit-0.luna.by90.located.count\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.orbit-0.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.acted\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.acted.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.correlated\endcsname{89}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.correlated.pct\endcsname{76}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.faults\endcsname{117}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.located\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.located.pct\endcsname{1}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.missed\endcsname{27}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.missed.pct\endcsname{23}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.orbit-0.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.0-10.act\endcsname{0.6}
\expandafter\def\csname val@rq.rag-b2r.kimi.0-10.claim\endcsname{5.6}
\expandafter\def\csname val@rq.rag-b2r.kimi.0-10.executed\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.kimi.0-10.read\endcsname{4.8}
\expandafter\def\csname val@rq.rag-b2r.kimi.10-20.act\endcsname{1.5}
\expandafter\def\csname val@rq.rag-b2r.kimi.10-20.claim\endcsname{26.9}
\expandafter\def\csname val@rq.rag-b2r.kimi.10-20.executed\endcsname{0.7}
\expandafter\def\csname val@rq.rag-b2r.kimi.10-20.read\endcsname{10.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.20-30.act\endcsname{2.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.20-30.claim\endcsname{37.1}
\expandafter\def\csname val@rq.rag-b2r.kimi.20-30.executed\endcsname{1.2}
\expandafter\def\csname val@rq.rag-b2r.kimi.20-30.read\endcsname{11.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.30-40.act\endcsname{2.6}
\expandafter\def\csname val@rq.rag-b2r.kimi.30-40.claim\endcsname{32.1}
\expandafter\def\csname val@rq.rag-b2r.kimi.30-40.executed\endcsname{1.5}
\expandafter\def\csname val@rq.rag-b2r.kimi.30-40.read\endcsname{9.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.40-50.act\endcsname{1.3}
\expandafter\def\csname val@rq.rag-b2r.kimi.40-50.claim\endcsname{42.2}
\expandafter\def\csname val@rq.rag-b2r.kimi.40-50.executed\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.kimi.40-50.read\endcsname{9.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.50-60.act\endcsname{2.5}
\expandafter\def\csname val@rq.rag-b2r.kimi.50-60.claim\endcsname{32.8}
\expandafter\def\csname val@rq.rag-b2r.kimi.50-60.executed\endcsname{1.1}
\expandafter\def\csname val@rq.rag-b2r.kimi.50-60.read\endcsname{7.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.60-70.act\endcsname{1.2}
\expandafter\def\csname val@rq.rag-b2r.kimi.60-70.claim\endcsname{34.6}
\expandafter\def\csname val@rq.rag-b2r.kimi.60-70.executed\endcsname{0.3}
\expandafter\def\csname val@rq.rag-b2r.kimi.60-70.read\endcsname{8.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.70-80.act\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.kimi.70-80.claim\endcsname{30.3}
\expandafter\def\csname val@rq.rag-b2r.kimi.70-80.executed\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.kimi.70-80.read\endcsname{8.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.80-90.act\endcsname{1.3}
\expandafter\def\csname val@rq.rag-b2r.kimi.80-90.claim\endcsname{26.6}
\expandafter\def\csname val@rq.rag-b2r.kimi.80-90.executed\endcsname{0.8}
\expandafter\def\csname val@rq.rag-b2r.kimi.80-90.read\endcsname{7.0}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions\endcsname{68}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.off\endcsname{32}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.off.pct\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.unrepaired\endcsname{36}
\expandafter\def\csname val@rq.rag-b2r.kimi.actions.unrepaired.pct\endcsname{53}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.correlated\endcsname{0.31}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.correlated.count\endcsname{5}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.injected\endcsname{16}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.located\endcsname{0.19}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.located.count\endcsname{3}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.correlated\endcsname{0.28}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.correlated.count\endcsname{10}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.injected\endcsname{36}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.located\endcsname{0.31}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.located.count\endcsname{11}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.correlated\endcsname{0.32}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.injected\endcsname{50}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.located\endcsname{0.30}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.located.count\endcsname{15}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.correlated\endcsname{0.31}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.correlated.count\endcsname{22}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.injected\endcsname{71}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.located\endcsname{0.35}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.located.count\endcsname{25}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.correlated\endcsname{0.36}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.correlated.count\endcsname{33}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.injected\endcsname{91}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.located\endcsname{0.36}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.located.count\endcsname{33}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.correlated\endcsname{0.40}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.correlated.count\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.injected\endcsname{117}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.located\endcsname{0.40}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.located.count\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.correlated\endcsname{0.43}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.correlated.count\endcsname{50}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.injected\endcsname{117}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.located\endcsname{0.40}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.located.count\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.correlated\endcsname{0.43}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.correlated.count\endcsname{50}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.injected\endcsname{117}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.located\endcsname{0.40}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.located.count\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.correlated\endcsname{0.43}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.correlated.count\endcsname{50}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.injected\endcsname{117}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.located\endcsname{0.40}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.located.count\endcsname{47}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.kimi.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.acted\endcsname{25}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.acted.pct\endcsname{21}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.correlated\endcsname{16}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.correlated.pct\endcsname{14}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.faults\endcsname{117}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.located\endcsname{26}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.located.pct\endcsname{22}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.missed\endcsname{50}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.missed.pct\endcsname{43}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.kimi.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.0-10.act\endcsname{1.2}
\expandafter\def\csname val@rq.rag-b2r.luna.0-10.claim\endcsname{9.5}
\expandafter\def\csname val@rq.rag-b2r.luna.0-10.executed\endcsname{0.9}
\expandafter\def\csname val@rq.rag-b2r.luna.0-10.read\endcsname{7.9}
\expandafter\def\csname val@rq.rag-b2r.luna.10-20.act\endcsname{1.3}
\expandafter\def\csname val@rq.rag-b2r.luna.10-20.claim\endcsname{22.4}
\expandafter\def\csname val@rq.rag-b2r.luna.10-20.executed\endcsname{1.3}
\expandafter\def\csname val@rq.rag-b2r.luna.10-20.read\endcsname{11.9}
\expandafter\def\csname val@rq.rag-b2r.luna.20-30.act\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.luna.20-30.claim\endcsname{27.9}
\expandafter\def\csname val@rq.rag-b2r.luna.20-30.executed\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.luna.20-30.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.30-40.act\endcsname{1.3}
\expandafter\def\csname val@rq.rag-b2r.luna.30-40.claim\endcsname{32.0}
\expandafter\def\csname val@rq.rag-b2r.luna.30-40.executed\endcsname{1.2}
\expandafter\def\csname val@rq.rag-b2r.luna.30-40.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.40-50.act\endcsname{1.0}
\expandafter\def\csname val@rq.rag-b2r.luna.40-50.claim\endcsname{34.0}
\expandafter\def\csname val@rq.rag-b2r.luna.40-50.executed\endcsname{0.9}
\expandafter\def\csname val@rq.rag-b2r.luna.40-50.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.50-60.act\endcsname{0.7}
\expandafter\def\csname val@rq.rag-b2r.luna.50-60.claim\endcsname{34.6}
\expandafter\def\csname val@rq.rag-b2r.luna.50-60.executed\endcsname{0.7}
\expandafter\def\csname val@rq.rag-b2r.luna.50-60.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.60-70.act\endcsname{0.5}
\expandafter\def\csname val@rq.rag-b2r.luna.60-70.claim\endcsname{35.6}
\expandafter\def\csname val@rq.rag-b2r.luna.60-70.executed\endcsname{0.4}
\expandafter\def\csname val@rq.rag-b2r.luna.60-70.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.70-80.act\endcsname{1.1}
\expandafter\def\csname val@rq.rag-b2r.luna.70-80.claim\endcsname{38.0}
\expandafter\def\csname val@rq.rag-b2r.luna.70-80.executed\endcsname{0.5}
\expandafter\def\csname val@rq.rag-b2r.luna.70-80.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.80-90.act\endcsname{0.7}
\expandafter\def\csname val@rq.rag-b2r.luna.80-90.claim\endcsname{38.1}
\expandafter\def\csname val@rq.rag-b2r.luna.80-90.executed\endcsname{0.3}
\expandafter\def\csname val@rq.rag-b2r.luna.80-90.read\endcsname{12.0}
\expandafter\def\csname val@rq.rag-b2r.luna.actions\endcsname{99}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.off\endcsname{51}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.off.pct\endcsname{52}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.unrepaired\endcsname{48}
\expandafter\def\csname val@rq.rag-b2r.luna.actions.unrepaired.pct\endcsname{48}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.correlated\endcsname{0.42}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.correlated.count\endcsname{10}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.located\endcsname{0.12}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.located.count\endcsname{3}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.correlated\endcsname{0.30}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.correlated.count\endcsname{16}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.injected\endcsname{53}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.located\endcsname{0.08}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.located.count\endcsname{4}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.correlated\endcsname{0.23}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.correlated.count\endcsname{17}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.injected\endcsname{74}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.located\endcsname{0.08}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.located.count\endcsname{6}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.correlated\endcsname{0.23}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.correlated.count\endcsname{24}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.injected\endcsname{106}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.located\endcsname{0.10}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.located.count\endcsname{11}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.correlated.count\endcsname{27}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.injected\endcsname{134}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.located\endcsname{0.10}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.located.count\endcsname{13}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.correlated\endcsname{0.19}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.correlated.count\endcsname{32}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.injected\endcsname{171}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.located\endcsname{0.10}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.located.count\endcsname{17}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.correlated.count\endcsname{34}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.injected\endcsname{171}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.located\endcsname{0.11}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.located.count\endcsname{18}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.correlated.count\endcsname{34}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.injected\endcsname{171}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.located\endcsname{0.11}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.located.count\endcsname{18}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.correlated\endcsname{0.20}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.correlated.count\endcsname{34}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.injected\endcsname{171}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.located\endcsname{0.11}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.located.count\endcsname{18}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.rag-b2r.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.acted\endcsname{23}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.acted.pct\endcsname{13}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.correlated\endcsname{23}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.correlated.pct\endcsname{13}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.faults\endcsname{171}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.located\endcsname{10}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.located.pct\endcsname{6}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.missed\endcsname{115}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.missed.pct\endcsname{67}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.rag-b2r.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.held10.outcome.acted\endcsname{33}
\expandafter\def\csname val@rq.react-b2.held10.outcome.acted.pct\endcsname{56}
\expandafter\def\csname val@rq.react-b2.held10.outcome.correlated\endcsname{7}
\expandafter\def\csname val@rq.react-b2.held10.outcome.correlated.pct\endcsname{12}
\expandafter\def\csname val@rq.react-b2.held10.outcome.faults\endcsname{59}
\expandafter\def\csname val@rq.react-b2.held10.outcome.handled\endcsname{4}
\expandafter\def\csname val@rq.react-b2.held10.outcome.handled.pct\endcsname{7}
\expandafter\def\csname val@rq.react-b2.held10.outcome.located\endcsname{1}
\expandafter\def\csname val@rq.react-b2.held10.outcome.located.pct\endcsname{2}
\expandafter\def\csname val@rq.react-b2.held10.outcome.missed\endcsname{7}
\expandafter\def\csname val@rq.react-b2.held10.outcome.missed.pct\endcsname{12}
\expandafter\def\csname val@rq.react-b2.held10.outcome.repaired-only\endcsname{7}
\expandafter\def\csname val@rq.react-b2.held10.outcome.repaired-only.pct\endcsname{12}
\expandafter\def\csname val@rq.react-b2.held5.outcome.acted\endcsname{12}
\expandafter\def\csname val@rq.react-b2.held5.outcome.acted.pct\endcsname{40}
\expandafter\def\csname val@rq.react-b2.held5.outcome.correlated\endcsname{0}
\expandafter\def\csname val@rq.react-b2.held5.outcome.correlated.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.held5.outcome.faults\endcsname{30}
\expandafter\def\csname val@rq.react-b2.held5.outcome.handled\endcsname{5}
\expandafter\def\csname val@rq.react-b2.held5.outcome.handled.pct\endcsname{17}
\expandafter\def\csname val@rq.react-b2.held5.outcome.located\endcsname{0}
\expandafter\def\csname val@rq.react-b2.held5.outcome.located.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.held5.outcome.missed\endcsname{3}
\expandafter\def\csname val@rq.react-b2.held5.outcome.missed.pct\endcsname{10}
\expandafter\def\csname val@rq.react-b2.held5.outcome.repaired-only\endcsname{10}
\expandafter\def\csname val@rq.react-b2.held5.outcome.repaired-only.pct\endcsname{33}
\expandafter\def\csname val@rq.react-b2.kimi.0-10.act\endcsname{0.7}
\expandafter\def\csname val@rq.react-b2.kimi.0-10.claim\endcsname{3.9}
\expandafter\def\csname val@rq.react-b2.kimi.0-10.executed\endcsname{0.6}
\expandafter\def\csname val@rq.react-b2.kimi.0-10.read\endcsname{8.9}
\expandafter\def\csname val@rq.react-b2.kimi.10-20.act\endcsname{1.1}
\expandafter\def\csname val@rq.react-b2.kimi.10-20.claim\endcsname{8.3}
\expandafter\def\csname val@rq.react-b2.kimi.10-20.executed\endcsname{1.1}
\expandafter\def\csname val@rq.react-b2.kimi.10-20.read\endcsname{14.9}
\expandafter\def\csname val@rq.react-b2.kimi.20-30.act\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.20-30.claim\endcsname{18.7}
\expandafter\def\csname val@rq.react-b2.kimi.20-30.executed\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.20-30.read\endcsname{15.8}
\expandafter\def\csname val@rq.react-b2.kimi.30-40.act\endcsname{0.5}
\expandafter\def\csname val@rq.react-b2.kimi.30-40.claim\endcsname{23.7}
\expandafter\def\csname val@rq.react-b2.kimi.30-40.executed\endcsname{0.5}
\expandafter\def\csname val@rq.react-b2.kimi.30-40.read\endcsname{15.0}
\expandafter\def\csname val@rq.react-b2.kimi.40-50.act\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.40-50.claim\endcsname{27.7}
\expandafter\def\csname val@rq.react-b2.kimi.40-50.executed\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.40-50.read\endcsname{16.4}
\expandafter\def\csname val@rq.react-b2.kimi.50-60.act\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.50-60.claim\endcsname{32.3}
\expandafter\def\csname val@rq.react-b2.kimi.50-60.executed\endcsname{0.3}
\expandafter\def\csname val@rq.react-b2.kimi.50-60.read\endcsname{13.9}
\expandafter\def\csname val@rq.react-b2.kimi.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.60-70.claim\endcsname{30.2}
\expandafter\def\csname val@rq.react-b2.kimi.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.60-70.read\endcsname{14.2}
\expandafter\def\csname val@rq.react-b2.kimi.70-80.act\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.70-80.claim\endcsname{34.1}
\expandafter\def\csname val@rq.react-b2.kimi.70-80.executed\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.70-80.read\endcsname{12.9}
\expandafter\def\csname val@rq.react-b2.kimi.80-90.act\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.80-90.claim\endcsname{35.5}
\expandafter\def\csname val@rq.react-b2.kimi.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.kimi.80-90.read\endcsname{13.8}
\expandafter\def\csname val@rq.react-b2.kimi.actions\endcsname{46}
\expandafter\def\csname val@rq.react-b2.kimi.actions.off\endcsname{2}
\expandafter\def\csname val@rq.react-b2.kimi.actions.off.pct\endcsname{4}
\expandafter\def\csname val@rq.react-b2.kimi.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.react-b2.kimi.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.kimi.actions.unrepaired\endcsname{44}
\expandafter\def\csname val@rq.react-b2.kimi.actions.unrepaired.pct\endcsname{96}
\expandafter\def\csname val@rq.react-b2.kimi.by10.correlated\endcsname{0.75}
\expandafter\def\csname val@rq.react-b2.kimi.by10.correlated.count\endcsname{18}
\expandafter\def\csname val@rq.react-b2.kimi.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.react-b2.kimi.by10.located\endcsname{0.12}
\expandafter\def\csname val@rq.react-b2.kimi.by10.located.count\endcsname{3}
\expandafter\def\csname val@rq.react-b2.kimi.by10.repaired\endcsname{0.04}
\expandafter\def\csname val@rq.react-b2.kimi.by10.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by20.correlated\endcsname{0.74}
\expandafter\def\csname val@rq.react-b2.kimi.by20.correlated.count\endcsname{40}
\expandafter\def\csname val@rq.react-b2.kimi.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.react-b2.kimi.by20.located\endcsname{0.15}
\expandafter\def\csname val@rq.react-b2.kimi.by20.located.count\endcsname{8}
\expandafter\def\csname val@rq.react-b2.kimi.by20.repaired\endcsname{0.02}
\expandafter\def\csname val@rq.react-b2.kimi.by20.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by30.correlated\endcsname{0.77}
\expandafter\def\csname val@rq.react-b2.kimi.by30.correlated.count\endcsname{58}
\expandafter\def\csname val@rq.react-b2.kimi.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.react-b2.kimi.by30.located\endcsname{0.13}
\expandafter\def\csname val@rq.react-b2.kimi.by30.located.count\endcsname{10}
\expandafter\def\csname val@rq.react-b2.kimi.by30.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by30.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by40.correlated\endcsname{0.72}
\expandafter\def\csname val@rq.react-b2.kimi.by40.correlated.count\endcsname{77}
\expandafter\def\csname val@rq.react-b2.kimi.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.react-b2.kimi.by40.located\endcsname{0.09}
\expandafter\def\csname val@rq.react-b2.kimi.by40.located.count\endcsname{10}
\expandafter\def\csname val@rq.react-b2.kimi.by40.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by40.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by50.correlated\endcsname{0.64}
\expandafter\def\csname val@rq.react-b2.kimi.by50.correlated.count\endcsname{88}
\expandafter\def\csname val@rq.react-b2.kimi.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.react-b2.kimi.by50.located\endcsname{0.07}
\expandafter\def\csname val@rq.react-b2.kimi.by50.located.count\endcsname{10}
\expandafter\def\csname val@rq.react-b2.kimi.by50.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by50.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by60.correlated\endcsname{0.69}
\expandafter\def\csname val@rq.react-b2.kimi.by60.correlated.count\endcsname{122}
\expandafter\def\csname val@rq.react-b2.kimi.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.kimi.by60.located\endcsname{0.07}
\expandafter\def\csname val@rq.react-b2.kimi.by60.located.count\endcsname{13}
\expandafter\def\csname val@rq.react-b2.kimi.by60.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by60.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by70.correlated\endcsname{0.69}
\expandafter\def\csname val@rq.react-b2.kimi.by70.correlated.count\endcsname{123}
\expandafter\def\csname val@rq.react-b2.kimi.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.kimi.by70.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.kimi.by70.located.count\endcsname{14}
\expandafter\def\csname val@rq.react-b2.kimi.by70.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by70.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by80.correlated\endcsname{0.69}
\expandafter\def\csname val@rq.react-b2.kimi.by80.correlated.count\endcsname{123}
\expandafter\def\csname val@rq.react-b2.kimi.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.kimi.by80.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.kimi.by80.located.count\endcsname{14}
\expandafter\def\csname val@rq.react-b2.kimi.by80.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by80.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.by90.correlated\endcsname{0.69}
\expandafter\def\csname val@rq.react-b2.kimi.by90.correlated.count\endcsname{123}
\expandafter\def\csname val@rq.react-b2.kimi.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.kimi.by90.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.kimi.by90.located.count\endcsname{14}
\expandafter\def\csname val@rq.react-b2.kimi.by90.repaired\endcsname{0.01}
\expandafter\def\csname val@rq.react-b2.kimi.by90.repaired.count\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.acted\endcsname{41}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.acted.pct\endcsname{23}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.correlated\endcsname{84}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.correlated.pct\endcsname{47}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.located\endcsname{3}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.located.pct\endcsname{2}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.missed\endcsname{48}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.missed.pct\endcsname{27}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.repaired-only\endcsname{1}
\expandafter\def\csname val@rq.react-b2.kimi.outcome.repaired-only.pct\endcsname{1}
\expandafter\def\csname val@rq.react-b2.luna.0-10.act\endcsname{0.9}
\expandafter\def\csname val@rq.react-b2.luna.0-10.claim\endcsname{4.1}
\expandafter\def\csname val@rq.react-b2.luna.0-10.executed\endcsname{0.9}
\expandafter\def\csname val@rq.react-b2.luna.0-10.read\endcsname{10.9}
\expandafter\def\csname val@rq.react-b2.luna.10-20.act\endcsname{1.6}
\expandafter\def\csname val@rq.react-b2.luna.10-20.claim\endcsname{8.9}
\expandafter\def\csname val@rq.react-b2.luna.10-20.executed\endcsname{1.3}
\expandafter\def\csname val@rq.react-b2.luna.10-20.read\endcsname{13.4}
\expandafter\def\csname val@rq.react-b2.luna.20-30.act\endcsname{0.2}
\expandafter\def\csname val@rq.react-b2.luna.20-30.claim\endcsname{12.3}
\expandafter\def\csname val@rq.react-b2.luna.20-30.executed\endcsname{0.2}
\expandafter\def\csname val@rq.react-b2.luna.20-30.read\endcsname{21.3}
\expandafter\def\csname val@rq.react-b2.luna.30-40.act\endcsname{0.4}
\expandafter\def\csname val@rq.react-b2.luna.30-40.claim\endcsname{12.5}
\expandafter\def\csname val@rq.react-b2.luna.30-40.executed\endcsname{0.4}
\expandafter\def\csname val@rq.react-b2.luna.30-40.read\endcsname{14.7}
\expandafter\def\csname val@rq.react-b2.luna.40-50.act\endcsname{1.9}
\expandafter\def\csname val@rq.react-b2.luna.40-50.claim\endcsname{15.9}
\expandafter\def\csname val@rq.react-b2.luna.40-50.executed\endcsname{1.2}
\expandafter\def\csname val@rq.react-b2.luna.40-50.read\endcsname{13.3}
\expandafter\def\csname val@rq.react-b2.luna.50-60.act\endcsname{0.1}
\expandafter\def\csname val@rq.react-b2.luna.50-60.claim\endcsname{21.2}
\expandafter\def\csname val@rq.react-b2.luna.50-60.executed\endcsname{0.1}
\expandafter\def\csname val@rq.react-b2.luna.50-60.read\endcsname{14.3}
\expandafter\def\csname val@rq.react-b2.luna.60-70.act\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.luna.60-70.claim\endcsname{42.6}
\expandafter\def\csname val@rq.react-b2.luna.60-70.executed\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.luna.60-70.read\endcsname{17.3}
\expandafter\def\csname val@rq.react-b2.luna.70-80.act\endcsname{0.1}
\expandafter\def\csname val@rq.react-b2.luna.70-80.claim\endcsname{49.1}
\expandafter\def\csname val@rq.react-b2.luna.70-80.executed\endcsname{0.1}
\expandafter\def\csname val@rq.react-b2.luna.70-80.read\endcsname{14.5}
\expandafter\def\csname val@rq.react-b2.luna.80-90.act\endcsname{0.7}
\expandafter\def\csname val@rq.react-b2.luna.80-90.claim\endcsname{51.1}
\expandafter\def\csname val@rq.react-b2.luna.80-90.executed\endcsname{0.0}
\expandafter\def\csname val@rq.react-b2.luna.80-90.read\endcsname{13.0}
\expandafter\def\csname val@rq.react-b2.luna.actions\endcsname{63}
\expandafter\def\csname val@rq.react-b2.luna.actions.off\endcsname{14}
\expandafter\def\csname val@rq.react-b2.luna.actions.off.pct\endcsname{22}
\expandafter\def\csname val@rq.react-b2.luna.actions.repaired\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.actions.repaired.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.actions.unrepaired\endcsname{49}
\expandafter\def\csname val@rq.react-b2.luna.actions.unrepaired.pct\endcsname{78}
\expandafter\def\csname val@rq.react-b2.luna.by10.correlated\endcsname{0.38}
\expandafter\def\csname val@rq.react-b2.luna.by10.correlated.count\endcsname{9}
\expandafter\def\csname val@rq.react-b2.luna.by10.injected\endcsname{24}
\expandafter\def\csname val@rq.react-b2.luna.by10.located\endcsname{0.12}
\expandafter\def\csname val@rq.react-b2.luna.by10.located.count\endcsname{3}
\expandafter\def\csname val@rq.react-b2.luna.by10.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by10.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by20.correlated\endcsname{0.35}
\expandafter\def\csname val@rq.react-b2.luna.by20.correlated.count\endcsname{19}
\expandafter\def\csname val@rq.react-b2.luna.by20.injected\endcsname{54}
\expandafter\def\csname val@rq.react-b2.luna.by20.located\endcsname{0.09}
\expandafter\def\csname val@rq.react-b2.luna.by20.located.count\endcsname{5}
\expandafter\def\csname val@rq.react-b2.luna.by20.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by20.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by30.correlated\endcsname{0.37}
\expandafter\def\csname val@rq.react-b2.luna.by30.correlated.count\endcsname{28}
\expandafter\def\csname val@rq.react-b2.luna.by30.injected\endcsname{75}
\expandafter\def\csname val@rq.react-b2.luna.by30.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.luna.by30.located.count\endcsname{6}
\expandafter\def\csname val@rq.react-b2.luna.by30.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by30.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by40.correlated\endcsname{0.37}
\expandafter\def\csname val@rq.react-b2.luna.by40.correlated.count\endcsname{40}
\expandafter\def\csname val@rq.react-b2.luna.by40.injected\endcsname{107}
\expandafter\def\csname val@rq.react-b2.luna.by40.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.luna.by40.located.count\endcsname{9}
\expandafter\def\csname val@rq.react-b2.luna.by40.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by40.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by50.correlated\endcsname{0.35}
\expandafter\def\csname val@rq.react-b2.luna.by50.correlated.count\endcsname{48}
\expandafter\def\csname val@rq.react-b2.luna.by50.injected\endcsname{137}
\expandafter\def\csname val@rq.react-b2.luna.by50.located\endcsname{0.08}
\expandafter\def\csname val@rq.react-b2.luna.by50.located.count\endcsname{11}
\expandafter\def\csname val@rq.react-b2.luna.by50.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by50.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by60.correlated\endcsname{0.40}
\expandafter\def\csname val@rq.react-b2.luna.by60.correlated.count\endcsname{70}
\expandafter\def\csname val@rq.react-b2.luna.by60.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.luna.by60.located\endcsname{0.09}
\expandafter\def\csname val@rq.react-b2.luna.by60.located.count\endcsname{16}
\expandafter\def\csname val@rq.react-b2.luna.by60.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by60.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by70.correlated\endcsname{0.42}
\expandafter\def\csname val@rq.react-b2.luna.by70.correlated.count\endcsname{74}
\expandafter\def\csname val@rq.react-b2.luna.by70.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.luna.by70.located\endcsname{0.12}
\expandafter\def\csname val@rq.react-b2.luna.by70.located.count\endcsname{22}
\expandafter\def\csname val@rq.react-b2.luna.by70.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by70.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by80.correlated\endcsname{0.42}
\expandafter\def\csname val@rq.react-b2.luna.by80.correlated.count\endcsname{74}
\expandafter\def\csname val@rq.react-b2.luna.by80.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.luna.by80.located\endcsname{0.12}
\expandafter\def\csname val@rq.react-b2.luna.by80.located.count\endcsname{22}
\expandafter\def\csname val@rq.react-b2.luna.by80.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by80.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.by90.correlated\endcsname{0.42}
\expandafter\def\csname val@rq.react-b2.luna.by90.correlated.count\endcsname{74}
\expandafter\def\csname val@rq.react-b2.luna.by90.injected\endcsname{177}
\expandafter\def\csname val@rq.react-b2.luna.by90.located\endcsname{0.12}
\expandafter\def\csname val@rq.react-b2.luna.by90.located.count\endcsname{22}
\expandafter\def\csname val@rq.react-b2.luna.by90.repaired\endcsname{0.00}
\expandafter\def\csname val@rq.react-b2.luna.by90.repaired.count\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.outcome.acted\endcsname{42}
\expandafter\def\csname val@rq.react-b2.luna.outcome.acted.pct\endcsname{24}
\expandafter\def\csname val@rq.react-b2.luna.outcome.correlated\endcsname{44}
\expandafter\def\csname val@rq.react-b2.luna.outcome.correlated.pct\endcsname{25}
\expandafter\def\csname val@rq.react-b2.luna.outcome.faults\endcsname{177}
\expandafter\def\csname val@rq.react-b2.luna.outcome.handled\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.outcome.handled.pct\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.outcome.located\endcsname{12}
\expandafter\def\csname val@rq.react-b2.luna.outcome.located.pct\endcsname{7}
\expandafter\def\csname val@rq.react-b2.luna.outcome.missed\endcsname{79}
\expandafter\def\csname val@rq.react-b2.luna.outcome.missed.pct\endcsname{45}
\expandafter\def\csname val@rq.react-b2.luna.outcome.repaired-only\endcsname{0}
\expandafter\def\csname val@rq.react-b2.luna.outcome.repaired-only.pct\endcsname{0}
\expandafter\def\csname val@rq.rows\endcsname{21}
\expandafter\def\csname val@rq.run.act.pct\endcsname{1.1}
\expandafter\def\csname val@rq.run.claim.pct\endcsname{74.6}
\expandafter\def\csname val@rq.run.read.pct\endcsname{24.3}
\expandafter\def\csname val@rq.runs\endcsname{52}
\expandafter\def\csname val@rq.runs.kimi\endcsname{24}
\expandafter\def\csname val@rq.runs.none\endcsname{3}
\expandafter\def\csname val@rq.settle.correlated\endcsname{45}
\expandafter\def\csname val@rq.settle.faults\endcsname{1408}
\expandafter\def\csname val@rq.settle.located\endcsname{8}
\expandafter\def\csname val@rq.settle.repaired\endcsname{2}
\makeatother

